A General Theory for Federated Optimization with Asynchronous and Heterogeneous Clients Updates

We propose a novel framework to study asynchronous federated learning optimization with delays in gradient updates. Our theoretical framework extends the standard FedAvg aggregation scheme by introducing stochastic aggregation weights to represent the variability of the clients update time, due for example to heterogeneous hardware capabilities. Our formalism applies to the general federated setting where clients have heterogeneous datasets and perform at least one step of stochastic gradient descent (SGD). We demonstrate convergence for such a scheme and provide sufficient conditions for the related minimum to be the optimum of the federated problem. We show that our general framework applies to existing optimization schemes including centralized learning, FedAvg, asynchronous FedAvg, and FedBuff. The theory here provided allows drawing meaningful guidelines for designing a federated learning experiment in heterogeneous conditions. In particular, we develop in this work FedFix, a novel extension of FedAvg enabling efficient asynchronous federated training while preserving the convergence stability of synchronous aggregation. We empirically demonstrate our theory on a series of experiments showing that asynchronous FedAvg leads to fast convergence at the expense of stability, and we finally demonstrate the improvements of FedFix over synchronous and asynchronous FedAvg.

==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/delayed_proofs/Calculus_applications.tex <==
\section{Calculus Applications}\label{app:sec:calculus_applications}

We assume that $\tau$, $W$, $\nu$, $\beta$ are independent from $N$, and $K \ll N$, $M \ll N$

\begin{align}
\epsilon_{F}
= \Ocal\left(\frac{\sqrt{W}}{\sqrt{K N}}\right)
+ \Ocal \left( \frac{1}{W N } \sigma^2 \right)
,
\end{align}

\begin{align}
\epsilon_{opt}
&= \Ocal\left(\frac{1}{\sqrt{WKN}} \nu \sigma^2 \right)
+ \Ocal \left(\frac{(\tau +  1)  \tau}{WN } \nu \sigma^2 \right)
+ \Ocal\left(\frac{\sqrt{K}}{W^{3/2}N^{3/2}}  \beta   \sigma^2 \right)
\nonumber\\
&+ \Ocal \left( \frac{\tau}{WN} \sigma^2 \right)
+ \Ocal \left(\beta \frac{K(\tau+1)\tau}{W^2N^2 }\sigma^2 \right)
\\
&= \Ocal\left(\frac{1}{\sqrt{WKN}} \nu \sigma^2 \right)
,
\end{align}
\begin{align}
\epsilon_H
= \Ocal\left(\frac{\sqrt{K}}{\sqrt{WN}} \right)
+ \Ocal \left( \frac{\tau}{WN} K \right)
+ \Ocal \left((\tau +  1) \frac{\tau}{WN} K \right)
= \Ocal\left(\frac{\sqrt{K}}{\sqrt{WN}} \right)
%+ \Ocal \left( \frac{\tau}{WN} K \right)
%+ \Ocal \left((\tau +  1) \frac{\tau}{WN} K \right)
,
\end{align}
\begin{equation}
\nu 
= \frac{1}{N}\sum_{ n = 0 }^{N-1} \sum_{i=1}^M \mathbb{P}( T_i^n \le \Delta t^n ) d_i^2(n) 
,
\end{equation}
and
\begin{equation}
\beta = \nu + \frac{1}{N}\sum_{ n = 0 }^{N-1}
\left[
\left[\sum_{i=1}^M  R_i(n) d_i(n)\right]^2
- \sum_{i=1}^M R_i^2(n) d_i^2(n)
\right]
.
\end{equation}




\begin{equation}
	\epsilon_W = \Ocal( \frac{\sqrt{K (W-1)}}{\sqrt{N}})
\end{equation}

As a result, we have 

\begin{align}
\epsilon_{iid}
= \Ocal \left(\frac{1}{\sqrt{KN}}\right)
%+ \Ocal\left(\frac{\sqrt{K(W-1)}}{\sqrt{N}}\right)
+ \Ocal\left(\frac{1}{\sqrt{KN}} \nu \sigma^2 \right)
\end{align}

\begin{align}
	\epsilon_{non-iid}
	= \Ocal \left(\frac{\sqrt{K}}{\sqrt{WN}}\right)
	+ \Ocal\left(\frac{\sqrt{K(W-1)}}{\sqrt{N}}\right)
	+ \Ocal\left(\frac{1}{\sqrt{WKN}} \nu \sigma^2 \right)
\end{align}


\subsection{Synchronous FL: naive FedAvg}





\begin{equation}
\nu 
= \sum_{i=1}^M p_i^2
,
\end{equation}
and
%\begin{equation}
%\beta = \sum_{i=1}^M p_i^2 + 
%\left[ 1 - \sum_{i=1}^M p_i^2
%\right] =1 
%.
%\end{equation}
$W=1$, $\tau = 0$.

Hence, we have
\begin{align}
\epsilon
= \Ocal \left(\frac{\sqrt{K}}{\sqrt{WN}}\right)
+ \Ocal\left(\frac{\sqrt{K(W-1)}}{\sqrt{N}}\right)
+ \Ocal\left(\frac{1}{\sqrt{WKN}} \nu \sigma^2 \right)
\end{align}



\subsection{Synchronous FL : sampling with windows}




==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/delayed_proofs/Lemma_equality.tex <==
\begin{lemma}\label{lem:decompo_Xi}
	Let us consider $n$ vectors $\vx_i, ..., \vx_n$ and assume Assumption \ref{ass:clients_covariance}. We have
	\begin{equation}
	\EE{S_n}{\norm{\sum_{i=1}^M\omega_i(n)\vx_i}^2} 
	= \sum_{i=1}^M \gamma_i(n) \norm{\vx_i}^2
	+ \alpha \norm{\sum_{i=1}^M q_i(n) \vx_i}^2
	,
	\end{equation}
	where $\gamma_i(n)
	= \EE{S_n}{\omega_i^2(n)} - \alpha q_i^2(n)
	\ge 0$, and $\gamma_i(n) \le \beta q_i(n)$ with $\beta \coloneqq \max\{d_i(n) - \alpha q_i(n)\}$.
\end{lemma}

\begin{proof}
	\begin{align}
	\EE{S_n}{\norm{\sum_{i=1}^M\omega_i(n)\vx_i}^2} 
	& = \sum_{i=1}^M \EE{S_n}{\omega_i^2(n)} \norm{\vx_i}^2
	+ \sum_{i=1}^M\sum_{\substack{j=1\\ j\neq i}}^M\EE{S_n}{\omega_i(n)\omega_j(n)}\inner{\vx_i}{\vx_j}
	\\
	& = \sum_{i=1}^M \EE{S_n}{\omega_i^2(n)} \norm{\vx_i}^2
%	\nonumber\\
	+ \sum_{i=1}^M \sum_{\substack{j=1\\ j\neq i}}^M \alpha q_i(n) q_j(n) \inner{\vx_i}{\vx_j}
	\label{app:eq:AA1}
	.
	\end{align}
	In addition, we have
	\begin{equation}
	\sum_{i=1}^M\sum_{\substack{j=1\\ j\neq i}}^M\inner{q_i(n) \vx_i}{q_j(n) \vx_j} 
	= \norm{\sum_{i=1}^M q_i(n) \vx_i}^2 - \sum_{i=1}^M q_i^2(n) \norm{\vx_i}^2
	\label{app:eq:AA3}
	.
	\end{equation}
	Substituting equation (\refeq{app:eq:AA3}) in equation (\refeq{app:eq:AA1}) completes the first claim.
	
	Considering that $\EE{S_n}{\omega_i^2(n)} = \VAR{\omega_i(n)} + q_i^2(n) \ge q_i^2(n)$ and $\alpha \le 1$, we have $\gamma_i(n) \ge 0$ which completes the second claim.
	
	Finally, the third claim follows directly from the close-form of the clients aggregation weights, equation (\refeq{eq:agg_weights}).
	

	\textbf{Remark.}
	We can also provide the following lower bound for equation (\refeq{app:eq:AA3}) using Jensen inequality
	\begin{equation}
	\sum_{i=1}^M\sum_{\substack{j=1\\ j\neq i}}^M\inner{q_i(n) \vx_i}{q_j(n) \vx_j} 
	\ge \norm{\sum_{i=1}^M q_i(n) \vx_i}^2 - \frac{\max q_i(n)}{q(n)}\norm{\sum_{i=1}^M q_i(n) \vx_i}^2
	\ge 0
	\label{app:eq:AA4}
	.
	\end{equation}
	Therefore, $\EE{S_n}{\norm{\sum_{i=1}^M\omega_i(n)\vx_i}^2} $ is linearly proportional to $\alpha$.
	
\end{proof}




\begin{lemma}\label{lemma:one_SGD}
	%	We consider clients send at optimization round $n$ their contribution $\vDelta^n$.
	Under Assumption \ref{ass:clients_covariance}, the following equation holds for any vector $\vx$:
	\begin{align}
	\Delta(n)
	&\le - 2 \tilde{\eta} D(\vx, n)
	+ \tilde{\eta}^2 \alpha q^2(n) R(n)
	+ \tilde{\eta}^2 \beta q(n) S(n)
	.
	\end{align}
	
	
\end{lemma}


\begin{proof}
	We consider $S_n$, the set of participating clients at optimization round $n$, i.e. $S_n = \{n: T_i^n \le \Delta t^n\}$. We have
	\begin{align}
	\EE{S_n}{\norm{\vtheta^{n, k+1} - \vtheta^*}^2} 
	&= \EE{S_n}{\norm{(\vtheta^{n, k+1} - \vtheta^{n ,k}) + (\vtheta^{n, k} - \vtheta^*)}^2}\\
	&= \norm{\vtheta^{n, k} - \vtheta^*}^2 
	+ 2 \inner{\EE{S_n}{\vtheta^{n, k+1} - \vtheta^{n,k}}}{\vtheta^{n ,k} - \vtheta^*} \nonumber\\
	& + \EE{S_n}{\norm{\vtheta^{n, k+1} - \vtheta^{n, k}}^2} 
	\label{app:eq:decomposition}
	.
	\end{align}
	By construction, we have 
	$\vtheta^{n, k+1} - \vtheta^{n , k} 
	=  - \tilde{\eta} \sum_{i=1}^M \omega_i(n) g_i(\vtheta_i^{\rho_i(n) , k})$.
	Taking the expectation over $S_n$, we can simplify the second term of equation (\refeq{app:eq:decomposition}) with 
	$\EE{S_n}{\vtheta^{n, k+1} - \vtheta^{n , k}} 
	= - \tilde{\eta} \sum_{i=1}^M q_i(n) g_i(\vtheta_i^{\rho_i(n) , k})$. 
	Finally, using Lemma \ref{lem:decompo_Xi}, we can bound the third term.
	Therefore, we have
	\begin{align}
	\EE{S_n}{\norm{\vtheta^{n, k+1} - \vtheta^*}^2} 
	&= \norm{\vtheta^{n, k} - \vtheta^*}^2 
	+ 2 \tilde{\eta} \inner{\sum_{i=1}^M q_i(n)  g_i(\vtheta_i^{\rho_i(n) , k})}{\vtheta^n - \vtheta^*} 
	\nonumber\\
	&+ \tilde{\eta}^2 \sum_{i=1}^M \gamma_i(n)  \norm{g_i(\vtheta_i^{\rho_i(n) , k})}^2 
	+ \tilde{\eta}^2 \alpha  \norm{\sum_{i=1}^M  q_i(n) g_i(\vtheta_i^{\rho_i(n) , k})}^2 
	\label{app:eq:A1}
	.
	\end{align}
	Considering $\gamma_i(n) \le \beta q_i(n)$, taking the expected value over the iteration random batches $\vxi^{\rho_i(n), k}$, and finally taking the expected value over the remaining random variables gives
	\begin{align}
	\Delta(n, k)
	&\le - 2 \tilde{\eta} D(\vx, n, k)
	+ \tilde{\eta}^2 \alpha q^2(n) R(n ,k)
	+ \tilde{\eta}^2 \beta q(n) S(n ,k)
	.\label{eq:one_server_iteration}
	\end{align}
	Taking the mean over $K$ completes the proof.
	
\end{proof}

==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/delayed_proofs/app_bias_bound.tex <==
\section{Proof of Theorem \ref{theo:bias_convex}}\label{app:sec:theo_bias}

In this proof, we consider $\tilde{\Lcal}^n = q^{-1}(n) \Lcal^n$.

\subsection{Useful Lemma}
\begin{lemma} \label{lem:async_FL_bias}
	The difference between the gradients of $\Lcal(\vtheta)$ and $\Lcal(\vtheta)$ can be bounded as follow
%	\begin{align}
%	\norm{\nabla \Lcal(\vtheta) - \nabla \Lcal^n (\vtheta)}^2
%	& \le 4L \chi_n^2 [ \Lcal^n(\vtheta) - \Lcal^n(\tilde{\vtheta}^n)] \nonumber\\
%	& + 4L \chi_n^2 [ \Lcal^n(\tilde{\vtheta}^n) -\sum_{j \in W_n} r_j^n \Lcal_j(\vtheta_j^*)] \nonumber\\
%	&+ 4L  \sum_{j \notin W_n} r_j  [ \Lcal_j(\vtheta) - \Lcal_j(\vtheta_j^*)] ,
%%	\label{app:eq:U_1}
%	\end{align}
	\begin{align}
	\norm{\nabla \Lcal(\vtheta) - \nabla \tilde{\Lcal}^n (\vtheta)}^2
	 \le 4L \chi_n^2 [ \tilde{\Lcal}^n(\vtheta) -\sum_{j \in W_n} \tilde{s}_j(n) \Lcal_j(\vtheta_j^*)] 
	+ 4L \sum_{j \notin W_n} r_j  [ \Lcal_j(\vtheta) - \Lcal_j(\vtheta_j^*)] ,
	\end{align}
	where $W_n = \{j : s_j(n) > 0\}$ and $\chi_n^2 = \sum_{j \in W_n } (r_j - \tilde{s}_j(n))^2/\tilde{s}_j(n)$.
\end{lemma}

\begin{proof}
	We have $\sum_{ j = 1 }^J s_j(n) = \sum_{ i = 1 }^M q_i(n) = q(n)$.
	Hence, by definition of $\Lcal(\vtheta)$ and $\Lcal^n(\vtheta)$, we have
	\begin{align}
		\nabla \Lcal(\vtheta) - \nabla \tilde{\Lcal}^n(\vtheta)
		& = \sum_{j=1}^{J} (r_j - \tilde{s}_j(n) ) \nabla \Lcal_j(\vtheta)\\
		& = \sum_{j \in W_n} \frac{r_j - \tilde{s}_j(n)}{\sqrt{\tilde{s}_j(n)}} \sqrt{\tilde{s}_j(n)}\nabla \Lcal_j(\vtheta)
		+ \sum_{j \notin W_n} r_j \nabla \Lcal_j(\vtheta)
		.
	\end{align}
	Applying Jensen and Cauchy-Schwartz inequality gives
	\begin{align}
		\norm{\nabla \Lcal(\vtheta) - \nabla \tilde{\Lcal}^n (\vtheta)}^2
		& \le 2 \norm{ \sum_{j \in W_n} \frac{r_j - \tilde{s}_j(n)}{\sqrt{\tilde{s}_j(n)}} \sqrt{\tilde{s}_j(n)} \nabla \Lcal_j(\vtheta) }^2 
		+ 2 \norm{ \sum_{j \notin W_n} r_j \nabla \Lcal_j(\vtheta)}^2 
		\\
		& \le 2 \left[\sum_{j \in W_n} \frac{(r_j - \tilde{s}_j(n))^2}{\tilde{s}_j(n)}  \right] 
		\sum_{j = 1}^J \tilde{s}_j(n) \norm{ \nabla \Lcal_j(\vtheta) }^2 
		\nonumber\\
		& + 2  \left[\sum_{j \notin W_n}  r_j\right] \sum_{j \notin W_n} r_j  \norm{ \nabla \Lcal_j(\vtheta) }^2 
	\end{align}
	Considering the Lipschitz smoothness of the clients loss function, and $\sum_{ j \notin W_n} r_j \le  1$ completes the proof.
	
%	\begin{align}
%	\norm{\nabla \Lcal(\vtheta) - \frac{1}{q(n)}\nabla \Lcal^n (\vtheta)}^2
%	& \le 4L \chi_n^2 \frac{1}{q(n)} [ \Lcal^n(\vtheta) - \Lcal^n(\bar{\vtheta}^n) + \Lcal^n(\bar{\vtheta}^n) -\sum_{j \in W_n} \tilde{s}_j(n) \Lcal_j(\vtheta_j^*)] \nonumber\\
%	&+ 4L \sum_{j \notin W_n} r_j  [ \Lcal_j(\vtheta) - \Lcal_j(\vtheta_j^*)] ,
%	\end{align}
	
\end{proof}


\subsection{Proof of Theorem \ref{theo:bias_convex}}
\begin{proof}
	Using Jensen inequality and Lemma \ref{lem:async_FL_bias} gives
	\begin{align}
	\norm{\nabla \Lcal (\vtheta)}^2
	& \le 2 \norm{\nabla \Lcal ( \vtheta) - \frac{1}{q(n)}\nabla \Lcal^n( \vtheta)}^2 
	+ 2 \norm{\frac{1}{q(n)} \nabla \Lcal^n (\vtheta)}^2\\
	& \le 4L \left[\chi_n^2 \frac{1}{q(n)} + \frac{1}{q^2(n)} \right] [ \Lcal^n(\vtheta) - \Lcal^n(\bar{\vtheta}^n)] \nonumber\\
	& + \chi_n^2 \frac{1}{q(n)}4L [ \Lcal^n(\bar{\vtheta}^n) -\sum_{j \in W_n} s_j(n) \Lcal_j(\vtheta_j^*)] \nonumber\\
	&+ 4L  \sum_{j \notin W_n} r_j  [ \Lcal_j(\vtheta) - \Lcal_j(\vtheta_j^*)]
	\end{align}
	We take the maximum of $\chi_n^2$ and $q(n)$, the mean over the $KN$ serial SGD steps, and use Theorem \ref{theo:convergence_convex} to complete the proof
	.
%	, i.e.
%	\begin{align}
%	\frac{1}{N}\sum_{n=0}^{N-1} \norm{\nabla \Lcal (\vtheta^n)}^2
%	& \le 4L \max_n\left[\chi_n^2 \frac{1}{s(n)}+ \frac{1}{s^2(n)}\right] \left[ R(\{\Lcal^n\}) + \epsilon'\right]   
%	\nonumber\\
%	& + 4L \frac{1}{N}\sum_{n=0}^{N-1}\chi_n^2 \frac{1}{s(n)}[\Lcal^n(\tilde{\vtheta}^n) -\sum_{j \in W_n} {q}_j^n \Lcal_j(\vtheta_j^*)])
%	\nonumber\\
%	& + 4L \frac{1}{N}\sum_{n=0}^{N-1}\sum_{j \notin W_n} r_j [\Lcal_j(\vtheta^n) - \Lcal_j(\vtheta_j^*)]) 
%	,
%	\end{align}	
	
	

\end{proof}












==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/delayed_proofs/app_bias_bound_2.tex <==
\section{Include Bias in the error bound}

\begin{lemma} \label{lem:async_FL_bias}
%	For any model parameters $\theta$, the difference between the gradients of $\Lcal(\theta)$ and $\tilde{\Lcal}(\theta)$ can be bounded as follow:
	\begin{align}
	\norm{\nabla \Lcal(\theta) - \nabla \Lcal^n (\theta)}^2
	\le 2 \chi^n \norm{\nabla \Lcal^n (\theta)}^2 
+ 2  \norm{ \sum_{j \notin W_n} r_j  \nabla \Lcal_j(\theta) }^2  ,
%	\label{app:eq:U_1}
	\end{align}
	where $\chi^n$ denote the chi-square distance between $p$ and $q^n$, i.e. $\chi^n = \sum_{j \in W_n } (r_j - s_j^n)^2/s_j^n$ and $W_n = \{j | s_j^n > 0\}$.
\end{lemma}

\begin{proof}
	We define $s_j^n = \frac{1}{\bar{q}^n}q_j^n $ and $\bar{q}^n = \sum_{j=1}^{J}q_j^n = \sum_{i=1}^{C}q_i^n $.
	
	According to the definition of $\Lcal(\theta)$ and $\Lcal^n(\theta)$, we have:
	\begin{align}
		\nabla \Lcal(\theta) - \nabla \Lcal^n(\theta)
		& = \sum_{j=1}^{J} (r_j - s_j^n ) \nabla \Lcal_j(\theta)
		\\
%		& = \sum_{i=1}^{n} (r_j - s_j^n) [\nabla \Lcal_j(\theta) -  \nabla \Lcal^n (\theta)]\\
		& = \sum_{j \in W_n} \frac{r_j - s_j^n}{\sqrt{s_j^n}} \sqrt{s_j^n}\nabla \Lcal_j(\theta)
		+ \sum_{j \notin W_n} r_j \nabla \Lcal_j(\theta) ,
	\end{align}
	where 
%	the second equality comes from $\sum_{i=1}^{n}r_j = \sum_{i=1}^{n}s_j^n = 1$ and 
	$W_n = \{j | s_j^n > 0\}$.
	
	Applying the Jensen inequality and the Cauchy-Schwartz inequality, it follows that:
	\begin{align}
		\norm{\nabla \Lcal(\theta) - \nabla \Lcal^n (\theta)}^2
		& \le 2 \norm{ \sum_{j \in W_n} \frac{r_j - s_j^n}{\sqrt{s_j^n}} \sqrt{s_j^n} \nabla \Lcal_j(\theta) }^2 
		+ 2 \norm{ \sum_{j \notin W_n} r_j \nabla \Lcal_j(\theta)}^2 
		\\
		& \le 2 \left[\sum_{j \in W_n} \frac{(r_j - s_j^n)^2}{s_j^n}  \right] \norm{\sum_{j \in W_n} s_j^n \nabla \Lcal_j(\theta) }^2 
		+ 2  \norm{ \sum_{j \notin W_n} r_j  \nabla \Lcal_j(\theta) }^2 
%	& \le  \left[\sum_{j \notin W_n}  r_j\right] \sum_{j \notin W_n} r_j  [\Lcal_j(\theta^n) - \Lcal_j(\theta_j^*)] 
	\end{align}
	
	
	
\end{proof}

\begin{proof}	
	\begin{align}
	\norm{\nabla \Lcal (\theta)}^2
	& \le 2 \norm{\nabla \Lcal ( \theta) - \nabla \Lcal^n( \theta)}^2 
	+ 2 \norm{ \nabla \Lcal^n (\theta)}^2\\
	& \le \left[ 4 \chi^n + 2 \right] \norm{ \nabla \Lcal^n (\theta)}^2 
	+ 4  \norm{ \sum_{j \notin W_n} r_j  \nabla \Lcal_j(\theta) }^2 
	,
	%	\label{app:eq:U_1}
	\end{align}
	We define $B = \frac{1}{N}\sum_{i=0}^{N-1}B^n$. 
%	We define $\chi_{p ||q}^2 = \max_n \chi^n$.  
	Hence, using Theorem XX, we have:
	\begin{align}
	\frac{1}{N}\sum_{n=0}^{N-1} \norm{\nabla \Lcal (\theta^n)}^2
	& \le 
%	4L \left[\chi_{p ||q}^2 + 1\right] \epsilon_{opt}
	\epsilon
	+ \frac{1}{N}\sum_{n=0}^{N-1}\chi^n A^n 
	+ B \nonumber\\
	& + 4L \max_n\left[\left[\chi^n + 1\right]\frac{1}{\bar{q}^n}\right] 
	\min_x\left[ \frac{1}{N}  \sum_{n=0}^{N-1} \left[ \E{\Lcal^n(x)} - \Lcal^n(\tilde{\theta}^n) \right] \right]
	,
	%	\label{app:eq:U_1}
	\end{align}	
	
	\begin{align}
	\frac{1}{N}\sum_{n=0}^{N-1} \norm{\nabla \Lcal (\theta^n)}^2
	& \le 
	%	4L \left[\chi_{p ||q}^2 + 1\right] \epsilon_{opt}
	\epsilon
	+ \Ocal (\frac{1}{N}\sum_{n=0}^{N-1}\chi^n [\Lcal^n(\tilde{\theta}^n) -\sum_{j \in W_n} {q}_j^n \Lcal_j(\theta_j^*)])\nonumber\\
	& + \Ocal(\frac{1}{N}\sum_{n=0}^{N-1}\sum_{j \notin W_n} r_j [\Lcal_j(\theta^n) - \Lcal_j(\theta_j^*)]) \nonumber\\
	& + \Ocal(\min_x \{\frac{1}{N} \sum_{n=0}^{N-1} \left[ \E{\Lcal^n(x)} - \Lcal^n(\tilde{\theta}^n) \right]\} )
	\end{align}	
	
	

\end{proof}














==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/delayed_proofs/app_convergence_convexity.tex <==

\section{Convergence Guarantees Proofs}

\begin{table}
	\caption{Common Notation Summary.}
	\label{table:parameters}
	\centering
	\begin{tabular}{cc}
%		\toprule
		Symbol     & Description    \\
%		\midrule
		$C$ & Number of clients. \\
		$K$ & Number of local SGD.  \\
		$\eta_l$ & Local/Client learning rate.\\
		$\eta_g$ & Global/Server learning rate.\\
		$\tilde{\eta}$ & Effective learning rate, $\tilde{\eta} = \eta_l \eta_g$.\\
		
		$n$ & optimization round. \\
		$\theta^n$ & Global model at server iteration $n$.  \\
		$\tilde{\theta}$ & Optimum of the federated loss function, equation (\ref{eq:global_loss}). \\
		$\theta_i^{n+1}$ & Local update of client $i$ on model $\theta^n$.\\
		$y_{i, k}^n$ & Local model of client i after $k$ SGD updates ($y_{i, k}^n = \theta_i^{n+1}$ and $y_{i, 0}^{t} = \theta^n$). \\
		
		$p_i$ & Importance of client $i$ in the federated loss function, equation (\ref{eq:global_loss}).  \\
		$m$ & Maximum amount of clients the server can communicate with.\\
		$S_n$ & Set of participating clients considered at iteration $n$.\\
		$\omega_i(S_n)$ & Aggregation weight for client $i$ given $S_n$.\\
		$\alpha$ & Covariance parameter.\\
		$\delta_i, \delta_i^*$ & cf Section \ref{sec:convergence}\\
		$\gamma^*$ & Jensen gap upper bound parameter, cf Section \ref{sec:convergence}\\
		
		$n$ & time variable since the start of the learning process.\\
		$t^n$ & time at the aggregation $n$.\\
		$\rho_i(n)$ & expected computation time of client $i$. \\
		
		$\EE{n}{\cdot}$ & Expected value conditioned on $\theta^n$.\\
		$\Lcal(\cdot)$ & Federated loss function, equation \ref{eq:global_loss}\\
		$\Lcal_i(\cdot)$ & Local loss function of client $i$.\\
		$g_i(\cdot)$ & SGD. We have $\EE{\xi_i}{g_i(\cdot)} = \nabla \Lcal_i(\cdot)$ with Assumption \ref{ass:unbiased}.\\
		$\xi_i$ & Random batch of samples from client $i$ of size $B$.\\

		
		$L$ & Lipschitz smoothness parameter, Assumption \ref{ass:smoothness}.\\
		$\sigma^2$ & Uniform bound on the variance of the stochastic gradients, Assumption \ref{ass:unbiased}.\\
		$\beta$, $\kappa$ & Assumption \ref{ass:dissimilarity} parameters on the clients gradient bounded dissimilarity.\\
		$\mu$ & Strong convexity parameter. \\
		
%		$\rho_i(n)$ & step at which the server communicated to client $i$ its global model for local computation.\\
		
		
%		\bottomrule
	\end{tabular}
\end{table}


In Table \ref{table:parameters}, we provide the definition of the different notation used in this work.






\begin{equation}
\label{app:eq:SGD_process}
y_{i, k}^{\rho_i(n)} - \theta^{\rho_i(n)} 
= - \eta_l \sum_{l=0}^{k-1} g_i( y_{i, l}^{\rho_i(n)})
\end{equation}
By taking the expected value while considering Assumption \ref{ass:unbiased} we get:
\begin{equation}
\label{app:eq:E_SGD_process}
\E{y_{i, k}^{\rho_i(n)} - \theta^{\rho_i(n)}} 
= - \eta_l \sum_{ l = 0 }^{k - 1} \nabla \Lcal_i( y_{i, l}^{\rho_i(n)})
\end{equation}


By rewriting equation (\ref{eq:aggreg_SCAFFOLD_general}) with equation (\ref{app:eq:SGD_process}), we get:
\begin{align}
\label{app:eq:global_update_rewrote}
\theta^{n+1} - \theta^n
& = \eta_g \sum_{i=1}^n \omega_i^n \left[\theta_i^{\rho_i(n)+1} - \theta^{\rho_i(n)} \right] \\
& = -\tilde{\eta} \sum_{i=1}^n \omega_i^n \sum_{k=1}^{K} g_i( y_{i, k}^{\rho_i(n)})
\end{align}
We take the expected value of equation (\ref{app:eq:global_update_rewrote}). The aggregation weight $\omega_i^n$ is independent from the local work $\theta_i^{\rho_i(n)+1} - \theta^{\rho_i(n)}$. Hence, using equation (\ref{app:eq:E_expected_weight}) and (\ref{app:eq:E_SGD_process}), one gets:
\begin{equation}
\label{app:eq:E_global_update_rewrote}
\E{\theta^{n+1} - \theta^n}
= -\tilde{\eta} \sum_{i=1}^n q_i^n \sum_{k=1}^{K} \nabla \Lcal_i( y_{i, k}^{\rho_i(n)})
\end{equation}



%\input{./tex/Lemma_equality.tex}
\input{./tex/bounding_client_drift.tex}
\input{./tex/property_convex_functions.tex}
\input{./tex/convergence_convex.tex}


















%\subsection{Proof of Theorem \ref{theo:convergence}}\label{app:proof:convergence}
%
%\begin{proof}
%	
%	With Lemma \ref{lem:equality_update_without_Jenken}, we get:
%	\begin{align}
%	\EE{n}{\norm{\theta^{n+1} - \tilde{\theta}}^2} 
%	&\le \norm{\theta^n - \tilde{\theta}}^2 
%	\underbrace{- 2 \tilde{\eta} \inner{\sum_{k, i}d_i \nabla \Lcal_i(y_{i,k}^{\rho_i(n)})}{\theta^n - \tilde{\theta}}}_{T_1} \nonumber\\
%	&+ \underbrace{\eta_g^2 \sum_{i=1}^{n} \EE{n}{\omega_i^2} \EE{n}{\norm{\theta_i^{\rho_i(n) + 1} - \theta^{\rho_i(n)}}^2 }}_{T_2}. \label{app:eq:C_1}
%	\end{align}
%	
%	
%	
%	
%	\subsubsection*{Bounding $T_1$}
%	Using Lemma \ref{lem:perturbed_strong_convexity} with convex functions ($\mu = 0$), we can bound $T_1$ as :
%	\begin{align}
%	T_1 
%	&\le - 2 \tilde{\eta} \sum_{k, i}d_i \left[ \Lcal_i(\theta^n) - \Lcal_i(\tilde{\theta}) - L \norm{y_{i, k}^{\rho_i(n)} - \theta^n}^2
%	%			+ \frac{\mu}{4}\norm{\theta^n - \tilde{\theta}}^2
%	\right]\\
%	&\le - 2 \tilde{\eta} K \left[ \Lcal(\theta^n) - \Lcal(\tilde{\theta}) 
%	%			+ \frac{\mu}{4}\norm{\theta^n - \tilde{\theta}}^2
%	\right] 
%	+ 2 L \tilde{\eta} \sum_{i}d_i\sum_{k}\EE{n}{\norm{y_{i,k}^{\rho_i(n)} - \theta^n}^2},
%	\end{align}
%	where $\EE{n}{\norm{y_{i,k}^{\rho_i(n)} - \theta^n}^2}$ can be bounded using Lemma \ref{lem:bounded_drift_asynchronous}:
%	\begin{align}
%	T_1 
%	&\le - 2 \tilde{\eta} K\left[ \Lcal(\theta^n) - \Lcal(\tilde{\theta}) 
%	%		+ \frac{\mu}{4}\norm{\theta^n - \tilde{\theta}}^2
%	\right] 
%	+ 4 L \tilde{\eta} \eta_l^2 K^2 (\Delta \tau + 1) \left[ [\sigma^2 + 3 L^2 G^2 ][1 + \eta_g^2 \delta^{t, \Delta \tau}]  
%	+3 \rho
%	+ 3 \eta_g^2 \nu^t \right],
%	\label{app:eq:C_2}
%	\end{align}
%	where $\rho = \sum_{i=1}^{n} d_i \EE{\xi_i}{\norm{\nabla \Lcal_i (\tilde{\theta})}^2}$.
%	
%	
%	
%	
%	
%	
%	
%	\subsubsection*{Bounding $T_2$}
%	Using Lemma \ref{lem:bounded_drift_asynchronous}, we can rewrite $T_2$ as :
%	\begin{equation}
%	T_2
%	\le 2 \tilde{\eta}^2 K^2 (\Delta \tau + 1) \left[ \delta [\sigma^2 + 3 L^2 G^2 ][1 + \eta_g^2 \delta^{t, \Delta \tau}]  
%	+3 \epsilon 
%	+ 3 \eta_g^2 \delta  \nu^t \right], 
%	\label{app:eq:C_4}
%	\end{equation}
%	where we define $\delta_i  = \EE{n}{{\omega_i^n}^2}$, $\delta = \sum_{i=1}^{n}\delta_i$, and $\epsilon =\sum_{i=1}^{n}\delta_i \EE{\xi_i}{\norm{\nabla \Lcal_i(\tilde{\theta})}^2 }$. 
%	
%	
%	
%	
%	\subsubsection*{Bounding equation (\ref{app:eq:C_1})}
%	
%	
%	Substituting equation (\ref{app:eq:C_4}) and (\ref{app:eq:C_2}) in equation (\ref{app:eq:C_1}), we get:	
%	
%	\begin{align}
%	\EE{n}{\norm{\theta^{n+1} - \tilde{\theta}}^2} 
%	&\le \norm{\theta^n - \tilde{\theta}}^2 
%	- 2 \tilde{\eta} K\left[ \Lcal(\theta^n) - \Lcal(\tilde{\theta}) 
%	%	+ \frac{\mu}{4}\norm{\theta^n - \tilde{\theta}}^2
%	\right] \nonumber\\
%	& + 4 L \tilde{\eta} \eta_l^2 K^2 (\Delta \tau + 1) \left[ [\sigma^2 + 3 L^2 G^2 ][1 + \eta_g^2 \delta^{t, \Delta \tau}]  
%	+3 \rho
%	+ 3 \eta_g^2 \nu^t \right] \nonumber\\
%	&+ 2 \tilde{\eta}^2 K^2 (\Delta \tau + 1) \left[ \delta [\sigma^2 + 3 L^2 G^2 ][1 + \eta_g^2 \delta^{t, \Delta \tau}]  
%	+3 \epsilon 
%	+ 3 \eta_g^2 \delta  \nu^t \right]. 
%	\end{align}
%	
%	Finally, by rearranging the terms, we get:
%	\begin{align}
%	\E{\Lcal(\theta^n)} - \Lcal(\tilde{\theta}) 	
%	& \le \frac{1}{2 \tilde{\eta} K} \left[\E{\norm{\theta^n - \tilde{\theta}}^2} - \E{\norm{\theta^{n+1} - \tilde{\theta}}^2}  \right] \nonumber\\
%	& + 2 L \eta_l^2 K (\Delta \tau + 1) \left[ [\sigma^2 + 3 L^2 G^2 ][1 + \eta_g^2 \delta^{t, \Delta \tau}]  
%	+3 \rho
%	+ 3 \eta_g^2 \nu^t \right] \nonumber\\
%	&+ \tilde{\eta} K (\Delta \tau + 1) \left[ \delta [\sigma^2 + 3 L^2 G^2 ][1 + \eta_g^2 \delta^{t, \Delta \tau}]  
%	+3 \epsilon 
%	+ 3 \eta_g^2 \delta  \nu^t \right],
%	\label{app:eq:C_5}
%	\end{align}
%	
%	We note that we have:
%	\begin{align}
%	\delta = 
%	&\frac{1}{T+1}\sum_{t=0}^{T} \delta^{t, \Delta \tau}\\
%	& =  \frac{1}{T+1}\sum_{t=0}^{T}\sum_{s=0}^{\Delta \tau - 1} \delta^{t-s}\\
%	& \le \frac{1}{T+1}\sum_{t=0}^{T}\sum_{s=0}^{\Delta \tau - 1}  \sum_{i=1}^C \E{{\omega_i^{t-s}}^2}\\
%	& \le \frac{1}{T+1}\sum_{t=0}^{T}\Delta \tau \sum_{i=1}^C \E{{\omega_i^{t}}^2}
%	\label{app:eq:C_6}
%	\end{align}
%	Similarly, we have:
%	\begin{equation}
%	\nu
%	= \frac{1}{T+1 } \sum_{t=0}^{T} \nu^{t} 
%	\le \frac{\Delta \tau}{T+1}\sum_{t=0}^{T}  \sum_{i=1}^C \EE{n}{{\omega_i^n}^2}
%	\EE{\xi_i}{\norm{\nabla \Lcal_i(\tilde{\theta}) }^2}
%	\label{app:eq:C_7}
%	\end{equation}
%	Substituting equation (\ref{app:eq:C_6}) and equation (\ref{app:eq:C_7}) in equation (\ref{app:eq:C_5}) gives:
%	\begin{align}
%	\frac{1}{T+1} \sum_{t=0}^{T}\E{\Lcal(\theta^n)} - \Lcal(\tilde{\theta}) 	
%	& \le \frac{1}{2 \tilde{\eta} K(T+1)} \E{\norm{\theta^0 - \tilde{\theta}}^2} \nonumber\\
%	& + 2 L \eta_l^2 K (\Delta \tau + 1) \left[ [\sigma^2 + 3 L^2 G^2 ][1 + \eta_g^2 \delta]  
%	+3 \rho
%	+ 3 \eta_g^2 \nu \right] \nonumber\\
%	&+ \tilde{\eta} K (\Delta \tau + 1) \left[ \delta [\sigma^2 + 3 L^2 G^2 ][1 + \eta_g^2 \delta]  
%	+3 \epsilon 
%	+ 3 \eta_g^2 \delta  \nu \right]\\
%	& = \Ocal (\frac{1}{\tilde{\eta} K(T+1)}) \nonumber\\
%	& + \Ocal( \eta_l^2 K (\Delta \tau + 1) [1 + \eta_g^2 \delta])
%	+ \Ocal( \eta_l^2 K (\Delta \tau + 1) (\rho
%	+ \eta_g^2 \nu ))\nonumber\\
%	&+ \Ocal( \tilde{\eta} K (\Delta \tau + 1) \delta [1 + \eta_g^2 \delta] ) 
%	+ \Ocal (\tilde{\eta} K (\Delta \tau + 1) (\epsilon 
%	+ \eta_g^2 \delta  \nu )).
%	\end{align}
%	
%	
%	
%	
%	
%	
%\end{proof}




==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/delayed_proofs/app_convergence_without_convexity.tex <==
\section{No convexity}


\begin{proof}
	With the Lipschitz-smooth assumption \ref{ass:smoothness}, it follows:
	\begin{equation}
		\EE{n}{\Lcal^n(\theta^{n+1})} - \Lcal^n(\theta^n)
		\le \underbrace{\EE{n}{\inner{\nabla \Lcal^n(\theta^n)}{\theta^{n+1} - \theta^n}}}_A 
		+ \frac{L}{2}\underbrace{\EE{n}{\norm{\theta^{n+1} - \theta^n}^2}}_B
		\label{app:eq:M_0}
	\end{equation}	
	By construction, equation (\ref{eq:aggreg_SCAFFOLD_general}), we have $\theta^{n+1} - \theta^n =  \eta_g \sum_{i}\omega_i^n(\theta_i^{\rho_i(n) +  1} - \theta^{\rho_i(n)})$. The considered client sampling satisfies $\EE{n}{\omega_i^n} = q_i^n$ and the aggregation weight is independent of a client's local work. Therefore, $\EE{n}{\theta^{n+1} - \theta^n} = \eta_g \sum_{i} q_i^n \EE{n}{\theta_i^{\rho_i(n)+1} - \theta^{\rho_i(n)}}$. 
	\begin{align}
	A 
	&= \eta_g \inner{\nabla \Lcal^n(\theta^n)}{\sum_{i} q_i^n \EE{n}{\theta_i^{t+1} - \theta_i^{\rho_i(n)}}}
	\\
	&= - \tilde{\eta}\inner{\nabla \Lcal^n(\theta^n)}{\sum_{i, k} q_i^n \EE{n}{\nabla \Lcal^n_i(y_{k, i}^{\rho_i(n)})}}
	\\
	&= - K\bar{q}^n\tilde{\eta}\inner{\nabla \Lcal^n(\theta^n)}{\sum_{i, k} \frac{1}{\bar{q}^n} q_i^n \frac{1}{K}\EE{n}{\nabla \Lcal^n_i(y_{k, i}^{\rho_i(n)})}}
	\\
	&= - K\tilde{\eta} \bar{q}^n\frac{1}{2} 
	[\norm{\nabla \Lcal^n(\theta^n)}^2 
	+ \EE{n}{\norm{\sum_{i, k}\frac{1}{\bar{q}^n} q_i^n \frac{1}{K}\nabla \Lcal^n_i(y_{k, i}^{\rho_i(n)})}^2} \nonumber\\
	&- \underbrace{\EE{n}{\norm{\nabla \Lcal^n(\theta^n) - \sum_{i, k} \frac{1}{\bar{q}^n} q_i^n\frac{1}{K} \nabla \Lcal^n_i(y_{k, i}^{\rho_i(n)})}^2}}_C]
	\\
	&\le - K\tilde{\eta} \bar{q}^n\frac{1}{2} 
	[\norm{\nabla \Lcal^n(\theta^n)}^2 
	+ H^2 - C ],
	\label{app:eq:M_1}
	\end{align}
	where the second equality comes from XXX and the last inequality comes from using $2 \inner{a}{b} = \norm{a}^2 + \norm{b}^2 - \norm{a-b}^2$.
	
	
	\begin{align}
		C 
		&=  \EE{n}{\norm{\sum_{i} \frac{1}{\bar{q}^n} q_i^n [\nabla \Lcal_i(\theta^n) - \sum_{k}\frac{1}{K} \nabla \Lcal_i(y_{k, i}^{\rho_i(n)})]}^2}
		\\
%		& \le \sum_{i} q_i^n  \EE{n}{\norm{ \sum_{k}\frac{1}{K} [\nabla \Lcal_i(\theta^n) - \nabla \Lcal_i(y_{k, i}^{\rho_i(n)}) ] }^2}\\
		& \le \sum_{k, i} \frac{1}{\bar{q}^n}q_i^n  \frac{1}{K}\EE{n}{\norm{ \nabla \Lcal_i(\theta^n) - \nabla \Lcal_i(y_{k, i}^{\rho_i(n)}) }^2}\\
		& \le \sum_{k, i} \frac{1}{\bar{q}^n} q_i^n  \frac{1}{K} L^2 \EE{n}{\norm{ \theta^n - y_{k, i}^{\rho_i(n)} }^2}
		\\
		& = \sum_{i} \frac{1}{\bar{q}^n} q_i^n  L^2 \left[ (\Delta \tau + 1 ) (\eta_l^2 K^2 (\sigma^2 + H^2 )) + (\Delta \tau + 1 ) \eta_g^2 \beta(n) (\eta_l^2 K^2 (\sigma^2 + H^2 )) \right]
		\\
		& = L^2 (\Delta \tau + 1 ) (\eta_l^2 K^2 (\sigma^2 + H^2 )) ( 1 + \eta_g^2 \beta(n) )
		\label{app:eq:M_2}
	\end{align}
	
	
	
	
	
	
	
	
	\begin{align}
		B 
		& = \EE{n}{\norm{\theta^{n+1} - \theta^n}^2}
		\\
		&  \le \eta_g^2 \sum_{i=1}^{C}\beta_i^n \EE{n}{\norm{\theta_i^{\rho_i(n)+1} - \theta_i^{\rho_i(n)}}^2}
		\\
		&  \le \tilde{\eta}^2 \sum_{i=1}^{C}\beta_i^n \EE{n}{\norm{\sum_{k=0}^{K-1} g_i(y_{i, k}^{\rho_i(n)})}^2}
		\\
		&  \le \tilde{\eta}^2 \sum_{i=1}^{C}\beta_i^n \left[ K \sigma^2 + \EE{n}{\norm{\sum_{k=0}^{K-1} \nabla \Lcal_i(y_{i, k}^{\rho_i(n)})}^2} \right]
		\\
		&  \le \tilde{\eta}^2 \sum_{i=1}^{C}\beta_i^n 
		\left[ K \sigma^2 
		+ K H^2\right]
		\label{app:eq:M_3}
	\end{align}
	where the last inequality comes from using Assumption \ref{ass:unbiased}.
	
	Substituting equation (\ref{app:eq:M_2}) and equation (\ref{app:eq:M_3}) in equation (\ref{app:eq:M_0}), we get:
	\begin{equation}
		\EE{n}{\Lcal^n(\theta^{n+1})} - \Lcal^n(\theta^n)
		\le \EE{n}{\inner{\nabla \Lcal^n(\theta^n)}{\theta^{n+1} - \theta^n}}
		+ \frac{L}{2}\EE{n}{\norm{\theta^{n+1} - \theta^n}^2}
	\end{equation}
	
	
	
	
	
	
	
	
\end{proof}

==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/delayed_proofs/bounding_Q.tex <==


\begin{lemma}\label{lem:bound_Q}
	Under Assumption \ref{ass:smoothness} and \ref{ass:unbiased}, 
	considering that $\gamma_i(n) \le \beta q_i(n)$, 
	and considering $12 \rho^2 \left[ \alpha + \beta\right]  \tilde{\eta}^2 K^2 \tau^2 L^2
	\le 1/2$, we have
	\begin{align}
	\bar{Q}(N)
	& \le
	24 \rho \left[2 \alpha + \beta \right] \tilde{\eta}^2 K^2 L \bar{Z}(N)
	+ 6  \rho^2 \left[ \alpha D + 2 \beta \right] \tilde{\eta}^2 K^2 \Sigma_1(N)
	+ 12  \rho^2 \alpha \tilde{\eta}^2 K^2  \Sigma_2(N) 
	.
	\end{align}
	
\end{lemma}


\begin{proof}
	Considering the proof of Lemma \ref{lemma:one_SGD}, using the fact that $\gamma_i(n) \le \beta q_i(n)$, and Jensen inequality, we have	
	\begin{align}
	Q(n)
	&\le 
	q^2(n) \alpha  \tilde{\eta}^2 \E{\norm{\sum_{ i = 1 }^M \tilde{q}_i(n)\sum_{ k = 0 }^{K-1} g_i(\vtheta_i^{\rho_i(n), k}) }^2}
	+ q(n) \beta  \tilde{\eta}^2 \sum_{ i = 1 }^M \tilde{q}_i(n) \E{\norm{\sum_{ k = 0 }^{K-1} g_i(\vtheta_i^{\rho_i(n), k})}^2}
	\nonumber\\
	&\le 
	q^2(n) \alpha  \tilde{\eta}^2 K^2 R(n)
	+ q(n) \beta  \tilde{\eta}^2 K^2 S(n)
%	=\tilde{\eta}^2  Q(n)
	%	\label{app:eq:Q}
	\end{align}
	Using Lemma \ref{lem:bounding_R} to bound $R(n)$ and Lemma \ref{lem:phi_nk} to bound $S(n)$, we can thus bound $Q(n)$ with the previous global model distances to the optimum $Q(s)$, where $ \max(0, n - \tau) \le s \le n -1$, we thus have 	
	\begin{align}
	\frac{1}{\rho \tilde{\eta}^2 K^2}Q(n)
	& \le 12 \rho  \left[\alpha + \beta\right] \tau L^2 \sum_{ s = 1 }^\tau Q(n - s)
	+ 12 \left[2 \alpha + \beta \right] L Z(n)
	\nonumber\\
	& 
	+ 3 \rho  \left[ \alpha D + 2 \beta \right] \sigma_1(n)
	+ 6 \rho  \alpha \sigma_2(n) 
	.\label{app:eq:J1}
	\end{align}
	We can thus define $A(n)$ and $B(n)$ such that the bound of of equation (\refeq{app:eq:J1}) can be rewritten as in equation (\refeq{app:eq:rewriting}),  with its associated implications when taking the mean over $N$, reordering, and considering that $\tau A(n) \le 1/2$:
	\begin{align}
	Q(n)
	\le A(n) \sum_{ s = 1 }^\tau Q(n -s) 
	+ B(n)
	\Rightarrow
	\bar{Q}(N) 
	= \frac{1}{N}\sum_{ n = 0 }^{N-1} Q(n)
	\le 2 \frac{1}{N}  \sum_{ n = 0 }^{N-1} B(n)
	.
	\label{app:eq:rewriting}
	\end{align}
	Therefore, considering $12 \rho^2 \left[ \alpha + \beta\right]  \tilde{\eta}^2 K^2 \tau^2 L^2
	\le 1/2$ completes the proof.
	
%	\begin{align}
%	\bar{Q}(N)
%	& \le
%	24 L \left[2 \alpha + \beta \right] \rho \tilde{\eta}^2 K^2 \bar{Z}(N)
%	+ 6  \rho^2\tilde{\eta}^2 K^2\left[ \alpha D + 2 \beta \right] \Sigma_1(N)
%	+ 12  \rho^2\tilde{\eta}^2 K^2 \alpha \Sigma_2(N) 
%	\end{align}
	
\end{proof}



%\begin{proof}
%	Considering the proof of Lemma \ref{lemma:one_SGD}, using the fact that $\gamma_i(n) \le \beta q_i(n)$, and Jensen inequality, we have	
%	\begin{align}
%	Q(n)
%	&\le 
%	\tilde{\eta}^2  \alpha q^2(n)\E{\norm{\sum_{ i = 1 }^M \tilde{q}_i(n)\sum_{ k = 0 }^{K-1} g_i(\vtheta_i^{\rho_i(n), k}) }^2}
%	+ \tilde{\eta}^2 \beta q(n) \sum_{ i = 1 }^M \tilde{q}_i(n) \E{\norm{\sum_{ k = 0 }^{K-1} g_i(\vtheta_i^{\rho_i(n), k})}^2}
%	\nonumber\\
%	&\le 
%	\tilde{\eta}^2  \alpha q^2(n)K^2 R(n)
%	+ \tilde{\eta}^2 \beta q(n) K^2 S(n)
%%	\label{app:eq:Q}
%	\end{align}
%	Using Lemma \ref{lem:bounding_R} to bound $R(n)$ and Lemma \ref{lem:phi_nk} to bound $S(n)$, we can thus bound $Q(n)$ with the previous global model distances to the optimum $Q(s)$, where $ \max(0, n - \tau) \le s \le n -1$, we thus have 	
%	\begin{align}
%	\frac{1}{\rho q(n)\tilde{\eta}^2 K^2}Q(n)
%	& \le 12  L^2 \left[\alpha + \beta\right] \tau \sum_{ s = 1 }^\tau Q(n - s)
%	+ 12 L \left[2 \alpha + \beta \right] q^{-1}(n) Z(n)
%	\nonumber\\
%	& 
%	+ 3  \left[ \alpha D + 2 \beta \right] \sigma_1(n)
%	+ 6  \alpha \sigma_2(n) 
%	.\label{app:eq:J1}
%	\end{align}
%	We can thus define $A(n)$ and $B(n)$ such that the bound of of equation (\refeq{app:eq:J1}) can be rewritten as in equation (\refeq{app:eq:rewriting}),  with its associated implications when taking the mean over $N$, reordering, and considering that $\tau A(n) \le 1/2$:
%	\begin{align}
%		Q(n)
%		\le A(n) \sum_{ s = 1 }^\tau Q(n -s) 
%		+ B(n)
%		\Rightarrow
%		\bar{Q}(N) 
%		= \frac{1}{N}\sum_{ n = 0 }^{N-1} Q(n)
%		\le 2 \frac{1}{N}  \sum_{ n = 0 }^{N-1} B(n)
%		.
%		\label{app:eq:rewriting}
%	\end{align}
%	Therefore, considering 
%	$12 \rho^2 \tilde{\eta}^2 K^2 L^2 \left[\alpha + \beta\right] \tau^2
%	\le 1/2$ completes the proof.
%	
%	\begin{align}
%	\bar{Q}(N)
%	& \le
%	24 L \left[2 \alpha + \beta \right] \rho \tilde{\eta}^2 K^2 \bar{Z}(N)
%	+ 6  \rho^2\tilde{\eta}^2 K^2\left[ \alpha D + 2 \beta \right] \Sigma_1(N)
%	+ 12  \rho^2\tilde{\eta}^2 K^2 \alpha \Sigma_2(N) 
%	\end{align}
%
%\end{proof}





==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/delayed_proofs/bounding_R.tex <==
\begin{lemma}\label{lem:bounding_R}
	Under Assumption \ref{ass:smoothness} and \ref{ass:unbiased}, and 
	considering $D \le 1/2$, we have
	\begin{align}
	R(n)
	&\le 12 L^2 \tau \sum_{s=1}^\tau  Q(n - s) 
	+ 24 L q^{-1}(n) Z(n)
	+ 3 D \sigma_1(n)
	+ 6  \sigma_2(n) 
	.
	\end{align}
	
\end{lemma}


\begin{proof}
	\begin{align}
	R(n, k)
	&\le 3 \E{\norm{\sum_{ i = 1 }^M \tilde{q}_i(n)\left[ g_i(\vtheta_i^{\rho_i(n), k}) - \nabla \Lcal_i(\vtheta^{n, k}, \vxi_{i, k}^{\rho_i(n)}) \right]}^2}
	\nonumber\\
	&+ 3  \E{\norm{\sum_{ i = 1 }^M \tilde{q}_i(n) \left[\nabla \Lcal_i(\vtheta^{n, k}, \vxi_i) - \nabla \Lcal_i(\vtheta^{n, k})\right]}^2}
	\nonumber\\
	& + 3 \E{\norm{\sum_{ i = 1 }^M \tilde{q}_i(n) \nabla \Lcal_i(\vtheta^{n, k})}^2}
	\label{app:eq:S1}
	.
	\end{align}
	We respectively call the three terms of equation (\refeq{app:eq:S1}), $a(n , k)$, $b(n, k)$, and $c(n, k)$.
	Using the local loss functions Lipschitz smoothness, Assumption \ref{ass:smoothness}, and Jensen inequality, we can bound $a(n, k)$ as
	\begin{equation}
	a(n, k)
	\le 3\sum_{ i = 1 }^M \tilde{q}_i(n)\E{\norm{ g_i(\vtheta_i^{\rho_i(n), k}) - \nabla \Lcal_i(\vtheta^{n, k}, \vxi_{i, k}^{\rho_i(n)}) }^2}
	\le 3 L^2 \phi(n, k)
	\label{app:eq:S1_1}
	.
	\end{equation}
	Using the unbiasedness of the gradient estimator, Assumption \ref{ass:unbiased}, and the local loss function  Lipschitz smoothness, Assumption \ref{ass:smoothness}, we can bound $b(n, k)$ as
	\begin{align}
	b(n, k)
	&=  3\sum_{ i = 1 }^M \tilde{q}_i^2(n)\E{\norm{ \nabla\Lcal_i(\vtheta^{n, k}, \vxi_i) - \nabla \Lcal_i(\vtheta^{n, k})}^2}
	\\
	& \le  3\sum_{ i = 1 }^M \tilde{q}^2_i(n)\E{\norm{ \nabla\Lcal_i(\vtheta^{n, k}, \vxi_i) }^2}
	\\
	& \le  6 \sum_{ i = 1 }^M \tilde{q}^2_i(n)
	\left[\E{\norm{ \nabla\Lcal_i(\vtheta^{n, k}, \vxi_i) - \nabla\Lcal_i(\bar{\vtheta}^n, \vxi_i)}^2}
	+ \E{\norm{ \nabla\Lcal_i(\bar{\vtheta}^n, \vxi_i)}^2}
	\right]
	\\
	& \le 12 L \max_i (\tilde{q}_i(n)) \left[\tilde{\Lcal}^n(\vtheta^{n, k}) - \tilde{\Lcal}^n(\bar{\vtheta}^n)\right]
	+ 6  \sum_{ i = 1 }^M \tilde{q}_i^2(n)\E{\norm{ \nabla\Lcal_i(\bar{\vtheta}^n, \vxi_i))}^2}
	.
	\label{app:eq:S1_2}
	\end{align}
	
	Using the Lipschitz smoothness of the local loss functions, Assumption \ref{ass:smoothness} and Jensen inequality, we can bound $c(n, k)$ as
	\begin{align}
	c(n , k)
	\le  3 \E{\norm{\nabla \tilde{\Lcal}^n(\vtheta^{n, k}) - \nabla \tilde{\Lcal}^n(\bar{\vtheta}^n)}^2}
	\le 6 L \left[\tilde{\Lcal}^n(\vtheta^{n, k}) - \tilde{\Lcal}^n(\bar{\vtheta}^n)\right]
	\label{app:eq:S1_3}
	.
	\end{align}
	Substituting equation (\refeq{app:eq:S1_1}), equation (\refeq{app:eq:S1_2}), and equation (\refeq{app:eq:S1_3}) in equation (\refeq{app:eq:S1}),
	considering that 
	$ \max_i (\tilde{q}_i(n)) \le 1$, 
	 and summing over $K$
	 gives
	\begin{align}
	R(n)
	&\le 3  L^2 \phi(n)
	+ 18 L q^{-1}(n) Z(n)
	+ 6  \sigma_2(n) 
	\end{align}
	Using Lemma \ref{lem:phi_nk} to replace $\phi(n)$, and considering that $D \le 1 /2 < 1$ completes the proof.
%	\begin{align}
%	R(n)
%	&\le 12 L^2 \tau \sum_{s=1}^\tau  Q(n - s) 
%	+ 24 L q^{-1}(n) Z(n)
%	+ 3 D \sigma_1(n)
%	+ 6  \sigma_2(n) 
%	\label{app:eq:R2f}
%	\end{align}
	
\end{proof}

==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/delayed_proofs/bounding_client_drift.tex <==
\begin{lemma}\label{lem:phi_nk}
	
	Under Assumption \ref{ass:unbiased} and \ref{ass:smoothness}, and $D \coloneqq 6 \eta_l^2 (K-1)^2 L^2 \le 1/2$, we have
	\begin{align}
	\phi(n)
	&\le  4 q(n) \tau \sum_{s=1}^\tau  Q(n - s) 
	+ 4 D \frac{1}{L} q^{-1}(n) Z(n)
	+ 6 \eta_l^2 (K-1)^2 \sigma_1(n)
	,
	\end{align}
	\begin{align}
	\text{and } S(n)
	\le 12 q(n) L^2 \tau \sum_{ s = 1 }^\tau Q(n - s)
	+ 12 L q^{-1}(n) Z(n)
	+ 6 \sigma_1(n)
	.
	\end{align}
\end{lemma}

\begin{proof}
	Let us decompose the difference $\vtheta_i^{\rho_i(n), k} - \vtheta^{n,k}$ as
	\begin{equation}
		\vtheta_i^{\rho_i(n), k} - \vtheta^{n,k}
		= \left[\vtheta^{\rho_i(n)} - \eta_l\sum_{ l = 0 }^{k-1} g_i(\vtheta_i^{\rho_i(n), l})\right]
		- \left[\vtheta^n - \eta_l\sum_{ l = 0 }^{k-1}\sum_{ i = 1 }^M \tilde{q}_i(n) g_i(\vtheta_i^{\rho_i(n), l})\right]
	.
	\end{equation}
	Using Jensen inequality, we split the difference between the global models and the one between the gradients to get
	\begin{equation}
	\norm{\vtheta_i^{\rho_i(n), k} - \vtheta^{n,k}}^2
	\le  2 \norm{\vtheta^{\rho_i(n)} - \vtheta^n}^2
	+ 2 \eta_l^2 k \sum_{ l = 0 }^{k-1}\norm{ g_i(\vtheta_i^{\rho_i(n), l})
	- \sum_{ i = 1 }^M \tilde{q}_i(n) g_i(\vtheta_i^{\rho_i(n), l})}^2
	.
	\label{app:eq:O1}
	\end{equation}
	Therefore, by taking the expectations of equation (\refeq{app:eq:O1}) and summing over $M$ gives
	\begin{align}
	\phi(n , k)
	&\le  2 \sum_{ i = 1 }^M \tilde{q}_i(n) \E{\norm{\vtheta^{\rho_i(n)} - \vtheta^n}^2}
	\nonumber\\
	& + 2 \eta_l^2 k \sum_{ l = 0 }^{ k - 1} \sum_{ i = 1 }^M \tilde{q}_i(n)\E{\norm{ g_i(\vtheta_i^{\rho_i(n), l})
		- \sum_{ i = 1 }^M \tilde{q}_i(n) g_i(\vtheta_i^{\rho_i(n), l})}^2}
	\\
	&\le  2 \sum_{ i = 1 }^M \tilde{q}_i(n) \E{\norm{\vtheta^{\rho_i(n)} - \vtheta^n}^2} 
	+ 2 \eta_l^2 k \sum_{ l = 0 }^{k-1}\sum_{ i = 1 }^M \tilde{q}_i(n)\E{\norm{ g_i(\vtheta_i^{\rho_i(n), l})}^2}
	\label{app:eq:O2}
	,
	\end{align}
	where we see that $S(n, l)$ appears in the second term of equation (\refeq{app:eq:O2}). We consider now bounding $S(n , k)$, and first note that a stochastic gradient can be bounded as follow
	\begin{align}
	\E{\norm{g_i(\vtheta_i^{\rho_i(n), k})}^2}
	& \le 3 \E{\norm{\nabla \Lcal_i(\vtheta_i^{\rho_i(n),k}, \vxi_{i, k}^{\rho_i(n)}) - \nabla \Lcal_i(\vtheta^{n,k}, \vxi_{i, k}^{\rho_i(n)}) }^2} 
	\nonumber\\
	&+ 3 \E{\norm{\nabla \Lcal_i(\vtheta^{n,k}, \vxi_i) - \nabla \Lcal_i(\bar{\vtheta}^n, \vxi_i) }^2} 
	+ 3 \E{\norm{\nabla \Lcal_i(\bar{\vtheta}^n, \vxi_i) }^2} 
	.
	\label{app:eq:F_0}
	\end{align}
	When summing equation (\refeq{app:eq:F_0}) over $M$, and considering the clients loss functions Lipschitz smoothness, Assumption \ref{ass:smoothness}, we have
	\begin{align}
	S(n, k)
	=	\sum_{ i = 1 }^M \tilde{q}_i(n)\E{\norm{g_i(\vtheta_i^{\rho_i(n), k})}^2}
	\le 3 L^2 \phi(n , k)
	+ 6 L q^{-1}(n)Z(n , k)
	+ 3  \sigma_1(n)
	.
	\label{app:eq:F_11}
	\end{align}
	We also note the following intermediary results 
	\begin{equation}
	\sum_{ k = 0 }^{K-1} k \sum_{ l = 0 }^{k-1}x_l
	\le (K-1)\sum_{ k = 1 }^{K-1} \sum_{ l = 0 }^{k-1}x_l
	\le (K - 1)^2 \sum_{ k = 0 }^{K-2}x_k
	\le (K - 1)^2 \sum_{ k = 0 }^{K-1}x_k
	\label{app:eq:O3}
	.
	\end{equation}
	We substitute equation (\refeq{app:eq:F_11}) in equation (\refeq{app:eq:O2}) such that $D$ appears, take the mean over $K$ to introduce $\phi(n)$ on the two sides of the equation, and use equation (\refeq{app:eq:O3}). We have
	\begin{align}
	\phi(n)
	\le  2 \sum_{ i = 1 }^M \tilde{q}_i(n) \E{\norm{\vtheta^{\rho_i(n)} - \vtheta^n}^2} 
	+ D \phi(n) 
	+ 2 D \frac{1}{L} q^{-1}(n) Z(n)
	+ 6 \eta_l^2 (K-1)^2 \sigma_1(n)
	.
	\label{app:eq:phin}
	\end{align}
	Finally, reminding that $D \le 1/2$, which gives $1 - D \ge 1/2$, and 
	using Assumption \ref{ass:answering_time} to bound $\E{\norm{\vtheta^{\rho_i(n)} - \vtheta^n}^2}$  with Jensen inequality completes the first claim for $\phi(n)$, i.e.
	\begin{equation}
		\E{\norm{\vtheta^{\rho_i(n)} - \vtheta^n}^2}
		\le \tau \sum_{s=1}^\tau \E{\norm{\vtheta^{n - s+1 } - \vtheta^{n - s}}^2}
		= \tau \sum_{s=1}^\tau  Q(n - s)
		.
	\end{equation}
	
	Substituting the close-form of $\phi(n)$ in equation (\refeq{app:eq:F_11}) completes the claim for $S(n , k)$. 
	
	
	
	
\end{proof}






==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/delayed_proofs/common_ground.tex <==
We provide the following basic inequalities used in our proofs.

Let us consider $f$ a $L$-Lipschitz smooth and convex function with optimum $\vx^*$. 
For any vector $\vx$ and $\vy$, we have
\begin{equation}
\norm{\nabla f (\vx)}^2
\le 2 L [f(\vx) - f(\vx^*)]
,
\text{ and }
\norm{\nabla f (\vx) - \nabla f (\vy) }^2
\le L^2 \norm{\vx - \vy}^2
\label{app:eq:lipschitz}
.
\end{equation}

Let us consider $g$ a convex function and $d$ vectors $\{\vx_k\}$ each with importance $p_k$ such that $\sum_{ k = 1 }^d p_k = 1$. With Jensen inequality, we have
\begin{equation}
	g(\sum_{ k = 1 }^d p_k \vx_k) 
	\le \sum_{k=1}^d p_k g(\vx_k)
	.
\end{equation}

Let us consider the random variable $X$, we have
\begin{equation}
	\E{\norm{X - \E{X}}^2}
	\le \E{\norm{X}^2}
	.
\end{equation}


==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/delayed_proofs/constraints_lr.tex <==
The constraints on the learning rate can be summarized as 
$D = 6 \eta_l^2 (K-1)^2 L^2 \le 1/2$ (Lemma \ref{lem:phi_nk}),
$12 \rho^2 \left[ \alpha + \beta\right]  \tilde{\eta}^2 K^2 \tau^2 L^2
\le 1/2$ (Lemma \ref{lem:bound_Q}),
$3 \rho  \left[\alpha + \beta\right] \tilde{\eta} L \le 1$ (Theorem \ref{theo:convergence_convex}),
$2 
- 4 D 
- 12 \rho \left[2 \alpha + \beta \right] \left[\tilde{\eta} + \nu \tilde{\eta}^2 K^2 \tau^2 \right] L
\ge 1$ (Theorem \ref{theo:convergence_convex}),
$3 \rho^2 \tilde{\eta} L \le 1$ (Theorem \ref{theo:convergence_convex}), 
and $48 \rho^3 \tilde{\eta}^2 K^2 \tau^2 L^2 \le1$ (Theorem \ref{theo:convergence_convex}).

We note that $\alpha \le 1$, and $\beta \le 1$. We thus propose the following sufficient conditions to satisfy the conditions above
\begin{align}
	48 \eta_l^2 (K-1)^2 L^2 \le 1,
	144 \rho^2 \tilde{\eta} L \le 1,
	\text{ and }
	2304 \rho^3 \tilde{\eta}^2 K^2 \tau^2 L^2 \le 1
	,
\end{align}
which can further be simplified with
\begin{equation}
	\eta_l
	\le \frac{1}{48 K L }
	\min \left(1, \frac{1}{3 \rho^{2} \eta_g (\tau+1)}\right)
	.
\end{equation}

==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/delayed_proofs/convergence_convex.tex <==
\subsection{Proof of Theorem \ref{theo:convergence_convex}}\label{sec:app:proof:convergence}

\begin{proof}
	Equation (\ref{eq:FedAvg_one_server_iteration_bound})
	\begin{align}
	\E{\norm{\vtheta^{n+1} - \vx}^2} 
	&= \E{ \norm{\vtheta^n - \vx}^2 }
	\underbrace{- 2 \eta_g \E{ \inner { \sum_{i=1}^M q_i(n) \E{\vtheta_i^{\rho_i(n)+1} - \vtheta^{\rho_i(n)}} }{x - \vtheta^n} }}_{T_1}
	+ \tilde{\eta}^2 Q(\vtheta^n)
%	\nonumber\\
%	&+ \underbrace{\eta_g^2 \sum_{i=1}^M \beta_i^n \E{\norm{\vtheta_i^{\rho_i(n) + 1} - \vtheta^{\rho_i(n)}}^2}}_{T_2},
	\label{app:eq:C_1}
	\end{align}
	
	
	
	
	\subsubsection*{Bounding $T_1$}
	\begin{align}
	T_1 
	& = - 2 \tilde{\eta} \sum_{i=1}^M q_i(n) \sum_{k=0}^{K-1}  \underbrace{\E{ \inner { \nabla \Lcal_i (\vy_{i, k}^{\rho_i(n)}) }{\vx - \vtheta^n} }}_{T_2}
%	\\
	\end{align}
	
	\begin{align}
	T_2 
	& = \E{ \inner { \nabla \Lcal_i (\vy_{i, k}^{\rho_i(n)}) }{\vx - y_{i, k}^{\rho_i(n)}} }
	\nonumber\\
	& + \E{ \inner { \nabla \Lcal_i (\vy_{i, k}^{\rho_i(n)}) }{y_{i, k}^{\rho_i(n)} - \vtheta^{\rho_i(n)}} }
	\nonumber\\
	& + \E{ \inner { \nabla \Lcal_i (\vy_{i, k}^{\rho_i(n)}) }{\vtheta^{\rho_i(n)} - \vtheta^n} }
	\end{align}
	
	Using Cauchy Schwartz inequality and AM-GM inequality, we have
	\begin{equation}
		- 2 \inner{\va}{\vb} 
		\le 2 \sqrt{\norm{\va}^2\norm{\vb}^2}
		= 2 \sqrt{\frac{1}{\tilde{\eta}}\norm{\va}^2 \tilde{\eta} \norm{\vb}^2}
		\le \left[ \frac{1}{\tilde{\eta}}\norm{\va}^2 + \tilde{\eta} \norm{\vb}^2\right] 
	\end{equation}
	Also, the strong convexity of $\Lcal_i$ gives us:
	\begin{equation}
		\inner { \nabla \Lcal_i (\vy_{i, k}^{\rho_i(n)}) }{\vx - y_{i, k}^{\rho_i(n)}} 
		\ge \Lcal_i(\vy_{i, k}^{\rho_i(n)}) - \Lcal_i(\vx) + \frac{\mu}{2}\norm{\vy_{i, k}^{\rho_i(n)} - \vx}^2
	\end{equation}
	
	\begin{align}
	T_1 
	& \le - 2 \tilde{\eta} \sum_{i=1}^M q_i(n) \sum_{k=0}^{K-1} 
	\E{
	\Lcal_i(\vy_{i, k}^{\rho_i(n)}) - \Lcal_i(\vx) + \frac{\mu}{2}\norm{\vy_{i, k}^{\rho_i(n)} - \vx}^2
}
	\nonumber\\
	& + \sum_{i=1}^M q_i(n) \sum_{k=0}^{K-1}
	\E{
	2 \tilde{\eta}^2 \norm{\nabla \Lcal_i (\vy_{i, k}^{\rho_i(n)})}^2 
	+  \norm{y_{i, k}^{\rho_i(n)} - \vtheta^{\rho_i(n)}}^2 
	+ \norm{\vtheta^{\rho_i(n)} - \vtheta^n}^2
}
	%	\\
	\end{align}
	


	
	
	
	\subsubsection*{Bounding $T_2$}
	Using Lemma \ref{lem:bounded_drift_convex}, we can rewrite $T_2$ as :	
%	\begin{align}
%	T_2
%	&\le 2\tilde{\eta}^2  (H +  1) K^2 \underbrace{ \sum_{i=1}^{C}\beta_i^n \phi_i(x)}_{U^n}\nonumber\\
%	& + 2 \tilde{\eta}^2  (H +  1) K^2  \eta_g^2 H \underbrace{\left[\sum_{i=1}^{C}\beta_i^n \right]\frac{1}{\max(H, 1)}\sum_{s=0}^{H - 1} \sum_{i=1}^{C} \beta_i^{n-s}
%	\phi_i(x)}_{V^n} 
%	,
%	\label{app:eq:C_4}
%	\end{align}
%
	\begin{align}
	T_2
	&\le 2 \tilde{\eta}^2 K^2 \underbrace{\sum_{i=1}^{C} \beta_i^n \phi_i(x)}_{U^n}
	,
	\label{app:eq:C_4}
	\end{align}
	
	
	
	\subsubsection*{Bounding equation (\ref{app:eq:C_1})}
	
	
	Substituting equation (\ref{app:eq:C_4}) and (\ref{app:eq:C_2}) in equation (\ref{app:eq:C_1}), we get:	
	\begin{align}
	\E{\norm{\vtheta^{n+1} - \vx}^2} 
	&\le \E{ \norm{\vtheta^n - \vx}^2 }
	- 2 \tilde{\eta} K  \E{ \Lcal^n(\vtheta^n) - \Lcal^n(x) 
	%	+ \frac{\mu}{4}\norm{\vtheta^n - \vx}^2
	}\nonumber\\
	&+ 2 \tilde{\eta} (H +  1) \eta_l^2 K^3 [R^n + \eta_g^2 H S^n] 
	+ 2 \tilde{\eta}^2  K^2 U^n . 
	\end{align}	

	Finally, by rearranging the terms, we get:
	\begin{align}
	\E{\Lcal^n(\vtheta^n)} - \Lcal^n(x) 	
	& \le \frac{1}{2  \tilde{\eta} K} \left[\E{\norm{\vtheta^n - \vx}^2} - \E{\norm{\vtheta^{n+1} - \vx}^2}  \right] \nonumber\\
	&+ (H +  1) \eta_l^2 K^2 [R^n + \eta_g^2 H S^n ]  
	+ \tilde{\eta}  K . 
	\label{app:eq:C_5}
	\end{align}

	Summing over $N$ gives:
	\begin{align}
	\frac{1}{N} \sum_{n=0}^{N-1} \left[ \E{\Lcal^n(\vtheta^n)} - \Lcal^n(x) \right]	
	& \le \frac{1}{2 \tilde{\eta} K N} \E{\norm{\vtheta^0 - \vx}^2} \nonumber\\
	& + (H +  1) \eta_l^2 K^2 \frac{1}{N} \sum_{n=0}^{N-1} [R^n + \eta_g^2 H S^n ] 
	+ \tilde{\eta}   K \frac{1}{N} \sum_{n=0}^{N-1} U^n  
	\\
	& = \Ocal(\frac{1}{\tilde{\eta} K N})
	+\Ocal[(H +  1) \eta_l^2 K^2] 
	+ \Ocal[\tilde{\eta}^2  (H +  1)H  K ]
	+\Ocal[\tilde{\eta} K] 
	\label{app:eq:R_1}
	.
	\end{align}
	
	We note that the result in equation (\ref{app:eq:R_1}) works for any model $x$. FL is a succession of minimization problems $\Lcal^n$ with respective optimum $\tilde{\vtheta}^n$. 
	As a result, we have:
	\begin{align}
	\frac{1}{N} \sum_{n=0}^{N-1} \left[ \E{\Lcal^n(\vtheta^n)} - \Lcal^n(\tilde{\vtheta}^n) \right]
	& \le \frac{1}{N} \sum_{n=0}^{N-1} \left[ \E{\Lcal^n(x)} - \Lcal^n(\tilde{\vtheta}^n) \right]
	 + \Ocal(\frac{1}{\tilde{\eta} K N}) \nonumber\\
	&+\Ocal[(H +  1) \eta_l^2 K^2] 
	+ \Ocal[\tilde{\eta}^2  (H +  1)H  K ]
	+\Ocal[\tilde{\eta} K]
	\label{app:eq:R_2}
	.
	\end{align}
	


	

	
	
\end{proof}

==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/delayed_proofs/convergence_convex_2.tex <==
\begin{proof}
	Using Lemma \ref{lemma:one_SGD}, we have 
	\begin{align}
	\frac{1}{\tilde{\eta}}\Delta(n)
	&\le - 2  D(\vx, n)
	+ \rho^2 \alpha \tilde{\eta}  R(n)
	+  \rho  \beta \tilde{\eta} S(n)
	\end{align}
	Using Lemma \ref{lem:Dxn} to bound $D(\vx, n)$, Lemma \ref{lem:bounding_R} to bound $R(n)$, Lemma \ref{lem:phi_nk} to bound $S(n)$, and $3 \rho  \left[\alpha + \beta\right] \tilde{\eta} L \le 1$, we get
	\begin{align}
	\frac{1}{\tilde{\eta}}\Delta(n)
	&\le -2  \Xi(n)
	 + 8 \rho \tau L \sum_{s=1}^\tau  Q(n - s) 
	+ 4 D Z(n)
	+ 6 \rho \eta_l^2 (K-1)^2 L \sigma_1(n)
%	+ \frac{1}{K \tilde{\eta}} Q(n)
	\nonumber\\
	& 
	+ 12 \left[2 \alpha + \beta \right] \rho \tilde{\eta} L Z(n) 
	+ 3 \rho^2 \tilde{\eta} \left[ \alpha D + 2 \beta \right]  \sigma_1(n)
	+ 6  \rho^2 \alpha \tilde{\eta} \sigma_2(n) 
	\label{app:eq:C_12}
	.
\end{align}
	When considering the following intermediary result
	\begin{equation}
	\sum_{ n = 0 }^{N-1} K \Delta(n) \\
	= \E{\norm{\vtheta^{KN} - \vx}^2} - \norm{\vtheta^{0} - \vx}^2
	\ge - \norm{\vtheta^{0} - \vx}^2
	,
	\end{equation}
	reordering the terms, and taking the mean over $N$, we get
	\begin{align}
	2  \bar{\Xi}(N)
	&\le \frac{1}{ \tilde{\eta} KN }\E{ \norm{\vtheta^{0} - \vx}^2 }
	+ 8 \rho L \tau^2 \bar{Q}(N) 
	+ 4 D \bar{Z}(N)
	+ 6 \rho \eta_l^2 (K-1)^2 L \Sigma_1(N)
	%	+ \frac{1}{K \tilde{\eta}} Q(n)
	\nonumber\\
	& 
	+ 12 \rho  \left[2 \alpha + \beta \right] \tilde{\eta} L \bar{Z}(N) 
	+ 3 \rho^2 \left[ \alpha D + 2 \beta \right] \tilde{\eta} \Sigma_1(N)
	+ 6  \rho^2 \alpha \tilde{\eta} \Sigma_2(N) 
%	\label{app:eq:C_12}
	.
	\end{align}
	Using Lemma \ref{lem:bound_Q} to bound $\bar{Q}(N)$, and with $\nu = 16 \rho L$, we have
	\begin{align}
	2  \bar{\Xi}(N)
	&\le \frac{1}{\tilde{\eta} KN }\E{ \norm{\vtheta^{0} - \vx}^2 }
	+ 4 D \bar{Z}(N)
	+ 6 \rho \eta_l^2 (K-1)^2 L \Sigma_1(N)
	\nonumber\\
	& 
	+ 12 \rho \left[2 \alpha + \beta \right] \left[\tilde{\eta} + \nu \tilde{\eta}^2 K^2 \tau^2 \right] L \bar{Z}(N) 
	+ 3 \rho^2 \left[ \alpha D + 2 \beta \right] \left[\tilde{\eta} + \nu \tilde{\eta}^2 K^2 \tau^2 \right] \Sigma_1(N)
	\nonumber\\
	&+ 6  \rho^2 \alpha \left[\tilde{\eta} + \nu \tilde{\eta}^2 K^2 \tau^2 \right] \Sigma_2(N) 
	.
	\end{align}
	We note that when $ \bar{\Xi}(N) \le 0$, the claim follows directly. Therefore, we consider $ \bar{\Xi}(N) \ge 0$ for the rest of this proof. 
	We first note that 
	\begin{equation}
		\bar{Z}(N)
		= \bar{\Xi}(N)
		+ R(\{\Lcal^n\})
		\label{app:eq:decompo_loss}
		,
	\end{equation}
	and consider $\eta_l$ such that
	\begin{equation}
%		\zeta \coloneqq
		2 
		- 4 D 
		- 12 \rho \left[2 \alpha + \beta \right] \left[\tilde{\eta} + \nu \tilde{\eta}^2 K^2 \tau^2 \right] L
		\ge 1 
		,
	\end{equation}
	which gives
	\begin{align}
	\bar{\Xi}(N)
	&\le \frac{1}{\tilde{\eta} KN}\E{ \norm{\vtheta^{0} - \vx}^2 }
	+ 4 D R(\{\Lcal^n\})
	+ 6 \rho \eta_l^2 (K-1)^2 L \Sigma_1(N)
	\nonumber\\
	& 
	+ 12 \rho \left[2 \alpha + \beta \right] \left[\tilde{\eta} + \nu \tilde{\eta}^2 K^2 \tau^2 \right] L R(\{\Lcal^n\})
	+ 3 \rho^2 \left[ \alpha D + 2 \beta \right] \left[\tilde{\eta} + \nu \tilde{\eta}^2 K^2 \tau^2 \right] \Sigma_1(N)
	\nonumber\\
	&+ 6  \rho^2 \alpha \left[\tilde{\eta} + \nu \tilde{\eta}^2 K^2 \tau^2 \right] \Sigma_2(N) 
	.
	\end{align}
	The 5th term can be simplified with the third one. Indeed, we consider a local learning rate such that $3 \rho^2 \tilde{\eta} L \le 1$, $48 \rho^3 \tilde{\eta}^2 K^2 \tau^2 L^2 \le1$, and we remind that $\alpha \le 1$. We thus have
	\begin{align}
	\bar{\Xi}(N)
	&\le \frac{1}{ \tilde{\eta} KN}\E{ \norm{\vtheta^{0} - \vx}^2 }
	+ \Ocal \left(\eta_l^2 (K-1)^2 \left[ R(\{\Lcal^n\}) + \Sigma_1(N) \right] \right) 
	\nonumber\\
	& 
	+ \Ocal \left( \alpha \left[\tilde{\eta} + \tilde{\eta}^2 K^2 \tau^2 \right] \left[ R(\{\Lcal^n\}) + \Sigma_2(N) \right] \right)
	\nonumber\\
	&+ \Ocal\left(\beta \left[\tilde{\eta} + \tilde{\eta}^2 K^2 \tau^2 \right] \left[ R(\{\Lcal^n\}) + \Sigma_1(N)\right]\right)
	.\label{app:eq:final_theo}
	\end{align}
	
	With 
	\begin{equation}
		\norm{\nabla \Lcal_i(\vtheta, \xi)}^2 
		\le 2 \norm{\nabla \Lcal_i(\vtheta, \xi) - \nabla \Lcal_i(\bar{\vtheta}, \xi)}^2
		+ 2 \norm{\nabla \Lcal_i(\bar{\vtheta}, \xi)}^2
		,
	\end{equation}
	we have 
	\begin{equation}
		\Sigma_2(N) 
		\le \max q_i(n) \Sigma_1(N) 
		\le \max q_i(n) \left[4L R({\Lcal^n}) + 2 \Sigma \right]
		.\label{app:eq:bound_Sigma}
	\end{equation}	
	Finally, substituting equation (\refeq{app:eq:decompo_loss}) and (\refeq{app:eq:bound_Sigma}) in equation (\refeq{app:eq:final_theo}) completes the proof.

	
\end{proof}





















==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/delayed_proofs/decomposition_theorem.tex <==
\section{Decomposition Theorem \ref{theo:decomposition_theorem}} \label{app:sec:decomposition_theorem}

\input{tex/variables}
In Table \ref{table:parameters}, we provide the definition of the different notations used in this work.

%\input{./tex/Lemma_equality.tex}

\subsection{Useful Lemma}
We first introduce and prove the following useful lemma before introducing the proof of Decomposition Theorem \ref{theo:decomposition_theorem}.

\begin{lemma}\label{lem:decompo_Xi}
	Let us consider $n$ vectors $\vx_i, ..., \vx_n$ and a client sampling satisfying $\EE{S_t}{\omega_i(S_t)} = p_i$ and $\COV{\omega_i(S_t)}{\omega_j(S_t)} = - \alpha p_i p_j$. We have:
	\begin{equation}
		\EE{S_t}{\norm{\sum_{i=1}^{n}\omega_i(S_t)\vx_i}^2} 
		= \sum_{i=1}^{n} \gamma_i \norm{\vx_i}^2
		+ (1 - \alpha)\norm{\sum_{i=1}^{n}p_i \vx_i}^2,
	\end{equation}
	where $\gamma_i =  \VARR{S_t}{\omega_i(S_t)} + \alpha p_i^2 $.
\end{lemma}


\begin{proof}
	\begin{align}
		\EE{S_t}{\norm{\sum_{i=1}^{n}\omega_i(S_t)\vx_i}^2} 
		& = \sum_{i=1}^{n} \EE{S_t}{\omega_i(S_t)^2} \norm{\vx_i}^2
		+ \sum_{i=1}^{n}\sum_{\substack{j=1\\ j\neq i}}^{n}\EE{S_t}{\omega_i(S_t)\omega_j(S_t)}\inner{\vx_i}{\vx_j}
		\label{app:eq:AA1}
	\end{align}
	
	In addition, we have:
	\begin{equation}
		\EE{S_t}{\omega_i(S_t)\omega_j(S_t)}
		= \COV{\omega_i(S_t)}{\omega_j(S_t)} + p_i p_j
		= (- \alpha + 1) p_i p_j,
		\label{app:eq:AA2}
	\end{equation}
	where the last equality comes from the client sampling covariance assumption.
	
	We also have:
	\begin{equation}
		\sum_{i=1}^{n}\sum_{\substack{j=1\\ j\neq i}}^{n}\inner{p_i \vx_i}{p_j \vx_j} 
		= \norm{\sum_{i=1}^{n}p_i \vx_i}^2 - \sum_{i=1}^{n}p_i^2 \norm{\vx_i}^2
		\label{app:eq:AA3}
	\end{equation}
	
	Substituting equation (\ref{app:eq:AA2})  and equation (\ref{app:eq:AA3}) in equation (\ref{app:eq:AA1}) gives:
	\begin{equation}
		\EE{S_t}{\norm{\sum_{i=1}^{n}\omega_i(S_t)\vx_i}^2} 
		= \sum_{i=1}^{n} \left[ \EE{S_t}{\omega_i(S_t)^2} - (-\alpha +1 )p_i^2 \right] \norm{\vx_i}^2
		+ (-\alpha +  1)\norm{\sum_{i=1}^{n}p_i \vx_i}^2
		\label{app:eq:AA4}
	\end{equation}
	
	Considering that we have $\EE{S_t}{\omega_i(S_t)^2} = \VAR{\omega_i(S_t)} + p_i^2$, we have :
	\begin{equation}
	\EE{S_t}{\omega_i(S_t)^2} + (\alpha - 1) p_i^2
	= \VARR{S_t}{\omega_i(S_t)} + \alpha p_i^2
	\label{app:eq:AA5}
	\end{equation}
	
	Substituting equation (\ref{app:eq:AA5}) in equation (\ref{app:eq:AA4}) completes the proof.

\end{proof}





\subsection{Proof of the Decomposition Theorem \ref{theo:decomposition_theorem}}
\begin{proof}
	\begin{align}
	\EE{t}{\norm{\theta^{t+1} - \theta^*}^2} 
	&= \EE{t}{\norm{(\theta^{t+1} - \theta^t) + (\theta^t - \theta^*)}^2}\\
	&= \norm{\theta^t - \theta^*}^2 
	+ 2 \inner{\EE{t}{\theta^{t+1} - \theta^t}}{\theta^t - \theta^*} + \EE{t}{\norm{\theta^{t+1} - \theta^t}^2} 
	\end{align}
	By construction, equation (\ref{eq:aggreg_SCAFFOLD_general}), we have 
	$\theta^{t+1} - \theta^t 
	=  \eta_g \sum_{i=1}^n\omega_i(S_t)(\theta_i^{t+1} - \theta^t) 
	%= - \tilde{\eta} \sum_{i, k}\omega_i(S_t)g_i(y_{i,k}^t)
	$. The sampling scheme follows Definition \ref{def:sampling} which gives $\EE{S_t}{\theta^{t+1} - \theta^t} = \eta_g \sum_{i=1}^n p_i (\theta_i^{t+1} - \theta^t)$. Hence , we get:
	\begin{align}
	\EE{t}{\norm{\theta^{t+1} - \theta^*}^2} 
	&= \norm{\theta^t - \theta^*}^2 
	+ 2 \eta_g \inner{\sum_{i=1}^n p_i \EE{t}{\theta_i^{t+1} - \theta^t}}{\theta^t - \theta^*} \nonumber\\
	&+ \eta_g^2 \underbrace{\EE{t}{\norm{\sum_{i=1}^n\omega_i(S_t) (\theta_i^{t+1} - \theta^t)}^2}}_{= \eta_l^2 Q(\theta^t)} 
	\label{app:eq:A1}
	\end{align}
	
	Using Lemma \ref{lem:decompo_Xi}, we bound $Q(\theta^t)$ as follow:
	\begin{equation}
		\eta_l^2 Q(\theta^t) 
		= \sum_{i=1}^n \gamma_i \EE{t}{\norm{ \theta_i^{t+1} - \theta^t}^2}
		+ (1 - \alpha) \EE{t}{\norm{\sum_{i=1}^n p_i (\theta_i^{t+1} - \theta^t)}^2}.
		\label{app:eq:A2}
	\end{equation}
	
	
	By construction, we have $\theta_i^{t+1} - \theta^t = - \sum_{k=0}^{K-1} \eta_l g_i(y_{i,k}^t)$. Considering Assumption \ref{ass:unbiased} gives
	\begin{align}
	\E{\norm{\theta_i^{t+1} - \theta^t}^2}
	%        = \E{\norm{\theta_i^{t+1}-\theta^t}^2}
	%        \\
%	= \eta_l^2 \E{\norm{d_i^t}^2}
	%        \\
	%        = \eta_l^2 \left[ \E{\norm{d_i^t - h_i^t}^2 }
	%        +  \E{\norm{h_i^t}^2}\right]
	%        \\
	= \eta_l^2 \left[ \E{\norm{\xi_i^t}^2 }
	+ \E{\norm{\Delta_i^t}^2} \right] 
	%        \\
	.
	\label{app:eq:A3}
	\end{align}
	
	Similarly by using twice Assumption \ref{ass:unbiased} for the global model drift, we have
	\begin{align}
%	G(\{p_i\}, \theta^t)
%	%        &= \E{\norm{\sum_{i=1}^n p_i (\theta_i^{t+1}-\theta^t)}^2}
%	%        \\
%	&= 
	\eta_l^2 \E{\norm{\sum_{i=1}^n p_id_i^t }^2}
%	&= \eta_l^2 \E{\norm{\sum_{i=1}^n p_i (d_i^t - h_i^t)}^2}
%	+ \eta_l^2 \E{\norm{\sum_{i=1}^n p_i h_i^t }^2}
%	\\
	&= \eta_l^2 \E{\norm{\sum_{i=1}^n p_i \xi_i^t }^2}
	+ \eta_l^2 \E{\norm{\sum_{i=1}^n p_i \Delta_i^t }^2}
	\\
	&= \eta_l^2 \left[ \sum_{i=1}^n p_i^2 \E{\norm{ \xi_i^t }^2}
	+ \E{\norm{\sum_{i=1}^n p_i \Delta_i^t }^2} \right],
	\label{app:eq:A4}
	\end{align}
	where, for the last equality, Assumption \ref{ass:unbiased} gives $\E{\inner{\xi_i^t}{\xi_j^t}} = \E{\xi_i^t}^T \E{\xi_j^t} =  0 $.
	
	Combining equation (\ref{app:eq:A3}) with equation (\ref{app:eq:A4}) gives
	\begin{align}
	Q(\theta^t)
%	& = \sum_{i=1}^{n} \left[ \VAR{\omega_i(S_t)} 
%	+ \alpha p_i^2\right] L_i(\theta^t) + ( 1- \alpha) G(\theta^t)
%	\\
%	& = \eta_l^2 \sum_{i=1}^{n} \left[ \VAR{\omega_i(S_t)} + \alpha p_i^2\right]  \left[ \E{\norm{\xi_i^t}^2 } + \E{\norm{h_i^t}^2} \right] 
%	\nonumber\\
%	& + \eta_l^2 ( 1- \alpha)  \left[ \sum_{i=1}^n p_i^2 \E{\norm{ \xi_i^t }^2}
%	+ \E{\norm{\sum_{i=1}^n p_i h_i^t }^2} \right]
%	\\
	& = \sum_{i=1}^{n} \left[ \VAR{\omega_i(S_t)} + p_i^2 \right] \E{\norm{\xi_i^t}^2 } 
	\nonumber\\
	& +  \sum_{i=1}^{n} \gamma_i  \E{\norm{\Delta_i^t}^2} 
	+ ( 1- \alpha)  \E{\norm{\sum_{i=1}^n p_i \Delta_i^t }^2} .
	\label{app:eq:A5}
%	\\
%	& = \eta_l^2 \sum_{i=1}^{n} \left[ \VAR{\omega_i(S_t)} + p_i^2 \right] \E{\norm{\xi_i^t}^2 } 
%	\nonumber\\
%	& + \eta_l^2 \sum_{i=1}^{n} \left[\VAR{\omega_i(S_t)} + p_i^2 \right]  \E{\norm{h_i^t}^2} 
%	+ \eta_l^2 ( 1- \alpha) \sum_{i=1}^{n}\sum_{\substack{j=1\\ j\neq i}}^{n} \E{\inner{h_i^t}{h_j^t}} 
	\end{align}
	
%	where the equality comes from the unbiasedness of the SGD estimator, Assumption \ref{ass:unbiased}, and the last inequality comes from the bounded variance of the SGD estimator, Assumption \ref{ass:unbiased}.
%	
%	
%	Let us consider the special case where clients have the same data distribution. Clients perform identical local work. Therefore, we can define $h^t \coloneqq h_i^t$. By definition, equation (\ref{eq:global_loss}), we have $\sum_{i=1}^{n}p_i = 1$ which gives $h^t = \sum_{i=1}^{n} p_i h_i^t$ which gives	
%	\begin{align}
%	\sum_{i=1}^{n} \gamma_i L_i(\theta^t) + ( 1- \alpha) G(\theta^t)
%	& \le \eta_l^2 \sum_{i=1}^{n} \left[ \VAR{\omega_i(S_t)} + p_i^2 \right] K \sigma^2 
%	\nonumber\\
%	& + \eta_l^2 \left[ \sum_{i=1}^{n} \gamma_i  + (1 - \alpha ) \right] \E{\norm{h^t}^2} 
%	%	+ \eta_l^2 ( 1- \alpha)  \E{\norm{\sum_{i=1}^n p_i h_i^t }^2} 
%	\\& = \eta_l^2 \sum_{i=1}^{n} \left[ \VAR{\omega_i} + p_i^2 \right] K \sigma^2 
%	+ \eta_l^2 \left[ \VAR{\sum_{i=1}^{n}\omega_i}  + 1 \right] \E{\norm{h^t}^2} 
%	\end{align}
	
	Substituting equation (\ref{app:eq:A5}) in equation (\ref{app:eq:A1}) completes the proof.
	
\end{proof}


\subsection{Adaptation to Clustered Sampling}

Instead of Lemma \ref{lem:decompo_Xi} which requires $\COV{\omega_i(S_t)}{\omega_j(S_t)} = - \alpha p_i p_j$, we propose the following Lemma for clustered sampling expressed in function of MD sampling covariance parameter $\alpha_{MD}$ showing that a sufficient condition for MD sampling to perform as Clustered sampling is $\vx_i$ to all be identical or for all the distributions to be identical, i.e. $r_{k, i} = p_i$. 

\begin{lemma}\label{lem:decompo_Xiclustered}
	Let us consider $n$ vectors $\vx_i, ..., \vx_n$ and a client sampling satisfying $\EE{S_t}{\omega_i(S_t)} = p_i$ and $\COV{\omega_i(S_{Cl})}{\omega_j(S_{Cl})} = - \alpha p_i p_j$. We have:
	\begin{equation}
	\EE{S_{Cl}}{\norm{\sum_{i=1}^{n}\omega_i(S_{Cl})\vx_i}^2} 
	\le \sum_{i=1}^{n} \gamma_i(MD) \norm{\vx_i}^2
	+ (1 - \alpha_{MD})\norm{\sum_{i=1}^{n}p_i \vx_i}^2,
	\label{eq:decompo_clustered}
	\end{equation}
	where $\gamma_i(MD)$ and $\alpha_{MD}$ are the aggregation weights statistics of MD sampling. Equation (\ref{eq:decompo_clustered}) is an equality if and only if $\sum_{i=1}^{n} r_{k, i} \vx_i = \sum_{j=1}^{n} r_{k, j} \vx_j$.
\end{lemma}


\begin{proof}
	Substituting equation (\ref{app:eq:T1}) in equation (\ref{app:eq:AA1}) gives
	\begin{align}
	\EE{S_{Cl}}{\norm{\sum_{i=1}^{n}\omega_i(S_{Cl})\vx_i}^2} 
	& = \sum_{i=1}^{n} \EE{ S_{Cl} }{\omega_i( S_{Cl} )^2} \norm{\vx_i}^2
	+ \sum_{i=1}^{n}\sum_{\substack{j=1\\ j\neq i}}^{n} p_i p_j \inner{\vx_i}{\vx_j}
	\nonumber\\
	&- \frac{1}{m^2} \sum_{k=1}^{m} \sum_{i=1}^{n}\sum_{\substack{j=1\\ j\neq i}}^{n}  r_{k, i}r_{k, j} \inner{\vx_i}{\vx_j}
	\label{app:eq:U1}
	\end{align}
	
	Substituting equation (\ref{app:eq:AA3}) in equation (\ref{app:eq:AA1}) gives:
	\begin{align}
	\EE{ S_{Cl} }{\norm{\sum_{i=1}^{n}\omega_i( S_{Cl} )\vx_i}^2} 
	& = \sum_{i=1}^{n} \EE{ S_{Cl} }{\omega_i( S_{Cl} )^2} \norm{\vx_i}^2
	+ \norm{\sum_{i=1}^{n}p_i \vx_i }^2 
	- \sum_{i=1}^{n}p_i^2 \norm{ \vx_i }^2 
	\nonumber\\
	&- \frac{1}{m^2} \sum_{k=1}^m \left[\norm{\sum_{i=1}^{n}r_{k, i} \vx_i }^2 
	- \sum_{i=1}^{n} r_{k, i}^2 \norm{ \vx_i }^2 \right]
	\label{app:eq:U2}
	\end{align}
	
	With rearrangements and using equation (\ref{app:eq:clustered_prop}) we get:
	\begin{align}
	\EE{ S_{Cl} }{\norm{\sum_{i=1}^{n}\omega_i( S_{Cl} )\vx_i}^2} 
	& = \sum_{i=1}^{n} \left[ \VAR{\omega_i( S_{Cl} )} + \frac{1}{m^2}\sum_{k=1}^m r_{k, i}^2 \right] \norm{\vx_i}^2
	+ \norm{\sum_{i=1}^{n}p_i \vx_i }^2 
	\nonumber\\
	&- \frac{1}{m^2} \sum_{k=1}^m \norm{\sum_{i=1}^{n}r_{k, i} \vx_i }^2 
	\label{app:eq:U3}
	\end{align}
	
	Using the expression of clustered sampling variance, equation (\ref{app:eq:T2}), for the first term and using Jensen inequality on the third term completes the proof. Jensen inequality is an equality if and only if $\sum_{i=1}^{n} r_{k, i} \vx_i = \sum_{j=1}^{n} r_{k, j} \vx_j$.
%	\begin{align}
%	\EE{S_t}{\norm{\sum_{i=1}^{n}\omega_i(S_t)\vx_i}^2} 
%	& = \frac{1}{m}\sum_{i=1}^{n} p_i \norm{\vx_i}^2
%	+ \norm{\sum_{i=1}^{n}p_i \vx_i }^2 
%	- \frac{1}{m^2} \sum_{k=1}^m \norm{\sum_{i=1}^{n}r_{k, i} \vx_i }^2 
%	\label{app:eq:U4}
%	\end{align}
%	Substituting equation (\ref{app:eq:AA5}) in equation (\ref{app:eq:AA4}) completes the proof.
	
\end{proof}



%\input{tex/coro_decomposition_theorem}

==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/delayed_proofs/new_quantities.tex <==
In Table \ref{tab:aggregation_weights}, we synthesize the different random variables associated to the clients aggregation weights. 
In Table \ref{tab:parameters}, we synthesize the remaining random variables.

We introduce the following notations to provide clear and compact proofs.
Whenever considering a function $f(n, k)$, we define $f(n) \coloneqq 1/K \sum_{ k = 0 }^{K-1} f(n , k)$, and $\bar{f}(N) \coloneqq 1/N \sum_{ n = 0 }^{N-1} f(n)$.
We introduce the following quantities
\begin{align}
D(\vx, n, k)
\coloneqq
\E{ \inner { \sum_{i=1}^M q_i(n) \nabla \Lcal_i (\vtheta_i^{\rho_i(n), k})}{\vtheta^{n,k} - \vx}}
,
&&
Q(n)
\coloneqq \E{\norm{\vtheta^{n+1, 0} - \vtheta^{n ,0}}^2} 
,
\end{align}
\begin{align}
R(n , k) 
\coloneqq \E{\norm{\sum_{ i = 1 }^M \tilde{q}_i(n) g_i(\vtheta_{i}^{\rho_i(n), k})}^2}
,
&&
S(n , k) 
\coloneqq \sum_{ i = 1 }^M \tilde{q}_i(n) \E{\norm{g_i(\vtheta_{i}^{\rho_i(n), k})}^2}
,
\end{align}
\begin{align}
Z(n , k)
= \Lcal^n(\vtheta^{n, k}) - \Lcal^n(\bar{\vtheta}^n)
,
&&
\Delta(n, k) 
\coloneqq \E{\norm{\vtheta^{n, k+ 1} - \vx}^2} - \E{ \norm{\vtheta^{n, k} - \vx}^2 }
,
\end{align} 
\begin{align}
\phi(n, k )
\coloneqq \sum_{ i = 1 }^M \tilde{q}_i(n) \E{\norm{\vtheta_i^{\rho_i(n), k} - \vtheta^{n,k}}^2 }
,
&&
\sigma_1(n) 
\coloneqq \sum_{ i = 1 }^M \tilde{q}_i(n)\E{\norm{ \nabla \Lcal_i(\bar{\vtheta}^n, \vxi_i)}^2}
,
\end{align}
\begin{align}
\sigma_2(n) 
\coloneqq \sum_{ i = 1 }^M \tilde{q}_i^2(n)\E{\norm{ \nabla\Lcal_i(\bar{\vtheta}^n, \vxi_i)}^2}
,
\text{ and }
\Xi(n , k)
= \Lcal^n(\vtheta^{n, k}) - \Lcal^n(\vx)
.
\end{align}
%We also define $\rho \coloneqq \max \left(1, q(n)\right)$. 
Finally, we define $g_i(\vy) = \nabla \Lcal_i(\vy, \vxi_i)$ the SG of client $i$ evaluated on model parameters $\vy$ and batch $\vxi_i$. We will thus write $g_i(\vtheta_{i, k}^{\rho_i(n)})$ instead of $\nabla \Lcal_i(\vtheta_{i, k}^{\rho_i(n)}, \vxi_{i, k}^{\rho_i(n)})$.

%We note that every client loss function satisfies Assumption \ref{ass:smoothness} and is thus $L$ smooth. Therefore, $\Lcal$ and is $L$-smooth and $\Lcal^n$ is $L q(n)$-smooth. Similarly, for the strong convexity parameter $\mu$, Assumption \ref{ass:strong_convexity}.


==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/delayed_proofs/proof_based_Wang.tex <==
\newpage
\section{FL Convergence}\label{app:sec:convergence_Wang}

Our work is made possible thanks to the one of \cite{FedNova}. We use their developed theoretical framework to prove Theorem \ref{theo:convergence_paper}. The focus of our work (and Theorem \ref{theo:convergence_paper}) is on FedAvg. Yet, the proof devised in this section, like in \cite{FedNova}, keeps $a_i$ which can account for a wide-range of regularization method on FedAvg or optimizer different of the Vanilla SGD one. This proof can easily be extended to account for different amount of local work from the clients \citep{FedNova}. 

Before diving in the proof of Theorem \ref{theo:convergence_paper} in Section \ref{app:sec:proof_convergence}, we introduce the notation we use in Section \ref{app:sec:notation}, some useful lemmas in Section \ref{app:sec:lemmas} and Theorem \ref{theo:intermediary} generalizing Theorem \ref{theo:convergence_paper} in Section \ref{app:sec:intermediary_theo}.



%\subsection{Notations}\label{app:sec:notation}
%We define by $\vy_{i, k}^n$ the local model of client $i$ after $k$ SGD initialized on $\vtheta^n$ which enables us to also define the normalized stochastic gradients $\vs_i^n$ and the normalized gradient $\vDelta_i^n$ defined as
%\begin{equation}
%\vs_i^n = \frac{1}{a_i} \sum_{k=0}^{K-1} a_{i,k} g_i(\vy_{i, k}^n)
%\text{ and }
%\vDelta_i^n = \frac{1}{a_i} \sum_{k=0}^{K-1} a_{i, k} \nabla \Lcal_i (\vy_{i, k}^n),
%\label{app:eq:formalism_sum_grad}
%\end{equation}
%where $a_{i, k}$ is an arbitrary scalar set by the client to its $k$th computed gradient, $\va_i = [a_{i, 0}, .., a_{i, K -1}]^T$, and $a_i = \norm{\va_i}_1$. In the special case of FedAvg, we have $\va_i = [1, ..., 1]$ and in the one of FedProx, we have $\va_i = [(1 - \mu)^{K-1}, ..., 1]$ where $\mu$ is the FedProx regularization parameter. 
%
%With the formalism in equation (\ref{app:eq:formalism_sum_grad}), we can express a client contribution as $\theta_i^{n+1} - \vtheta^n  = - \eta_l a_i \vs_i^n $ and rewrite the server aggregation scheme defined in equation (\ref{eq:aggreg_SCAFFOLD_general}) as 
%\begin{align}
%\vtheta^{n+1} - \vtheta^n  
%&= - \eta_g \eta_l \sum_{i=1}^M\omega_i(n) a_i \vs_i^{\rho_i(n)}
%%	& = - \tilde{\eta} \underbrace{\left(\sum_{i=1}^M\omega_i(n) a_i \right)}_{K_{eff}} \sum_{i=1}^M \underbrace{\left(\frac{\omega_i(n) a_i}{\sum_{i=1}^M\omega_i(n) a_i}\right)}_{w_i} \vs_i^n\\
%,
%\end{align}
%which in expectation over the set of sampled clients $S_n$ gives
%\begin{align}
%\EE{S_n}{\vtheta^{n+1} - \vtheta^n}  
%&= - \tilde{\eta} \sum_{i=1}^M q_i(n) a_i \vs_i^n
%\\
%& = - \tilde{\eta} \underbrace{\left(\sum_{i=1}^M q_i(n) a_i \right)}_{K_{eff}} \sum_{i=1}^M \underbrace{\left(\frac{q_i(n) a_i}{\sum_{i=1}^M q_i(n) a_i}\right)}_{q_i(n)} \vs_i^{\rho_i(n)}
%\label{app:eq:expected_client_contrib}
%\end{align}
%
%We define the surrogate objective $\Lcal^n(\vx) = \sum_{i=1}^M q_i(n) \Lcal_i(\vx)$, where $\sum_{i=1}^Mq_i(n) =1 $. 
%
%In what follows, for $\va_i$ we specify the norm used can either be L1, $\norm{\cdot}_1$, or L2, $\norm{\cdot}_2$, For other variables the norm is always the euclidean  one and $\norm{\cdot}$ is used instead of $\norm{\cdot}_2$. Also, regarding the client sampling metrics, for ease of writing, due to the independence of the client sampling statistics with the current optimization round we use $\omega_i(n)$ instead of $\omega_i(S_n)$.


\begin{align}
\EE{S_n}{\vtheta^{n+1} - \vtheta^n}  
&= - \tilde{\eta} \sum_{i=1}^M q_i(n) \Delta_i^n
%\\
%& = - \tilde{\eta} \underbrace{\left(\sum_{i=1}^M q_i(n) a_i \right)}_{K_{eff}} \sum_{i=1}^M \underbrace{\left(\frac{q_i(n) a_i}{\sum_{i=1}^M q_i(n) a_i}\right)}_{q_i(n)} \vs_i^{\rho_i(n)}
\label{app:eq:expected_client_contrib}
\end{align}



%
%\subsection{Useful Lemmas}\label{app:sec:lemmas}
%
%
%
%\begin{lemma}\label{lem:decompo_Xi}
%	Let us consider $n$ vectors $\vx_i, ..., \vx_n$ and a client sampling satisfying $\EE{S_n}{\omega_i(n)} = \mathbb{P}( T_i^n \le \Delta t^{n+1}) d_i^2(n)$ and $\EE{S_n}{\omega_i(n)\omega_j(n)} = - R_i(n) R_j(n) p_i p_j$. We have:
%	\begin{equation}
%	\EE{S_n}{\norm{\sum_{i=1}^M\omega_i(n)\vx_i}^2} 
%	= \sum_{i=1}^M \gamma_i(n) \norm{\vx_i}^2
%	+ \norm{\sum_{i=1}^MR_i(n)d_i(n) \vx_i}^2
%	\end{equation}
%	where $\gamma_i(n)=  \left[ \mathbb{P}( T_i^n \le \Delta t^n) -R_i^2(n) \right] d_i^2(n)$.
%\end{lemma}
%
%
%\begin{proof}
%	\begin{align}
%	\EE{S_n}{\norm{\sum_{i=1}^M\omega_i(n)\vx_i}^2} 
%	& = \sum_{i=1}^M \EE{S_n}{\omega_i^2(n)} \norm{\vx_i}^2
%	+ \sum_{i=1}^M\sum_{\substack{j=1\\ j\neq i}}^M\EE{S_n}{\omega_i(n)\omega_j(n)}\inner{\vx_i}{\vx_j}
%	\\
%	& = \sum_{i=1}^M \mathbb{P}( T_i^n \le \Delta t^n) d_i^2(n) \norm{\vx_i}^2 
%	+ \sum_{i, j \neq i}^M R_i(n) d_i(n) R_j(n) d_j(n) \inner{\vx_i}{\vx_j}
%	\label{app:eq:AA1}
%	\end{align}
%	In addition, we have:
%	\begin{equation}
%	\sum_{i=1}^M\sum_{\substack{j=1\\ j\neq i}}^M\inner{R_i(n)d_i(n) \vx_i}{R_j(n) d_j(n) \vx_j} 
%	= \norm{\sum_{i=1}^M R_i(n) d_i(n) \vx_i}^2 - \sum_{i=1}^MR_i^2(n) d_i^2(n) \norm{\vx_i}^2
%	\label{app:eq:AA3}
%	\end{equation}
%	Substituting equation (\ref{app:eq:AA3}) in equation (\ref{app:eq:AA1}) completes the proof.
%\end{proof}
%
%
%
%\begin{lemma}[\cite{OnTheImpact}]\label{lem:dif_grads}
%	Under Assumptions \ref{ass:unbiased} to \ref{ass:dissimilarity}, we can prove
%	\begin{align}
%%		\frac{1}{2}\sum_{i=1}^M q_i(n) 
%		\E{\norm{\nabla \Lcal_i(\vtheta^n) - \vDelta_i^n}^2}
%		&\le \frac{\eta_l^2 L^2 \sigma^2}{1 -R} 
%		\left( \norm{\va_i}_2^2 - a_{i, -1}^2\right)
%%		\nonumber\\
%%		&
%		+ \frac{R \beta^2 }{1 - R}\E{\norm{\nabla \Lcal^n(\vtheta^n)}^2}
%		+ \frac{R \kappa^2 }{ 1 -R},
%	\end{align}
%	with $R = 2 \eta_l^2 L^2 \max_{i}\{\norm{\va_i}_1 (\norm{\va_i}_1 - a_{i, -1})\}$ with a learning rate such that $R < 1$.
%	
%	\begin{align}
%	%		\frac{1}{2}\sum_{i=1}^M q_i(n) 
%	\E{\norm{\nabla \Lcal_i(\vtheta^n) - \vDelta_i^n}^2}
%	&\le \frac{3}{2}\eta_l^2 L^2 \sigma^2
%	\left( \norm{\va_i}_2^2 - a_{i, -1}^2\right)
%	%		\nonumber\\
%	%		&
%%	+ \frac{R \beta^2 }{1 - R}\E{\norm{\nabla \Lcal^n(\vtheta^n)}^2}
%	+ \frac{1}{2} \kappa^2 ,
%	\end{align}
%	
%	\begin{equation}
%	\E{\norm{\nabla \Lcal_i(\vtheta^n) - \vDelta_i^n}^2}
%	\le
%		L^2 \eta_l^2 \left[ \left(\norm{a_i}_2^2 - a_{i, -1}^2\right) \sigma^2 
%		+  a_i \left( a_i - a_{i, -1} \right) \kappa^2 \right]
%	\end{equation}
%\end{lemma}
%
%\begin{proof}
%	\begin{align}
%		\E{\norm{\nabla \Lcal_i(\vtheta^n) - h_i^n}^2}
%		& = \E{\norm{\frac{1}{a_i} \sum_{ k = 0 }^{K-1} a_{i, k} \left(\nabla \Lcal_i(\vtheta^n) - \nabla \Lcal_i(\vy_{i, k}^n)\right)}^2}
%		\\
%		& \le \frac{1}{a_i} \sum_{ k = 0 }^{K-1} a_{i, k}  \E{\norm{\nabla \Lcal_i(\vtheta^n) - \nabla \Lcal_i(\vy_{i, k}^n )}^2}
%		\\
%		& \le L^2 \frac{1}{a_i} \sum_{ k = 0 }^{K-1} a_{i, k}  \E{\norm{\vtheta^n - \vy_{i, k}^n }^2}
%		\label{app:eq:Q1}
%	\end{align}
%	
%	We also have:
%	\begin{align}
%		\E{\norm{\vtheta^n - \vy_{i, k}^n }^2}
%		& = \eta_l^2 \E{\norm{\sum_{s=0}^{k-1} a_{i, s} g_i(\vy_{i, s}^n)}^2}
%		\\
%		& = \eta_l^2 \left[ \E{\norm{\sum_{s=0}^{k-1} a_{i, s} \left(g_i(\vy_{i, s}^n) - \nabla \Lcal_i(\vy_{i, s}^n)\right)}^2}
%		+  \E{\norm{\sum_{s=0}^{k-1} a_{i, s} \nabla \Lcal_i(\vy_{i, s}^n)}^2}\right]
%		\\
%		& \le \eta_l^2 \left[ \sum_{s=0}^{k-1} a_{i, s}^2 \sigma^2 
%		+  \left( \sum_{s=0}^{k-1} a_{i, s}\right)^2 \kappa^2 \right]
%		\\
%		& \le \eta_l^2 \left[ \left(\norm{a_i}_2^2 - a_{i, -1}^2\right) \sigma^2 
%		+  a_i \left( a_i - a_{i, -1} \right) \kappa^2 \right]
%		\label{app:eq:Q2}
%	\end{align}
%	
%	Plugging equation (\ref{app:eq:Q2}) in equation (\ref{app:eq:Q1}) completes the proof.
%\end{proof}
%
%
%%\begin{proof}
%%	The proof is in Section C.5 of \cite{FedNova}.
%%	
%%	The bound provided here is slightly tighter in term of numerical constants than \cite{FedNova}. Indeed, equation (70) in \cite{FedNova} uses the Jensen inequality $\norm{ \va + \vb}^2 \le 2 \norm{\va}^2 + 2 \norm{\vb}^2$ which could instead be obtained with:
%%	\begin{equation}
%%		\E{\norm{\sum_{s=0}^{k-1}a_{i,s} g_i(\vy_{i, s}^n)}^2}
%%		= \E{\norm{\sum_{s=0}^{k-1}a_{i,s} \left(g_i(\vy_{i, s}^n ) - \nabla \Lcal_i(\vy_{i, s}^n) \right)}^2}
%%		+ \E{\norm{\sum_{s=0}^{k-1}a_{i,s} \nabla \Lcal_i(\vy_{i, s}^n)}^2},
%%	\end{equation}
%%	which uses Assumption \ref{ass:unbiased} giving $\E{\inner{\sum_{s=0}^{k-1}a_{i,s} \left(g_i(\vy_{i, s}^n ) - \nabla \Lcal_i(\vy_{i, s}^n )\right)}{\sum_{s=0}^{k-1}a_{i,s} \nabla \Lcal_i(\vy_{i, s}^n )}} = 0$ with the same reasoning as for $U$ in equation(\ref{app:eq:B2}).
%%\end{proof}
%
%
%
%
%
%\begin{lemma}[\cite{OnTheImpact}]\label{lem:contrib_client_sampling}
%	Under Assumptions \ref{ass:unbiased} to \ref{ass:dissimilarity}, we can prove
%	\begin{align}
%	\E{\norm{ a_i \vDelta_i^{n}}^2}
%	&\le \frac{1}{1 - R}  \left(\norm{\va_i}_2^2 - (a_{i, -1}^2) \right) \sigma^2 
%	+ 2  \left[ L^2 \frac{R}{1 - R} +1 \right] a_i^2 \left(\beta^2 \E{\norm{\nabla  \Lcal^n (\vtheta^n)}^2} + \kappa^2 \right)
%	%	\label{app:eq:C5}
%	\end{align}
%	where $2 \eta_l^2 L^2 \max_i \{ \norm{a_i}_1^2 \} <1$.
%%	 $R' = 2 \eta_l^2 L^2 \max_i \{ \norm{a_i}_1^2 \} <1$.
%
%	\begin{align}
%	\E{\norm{ a_i \vDelta_i^{n}}^2}
%	&\le \frac{3}{2}  \left(\norm{\va_i}_2^2 - (a_{i, -1}^2) \right) \sigma^2 
%	+ \left[ L^2 + 2\right] a_i^2 \kappa^2 
%	%	\label{app:eq:C5}
%	\end{align}
%	
%\end{lemma}
%
%\begin{proof}
%	Due to the definition of $\vDelta_i^n$, we have:
%	\begin{align}
%	\E{\norm{ \vDelta_i^{n}}^2}
%	= \E{\norm{\sum_{k=0}^{K-1} \frac{1}{a_i} a_{i, k} \nabla \Lcal_i (\vy_{i, k}^{n})}^2}
%	\le \sum_{k=0}^{K-1}\frac{1}{a_i} a_{i, k} \E{\norm{\nabla \Lcal_i (\vy_{i, k}^{n})}^2}
%	\le \kappa^2
%	,
%	\label{app:eq:C1}
%	\end{align}
%	where the first inequality comes from using Jensen inequality and the second inequality from using Assumption 
%	XX.
%\end{proof}
%
%
%%\begin{proof}
%%	Due to the definition of $\vDelta_i^n$, we have:
%%	\begin{align}
%%	\E{\norm{ a_i \vDelta_i^{\rho_i(n)}}^2}
%%	& = a_i^2 \E{\norm{\sum_{k=0}^{K-1} \frac{1}{a_i} a_{i, k} \nabla \Lcal_i (\vy_{i, k}^{\rho_i(n)})}^2}\\
%%	&\le a_i^2 \sum_{k=0}^{K-1}\frac{1}{a_i} a_{i, k} \E{\norm{\nabla \Lcal_i (\vy_{i, k}^{\rho_i(n)})}^2}
%%	\label{app:eq:C1}
%%	\end{align}
%%	
%%	Using Jensen inequality, we have
%%	\begin{align}
%%	\E{\norm{\nabla \Lcal_i (\vy_{i, k}^{\rho_i(n)})}^2}
%%	&\le 2 \E{ \norm{\nabla \Lcal_i (\vy_{i, k}^n) - \nabla \Lcal_i (\vtheta^n)}^2}
%%	+ 2 \E{\norm{\nabla \Lcal_i (\vtheta^n)}^2}\\
%%	&\le 2 L^2 \E{ \norm{ \vy_{i, k}^n - \vtheta^n}^2}
%%	+ 2 \E{\norm{\nabla \Lcal_i (\vtheta^n)}^2},
%%	\label{app:eq:C2}
%%	\end{align}
%%	where the second equality comes from using Assumption \ref{ass:smoothness}.
%%	
%%	Also, Section C.5 of \cite{FedNova} proves
%%	\begin{equation}
%%	\frac{1}{a_i} \sum_{k=0}^{K-1} a_{i, k}\E{ \norm{ \vy_{i, k}^n - \vtheta^n}^2}
%%	\le \frac{1}{1 - R}\eta_l^2 \sigma^2 \left(\norm{\va_i}_2^2 - (a_{i, -1}^2) \right)
%%	+ \frac{R}{1 - R} \E{\norm{\nabla \Lcal_i (\vtheta^n)}^2}
%%	.
%%	\label{app:eq:C3}
%%	\end{equation}
%%	
%%	Plugging equation (\ref{app:eq:C2}) and then equation (\ref{app:eq:C3}) in equation (\ref{app:eq:C1}), we get:
%%	\begin{align}
%%	\E{\norm{ a_i \vDelta_i^{\rho_i(n)}}^2}
%%	&\le a_i^2 \sum_{k=0}^{K-1}\frac{1}{a_i} a_{i, k} \left[2 L^2 \E{ \norm{ \vy_{i, k}^n - \vtheta^n}^2}
%%	+ 2 \E{\norm{\nabla \Lcal_i (\vtheta^n)}^2}\right]
%%	\\
%%	&= 2 L^2  a_i^2 \sum_{k=0}^{K-1}\frac{1}{a_i} a_{i, k}  \E{ \norm{ \vy_{i, k}^n - \vtheta^n}^2}
%%	+ 2 a_i^2 \E{\norm{\nabla \Lcal_i (\vtheta^n)}^2}
%%	\\
%%	&\le 2 L^2  a_i^2 \left[\frac{1}{1 - R}\eta_l^2 \sigma^2 \left(\norm{\va_i}_2^2 - (a_{i, -1}^2) \right)
%%	+ \frac{R}{1 - R} \E{\norm{\nabla \Lcal_i (\vtheta^n)}^2}\right]
%%	\nonumber\\
%%	&+ 2 a_i^2 \E{\norm{\nabla \Lcal_i (\vtheta^n)}^2}
%%	\\
%%	&\le \frac{R'}{1 - R} \sigma^2 \left(\norm{\va_i}_2^2 - (a_{i, -1}^2) \right)
%%	+ 2 a_i^2 \left[ L^2 \frac{R}{1 - R} +1 \right] \E{\norm{\nabla \Lcal_i (\vtheta^n)}^2}
%%	\label{app:eq:C4}
%%	\end{align}
%%	
%%	Summing over $M$ gives
%%	\begin{align}
%%	\sum_{i=1}^M \gamma_i(n) \E{\norm{ a_i \vDelta_i^{\rho_i(n)}}^2}
%%	&\le 2 L^2 \frac{1}{1 - R}\eta_l^2 \sigma^2 \sum_{i=1}^M \gamma_i(n) a_i^2\left(\norm{\va_i}_2^2 - (a_{i, -1}^2) \right)
%%	\nonumber\\
%%	&+ 2  \left[ L^2 \frac{R}{1 - R} +1 \right] \sum_{i=1}^M\gamma_i(n) a_i^2 \E{\norm{\nabla \Lcal_i (\vtheta^n)}^2}
%%	\label{app:eq:C5}
%%	\end{align}
%%	
%%	Using Assumption \ref{ass:dissimilarity} in equation (\ref{app:eq:C5}) and $R' < 1$ completes the proof.	
%%	
%%\end{proof}
%
%
%
%
%
%
%
\begin{lemma}\label{lem:delta_n}
	\begin{align}
	\Delta^n
	\coloneqq \E{\norm{\vtheta^{n+1} - \vtheta^n}^2}
	\le \tilde{\eta}^2 \alpha(n) \sigma^2
	+\tilde{\eta}^2 \beta(n)
	+\tilde{\eta}^2 U^2 K_{eff}^2 \Gamma(n)
	.
	\end{align}
	where $\alpha(n) = \sum_{i=1}^M \E{\omega_i^2(n)} \norm{\va_i}_2^2$, $\beta(n) = \sum_{i=1}^M \gamma_i(n) \E{\norm{ a_i \vDelta_i^{\rho_i(n)}}^2}$, and $\Gamma(n) =  \E{\norm{\sum_{i=1}^M q_i(n)\vDelta_i^{\rho_i(n)} }^2}$.
\end{lemma}
%
%\begin{proof}
%	
%	\begin{align}
%	\Delta^n 
%	& = \tilde{\eta}^2 \E{\norm{\sum_{i=1}^M \omega_i(n) a_i \vs_i^{\rho_i(n)}}^2}
%	\\
%	& = \tilde{\eta}^2 \E{\norm{\sum_{i=1}^M \omega_i(n) a_i \left(\vs_i^{\rho_i(n)} - \vDelta_i^{\rho_i(n)}\right) 
%			+ \sum_{i=1}^M \omega_i(n) a_i \vDelta_i^{\rho_i(n)}}^2}
%	\\
%	& = \tilde{\eta}^2 \E{\norm{\sum_{i=1}^M \omega_i(n) a_i \left(\vs_i^{\rho_i(n)} - \vDelta_i^{\rho_i(n)}\right) }^2 }
%	+\tilde{\eta}^2 \E{\norm{\sum_{i=1}^M \omega_i(n) a_i \vDelta_i^{\rho_i(n)}}^2}
%	\nonumber\\
%	& + 2 \tilde{\eta} \underbrace{\E{\inner{\sum_{i=1}^M \omega_i(n) a_i \left(\vs_i^{\rho_i(n)} - \vDelta_i^{\rho_i(n)}\right)}{\sum_{i=1}^M \omega_i(n) a_i \vDelta_i^{\rho_i(n)}}}}_V
%	.
%	\label{app:eq:B2}
%	\end{align}
%	Using Assumption \ref{ass:unbiased}, we have $\E{\inner{g_i(\vy_{i, k}^n) - \nabla \Lcal^n(\vy_{i, k}^n) }{\nabla \Lcal^n(\vy_{i, k}^n)}} = 0$. Hence, we get $V=0$ and can simplify $\Delta^n$ as: 
%	\begin{align}
%	\Delta^n
%	& = \tilde{\eta}^2 \sum_{i=1}^M \E{\omega_i^2(n)} a_i^2\E{\norm{ \vs_i^{\rho_i(n)} - \vDelta_i^{\rho_i(n)} }^2 }
%	+\tilde{\eta}^2 \E{\norm{\sum_{i=1}^M \omega_i(n) a_i \vDelta_i^{\rho_i(n)}}^2}
%	.
%	\label{app:eq:B3}
%	\end{align}
%	
%	Using Lemma \ref{lem:decompo_Xi} on the second term, we get:
%	\begin{align}
%	\Delta^n
%	& = \tilde{\eta}^2 \sum_{i=1}^M \E{\omega_i^2(n)} a_i^2\E{\norm{ \vs_i^{\rho_i(n)} - \vDelta_i^{\rho_i(n)} }^2 }
%	\nonumber\\
%	&+\tilde{\eta}^2 \sum_{i=1}^M \gamma_i(n) \E{\norm{ a_i \vDelta_i^{\rho_i(n)}}^2}
%	+\tilde{\eta}^2 \E{\norm{\sum_{i=1}^M R_i(n)d_i(n) a_i \vDelta_i^{\rho_i(n)} }^2}
%	.
%	\label{app:eq:B4}
%	\end{align} 
%	We can bound the first term using Assumption \ref{ass:unbiased}
%%	 and the second term with Lemma \ref{lem:contrib_client_sampling}
%	 . Also, using Assumption \ref{ass:clients_covariance} and the definition of $q_i(n)$, we can rewrite the third term as$\E{\norm{\sum_{i=1}^M R_i(n)d_i(n) a_i \vDelta_i^n}^2} = U^2 K_{eff}^2 \E{\norm{\sum_{i=1}^M q_i(n) \vDelta_i^n}^2}$. Hence, we have:
%	\begin{align}
%	\Delta^n
%	& = \tilde{\eta}^2 \sum_{i=1}^M \E{\omega_i^2(n)} \sum_{k=0}^{K-1} a_{i, k}^2 \E{\norm{ g_i(\vy_{i, k}^n) - \nabla \Lcal_i(\vy_{i, k}^n) }^2 }
%	\nonumber\\
%	&+\tilde{\eta}^2 \sum_{i=1}^M \gamma_i(n) \E{\norm{ a_i \vDelta_i^{\rho_i(n)}}^2}
%	+\tilde{\eta}^2 U^2 K_{eff}^2\E{\norm{\sum_{i=1}^M q_i(n)\vDelta_i^{\rho_i(n)} }^2}
%	\\
%	& \le \tilde{\eta}^2 \sum_{i=1}^M \E{\omega_i^2(n)} \norm{\va_i}_2^2 \sigma^2
%	+\tilde{\eta}^2 \sum_{i=1}^M \gamma_i(n) \E{\norm{ a_i \vDelta_i^{\rho_i(n)}}^2}
%	\nonumber\\
%	&
%	+\tilde{\eta}^2 U^2 K_{eff}^2\E{\norm{\sum_{i=1}^M q_i(n)\vDelta_i^{\rho_i(n)} }^2}
%	.
%	\label{app:eq:B5}
%	\end{align}
%\end{proof}
%
%
%
%\begin{lemma}\label{lem:dif_grads_async}
%	Under Assumptions \ref{ass:unbiased} to \ref{ass:dissimilarity}, we can prove
%	\begin{align}
%	\sum_{ i = 1 }^M q_i(n) \E{ \norm{\nabla \Lcal_i(\vtheta^n) - \vDelta_i^{\rho_i(n)}}^2}
%	& \le  \tilde{\eta}^2 L^2  (\tau+1) \sum_{s=1}^{H}
%	\left[ \alpha(n) \sigma^2
%	+\beta(n)
%	+U^2 K_{eff}^2 \Gamma(n) \right] 
%	\nonumber\\
%	&+ (\tau+1) 
%	\eta_l^2 \left[ \left(\norm{a_i}_2^2 - a_{i, -1}^2\right) \sigma^2 
%	+  a_i \left( a_i - a_{i, -1} \right) \kappa^2 \right]
%	.
%	\end{align}	
%	with $\Delta^n = \E{\norm{\vtheta^{n+1} - \vtheta^n}^2}$.
%	
%	with $R = 2 \eta_l^2 L^2 \max_{i}\{\norm{\va_i}_1 (\norm{\va_i}_1 - a_{i, -1})\}$ with a learning rate such that $R < 1$.
%\end{lemma}
%
%
%\begin{proof}
%	We note that we have:
%	\begin{align}
%		&\norm{\nabla \Lcal_i(\vtheta^n) - \vDelta_i^{\rho_i(n)}}^2
%		\nonumber\\
%		& = \norm{\sum_{s=0}^{n - \rho_i(n) -1 } \left[ \nabla \Lcal_i(\vtheta^{\rho_i(n)+ s + 1}) - \nabla \Lcal_i(\vtheta^{\rho_i(n) + s})\right] + \left[\nabla \Lcal_i(\vtheta^{\rho_i(n)}) - \vDelta_i^{\rho_i(n)}\right]}^2		
%		\nonumber\\
%		& \le (H +1 ) \sum_{s=0}^{n - \rho_i(n) -1 } \norm{ \nabla \Lcal_i(\vtheta^{\rho_i(n)+ s + 1}) - \nabla \Lcal_i(\vtheta^{\rho_i(n) + s})}^2 
%		+ (\tau+1)\norm{ \nabla \Lcal_i(\vtheta^{\rho_i(n)}) - \vDelta_i^{\rho_i(n)} }^2	
%		\nonumber\\
%		& \le (\tau+1) L^2  \sum_{s=0}^{n - \rho_i(n) -1 } \norm{ \vtheta^{\rho_i(n)+ s + 1} - \vtheta^{\rho_i(n) + s}}^2 
%		+ (\tau+1) \norm{ \nabla \Lcal_i(\vtheta^{\rho_i(n)}) - \vDelta_i^{\rho_i(n)} }^2	
%		,
%	\end{align}
%	where the first inequality comes from using Jensen inequality and the second inequality from using Assumption \ref{ass:smoothness}.
%	
%	Taking the expectation gives
%	\begin{align}
%	\E{\norm{\nabla \Lcal_i(\vtheta^n) - \vDelta_i^{\rho_i(n)}}^2}
%	\le  L^2  (\tau+1) \sum_{s=1}^{H} \Delta^{n - s} 
%	+ (\tau+1) \left[ \left(\norm{a_i}_2^2 - a_{i, -1}^2\right) \sigma^2 
%	+  a_i \left( a_i - a_{i, -1} \right) \kappa^2 \right]
%	,
%	\end{align}	
%	which with reordering completes the proof.
%	
%	
%	
%	Using Lemma \ref{lem:delta_n} and Lemma \ref{lem:dif_grads} yields, 
%	\begin{align}
%	\E{ \norm{\nabla \Lcal_i(\vtheta^n) - \vDelta_i^{\rho_i(n)}}^2}
%%	&\le  L^2  (\tau+1) \sum_{s=1}^{H} \Delta^{n - s} 
%%	+ (\tau+1) \E{ \norm{ \nabla \Lcal_i(\vtheta^{\rho_i(n)}) - \vDelta_i^{\rho_i(n)} }^2 }
%%	\\
%	& \le  \tilde{\eta}^2 L^2  (\tau+1) \sum_{s=1}^\tau
%	\left[ \alpha(n) \sigma^2
%	+\beta(n)
%	+U^2 K_{eff}^2 \Gamma(n) \right] 
%	\nonumber\\
%	&+ (\tau+1) 
%	\left[\frac{\eta_l^2 L^2 \sigma^2}{1 -R} 
%	\left( \norm{\va_i}_2^2 - a_{i, -1}^2\right)
%	+ \frac{1}{2}\E{\norm{\nabla \Lcal^n(\vtheta^{\rho_i(n)})}^2}
%	+ \frac{1}{2} \kappa^2  \right]
%	.
%	\end{align}	
%	
%	If we assume that $R \le \frac{1}{2 \beta^2 +1}$ and considering that $\beta^2 \ge 1$, then we have $\frac{1}{1 - R} \le 1 + \frac{1}{2 \beta^2}\le \frac{3}{2}$, $\frac{R}{1-R} \le \frac{1}{2}$ , $\frac{R \beta^2}{1 -R} \le \frac{1}{2 \beta^2 + 1} (1 + \frac{1}{2 \beta^2})\beta^2 = \frac{1}{2}$, and $1 - \frac{R \beta^2}{1 - R} \ge \frac{1}{2}$, which gives:
%	%	 We also define $\Omega = L \tilde{\eta} \frac{1}{K_{eff}}   \left[ L^2  + 2 \right] \left(\sum_{i=1}^M\gamma_i(n)a_i^2\right)\beta^2 \le \frac{1}{2}$. Plugging all these components in equation (\ref{app:eq:B66}) gives
%	\begin{align}
%	\E{ \norm{\nabla \Lcal_i(\vtheta^n) - \vDelta_i^{\rho_i(n)}}^2}
%	%	&\le  L^2  (\tau+1) \sum_{s=1}^{H} \Delta^{n - s} 
%	%	+ (\tau+1) \E{ \norm{ \nabla \Lcal_i(\vtheta^{\rho_i(n)}) - \vDelta_i^{\rho_i(n)} }^2 }
%	%	\\
%	& \le  \tilde{\eta}^2 L^2  (\tau+1) \sum_{s=1}^{H}
%	\left[ \alpha(n) \sigma^2
%	+\beta(n)
%	+U^2 K_{eff}^2 \Gamma(n) \right] 
%	\nonumber\\
%	&+ (\tau+1) 
%	\eta_l^2 \left[ \left(\norm{a_i}_2^2 - a_{i, -1}^2\right) \sigma^2 
%	+  a_i \left( a_i - a_{i, -1} \right) \kappa^2 \right]
%	.
%	\end{align}	
%	
%	Taking the summation over $M$ completes the proof.	
%
%	
%	
%	
%\end{proof}
%







\subsection{Intermediary Theorem}\label{app:sec:intermediary_theo}

%\begin{theorem}\label{theo:intermediary}
%\begin{align}
%\frac{1}{T}\sum_{t=0}^{T-1} \E{\norm{\nabla \Lcal^n(\vtheta^n)}^2}
%&\le \Ocal(\frac{1}{ ( 1 - \Omega) \tilde{\eta} \left(\sum_{i=1}^M p_i a_i\right) T}) 
%+ \Ocal (\tilde{\eta}A' \sigma^2\frac{1}{m})
%+ \Ocal( \eta_l^2 \sigma^2 B')
%\nonumber\\
%& + \Ocal (\eta_l^2 C' \kappa^2 )
%+ \Ocal(\tilde{\eta} D' \sigma^2)
%+ \Ocal(\tilde{\eta} E' \kappa^2)
%,
%\end{align}
%where $A$-$E$ are defined in the following proof from equation (\ref{app:eq:def_A}) to equation (\ref{app:eq:def_E}).
%\end{theorem}


\begin{proof}
$\Lcal^n$ is $L$-Lipschitz smooth, Assumption \ref{ass:smoothness}, which gives
\begin{equation}
	\E{\Lcal^n(\vtheta^{n+1}) - \Lcal^n(\vtheta^n)}
	\le \underbrace{\E{\inner{\nabla \Lcal^n(\vtheta^n)}{\vtheta^{n+1} - \vtheta^n}}}_{T_1}
	+ \frac{L}{2}\underbrace{\E{\norm{\vtheta^{n+1} - \vtheta^n }^2}}_{ T_2 }
%	\le \underbrace{\E{\inner{\nabla \Lcal^n(\vtheta^n)}{- \tilde{\eta} \sum_{i=1}^M \omega_i(n) a_i \vs_i^n}}}_{T_1}
%	+ \frac{L}{2}\underbrace{\E{\norm{\tilde{\eta}\sum_{i=1}^M\omega_ia_i \vs_i^n}^2}}_{T_2}
,
\label{app:eq:B1}
\end{equation}
where the expectation is taken over the subset of randomly sampled clients $S_n$ and the clients gradient estimator noises $\xi_i^n$ but we use $\E{\cdot}$ instead of $\EE{\{\xi_i^n\}, S_n}{\cdot}$ for ease of writing.


\subsubsection*{Bounding $T_1$}
By conditioning on $\{\xi_i^n \}$ and using equation (\ref{app:eq:expected_client_contrib}), we get:
\begin{equation}
	T_1 
	= \E{\inner{\nabla \Lcal^n(\vtheta^n)}{{\EE{S_n}{\vtheta^{n+1} - \vtheta^n}}}} 
	= - \tilde{\eta} \E{\inner{\nabla \Lcal^n(\vtheta^n)}{ \sum_{i=1}^M q_i(n) \vDelta_i^{\rho_i(n)}}},
\end{equation}
which, using $2 \inner{a}{b} = \norm{a}^2 + \norm{b}^2 - \norm{a - b}^2$ can be rewritten as:
\begin{equation}
T_1 
= - \frac{1}{2}\tilde{\eta} K \E{ \norm{\nabla \Lcal^n(\vtheta^n)}^2 
+ \norm{ \sum_{i=1}^M q_i(n) \frac{1}{K} \vDelta_i^{\rho_i(n)}}^2 
- \norm{\nabla \Lcal^n(\vtheta^n) -  \sum_{i=1}^M q_i(n) \frac{1}{K}\vDelta_i^{\rho_i(n)}}^2 } ,
\label{app:eq:BB1}
\end{equation}


\subsubsection*{Bounding $T_2$}

\begin{align}
	T_2 
	& = \tilde{\eta}^2 \E{\norm{\sum_{i=1}^M \omega_i(n) \left[\vtheta_i^{\rho_i(n)+1} - \vtheta^{\rho_i(n)}\right]}^2}
	\\
	& = \tilde{\eta}^2 \E{\norm{\sum_{i=1}^M \omega_i(n) \vxi_i^{\rho_i(n)}  
			+ \sum_{i=1}^M \omega_i(n) \vDelta_i^{\rho_i(n)}}^2|S_n}
	\\
	& = \tilde{\eta}^2 \sum_{i=1}^M \E{\omega_i^2(n)} \E{\norm{ \vxi^{\rho_i(n)} }^2 }
	+\tilde{\eta}^2 \E{\norm{\sum_{i=1}^M \omega_i(n) \vDelta_i^{\rho_i(n)}}^2}
%	\nonumber\\
%	& + 2 \tilde{\eta} \underbrace{\E{\inner{\sum_{i=1}^M \omega_i(n)  \left(\vs_i^{\rho_i(n)} - \vDelta_i^{\rho_i(n)}\right)}{\sum_{i=1}^M \omega_i(n) \vDelta_i^{\rho_i(n)}}}}_V
	.
	\label{app:eq:B2}
\end{align}
%Using Assumption \ref{ass:unbiased}, we have $\E{\inner{g_i(\vy_{i, k}^n) - \nabla \Lcal^n(\vy_{i, k}^n) }{\nabla \Lcal^n(\vy_{i, k}^n)}} = 0$. Hence, we get $V=0$ and can simplify $T_2$ as: 
%\begin{align}
%T_2 
%& = \tilde{\eta}^2 \sum_{i=1}^M \E{\omega_i^2(n)} a_i^2\E{\norm{ \vs_i^{\rho_i(n)} - \vDelta_i^{\rho_i(n)} }^2 }
%+\tilde{\eta}^2 \E{\norm{\sum_{i=1}^M \omega_i(n) a_i \vDelta_i^{\rho_i(n)}}^2}
%.
%\label{app:eq:B3}
%\end{align}
%
%
%Finally, by bounding the gradient estimators with Assumption \ref{ass:unbiased}, and noting that $p_i a_i = q_i(n)K_eff$. we get:
We note that $\E{\omega_i^2(n)} = \mathcal{P}(T_i^n \le \Delta t^n)d_i^2(n) = \nu_i(n)$. Therefore $\sum_{i=1}^M \E{\omega_i^2(n)}  = \nu(n)$.
Using Assumption \ref{ass:unbiased} on the first term and Lemma \ref{lem:decompo_Xi} on the second term, we get:
\begin{align}
T_2 
& = \tilde{\eta}^2 \left[ \nu(n) K \sigma^2
+  \sum_{i=1}^M \gamma_i(n) \E{\norm{ \vDelta_i^{\rho_i(n)}}^2}
+ U^2 \E{\norm{\sum_{i=1}^M q_i(n) \vDelta_i^{\rho_i(n)} }^2}
\right]
.
\label{app:eq:B4}
\end{align} 
%By  bounding the first term using Assumption \ref{ass:unbiased}, and noting that there exists $U$ such that $\E{\norm{\sum_{i=1}^M R_i(n)d_i(n) a_i \vDelta_i^n}^2} = U K_{eff}^2 \E{\norm{\sum_{i=1}^M q_i(n) \vDelta_i^n}^2}$ for the second term, we get:
%\begin{align}
%T_2 
%& = \tilde{\eta}^2 \sum_{i=1}^M \E{\omega_i^2(n)} \sum_{k=0}^{K-1} a_{i, k}^2 \E{\norm{ g_i(\vy_{i, k}^n) - \nabla \Lcal_i(\vy_{i, k}^n) }^2 }
%\nonumber\\
%&+\tilde{\eta}^2 \sum_{i=1}^M \gamma_i(n) \E{\norm{ a_i \vDelta_i^{\rho_i(n)}}^2}
%+\tilde{\eta}^2 U K_{eff}^2\E{\norm{\sum_{i=1}^M q_i(n)\vDelta_i^{\rho_i(n)} }^2}
%\\
%& \le \tilde{\eta}^2 \sum_{i=1}^M \E{\omega_i^2(n)} \norm{\va_i}_2^2 \sigma^2
%+\tilde{\eta}^2 \sum_{i=1}^M \gamma_i(n) \E{\norm{ a_i \vDelta_i^{\rho_i(n)}}^2}
%+\tilde{\eta}^2 U K_{eff}^2\E{\norm{\sum_{i=1}^M q_i(n)\vDelta_i^{\rho_i(n)} }^2}
%.
%\label{app:eq:B5}
%\end{align}


\subsubsection*{Going back to equation (\ref{app:eq:B1})}



Substituting equation (\ref{app:eq:BB1}) and equation (\ref{app:eq:B4})
%Lemma \ref{lem:delta_n} 
in equation (\ref{app:eq:B1}), we get:
\begin{align}
	\E{\Lcal^n(\vtheta^{n+1}) - \Lcal^n(\vtheta^n)}
	&\le - \frac{1}{2}\tilde{\eta} K \norm{\nabla \Lcal^n(\vtheta^n)}^2 
	+ \frac{1}{2}\tilde{\eta} K \E{\norm{\nabla \Lcal^n(\vtheta^n) -  \sum_{i=1}^M q_i(n) \frac{1}{K} \vDelta_i^{\rho_i(n)} }^2}
	\nonumber\\
	& - \frac{1}{2}\tilde{\eta} K \left[1 - L\tilde{\eta} U^2 K\right] \E{\norm{ \sum_{i=1}^M q_i(n) \frac{1}{K} \vDelta_i^{\rho_i(n)}}^2}
	\nonumber\\
	&+\frac{L}{2} \tilde{\eta}^2 \nu(n) K \sigma^2
	+ \frac{L}{2} \tilde{\eta}^2 \sum_{i=1}^M \gamma_i(n) \E{\norm{ \vDelta_i^{\rho_i(n)}}^2}
	,
	\label{app:eq:B55}
\end{align}
We consider that the local learning rate $\eta_l$ satisfies $1 - L\tilde{\eta} U^2 K>0$. Therefore, using Jensen inequality and with reordering equation (\ref{app:eq:B55}) can be simplified as
\begin{align}
\frac{\E{\Lcal^n(\vtheta^{n+1}) - \Lcal^n(\vtheta^n)}}{\frac{1}{2}\tilde{\eta} K}
&\le - \norm{\nabla \Lcal^n(\vtheta^n)}^2 
+ \sum_{i=1}^M q_i(n)\E{ \norm{\nabla \Lcal_i(\vtheta^n) -   \frac{1}{K}\vDelta_i^{\rho_i(n)}}^2}
\nonumber\\
%& - \frac{1}{2} \left[1 - L\tilde{\eta} U^2 K_{eff}\right] \Gamma(n)
%\nonumber\\
&+L \tilde{\eta} \nu(n) \sigma^2
+ L \tilde{\eta} \frac{1}{K} \sum_{i=1}^M \gamma_i(n) \E{\norm{ \vDelta_i^{\rho_i(n)}}^2}
.
\label{app:eq:B6}
\end{align}

Using Lemma \ref{lem:dif_grads} and \ref{lem:contrib_client_sampling}, we get:
\begin{align}
&\frac{\E{\Lcal^n(\vtheta^{n+1}) - \Lcal^n(\vtheta^n)}}{\tilde{\eta} K_{eff}}\\
&\le - \frac{1}{2}\norm{\nabla \Lcal^n(\vtheta^n)}^2 
+ \frac{1}{2}\tilde{\eta}^2 L^2  (\tau+1) \sum_{s=1}^{H}
\left[ \alpha(n) \sigma^2
+\beta(n)
+U^2 K_{eff}^2 \Gamma(n) \right] 
\nonumber\\
&
+ \frac{1}{2}(\tau+1) \eta_l^2 \left[ \left(\norm{a_i}_2^2 - a_{i, -1}^2\right) \sigma^2 
+  a_i \left( a_i - a_{i, -1} \right) \kappa^2 \right]
\nonumber\\
&
- \frac{1}{2}\left[1 - L\tilde{\eta} U^2 K_{eff}\right] \Gamma(n)
\nonumber\\
&+\frac{L}{2} \tilde{\eta} \frac{1}{K_{eff}} \sum_{i=1}^M \E{\omega_i^2(n)} \norm{\va_i}_2^2 \sigma^2
+ \frac{L}{2} \tilde{\eta} \frac{1}{K_{eff}} \sum_{i=1}^M \gamma_i(n) a_i^2 \kappa^2
.
\label{app:eq:B66}
\end{align}

We denote by $\bar{\alpha} = \frac{1}{N} \sum_{ n = 0 }^{N-1}\alpha(n)$. Hence, we have $\sum_{ n = 0 }^{N-1} \sum_{s=1}^\tau \alpha(n - s) \le \tau \bar{\alpha}$. We similarly define $\bar{\beta}$. Hence, by taking the average over $N$ rounds, we get:
\begin{align}
\frac{1}{N}\sum_{ n = 0 }^{N-1}\norm{\nabla \Lcal^n(\vtheta^n)}^2 
& \le 2 \frac{1}{N}\sum_{ n = 0 }^{N-1}\frac{\E{\Lcal^n(\vtheta^{n+1}) - \Lcal^n(\vtheta^n)}}{\tilde{\eta} K_{eff}}\\ 
&+ \tilde{\eta}^2 L^2  (\tau+1) 
\left[ \tau \bar{\alpha} \sigma^2
+ \bar{\beta} a_i^2 \kappa^2 
%+U^2 K_{eff}^2 \Gamma(n) 
\right] 
\nonumber\\
&
+ (\tau+1) \eta_l^2 \left[ \left(\norm{a_i}_2^2 - a_{i, -1}^2\right) \sigma^2 
+  a_i \left( a_i - a_{i, -1} \right) \kappa^2 \right]
\nonumber\\
&
- \frac{1}{N}\sum_{ n = 0 }^{N-1} \left[1 - L\tilde{\eta} U^2 K_{eff} + \tilde{\eta}^2 L^2 \tau (\tau+1) U^2 K_{eff}^2\right] \Gamma(n)
\nonumber\\
&+ L \tilde{\eta} \frac{1}{K_{eff}} \sum_{i=1}^M \E{\omega_i^2(n)} \norm{\va_i}_2^2 \sigma^2
+  L \tilde{\eta} \frac{1}{K_{eff}} \sum_{i=1}^M \gamma_i(n) a_i^2 \kappa^2
.
\label{app:eq:B66}
\end{align}




\begin{align}
\frac{\E{\Lcal^n(\vtheta^{n+1}) - \Lcal^n(\vtheta^n)}}{\tilde{\eta} K_{eff}}
&\le - \frac{1}{4}\left[1 - \Omega \right]\norm{\nabla \Lcal^n(\vtheta^n)}^2 
%	+ \norm{\sum_{i=1}^M q_i(n)\vDelta_i^n}^2 
+ \frac{3}{4} \eta_l^2 L^2 \sigma^2 \sum_{i=1}^M q_i(n)\left( \norm{\va_i}_2^2 - a_{i, -1}^2\right)
\nonumber\\
&+ \frac{3}{2}\eta_l^2 L^2\max_i\{a_i (a_i - a_{i, -1})\} \kappa^2 
\nonumber\\
&+\frac{L}{2} \tilde{\eta} \frac{1}{K_{eff}} \left[\sum_{i=1}^M \E{\omega_i^2(n)} \norm{\va_i}_2^2 
+ \frac{3}{2}\sum_{i=1}^M \gamma_i(n)\left(\norm{\va_i}_2^2 - (a_{i, -1}^2) \right)\right] \sigma^2
\nonumber\\
&+ L \tilde{\eta} \frac{1}{K_{eff}}   \left[  \frac{L^2}{2} +1 \right] \left(\sum_{i=1}^M\gamma_i(n)a_i^2\right)  \kappa^2
,
\end{align}


\subsection{Old}



Taking average across all rounds, we get:
\begin{align}
\frac{1 - \Omega}{T}\sum_{t=0}^{T-1} \E{\norm{\nabla \Lcal^n(\vtheta^n)}^2}
&\le 4   \frac{\Lcal^n(\theta^0) - \Lcal^n(\theta^*)}{\tilde{\eta} K_{eff}T} 
%	+ \norm{\sum_{i=1}^M q_i(n)\vDelta_i^n}^2 
+ 3 \eta_l^2 L^2 \sigma^2 \sum_{i=1}^M q_i(n)\left( \norm{\va_i}_2^2 - a_{i, -1}^2\right)
\nonumber\\
&+ 6\eta_l^2 L^2\max_i\{a_i (a_i - a_{i, -1})\} \kappa^2 
\nonumber\\
&+ L \tilde{\eta} \frac{1}{K_{eff}} \left[2 \sum_{i=1}^M \E{\omega_i^2(n)} \norm{\va_i}_2^2
+ 3  \sum_{i=1}^M \gamma_i(n)\left(\norm{\va_i}_2^2 - (a_{i, -1}^2) \right)\right] \sigma^2
\nonumber\\
&+ 4 L \tilde{\eta} \frac{1}{K_{eff}}   \left[ \frac{L^2}{2} +1 \right] \left(\sum_{i=1}^M\gamma_i(n)a_i^2\right)  \kappa^2
,
\end{align}


We define the following auxiliary variables
\begin{equation}
	A 
	= m \frac{1}{K_{eff}} \sum_{i=1}^M \E{\omega_i^2(n)} \norm{\va_i}_2^2 
	= m \frac{1}{\sum_{i=1}^Mp_i a_i} \sum_{i=1}^M \left[\VAR{\omega_i} + p_i^2\right] \norm{\va_i}_2^2 ,
	\label{app:eq:def_A}
\end{equation}

\begin{equation}
B
= \sum_{i=1}^M q_i(n)\left( \norm{\va_i}_2^2 - a_{i, -1}^2\right)
= \sum_{i=1}^M\frac{p_i a_i}{\sum_{j=1}^{n} p_j a _j}  \left( \norm{\va_i}_2^2 - a_{i, -1}^2\right)
,
\end{equation}

\begin{equation}
C
= \max_i\{a_i (a_i - a_{i, -1})\}
,
\end{equation}

\begin{equation}
D 
= \frac{1}{K_{eff}} \max_i\{a_i (a_i - a_{i, -1})\} \sum_{i=1}^M\gamma_i(n) 
= \frac{1}{\sum_{i=1}^Mp_i a_i} C \left( \sum_{i=1}^M \VAR{\omega_i} + \alpha \sum_{i=1}^Mp_i^2 \right)
,
\end{equation}

\begin{equation}
E 
%= \frac{1}{K_{eff}} \left(\sum_{i=1}^M\gamma_i(n)a_i^2\right)
= \frac{1}{K_{eff}}\max_{i} \{a_i^2\}\left(\sum_{i=1}^M\gamma_i(n)\right) 
= \frac{1}{\sum_{i=1}^Mp_i a_i} \max_{i} \{a_i^2\}\left(\sum_{i=1}^M \VAR{\omega_i} + \alpha \sum_{i=1}^M p_i^2 \right)
\label{app:eq:def_E}
.
\end{equation}
%where $E$ and $F$ are obtained using Property \ref{prop:sum_weights} with $\alpha
%= \frac{\sum_{i=1}^M\VAR{\omega_i(S_n)} - \VAR{ \sum_{i=1}^M  \omega_i(S_n)}}{1 - \sum_{i=1}^M p_i^2}$

%with $\gamma = \sum_{i=1}^M\gamma_i$.


We define for $A$ -$E$, $A'$-$E'$ such that $X' = \frac{1}{1 -\Omega} X$.
\begin{align}
\frac{1}{T}\sum_{t=0}^{T-1} \E{\norm{\nabla \Lcal^n(\vtheta^n)}^2}
&\le 4   \frac{\Lcal^n(\theta^0) - \Lcal^n(\theta^*)}{( 1- \Omega) \tilde{\eta} \left(\sum_{i=1}^M p_i a_i\right) T} 
+ 2L \tilde{\eta} A' \sigma^2\frac{1}{m}
+ 3 \eta_l^2 L^2 \sigma^2 B'
\nonumber\\
& + 6\eta_l^2 L^2 C' \kappa^2 
+ 3L \tilde{\eta} D\sigma^2
+ 4 L \left[  \frac{L^2}{2} +1 \right] \tilde{\eta} E \kappa^2
,
\label{app:eq:end_intermediary}
\end{align}

\end{proof}




\subsection{Theorem \ref{theo:convergence_paper}}\label{app:sec:proof_convergence}


\begin{proof}
With FedAvg, every client performs vanilla SGD. As such, we have $a_{i, k} = 1$ which gives $a_i = K$ and $\norm{a_i}_2 = \sqrt{K}$. In addition we consider a local learning rate $\eta_l$ such that $\Omega \le \frac{1}{2}$ as such we can bound $A'$-$E'$ as $ X' \le \frac{1}{2}X$. 

Finally, considering that the variables $A$ to $E$ can be simplified as
\begin{equation}
A 
= m \sum_{i=1}^M \left[\VAR{\omega_i} + p_i^2\right]
,
\end{equation}

\begin{equation}
B
= (K -1)
,
\end{equation}

\begin{equation}
C
= K (K-1)
,
\end{equation}

\begin{equation}
D 
= (K - 1) \left( \sum_{i=1}^M \VAR{\omega_i} + \alpha \sum_{i=1}^M p_i^2  \right)
,
\end{equation}

and
\begin{equation}
E 
= K  \left( \sum_{i=1}^M \VAR{\omega_i} + \alpha \sum_{i=1}^M p_i^2 \right)
,
\end{equation}
the convergence bound of Theorem \ref{theo:intermediary} can be reduced to
\begin{align}
\frac{1}{T}\sum_{t=0}^{T-1} \E{\norm{\nabla \Lcal^n(\vtheta^n)}^2}
&\le \Ocal \left( \frac{1}{\eta_g \eta_l K T} \right)
+  \Ocal \left( \eta_g \eta_l \sum_{i=1}^M \left[\VAR{\omega_i} + p_i^2\right] \sigma^2 \right)
\nonumber\\
&+ \Ocal \left(  \eta_l^2 (K-1) \sigma^2 \right)
+ \Ocal \left( \eta_l^2 K(K-1) \kappa^2 \right)
\nonumber\\
& + \Ocal \left( \eta_g \eta_l \left(\sum_{i=1}^M\VAR{\omega_i} + \alpha \sum_{i=1}^M p_i^2  \right) \left[(K-1)\sigma^2 + K \kappa^2 \right] \right)
\label{app:eq:F1}
,
\end{align}
which completes the proof.

\end{proof}    

$\Omega$ is proportional to $\sum_{i=1}^M\gamma_i(n)= \sum_{i=1}^M\VAR{\omega_i} + \alpha \sum_{i=1}^M p_i^2 $. With full participation, we have $\Omega = 0$. However, with client sampling, all the terms in equation (\ref{app:eq:F1}) are proportional with $\frac{1}{1 - \Omega}$. Yet, we provide a looser bound in equation (\ref{app:eq:F1}) independent from $\Omega$ as the conclusions drawn are identical. Through $\Omega$, $\sum_{i=1}^M\VAR{\omega_i}$ and  $\alpha$ needs to be minimized which are conclusions already reached with the impact of $E$ and $F$.

We note that equation (\ref{app:eq:F1}) is function of the client sampling through $\sigma^2$ an indicator of the clients SGD quality and $\kappa^2$ an indicator of the clients data heterogeneity. In the special case where clients have the same data distribution and perform full gradient descent, based on the arguments discussed in the previous paragraph, we can still provide the following bound showing the influence of a client sampling on the convergence speed and the interest of minimizing $\sum_{i=1}^M\VAR{\omega_i}$ and  $\alpha$.
\begin{align}
\frac{1}{T}\sum_{t=0}^{T-1} \E{\norm{\nabla \Lcal^n(\vtheta^n)}^2}
&\le \Ocal \left( \frac{1}{(1 - \Omega)\eta_g \eta_l K T} \right)
,
\end{align}

                                                                                                                                                                                                                       
                                                                                                                                                                                                                                      
                                                                                                                                                                                                                                      
When setting the server learning rate at 1, $\eta_g=1$ with client full participation, i.e. $\VAR{\omega_i} = \VAR{\sum_{i=1}^M\omega_i} = \alpha = 0$ and $m=n$, we have $E= F=0$ and can simplify $A$ to                          
\begin{equation}                                                                                                         
A
= n \sum_{i=1}^M p_i^2                                                                                                                                                                                                              
.                                                                                                                                                                                                                                     
\end{equation}                                                                                                                                                                                                                        
Therefore, our provided convergence guarantee is $\frac{1}{\eta_lKT} + \eta_l \sum_{i=1}^Mp_i^2 \sigma^2 + \eta_l^2 (K-1) \sigma^2 + \eta_l^2 K(K-1) \kappa^2 $ which is identical to the one of \cite{FedNova} (equation (97) in their work), where $\sum_{i=1}^Mp_i^2$ can be replaced by $1/n$ when clients have identical importance, i.e. $p_i = 1/n$.

In the special case, where we use $\eta_l = \sqrt{m/KT}$ \citep{FedNova}, we retrieve their asymptotic convergence bound $\frac{1}{\sqrt{mKT}} + \sqrt{\frac{m}{KT}} \sum_{i=1}^Mp_i^2 \sigma^2 + \frac{m}{T} \sigma^2 + \frac{m}{T} K \kappa^2 $.


\subsection{Application to Clustered Sampling}\label{app:sec:clustered_convergence}

We adapt Theorem \ref{theo:convergence_paper} to clustered sampling. \cite{ClusteredSampling} proves the convergence of FL with clustered sampling by giving identical convergence guarantees to the one of FL with MD sampling. As a result, their convergence bound does not depend of the clients selection probability in the different clusters $r_{k, i}$. \cite{ClusteredSampling} claim reducing the aggregation weight variance provides faster FL convergence while only providing experimental proofs. Corollary \ref{cor:clustered} complements \cite{ClusteredSampling} by theoretically proving the influence of one clustered sampling on the convergence rate. For ease of writing, Corollary \ref{cor:clustered} is formatted for FedAvg but can easily be extended to account for any local $\va_i$ using the proof of Theorem \ref{theo:intermediary} in Section \ref{app:sec:intermediary_theo}.

\begin{corollary}\label{cor:clustered}
	Even with no $\alpha$ such that $\COV{\omega_i(S_n)}{\omega_j(S_n)} = - \alpha p_i p_j$, the bound of Theorem \ref{theo:convergence_paper} still holds with $B$, $C$, and $D$ defined as in Section \ref{app:sec:intermediary_theo} and 
	\begin{equation}
	A = m \left[\frac{1}{m}
	- \frac{1}{m^2} \sum_{i=1}^M \sum_{k=1}^{m}r_{k, i}^2 + \sum_{i=1}^Mp_i^2\right]
	,\
	E 
	= \frac{1}{m}(K-1)
	,
	\text{ and }
	F
	= \frac{1}{m}K
	,
	\end{equation}
	where $E$ and $F$ are identical to the one for MD sampling and $A$ is smaller than the one for Clustered sampling.
\end{corollary}


\begin{proof}
	The covariance property required for Theorem \ref{theo:intermediary} is only used for Lemma \ref{lem:decompo_Xi}. In the proof of Theorem \ref{theo:intermediary}, Lemma \ref{lem:decompo_Xi} is only used in equation (\ref{app:eq:B4}). We can instead use Lemma \ref{lem:decompo_Xiclustered} and keep the rest of the proof as it is in Section \ref{app:sec:intermediary_theo}. Therefore, the bound of Theorem \ref{theo:intermediary} remains unchanged for clustered sampling where $E$ and $F$ use the aggregation weight statistics of MD sampling instead of clustered sampling. Statistics for MD sampling can be found in Section \ref{app:sec:MD} and gives
	\begin{equation}
	\VAR{\sum_{i=1}^M\omega_i(S_{MD})} =0
	\text{ and }
	\alpha_{MD} = \frac{1}{m}.
	\end{equation}
	and the ones of clustered sampling in Section \ref{app:sec:clustered} gives
	\begin{equation}
	\sum_{i=1}^M \VAR{\omega_i(S_{Cl})} 
	= \frac{1}{m}
	- \frac{1}{m^2} \sum_{i=1}^M \sum_{k=1}^{m}r_{k, i}^2
	\le \sum_{i=1}^M \VAR{\omega_i(S_{MD})} 
	.
	\end{equation}
	
\end{proof}



%\cite{ClusteredSampling} introduces \textit{clustered sampling}, a client sampling satisfying Definition \ref{def:sampling} and generalizing MD sampling. Coupling \textit{clustered sampling} with FL was proposed in \cite{ClusteredSampling} to improve MD sampling. Instead of sampling $m$ clients from $m$ the same distribution, $m$ clients are sampled from $m$ different distributions. As a result, clustered sampling generalizes MD sampling and $\VAR{\sum_{i=1}^M\omega_i(S_n)} = 0$. \cite{ClusteredSampling} provide identical convergence rate for clustered and MD sampling and experimentally show clustered sampling improvements over MD sampling. Based on the proof of Theorem \ref{theo:convergence_paper}, we differ to Appendix \ref{app:sec:clustered_convergence} the adjustment of Theorem \ref{theo:convergence_paper} for clustered sampling where we theoretically show the advantages of clustered sampling over MD sampling.




\subsection{ Proof of Corollary \ref{cor:sufficient_conditions}}\label{app:sec:sufficient_conditions} 

\begin{proof}
	
	Combining equation (\ref{app:eq:R1}) with equation (\ref{app:eq:S2}) gives
	\begin{align}
		\Sigma_{MD}
		- \Sigma_U
		& = \left[ - \frac{1}{m} \sum_{i=1}^Mp_i^2 + \frac{1}{m} \right]
		- \left( \frac{n}{m} - 1 \right) \sum_{i=1}^Mp_i^2
		\\
		& = - \frac{1}{m}\left[(n- m +1) \sum_{i=1}^M p_i^2 -1 \right]
		.
		\label{app:eq:N1}
	\end{align}
	Therefore, we have
	\begin{equation}
		\Sigma_{MD} \le \Sigma_U
		\Leftrightarrow
		\sum_{i=1}^Mp_i^2 
		\le 
		\frac{1}{n - m +1}
	\end{equation}
	
	Combining equation (\ref{app:eq:R2}), (\ref{app:eq:R3}), (\ref{app:eq:S5}), and (\ref{app:eq:S6}) gives
	\begin{align}
	\gamma_{MD} - \gamma_{U}
	&= \sum_{i=1}^M \VAR{  \omega_i(S_{MD})} + \alpha_{MD} \sum_{i=1}^M p_i^2
	- \left( \sum_{i=1}^M   \VAR{ \omega_i(S_{U})} + \alpha_U \sum_{i=1}^M  p_i^2 \right)
	\\
	& = \frac{1}{m} - \frac{n-m}{m (n-1)} n \sum_{i=1}^Mp_i^2
	.
	\label{app:eq:N2}
	\end{align}
	
	Therefore, we have
	\begin{equation}
	\gamma_{MD} \le \gamma_U
	\Leftrightarrow
	\sum_{i=1}^Mp_i^2 
	\le 
	\frac{1}{n-m} \frac{n-1}{n}
	.
	\end{equation}

	Noting that 
	\begin{equation}
		\frac{1}{n - m +1} - \frac{1}{n-m} \frac{n-1}{n} 
		= \frac{-m +1}{n (n-m )(n-m+1)}
		\le 0
	\end{equation}
	completes the proof.
%	We also consider a local learning rate $\eta_l$ such that $ \Omega_{MD} \ll 1$ and $ \Omega_{U} \ll 1$. Hence, subtracting equation (\ref{app:eq:end_intermediary}) estimated for FedAvg with Uniform sampling to equation (\ref{app:eq:end_intermediary}) estimated for FedAvg with MD sampling gives
%	\begin{align}
%		D
%		& =  2L  \tilde{\eta} \left[ \sum_{i=1}^M \VAR{\omega_i(S_{MD})}
%		- \sum_{i=1}^M \VAR{\omega_i(S_{U})} \right] \sigma^2 
%		\nonumber\\
%		& + \tilde{\eta} R \left[ 3L (K-1) \sigma^2 + 2 L \left( L^2 + 2 \right) K \kappa^2 \right]
%		\label{app:eq:N5}
%	\end{align}
%	Substituting equation (\ref{app:eq:N1}) and (\ref{app:eq:N2}) in equation (\ref{app:eq:N5}) gives
%	\begin{align}
%		D
%		& \le  2L  \tilde{\eta} \frac{1}{m} \abs{ 1 - (n- m +1) \sum_{i=1}^M p_i^2 } \sigma^2 
%		\nonumber\\
%		& + \tilde{\eta} \frac{1}{m} \abs{1 - \frac{n-m}{n-1} n \sum_{i=1}^Mp_i^2} \left[ 3L (K-1) \sigma^2 + 2 L \left( L^2 + 2 \right) K \kappa^2 \right]
%		\label{app:eq:N6}
%	\end{align}
%	Considering that clients importance satisfy $p_i = \Ocal(\frac{1}{n})$, we have $\sum_{i=1}^Mp_i^2 = \Ocal(\frac{1}{n})$ which gives
%	\begin{align}
%	D
%	& = \Ocal \left( \eta_g \eta_l \left(- \frac{1}{m}\left[(n- m +1) \frac{1}{n} -1 \right] \right) \sigma^2 \right)
%	\nonumber\\
%	& + \Ocal\left(\eta_g \eta_l \left( \frac{1}{m} - \frac{n-m}{m (n-1)} \right) [(K -1)\sigma^2 + K \kappa^2] \right)
%	\\
%	& = \Ocal \left( \eta_g \eta_l \frac{m-1}{m n} \sigma^2 \right)
%	+ \Ocal\left(\eta_g \eta_l \frac{m-1}{m (n-1)} [(K -1)\sigma^2 + K \kappa^2] \right)
%	\\
%	& = \Ocal \left( \eta_g \eta_l \frac{1}{n} \sigma^2 \right)
%	+ \Ocal\left(\eta_g \eta_l \frac{1}{n} [(K -1)\sigma^2 + K \kappa^2] \right)
%	\\
%	& = \Ocal\left(\eta_g \eta_l \frac{1}{n} K[\sigma^2 + \kappa^2] \right)
%	,
%	\label{app:eq:N7}
%	\end{align}
%	which completes the proof.
	
\end{proof}


































==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/delayed_proofs/proof_main_theorem.tex <==
\section{Proof of Theorem \ref{theo:convergence_convex}} 
\label{app:sec:convergence_convex}

We first provide in Section \ref{app:subsec:inequalities} the basic inequalities used in our proofs, and in Section \ref{app:subsec:notation} the basic notations used to provide clearer proofs.


\subsection{Basic Inequalities}\label{app:subsec:inequalities}
\input{./delayed_proofs/common_ground.tex}

\input{./delayed_proofs/variables}

\subsection{Additional Notation}\label{app:subsec:notation}
\input{./delayed_proofs/new_quantities.tex}




\subsection{Useful Lemmas}\label{app:subsec:useful_lemmas}
\input{./delayed_proofs/Lemma_equality.tex}
\input{./delayed_proofs/bounding_client_drift.tex}
\input{./delayed_proofs/property_convex_functions.tex}
\input{./delayed_proofs/bounding_R.tex}
\input{./delayed_proofs/bounding_Q.tex}

\subsection{Proof of Theorem \ref{theo:convergence_convex}}\label{app:subsec:proof_theo}
\input{./delayed_proofs/convergence_convex_2.tex}



\subsection{Simplifying the constraint on the learning rate}\label{app:subsec:learning_rate}
\input{./delayed_proofs/constraints_lr.tex}

==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/delayed_proofs/property_convex_functions.tex <==
\begin{lemma}\label{lem:Dxn}
	Under Assumption  \ref{ass:strong_convexity} and \ref{ass:unbiased}, we have
	\begin{align}
	-2 D(\vx, n)
	&\le -2 \Xi(n) 
	+ 4 L q(n) \tau \sum_{s=1}^\tau  Q(n - s) 
	+ 4 D Z(n)
	+ 6 \eta_l^2 (K-1)^2 q(n) L \sigma_1(n)
	.
	\end{align}
\end{lemma}

\begin{proof}
	Follows directly from using Lemma 12 in \cite{Khaled2020} on $D(\vx, n, k)$, taking the mean over $K$, and using Lemma \ref{lem:phi_nk} to bound $\phi(n)$ completes the proof.
	
%	Using Lemma 12 in \cite{Khaled2020}, we have
%	\begin{align}
%	- 2 D(\vx, n, k)
%	&\le -2 \sum_{ i = 1 }^M \tilde{q}_i(n) 
%	\E{ \Lcal_i(\vtheta^{n, k}) - \Lcal_i( \vx ) 
%	}
%	\nonumber\\
%	& +\sum_{ i = 1 }^M \tilde{q}_i(n) 
%	\E{ L \norm{\vtheta_i^{\rho_i(n), k} - \vtheta^{n, k}}^2
%		- \mu \norm{\vtheta^{n,k} - \vx}^2
%	}
%	\\
%	&= -2 \E{ \tilde{\Lcal}^n(\vtheta^{n,k}) - \tilde{\Lcal}^n(\vx)}
%	+ L \phi(n, k)
%	- \mu \E{\norm{\vtheta^{n,k} - \vx}^2}
%	.
%	\end{align}	
%	Summing over $K$ gives
%	\begin{align}
%	- 2 D(\vx, n)
%	&\le -2  \sum_{ k = 0 }^{K-1}\E{ \tilde{\Lcal}^n(\vtheta^{n, k}) - \tilde{\Lcal}^n(\vx)} 
%	+ L \phi(n)
%	- \mu \sum_{ k = 0 }^{K-1} \E{\norm{\vtheta^{n,k} - \vx}^2}
%	.
%	\end{align}
%	Replacing $\phi(n)$ by its close-form (Lemma \ref{lem:phi_nk}) completes the proof.

	
\end{proof}

==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/delayed_proofs/variables.tex <==
\begin{table}
	\caption{Common Notation Summary (addition to Table \ref{tab:aggregation_weights}).}
	\label{tab:parameters}
	\centering
	\begin{tabular}{cc}
		\hline
		Symbol     & Description    \\
		\hline
		$M$ & Number of clients. \\
		$K$ & Number of local SGD.  \\
		$\eta_g, \eta_l$ & Global/Local learning rate.\\
		$\tilde{\eta}$ & Effective learning rate, $\tilde{\eta} = \eta_l \eta_g$.\\
		
		$\vtheta^n$ & Global model at server iteration $n$.  \\
		$\vtheta_i^{n+1}$ & Local update of client $i$ on model $\vtheta^n$.\\
		$\vtheta^*$, $\vtheta_i^*$ & Optimum of the federated problem (\ref{eq:original_problem_general})/client $i$. \\
		$\vtheta^{(n, k)}$, $\vtheta_i^{(n, k)}$ & Global/Local update after $k$ SGD on global model $\vtheta^n$.\\
		$\alpha$ & Covariance parameter.\\
		$\beta$ & Defined in Theorem \ref{theo:convergence_convex}.\\
		% 		$\delta_i, \delta_i^*$ & cf Section \ref{sec:convergence}\\
		% 		$\mu^*$ & Jensen gap parameter, cf Section \ref{sec:convergence}\\
		
		% 		$\EE{n}{\cdot}$ & Expected value conditioned on $\vtheta^n$.\\
		$\Lcal(\cdot), \Lcal_i(\cdot)$ & Federated/local loss function.\\
		% 		$\Lcal_i(\cdot)$ & Local loss function of client $i$.\\
		$g_i(\cdot)$ & SG. We have $\EE{\xi_i}{g_i(\cdot)} = \nabla \Lcal_i(\cdot)$ with Assumption \ref{ass:unbiased}.\\
		$\vxi_i$ & Random batch of samples from client $i$ of size $B$.\\
		
		
		$L$ & Lipschitz smoothness parameter, Assumption \ref{ass:smoothness}.\\
		% 		$\mu$ & Strong convexity parameter. \\
		
		$T_i$ & Computation time of client $i$. \\
		$t^n$ & Time at aggregation $n$. \\
		$T_i^n$ & Remaining computation time of client $i$ at time $t^n$. \\
		$\Delta t^n$ & Time elapsed between two server aggregations. \\
		$\rho_i(n)$ & Last index at which a client $i$ received its global model. \\
		% 		& TO COMPLETE?\\
		
		$\rho$ & Highest sum of aggregation weights, i.e. $\rho \coloneqq \max \left(1, q(n)\right)$\\
		
		
		\hline
	\end{tabular}
\end{table}

==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/FL.tex <==
\section{Applications} \label{sec:applications}

In this section, we show that the formalism of Section \ref{sec:background} can be applied to a wide-range of optimization schemes, demonstrating the validity of the conclusions of Corollary \ref{cor:bias_distributions} and Theorem \ref{theo:relaxed_sufficient_conditions} (Section \ref{sec:convergence}). 
When clients have identical data distributions, the sufficient conditions of Corollary \ref{cor:bias_distributions} are always satisfied (Section \ref{sec:convergence}). 
In the heterogeneous case, these conditions can also (theoretically) be satisfied. It suffices that every client has a non-null participation probability, i.e. $\mathbb{P}( T_i^n \le \Delta t^n) >0$ such that there exists an appropriate $d_i(n)$ satisfying $\tilde{q}_i(n) = p_i$.
Yet, in practice clients generally may not even know their update time distribution $\mathbb{P}( T_i^n)$ making the computation of $d_i(n)$ intractable. In what follows, we thus focus on Theorem \ref{theo:relaxed_sufficient_conditions} to obtain the close-form of $\epsilon$, which only requires from the server to know the clients time $\tau_i$.

Theorem \ref{theo:relaxed_sufficient_conditions} provides a close-form for the convergence bound $\epsilon$ of an optimization scheme in function of the amount of server aggregation rounds $N$.
We first introduce in Section \ref{subsec:specifications} our considerations for the clients hardware and data to instead express $\epsilon$ in function of the training time $T$.
The quantity $\epsilon$ also depends on the optimization scheme time policy $\Delta t^n$ through $\alpha$, $\beta$ and $\tau$, and on the clients data heterogeneity through $R(\{\Lcal^n\})$ and $W$. We provide their close-form for synchronous \textsc{FedAvg} (Section \ref{subsec:synchronous}), asynchronous \textsc{FedAvg} (Section \ref{subsec:async_FL}), 
% where a new global model is created whenever a client updates its work to the server, 
and \textsc{FedFix} (Section \ref{subsec:FedFix}), a novel asynchronous optimization scheme motivated by Section \ref{subsec:relaxed_sufficient}.
% where aggregations are made at fixed clock times using all the available clients contribution received during the fixed time window.
Finally, in Section \ref{subsec:generalization}, we show that the conclusions drawn for synchronous/asynchronous \textsc{FedAvg} and \textsc{FedFix} can also be extended to other distributed optimization schemes with delayed gradients.
Of course, similar bounds can seamlessly be derived for centralized learning and client sampling, which we differ to Appendix \ref{app:sec:applying} to focus on asynchronous FL in this section.


% \input{tex/specifications}





% In this section, we show that the formalism of Section \ref{sec:background} can be applied to a wide-range of optimization schemes, demonstrating the validity of the conclusions of Corollary \ref{cor:bias_distributions} and Theorem \ref{theo:relaxed_sufficient_conditions} in Section \ref{sec:convergence}. 
% Theorem \ref{theo:relaxed_sufficient_conditions} provides a close-form for the convergence bound $\epsilon$ of an optimization scheme in function of the amount of server aggregation rounds $N$.
% The quantity $\epsilon$ depends on the optimization scheme time policy $\Delta t^n$ through $\alpha$, $\beta$ and $\tau$, and on the clients data heterogeneity through $R(\{\Lcal^n\})$ and $W$. In this section, we provide their close-form for each optimization scheme investigated in this section, and compare the resulting $\epsilon$ with the state-of-the-art bound for any given optimization scheme.

% This section is structured as follows. 
% In Section \ref{subsec:async_FL}, we provide the convergence bound of asynchronous \textsc{FedAvg}, where a new global model is created whenever a client updates its work to the server. In Section \ref{subsec:FedFix}, we introduce and provide the convergence bound of \textsc{FedFix}, a novel asynchronous optimization scheme motivated by Section \ref{subsec:relaxed_sufficient}, where aggregations are made at fixed clock times using all the available clients contribution received during the fixed time window. 
% Finally, in Section \ref{subsec:generalization}, we show that the conclusions drawn for asynchronous \textsc{FedAvg} and \textsc{FedFix} can also be extended to other distributed optimization schemes with delayed gradients.
% Of course, similar bounds can seamlessly be derived for centralized learning, synchronous \textsc{FedAvg}, and client sampling, which we differ to Appendix \ref{app:sec:applying} to focus on asynchronous FL in this section.

\input{tex/specifications}


% In what follows, we investigate (a) \textbf{centralized learning} where clients data is centralized to the server ($M=1$) before initiating the learning process, (b) \textbf{synchronous FL} with \textsc{FedAvg}, where the server waits for every participating clients to perform their local work before aggregating their contributions, (c) \textbf{asynchronous FL}, where a new global model is created whenever a client updates its work to the server, and (d) \textbf{\textsc{FedFix}}, a novel asynchronous FL setting motivated by Section \ref{subsec:relaxed_sufficient}, where aggregations are made at fixed clock times using all the available clients contribution received during the fixed time window. Finally, we show that the conclusions drawn for (a)-(d) can be extended to other distributed optimization schemes with delayed gradients.

%\input{./tex/one_client.tex}
%
\input{./tex/FedAvg.tex}

\input{./tex/async_FL.tex}

\input{./tex/hybrid_FL.tex}

\input{./tex/generalization.tex}



==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/FedAvg.tex <==
\subsection{\textsc{FedAvg}, Synchronous Federated Learning}\label{subsec:synchronous}

As described for \textsc{FedAvg} in Section \ref{subsec:agg_schem}, at every optimization round, the server sends to the clients the current global model to perform $K$ SGD steps on their own data before returning the resulting model to the server. Once every client performs its local work, the new global model is created as the weighted average of the clients contribution. 
The time required for an optimization step is therefore the one of the slowest client ($\Delta t^n = \max_i(T_i^n)$), and every client is considered ($\mathbb{P}( T_i^n \le \Delta t^n) = 1$). Hence, $\alpha= 1$, $\beta = 0$, and setting $d_i = p_i$ is sufficient to satisfy the conditions of Corollary \ref{cor:bias_distributions} (and thus the ones of Theorem \ref{theo:relaxed_sufficient_conditions}) ensuring that FL converges to its optimum \citep{FedNova}. The term $\epsilon$ then reduces to
\begin{align}
\epsilon_{\textsc{FedAvg}}
&=\frac{1}{\sqrt{K N} } \norm{\vtheta^0 -\vtheta^*}^2 
+ \Ocal \left(\frac{K-1}{N} \Sigma \right)
+ \Ocal\left(\frac{1}{\sqrt{K N} } \frac{1}{M} \Sigma 
\right)
\label{eq:epsilon_sync_FL}
.
\end{align}
The second element of equation (\refeq{eq:epsilon_sync_FL}) accounts for the clients update disparity through their amount of local work $K$ between two server aggregations, and is proportional to the SG variance $\Sigma$.
The third element benefits of the distributed computation by being proportional to $1/M$. Equation (\refeq{eq:epsilon_sync_FL}) is consistent with literature on convex distributed optimization with \textsc{FedAvg} including \cite{FedNova, Khaled2020}.


==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/abbreviations.tex <==
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\tabref}[1]{Tab.~\ref{#1}}
\newcommand{\eqnref}[1]{Eq.~(\ref{#1})}

\newcommand{\tbc}[0]{\textbf{> > > TO BE CHECKED < < <}}
\newcommand{\tbm}[0]{\textbf{> > > TO BE MODIFIED < < <}}
\newcommand{\tbe}[0]{\textbf{> > > TO BE EXPANDED < < <}}

\newcommand{\cf}[0]{\textit{cf. }}
\newcommand{\eg}[0]{\textit{e.g., }}
\newcommand{\ibid}[0]{\textit{ibid.}}
\newcommand{\ie}[0]{\textit{i.e.,}}

\newcommand{\suppmat}[0]{\hyperref[sec:supmat]{\textit{Supplementary Material}} }
\newcommand{\asuppmat}[0]{\hyperref[sec:supmat]{\textit{Sup. Mat.}} }


==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/abstracts.tex <==
\begin{abstract}%   <- trailing '%' for backward compatibility of .sty file
	We propose a novel framework to study asynchronous federated learning optimization with delays in gradient updates. Our theoretical framework extends the standard \textsc{FedAvg} aggregation scheme by introducing stochastic aggregation weights to represent the variability of the clients update time, due for example to heterogeneous hardware capabilities. Our formalism applies to the general federated setting where clients have heterogeneous datasets and perform at least one step of stochastic gradient descent (SGD). We demonstrate convergence for such a scheme and provide sufficient conditions for the related minimum to be the optimum of the federated problem. We show that our general framework applies to existing optimization schemes including centralized learning, \textsc{FedAvg}, asynchronous \textsc{FedAvg}, and \textsc{FedBuff}. The theory here provided allows drawing meaningful guidelines for designing a federated learning experiment in heterogeneous conditions. In particular, we develop in this work \textsc{FedFix}, a novel extension of \textsc{FedAvg} enabling efficient asynchronous federated training while preserving the convergence stability of synchronous aggregation. We empirically demonstrate our theory on a series of experiments showing that asynchronous \textsc{FedAvg} leads to fast convergence at the expense of stability, and we finally demonstrate  the improvements of \textsc{FedFix} over synchronous and asynchronous \textsc{FedAvg}.
\end{abstract}

% \begin{keywords}
% 	federated optimization, asynchronicity, heterogeneous data.
% \end{keywords}

==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/acknowledgements.tex <==
\subsection*{Acknowledgments}

This work has been supported by the French government, through the 3IA C\^ote d'Azur Investments in the Future project managed by the National Research Agency (ANR) with the reference number ANR-19-P3IA-0002, and by the ANR JCJC project Fed-BioMed 19-CE45-0006-01. The project was also supported by Accenture.
The authors are grateful to the OPAL infrastructure from Université C\^ote d'Azur for providing resources and support.

==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/additional_exp.tex <==
\section{Additional Experiments}\label{app:sec:experiments}

\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{./plots/app_fig_explore_opt_scheme_CIFAR10_20.pdf}
	\caption{Evolution of federated problem (\ref{eq:original_problem_general}) loss for CIFAR10 and time scenario $F80$ with $M=20$ and $K=10$.}
	\label{app:fig:explore_CIFAR10_20}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{./plots/app_fig_explore_opt_scheme_CIFAR10_50.pdf}
	\caption{Evolution of federated problem (\ref{eq:original_problem_general}) loss for CIFAR10 and time scenario $F80$ with $M=50$ and $K = 10$.}
	\label{app:fig:explore_CIFAR10_50}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{./plots/app_fig_explore_opt_scheme_Shakespeare_20.pdf}
	\caption{Evolution of federated problem (\ref{eq:original_problem_general}) loss for Shakespeare and time scenario $F80$ with $M=20$ and $K = 10$.}
	\label{app:fig:explore_Shakespeare_20}
\end{figure}



==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/applying_theo.tex <==
\section{Applying Theorem \ref{theo:relaxed_sufficient_conditions}}
\label{app:sec:applying}

This section extends Section \ref{sec:applications}, where we apply Theorem \ref{theo:relaxed_sufficient_conditions} to centralized learning (Section \ref{subsec:centralized_learning}) and synchronous \textsc{FedAvg} with unbiased and biased client sampling (Section \ref{subsec:client_sampling_unbiased} and \ref{subsec:client_sampling_biased} respectively).

\input{./tex/one_client.tex}
\input{./tex/client_sampling.tex}

==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/async_FL.tex <==
\subsection{Asynchronous \textsc{FedAvg}}
\label{subsec:async_FL}

With \textsc{FedAvg}, every client waits for the slowest one to perform its local work, and cannot contribute to the learning process during this waiting time. To remove this bottleneck, with asynchronous \textsc{FedAvg}, the server creates a new global model whenever it receives a client contribution before sending it back to this client. 
For in depth discussion of Asynchronous \textsc{FedAvg}, please refer to \cite{AFLsurvey}. 

With asynchronous \textsc{FedAvg},
clients always compute their local work but each on a different global model, giving $\Delta t^n = \min_i T_i^n$, $\alpha = 0$, and $\beta = \max_i d_i$. In addition, while the slowest client updates its local work, other clients performs a fix amount of updates (up to $\ceil{\tau_M/\tau_i}$). By scaling this amount of updates by the amount of clients sending updates to the server, we have 
\begin{equation}
    \tau = \Ocal\left(\frac{\tau_M}{\tau_0}(M-1)\right)
    .
\end{equation} 

We define $lcm(\{x_i\})$ the function returning the least common multiplier of the set of integers $\{x_i\}$. Hence, after every $\nu \coloneqq lcm(\{\tau_i\})$ time, each client has performed $\nu /\tau_i$ optimization rounds and the cycle of clients update repeats itself. Thus, the smallest window $W$ satisfies
\begin{equation}
	W
	= \sum_{ i = 1 }^M \nu / \tau_i
	.
\end{equation}
By construction, $\nu \ge \tau_M$ and thus $W = \Omega(M)$, with $W=M$ when clients have homogeneous hardware ($\tau_M = \tau_0$). In the worse case, every $\tau_i$ is a prime number, and we have $\nu / \tau_i \le \left(\tau_M\right)^{M-1}$, which gives $W = \Ocal(M \left( \tau_M\right)^{M-1})$. 
% When clients have homogeneous hardware, we have $W = \Ocal(M)$, while when their hardware is heterogeneous, $W$ is exponentially proportional to $M$. 
% This explains why convergence for asynchronous FL applications gets more challenging as the amount of clients $M$ increases, since $W$ captures the hardware heterogeneity among clients.
In a cycle of $W$ optimization rounds, every client participates $\nu /\tau_i$ times to the creation of a new global model. 
Therefore, we have $q_i(n) = d_i$ for the $\nu / \tau_i$ participation of client $i$, and $q_i(n) = 0$ otherwise.
Hence, the sufficient conditions of Theorem \ref{theo:relaxed_sufficient_conditions} are satisfied when 
\begin{equation}
\label{eq:aggreg_weights_async}
q_i
= \frac{1}{W}\sum_{ n = kW }^{(k+1)W - 1 }q_i(n) 
= \frac{1}{\sum_{ i = 1 }^M \nu / \tau_i}\frac{ \nu}{\tau_i }
d_i
= p_i
\Rightarrow
d_i
= \left[\sum_{ i = 1 }^M \frac{1}{\tau_i}\right] \tau_i p_i
.
\end{equation}
The client weight calculated in equation (\refeq{eq:aggreg_weights_async}) is constant and only depends on the client importance $p_i$ (set and thus known by the server), and on the clients computation time $\tau_i$ (eventually estimated by the server after some clients updates). The condition on $d_i$ can be further simplified by accounting for the server learning rate $\eta_g$. Coupling equation (\refeq{eq:aggreg_SCAFFOLD_general}) with equation (\refeq{eq:aggreg_weights_async}) gives $\eta_g d_i \propto \tau_i p_i$, which is sufficient to guarantee the convergence of asynchronous FL to its optimum. 
Finally, by bounding $\tau_i$, we also have $\beta = \max_i d_i \le \tau_M/ \tau_0$, bounded the hardware computation time heterogeneity.
%Therefore, knowing all the clients expected computation times $\tau_i$ is not needed to infer $d_i$. 

The disparity between the optimized objectives $R(\{\Lcal^n\})$ at different optimization rounds also slows down the learning process. Indeed, at every optimization round, only a single client can participate with probability $1$. As such, we have $\Lcal^n = d_i \Lcal_i$ which, thanks to the assumption $p_i = 1/M$, yields 
\begin{equation}
	R( \{\Lcal^n\})
	= \frac{1}{M} \sum_{ i = 1 }^M \left[\Lcal_i(\vtheta^*) - \Lcal_i(\vtheta_i^*)\right]
	.
\end{equation}
Finally, we simplify the close-form of $\epsilon$ (Theorem \ref{theo:relaxed_sufficient_conditions}) for asynchronous \textsc{FedAvg} to get
\begin{align}
\epsilon_{Async}
&= 
\frac{1}{\sqrt{KN}} \norm{\vtheta^0 -\vtheta^*}^2
+ \Ocal \left(\frac{K-1}{N} \Sigma \right)
% + \Ocal\left(\frac{1}{\sqrt{KN}}
% \left[R(\{\Lcal^n\})
% + \frac{\tau_M}{\tau_0}\Sigma\right]\right)
+ \Ocal\left(\frac{\tau_M}{\tau_0} \frac{1}{\sqrt{KN}} \left[ R(\{\Lcal^n\}) + \Sigma \right]\right)
\nonumber\\
&
% + \Ocal \left( \frac{K}{N} M^2 \left(\frac{\tau_M}{\tau_0}\right)^2
% \left[ \Sigma + R(\{\Lcal^n\}) \right]\right)
% &
+ \Ocal\left( \left(\frac{\tau_M}{\tau_0}\right)^3 \frac{K}{N} M^2 \left[ R(\{\Lcal^n\}) + \Sigma \right]\right)
+ \Ocal\left(  \frac{1}{\sqrt{KN}} (W-1)\right)
\label{eq:epsilon_async}
.
\end{align}
With equation (\refeq{eq:epsilon_async}), we can compare synchronous and asynchronous \textsc{FedAvg}.
The first and second asymptotic terms are identical for the two learning algorithms, while the third asymptotic term is scaled by the hardware characteristics $\tau_M/\tau_0$ instead of $1/M$ in $\textsc{FedAvg}$, with the addition of a non null residual $R(\{\Lcal^n\})$ for asynchronous \textsc{FedAvg}. 
However, the fourth and fifth term are unique to asynchronous \textsc{FedAvg}, and explains why its convergence gets more challenging as the amount of clients $M$ increases.
The impact of the hardware heterogeneity is also identified through the importance of $\tau_M/ \tau_0$ in the third term. With no surprise, for a given optimization round, synchronous \textsc{FedAvg} outperforms its asynchronous counterpart. However, in $T$ time, the server performs 
\begin{equation}
    N = \sum_{i=1}^M T / \tau_i
\end{equation}
aggregations with asynchronous \textsc{FedAvg} against $T/ \tau_M$ for synchronous \textsc{FedAvg}. With asynchronous \textsc{FedAvg}, the server thus performs at least $M$ times more aggregations than with synchronous \textsc{FedAvg}. As a result, the first two terms of equation (\ref{eq:epsilon_async}), which are proportional to how good the initial model is $\norm{\vtheta_0 - \vtheta^*}$, decrease faster with asynchronous \textsc{FedAvg} at the detriment of an higher convergence residual coming for the two last terms.


\textbf{Comparison with asynchronous DL and \textsc{FedAvg} literature.} The convergence rates obtained in the convex distributed optimization literature relies on additional assumptions to ours, with which we retrieve their proposed convergence rate. 
To the best of our knowledge, only \cite{SlowLearnersAreFast} considers non-iid data distributions for the clients. When assuming $W = \Ocal(\tau)$ and $\eta_l \propto 1/ \sqrt{\tau N}$, we retrieve a convergence rate$\sqrt{\tau/ N}$. 

We also match convergence rates for literature with iid client data distributions and $K=1$. With $M = \Ocal(\sqrt{N})$, then 
we have $\Ocal(1/\sqrt{N})$ \citep{DistributedDelayed, AsyncParallelSGDforNonconvex}.
When $\eta_l = \Ocal( 1 /\tau \sqrt{KN})$, we retrieve $\tau/N + 1/\sqrt{N}$ \citep{ErrorFeedbackFramework, StichCriticalParameters}. 


% With $\tau = \Ocal(M)$, we retrieve $\epsilon = \Ocal(M/T)$.\cite{arjevani20a}

% \textbf{Comparison with asynchronous \textsc{FedAvg} literature.}
% The authors of \cite{ErrorFeedbackFramework} consider similar assumptions to ours and provide a convergence rate of $\tau/N + 1/\sqrt{N}$.

% For asynchronous \textsc{FedAvg} in the non-iid case, we have
% \cite{ErrorFeedbackFramework}

% \cite{ErrorFeedbackFramework} for (asynchronous) FL. The authors make the same assumptions as us while also proving convergence for non convex functions. However, authors assume iid data distributions. Authors also introduce the notion of compressors. The delay scenario considered is $\tau = M$.
% Interesting, they have a convergence bound of the form $\epsilon = \Ocal ( M e(M/T)  + 1 / T )$ while we have $\epsilon = \Ocal ( 1/ \sqrt{MT} + M / T )$. However the learnt model is not the one at the end of the learning process but instead a weighted sum of all the global model with weights $(1 - \mu \eta_l)^{-n}$.  


% \cite{OptimalDistributedOnline} 



% Existing work on asynchronous \textsc{FedAvg} shows its interest over synchronous \textsc{FedAvg} through experimental comparison
% \cite{}
% \cite{RevisitingDistributedSynchronousSGD,EfficientAndRobust,PrivacyPreservingAsynchronous,HowSlowCanYouGo}

% Heterogeneous amount of local work \cite{AsynchronousFOpti}

% FedBuff
% \cite{FedBuff}
% \cite{RevisitingDistributedSynchronousSGD}

% Data shared across clients\cite{Hogwild}

% Synchronous aggregations but different amount of local work. \cite{AsynchronousFOpti}




% Interesting work on lower bounds \cite{GraphOracleModels}.

% Authors assume that $K + \tau = \Ocal\left( \sqrt{T/M}\right)$
% which gives them a convergence rate of $\Ocal(1/MT)$.
% \cite{stich2018local} Proposed optimization problem by bounding the clients gradient dissimilarity. A synchronous and asynchronous framework are proposed while considering non-iid data distributions. 

% \cite{Chen2021} strongly convex






==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/background.tex <==
\section{Background}\label{sec:background}

We define here the formalism  required by the theory that will be introduced in the following sections.
We first introduce in Section \ref{subsec:background_FedAvg} the FL optimization problem, and we adapt it in section \ref{subsec:formalize_delays} to account for delays in client contributions. We then generalize in Section \ref{subsec:agg_schem} the \textsc{FedAvg} aggregation scheme to account for contributions delays. 
In Section \ref{subsec:FL_one_SGD}, we introduce the notion of virtual global models as a direct generalization of gradient descent, and introduce in Section \ref{subsec:sequence_opt_problems} the final asynchronous FL optimization problem. Finally, we introduce in Section \ref{subsec:heterogeneity_across_clients} a formalization of the concept of data heterogeneity across clients.



\subsection{Federated Optimization Problem}\label{subsec:background_FedAvg}

We have $M$ participants owning $n_i$ data points $\{\vz_{k, i}\}_{k=1}^{n_i}$ independently sampled from a fixed 
unknown distribution over a sample space $\{\mathcal{Z}_i\}_{i=1}^M$.
We have $\vz_{k, i} = (\vx_{k, i}, \vy_{k, i})$ for supervised learning, where $\vx_{k, i}$ is the input of the statistical model,  and $\vy_{k, i}$ its desired target, while we denote $\vz_{k, i} = \vx_{k, i}$ for unsupervised learning.
Each client optimizes the model's parameters $\vtheta$ based on the estimated local loss $l(\vtheta, \vz_{k, i})$. 
The aim of FL is solving a distributed optimization problem associated with the averaged loss across clients
\begin{equation}
\Lcal(\vtheta) 
\coloneqq \EE{z \sim \hat{\mathcal{Z}}}{l(\vtheta, \vz)}
= \frac{1}{\sum_{i=1}^M n_i}\sum_{i=1}^M \sum_{k=1}^{n_i} l(\vtheta, \vz_{k, i}) \label{eq:original_problem}
,
\end{equation}
where the expectation is taken with respect to the sample distribution $\hat{\mathcal{Z}}$ across the $M$ participating clients.
We consider a general form of the federated loss of equation (\refeq{eq:original_problem}) where 
clients local losses are weighted by an associated parameter $p_i$ such that $\sum_{i=1}^{n} p_i = 1$, i.e.
\begin{equation}
\label{eq:original_problem_general}
\Lcal(\vtheta) = \sum_{i=1}^Mp_i \Lcal_i(\vtheta)
\text{ s.t. }
\Lcal_i(\vtheta) = \frac{1}{n_i}\sum_{k=1}^{n_i} l(\vtheta, \vz_{k, i})
.
\end{equation}
%where $\vtheta$ represents the model parameters. 
The weight $p_i$ can be interpreted as the importance given by the server to client $i$ in the federated optimization problem. While any combination of $\{p_i\}$ is possible, we note that in typical FL formulations, either (a) every client has equal importance, i.e. $p_i = 1 / M$, or (b) every data point is equally important, i.e. $p_i = n_i / \sum_{i=1}^Mn_i$. 
%Unless stated otherwise, in the rest of this work, we consider $\exists i, \ p_i \neq 1/n$.

%In this setting, to estimate a global model across clients, \textsc{FedAvg} \citep{FedAvg} is an iterative training strategy based on the aggregation of local model parameters. At each iteration step $n$, the server sends the current global model parameters $\vtheta^n$ to the clients. Each client updates the respective model by minimizing the local cost function $\Lcal_i(\vtheta)$ through a fixed amount $K$ of SGD initialized with $\vtheta^n$. Subsequently each client returns the updated local parameters ${\vtheta}_i^{n+1}$ to the server. The global model parameters $\vtheta^{n+1}$ at the iteration step $n+1$ are then estimated as a weighted average
%\begin{equation}
%\label{eq:FedAvg_server_aggregation}
%\vtheta^{n+1} = \sum_{i=1}^M p_i \vtheta_i^{(n , K)}
%.
%\end{equation}

%To estimate a global model across clients, \textsc{FedAvg} \citep{FedAvg} is an iterative training strategy based on the aggregation of local model parameters. 
%We define by $\vtheta^n$ the global model after $n$ server aggregations and $\vtheta_i^{(n, k)}$ the local model of client $i$ after $k$ SGD steps initialized with $\vtheta^n$. We set $\vtheta_i^{(n, 0)} = \vtheta^n$.




\subsection{Asynchronicity in Clients Updates}\label{subsec:formalize_delays}

An optimization round starts at time $t^n$ with global model $\vtheta^n$, finishes at time $t^{n+1}$ with the new global model $\vtheta^{n+1}$, and takes $\Delta t^{n} = t^{n+1} - t^n$ time to complete. No assumptions are made on $\Delta t^{n}$, which can be a random variable, and we set for convenience $t^0 = 0$. In this section, we introduce the random variables needed to develop in Section \ref{subsec:agg_schem} the server aggregation scheme connecting two consecutive global models $\vtheta^n$ and $\vtheta^{n+1}$.

We define the random variable $T_i$ representing the update time needed for client $i$ to perform its local work and send it to the server for aggregation. $T_i$ depends on the client computation and communication hardware, and is assumed to be independent from the current optimization round $n$. 
If the server sets the FL round time to $\Delta t^{n} = \max_i T_i$, the aggregation is performed by waiting for the contribution of every client, and we retrieve the standard client-server communication scheme of synchronous \textsc{FedAvg}.

With asynchronous \textsc{FedAvg}, we need to relate $T_i$ to the server aggregation time $\Delta t^n$. 
We introduce $\rho_i(n)$ the index of the most recent global model received by client $i$ at optimization round $n$ and, by construction, we have $0 \le \rho_i(n) \le n$.
We define by 
\begin{equation}
	T_i^n 
	\coloneqq T_i - (t^n - t^{\rho_i(n)})
\end{equation}the remaining time at optimization round $n$ needed by client $i$ to complete its local work. 
%Similarly to $\Delta t^n$, no assumptions are made for $T_i$ or $T_i^n$, which can thus both be random variables. 

Comparing $T_i^n$ with $\Delta t^n$ indicates whether a client is participating to the optimization round or not, through the stochastic event $\mathbb{I}( T_i^n \le \Delta t^{n})$. When $\mathbb{I}( T_i^n \le \Delta t^n) = 1$, the local work of client $i$ is used to create the new global model $\vtheta^{n+1}$, while client $i$ does not contribute when $\mathbb{I}( T_i^n \le \Delta t^n) = 0$. With synchronous \textsc{FedAvg}, we retrieve $\mathbb{I}( T_i^n \le \Delta t^n) = \mathbb{I}( T_i \le \max_i T_i) = 1$ for every client.

\begin{figure}
	\includegraphics[width=\linewidth]{./plots/schematic_cropped_ungroup.pdf}
	\caption{Illustration of the time notations introduced in Section \ref{subsec:formalize_delays} with $M=2$ clients. The frequency of the updates of Client 1 (C1) is twice the one of Client 2 (C2). If the server (S) creates the new global model after every fixed waiting time ($\Delta t^n = \Delta t$), C1 contributes at every optimization round, while C2 contributes once every two rounds. This aggregation policy define the federated learning strategy \textsc{FedFix} (Section \ref{subsec:FedFix})}
	\label{fig:illustration}
\end{figure}

Figure \ref{fig:illustration} illustrates the notations described in this section in a FL process with $M=2$ clients.









\subsection{Server Aggregation Scheme}\label{subsec:agg_schem}

We consider $\vDelta_i(n)$ the contribution of client $i$ received by the server at optimization round $n$.
In the rest of this work, we consider that clients perform $K$ steps of SGD on the model they receive from the server. By calling their trained model $\vtheta_i^{(n, k)}$ after $k$ SGD, we can rewrite clients contribution for \textsc{FedAvg} as $\vDelta_i(n) \coloneqq \vtheta_i^{(n, K)} - \vtheta^n$, and the \textsc{FedAvg} aggregation scheme as
\begin{equation}
\label{eq:FedAvg_server_aggregation}
\vtheta^{n+1} 
\coloneqq \vtheta^n + \sum_{i=1}^M p_i \vDelta_i(n)
.
\end{equation}
With \textsc{FedAvg}, the server waits for every client to send its contribution $\vDelta_i(n)$ to create the new global model. To allow for partial computation within the server aggregation scheme, we introduce the aggregation weight $d_i(n)$ corresponding to the weight given by the server to client $i$ at optimization round $n$. We can then define the stochastic aggregation weight $\omega_i(n)$ given to client $i$ at optimization step $n$ as
\begin{equation}
\label{eq:agg_weights}
\omega_i(n) 
\coloneqq
\mathbb{I}( T_i^n \le \Delta t^{n}) d_i(n) ,
\end{equation}
with $\omega_i(n)= d_i(n)$ if client $i$ updated its work at optimization round $n$ and $\omega_i(n)= 0$ otherwise. 
In the general setting, client $i$ receives $\vtheta^{\rho_i(n) }$ and its contribution is $\vDelta_i(\rho_i(n)) = \vtheta_i^{(\rho_i(n), K) }- \vtheta^{\rho_i(n)}$. 
By weighting each delayed contribution $\vDelta_i(\rho_i(n))$ with its stochastic aggregation weight $\omega_i(n)$, we propose the following aggregation scheme  
\begin{equation}
\label{eq:aggreg_SCAFFOLD_general}
\vtheta^{n+1}
\coloneqq \vtheta^n + \eta_g \sum_{i =1}^M \omega_i(n)\vDelta_i(\rho_i(n)),
\end{equation}
where $\eta_g$ is a global learning rate that the server can use to mitigate the disparity in clients contributions \citep{reddi2021adaptive, SCAFFOLD, Wang2020SlowMo}. 
%This disparity can be caused either by the clients data heterogeneity, consideration of a subset of clients, or delayed clients local work. 
Equation (\ref{eq:aggreg_SCAFFOLD_general}) generalizes FedAvg aggregation scheme (\refeq{eq:FedAvg_server_aggregation}) ($\eta_g =1$ and $\Delta t^n = \max_i T_i$), and the one of \cite{OnTheImpact} based on client sampling.

%In this work, we use aggregation scheme (\refeq{eq:aggreg_SCAFFOLD_general}) to provide a unique theoretical framework under which we can determine the convergence guarantees of a wide range of asynchronous federated optimization schemes (Section \ref{sec:applications}). In particular, under the conditions $\Delta t^n = \max_i T_i$, when $\vDelta_i(n) = \vtheta_i^{(n , K)} - \vtheta^n$, $\omega_i(n) = p_i$ with $\eta_g =1$, equation (\refeq{eq:aggreg_SCAFFOLD_general}) reduces to the standard aggregation scheme of \textsc{FedAvg}.

%To account for delays in local work manifesting in $\vDelta_i(n)$. 
%The local work of client $i$ is thus performed with initialization $\vtheta^{(\rho_i(n), 0) }$ and with resulting contribution $\vDelta_i(n) = \vtheta_i^{(\rho_i(n), K) }- \vtheta^{\rho_i(n)}$. 
%With \textsc{FedAvg}, the server waits for every client so $\rho_i(n) =n$ and we retrieve $\vDelta_i(n) = \vtheta_i^{ (n, K) }- \vtheta^{n}$. 

We introduce with Algorithm \ref{alg:FL_with_delayed_gradients} the implementation of the optimization schemes satisfying aggregation scheme (\refeq{eq:aggreg_SCAFFOLD_general}) with stochastic aggregation weights satisfying equation (\refeq{eq:agg_weights}). 


% \label{alg:FL_with_delayed_gradients}
\begin{algorithm}
	\caption{Asynchronous Federated Learning based on equation (\ref{eq:aggreg_SCAFFOLD_general})
	}\label{alg:FL_with_delayed_gradients}
	\begin{algorithmic}[1]
		\Require server learning rate $\eta_g$, aggregation weights $\{d_i(n)\}$, number of SGD $K$, learning rate $\eta_l$, batch size $B$, aggregation time policy $\Delta t^n$.
		\State The server sends to the $M$ clients the learning parameters ($K$, $\eta_l$, $B$) and the initial global model $\vtheta^0$.
		
		\For{$n \in \{0, ..., N-1\}$}
		
		\State Clients in $S_n = \{i: T_i^n \le \Delta t^n\}$ send their contribution $\vDelta_i(\rho_i(n)) = \vtheta_i^{\rho_i(n)+1} -\vtheta^{\rho_i(n)}$ to the server.
		
		\State The server creates the new global model $\vtheta^{n+1} = \vtheta^n + \eta_g \sum_{ i \in S_n } d_i(n) \vDelta_i(\rho_i(n))$, equation (\refeq{eq:aggreg_SCAFFOLD_general}).
		
		\State The global model  $\vtheta^{n+1}$ is sent back to the clients in $S_n$.
		
		\EndFor
	\end{algorithmic}
\end{algorithm}


\subsection{Expressing FL as cumulative GD steps}\label{subsec:FL_one_SGD}
To obtain the tightest possible convergence bound, we consider a convergence framework similar to the one of \cite{OnTheConvergence} and \cite{Khaled2020}. We introduced the aggregation rule for the server global models $\{\vtheta^n\}$ in Section \ref{subsec:agg_schem}, and we generalize it in this section by introducing the virtual sequence of global models $\vtheta^{n, k}$. This sequence corresponds to the \textit{virtual} global model that would be obtained with the clients contribution at optimization round $n$ computed on $k\le K$ SGD, i.e.
\begin{equation}
\vtheta^{n, k}
\coloneqq \vtheta^n  + \eta_g \sum_{ i = 1 }^M \omega_i(n) \left[\vtheta_i^{(\rho_i(n), k)} - \vtheta^{\rho_i(n)}\right]
.
\end{equation}
We retrieve $\vtheta^{n, 0} = \vtheta^n $ and $\vtheta^{n, K} = \vtheta^{n+1, 0} = \vtheta^{n+1}$. The server has not access to  $\vtheta^{n, k}$ when $k\neq 0$ or $k\neq K$. Hence the name virtual for the model $\vtheta^{n , k}$.

The difference between two consecutive global models in our virtual sequence depends on the sum of the differences between local models $\vtheta_i^{\rho_i(n), k+1} - \vtheta_i^{\rho_i(n), k} = - \eta_l \nabla \Lcal_i(\vtheta_i^{\rho_i(n), k}, \vxi_i)$, where $\vxi_i$ is a random batch of data samples of client $i$. Hence, we can rewrite the aggregation process as a GD step with
\begin{equation}
\vtheta^{n, k+1} =
\vtheta^{n, k} - \eta_g \eta_l \sum_{ i = 1 }^M \omega_i(n) \nabla \Lcal_i(\vtheta_i^{\rho_i(n), k}, \vxi_i)
.
\end{equation}


\subsection{Asynchronous FL as a Sequence of Optimization Problems}\label{subsec:sequence_opt_problems}

For the rest of this work, we define $q_i(n) \coloneqq \E{\omega_i(n)}$, the expected aggregation weight of client $i$ at optimization round $n$. 
No assumption is made on $q_i(n)$ which can vary across optimization rounds. The expected clients contribution $\sum_{ i = 1 }^M q_i(n)\vDelta_i(n)$ help minimizing the optimization problem $\Lcal^n$ defined as
\begin{equation}
\label{eq:surrogate_loss_fucntion}
\Lcal^n(\vtheta) 
\coloneqq
%\frac{1}{\bar{q}^n}
\sum _{i=1}^M q_i(n) \Lcal_i(\vtheta)
.
\end{equation}
We denote by $\bar{\vtheta}^n$ the optimum of $\Lcal^n$ and by $\vtheta^*$ the optimum of the optimization problem $\Lcal$ defined in equation (\refeq{eq:original_problem_general}). Finally, we define by $q_i = \frac{1}{N}\sum_{ n = 0 }^{N-1}q_i(n)$ the expected importance given to client $i$ over the $N$ server aggregations during the FL process,
and by $\tilde{q}_i(n)$ the normalized expected importance $\tilde{q}_i(n) = q_i(n) / (\sum_{ i = 1 }^M q_i(n))$. 
We define by $\bar{\Lcal}$ the associated optimization problem 
\begin{equation}
\label{eq:surrogate_problem}
\bar{\Lcal}(\vtheta) 
\coloneqq
%\frac{1}{\bar{q}^n}
\sum _{i=1}^M q_i \Lcal_i(\vtheta)
=
\frac{1}{N}\sum _{ n = 0}^{N-1} \Lcal^n(\vtheta)
,
\end{equation}
and we denote by $\bar{\vtheta}$ the associated optimum.

Finally, we introduce the following expected convergence residual, which quantifies the variance at the optimum in function of the relative clients importance $q_i(n)$ 
\begin{equation}
\Sigma
\coloneqq \sum_{ i = 1 }^M q_i \EE{\vxi_i}{\norm{\nabla \Lcal_i(\bar{\vtheta}, \vxi_i)}^2}
.
\end{equation}
% \begin{equation}
% \Sigma_1 
% \coloneqq \sum_{ i = 1 }^M q_i \EE{\vxi_i}{\norm{\nabla \Lcal_i(\bar{\vtheta}, \vxi_i)}^2}
% \text{ and }
% \Sigma_2 
% \coloneqq \sum_{ i = 1 }^M \left[ \frac{1}{N}\sum_{ n = 0 }^{N-1} q_i^2(n) \right] 
% \EE{\vxi_i}{\norm{\nabla \Lcal_i(\bar{\vtheta}, \vxi_i)}^2}
% .
% \end{equation}
The convergence guarantees provided in this work (Section \ref{sec:convergence}) are proportional to the expected convergence residual.
$\Sigma$ is positive and null only when clients have the same loss function and perform GD steps for local optimization.



\subsection{Formalizing Heterogeneity across Clients}\label{subsec:heterogeneity_across_clients}

We assume the existence of $J \le M$ different clients feature spaces $\Zcal_i$ and, without loss of generality, assume that the first $J$ clients feature spaces are different. 
This formalism allows us to represent the heterogeneity of data distribution across clients. 
In DL problems, we have $J <M$ when the same dataset split is accessible to many clients. 
When clients share the same distribution, we assume that their optimization problem is equivalent. In this case, we call $F_j(\vtheta)$ their loss function with optimum $\vtheta_j^*$.
The federated problem of equation (\refeq{eq:original_problem_general}) can thus be formalized with respect to the discrepancy between the clients feature spaces $\Zcal_i$. To this end, we define $Q_j$ the set of clients with the same feature space of client $j$, i.e. $Q_j \coloneqq \{i: \Zcal_i = \Zcal_j\}$. Each feature space as thus importance $r_j = \sum_{ i \in Q_j } p_i$, and expected importance $s_j(n) = \sum_{ i \in Q_j } q_i(n)$ such that
\begin{equation}
\Lcal (\vtheta) 
= \sum_{j=1}^J r_j F_j (\vtheta)
\text{ and }
\Lcal^n (\vtheta)
= \sum_{j=1}^J s_j(n) F_j(\vtheta)
.
\end{equation}
As for $\tilde{q}_i(n)$, we define $\tilde{s}_j(n) = s_j(n)/ \sum_{ i = 1 }^M s_j(n)$. 

In Table \ref{tab:aggregation_weights}, we summarize the different weights used to adapt the federated optimization problem to account respectively for heterogeneity in clients importance and data distributions across rounds. 

%, e.g. in distributed learning where every client has access to the same dataset. 
%In the FL setting, considering that two clients have the same loss function and associated minimum is also a reasonable approximation if we assume that their samples are drawn from the same data distribution, e.g. when the server splits a dataset among clients.

\begin{table}
	\begin{center}
		\begin{tabular}{ | c || c | c |  }
			\hline
			& Client $i$ & Sample distribution $j$ \\
			\hline
			Importance   
			& $p_i$ 
			& $r_j$
			\\
			Stochastic aggregation weight 
			&   $\omega_i(n)  $
			& -
			\\
			Aggregation weight 
			& $d_i(n)$ 
			& -
			\\
			Expected agg. weight 
			& $q_i(n)$ 
			& $s_j(n)$
			\\
			Normalized expected agg. weight 
			& $\tilde{q}_i(n)$ 
			& $\tilde{s}_j(n)$
			\\
			Expected agg. weight over $N$ rounds 
			& $q_i$ 
			& $s_j$
			\\
			\hline
		\end{tabular}
	\end{center}
\caption{The different weights used to account for the importance of clients or data distributions at every optimization round and during the full FL process.}
\label{tab:aggregation_weights}
\end{table}





%\subsection{Assumptions}
%We also consider server aggregation schemes (\refeq{eq:aggreg_SCAFFOLD_general}) with clients stochastic aggregation weight covariance satisfying Assumption \ref{ass:clients_covariance} \citep{OnTheImpact}. We provide in Section \ref{sec:applications} $\alpha$ close-form for all the considered optimization schemes. 
%\begin{assumption}\label{ass:clients_covariance}
%	%	$\exists R_i(n),\ R_j(n)$ such that $\mathbb{P}( T_i^n \le \Delta t^n,\ T_j^n \le \Delta t^n) =  R_i(n)R_j(n)$ 
%	%	and there exists $U\ge 0$ such that $R_i(n) = U \mathbb{P}( T_i^n \le \Delta t^n)$
%	There exists $\alpha \in (0, 1)$ such that $\E{\omega_i(n)\omega_j(n)} = \alpha q_i(n) q_j(n) $.
%\end{assumption}




%\subsection{Server Aggregation Scheme}
%
%
%
%%Optimization with naive \textsc{FedAvg} is shown to have a couple of drawbacks. 
%%Aggregation scheme (\refeq{eq:FedAvg_server_aggregation}) forces the server to wait for every client updated model $\vtheta_i^{(n , K)}$ to create the new global model $\vtheta^{n+1}$.
%%This condition is constraining in FL applications where clients can have heterogeneous and unreliable communication and computation capabilities giving to an optimization round the speed of the slowest client. In addition, clients data heterogeneity can lead to disparity in the clients updates. 
%
%We propose the following formalism for the server aggregation scheme generalizing equation (\refeq{eq:FedAvg_server_aggregation}). We consider $\vDelta_i(n)$ the contribution of client $i$ at optimization round $n$. Each client contribution is considered with a stochastic aggregation weight $\omega_i(n)$. As a result, we have
%\begin{equation}
%\label{eq:aggreg_SCAFFOLD_general}
%\vtheta^{n+1}
%= \vtheta^n + \eta_g \sum_{i =1}^M \omega_i(n)\vDelta_i(n),
%\end{equation}
%where $\eta_g$ is a global learning rate the server can use to mitigate the disparity in clients contributions \citep{reddi2021adaptive, SCAFFOLD, Wang2020SlowMo}. 
%%This disparity can be caused either by the clients data heterogeneity, consideration of a subset of clients, or delayed clients local work.
%
%Equation (\refeq{eq:aggreg_SCAFFOLD_general}) is a generalization of the stochastic server aggregation scheme proposed in \cite{OnTheImpact}. With this work, we use aggregation scheme (\refeq{eq:aggreg_SCAFFOLD_general}) to provide a unique theoretical framework giving the convergence guarantees of a wide range of optimization schemes in Section \ref{sec:applications}. In particular, when $\vDelta_i(n) = \vtheta_i^{(n , K)} - \vtheta^n$, $\omega_i(n) = p_i$ with $\eta_g =1$, equation (\refeq{eq:aggreg_SCAFFOLD_general}) reduces to equation (\refeq{eq:FedAvg_server_aggregation}).
%
%For the rest of this work, we define $q_i(n) \coloneqq \E{\omega_i(n)}$, the expected aggregation weight of client $i$ at optimization round $n$. We also consider server aggregation schemes (\refeq{eq:aggreg_SCAFFOLD_general}) with clients stochastic aggregation weight covariance satisfying Assumption \ref{ass:clients_covariance} \citep{OnTheImpact}. We provide in Section \ref{sec:applications} $\alpha$ close-form for all the considered optimization schemes. Lastly, we define $\tilde{q}_i(n)$ the normalized expected aggregation weight such that $\tilde{q}_i(n) = q_i(n) / \sum_{ i = 1 }^M q_i(n)$. 
%\begin{assumption}\label{ass:clients_covariance}
%%	$\exists R_i(n),\ R_j(n)$ such that $\mathbb{P}( T_i^n \le \Delta t^n,\ T_j^n \le \Delta t^n) =  R_i(n)R_j(n)$ 
%%	and there exists $U\ge 0$ such that $R_i(n) = U \mathbb{P}( T_i^n \le \Delta t^n)$
%	There exists $\alpha \in (0, 1)$ such that $\E{\omega_i(n)\omega_j(n)} = \alpha q_i(n) q_j(n) $.
%\end{assumption}
%
%We want a framework accounting for delays in local work manifesting in $\vDelta_i(n)$. We introduce $\rho_i(n)$ the index of the most recent global model received by client $i$ at optimization round $n$.
%By construction, we have $0 \le \rho_i(n) \le n$.
%Client $i$ local work is thus performed on $\vtheta^{\rho_i(n)}$ and $\vDelta_i(n) = \vtheta_i^{\rho_i(n)+1 }- \vtheta^{\rho_i(n) }$. 
%With \textsc{FedAvg}, the server waits for every client so $\rho_i(n) =n$ and we retrieve $\vDelta_i(n) = \vtheta_i^{ n + 1 }- \vtheta^{ n }$. 
%In the rest of this work, we define $\tau$ the maximum amount of optimization rounds needed for a client to update its work to the server, i.e.
%\begin{equation}
%	\tau 
%	\coloneqq
%	\max_{i, n} \left(n - \rho_i(n) \right)
%	.
%\end{equation}





%Before introducing our theoretical results, we also define $q_i(n)$ as the expected aggregation weight of client $i$ at optimization step $n$, i.e. $q_i(n) \coloneqq \E{\omega_i(n)}$. Hence, taking the expectation of equation (\refeq{eq:agg_weights}) gives 
%\begin{equation}
%\label{eq:E_agg_weights}
%q_i(n) = \mathbb{P}( T_i^n \le \Delta t^{n})d_i(n) .
%\end{equation}
%We do not make any assumption on $\sum_{ i = 1 }^M q_i(n)$. Therefore, we also introduce the normalized expected importance $\tilde{q}_i(n) = q_i(n) / \sum_{ i = 1 }^M q_i(n)$ such that $\sum_{ i = 1 }^M \tilde{q}_i(n) = 1$. 

















==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/client_sampling.tex <==
% \subsection{Synchronous Federated Learning}\label{subsec:client_sampling}

% %\begin{table}
% %	\begin{center}
% %	\begin{tabular}{ |c|c|c|c| } 
% %		\hline
% %		FL type  
% %		& $\Delta t^n = $ 
% %		& $\mathbb{P}(T_i^n \le \Delta t^n) = $ 
% %		& $R_i(n) = $
% %		\\ \hline
% %		
% %		Sync.
% %		& $\max_i T_i^n$
% %		& 1
% %		& 1
% %		\\ \hline
% %		 
% %		Async. Theorem
% %		& $\min_i T_i^n$
% %		& $(1/\tau_i) / (\sum_{ i = 1 }^C 1/\tau_i)$
% %		& 0
% %		\\ \hline
% %		
% %		Hybrid 
% %		& $T^n$
% %		& $ 1- e^{- T^n /\tau_i}$
% %		& $ 1- e^{- T^n /\tau_i}$
% %		\\ \hline
% %	\end{tabular}
% %
% %	\end{center}
% %	\caption{\label{tab:FL_statistics}Your caption.}
% %\end{table}

% %Instead of centralizing the dataset of the $M$ clients on a server, data never leaves their owner premises. 
% As described for \textsc{FedAvg} in Section \ref{subsec:agg_schem}, at every optimization round, the server sends to the clients the current global model to perform $K$ SGD steps on their own data before returning the resulting model to the server. Once every client performs its local work, the new global model is created as the weighted average of the clients contribution. 

% \subsubsection*{Full client participation, i.e. Vanilla \textsc{FedAvg}} 

% %\textbf{Full client participation, i.e. naive \textsc{FedAvg}}.
% The server waits for every client to update their local model before creating the new global model.
% The time required for an optimization step is therefore the one of the slowest client ($\Delta t^n = \max_i(T_i^n)$), and every client is considered ($\mathbb{P}( T_i^n \le \Delta t^n) = 1$). Therefore $\alpha= 1$, $\beta = 0$, and setting $d_i = p_i$ is sufficient to satisfy the conditions of Corollary \ref{cor:bias_distributions} (and thus the ones of Theorem \ref{theo:relaxed_sufficient_conditions}) ensuring that FL converges to its optimum \citep{FedNova}. The term $\epsilon$ then reduces to
% \begin{align}
% \epsilon_{\textsc{FedAvg}}
% &= \Ocal\left(\frac{\norm{\vtheta^0 -\vtheta^*}^2}{\eta_g \eta_l K N}\right)
% + \Ocal \left(\eta_g \eta_l \frac{1}{M} \Sigma \right)
% + \Ocal \left(\eta_l^2 (K-1)^2 \Sigma \right)
% % \label{eq:epsilon_sync_FL}
% .
% \end{align}
% The third element of equation (\refeq{eq:epsilon_sync_FL}) accounts for the amount $K$ of local work performed by clients between two server aggregations, and is proportional to the convergence residual $\Sigma$. Equation (\refeq{eq:epsilon_sync_FL}) is consistent with literature on optimization with \textsc{FedAvg} including \cite{FedNova, Khaled2020}.

% \textbf{iid data distributions}. When clients have identical data distributions, $\Sigma$ is identical for both centralized and synchronous FL. The second term of equation (\refeq{eq:epsilon_sync_FL}) benefits of the clients computation by being proportional to $1/M$. 

%The first two term are identical to centralized learning with an improvement for synchronous FL. The convergence residual $\Sigma$ 
%\begin{align}
%\epsilon'
%&= \Ocal\left(\frac{\norm{\vtheta^0 -\vtheta^*}^2\sqrt{\tau_M}}{\eta_g \sqrt{K T}}\right)
%+ \Ocal \left(\eta_g \frac{\sqrt{\tau_M}}{\sqrt{KT}}\frac{1}{M} \Sigma \right)
%+ \Ocal \left(\frac{\tau_M}{T}(K-1) \Sigma \right)
%\label{eq:convergence_FedAvg_Full}
%.
%\end{align}


\subsection{Unbiased client sampling ($q_i(n) = p_i$)}\label{subsec:client_sampling_unbiased}
% \subsubsection*{Partial Client Participation}
We define by $S_n$ the set of sampled clients performing their local work at optimization step $n$. Setting $\Delta t^n = \max_{i \in S_n } T_i$, with $T_i = \infty$ for the clients that are not sampled, and thus not in $S_n$, gives $\mathbb{P}( T_i \le \Delta t^n) = \mathbb{P}( i \in S_n )$. $S_n$ is independent from the clients hardware capabilities and is decided by the server. This allows to pre-compute $\mathbb{P}( T_i \le \Delta t^n)$ and to allocate to each client the aggregation weight $d_i$ such that $q_i = p_i$. 

Standard unbiased client sampling schemes include sampling $m$ clients uniformly without replacement \citep{OnTheConvergence} or sampling $m$ clients according to a Multinomial distribution \citep{FedProx}.
\cite{OnTheImpact} shows that both Uniform and MD sampling satisfy Assumption \ref{ass:clients_covariance}. 
In particular, in those setting, the term $\alpha\le 1$ is proportional to $m$, the amount of sampled clients, while $1 \ge \beta>0$ is inversely proportional to $m$. 
We get
\begin{align}
\epsilon
&= \Ocal\left(\frac{1}{\eta_g \eta_l K N}\right)
+ \Ocal \left(\eta_g \eta_l \alpha \frac{1}{M}\Sigma \right)
+ \Ocal \left(\eta_l^2 (K-1)^2 \Sigma \right)
+ \Ocal \left(\eta_g \eta_l \beta \Sigma \right)
\label{eq:epsilon_sync_unbiased}
.
\end{align}
The second term, proportional to $\alpha/M$, is reduced at the expense of the introduction of a fourth term proportional to $\beta$.
In turn, it still provides faster optimization rounds with $\Delta t^n = \max_{i \in S_n } T_i$ and $N = \Ocal \left(T/ \E{\max_{i \in S_n } T_i}\right)$. 
FedAvg with client sampling generalizes FedAvg with full client participation ($\alpha = 1$ and $\beta=0$).

\subsection{Biased client sampling ($q_i(n) \neq p_i$)} \label{subsec:client_sampling_biased}
The condition $q_i(n) = p_i$ imposes the design of new client sampling based on the clients data heterogeneity. Nevertheless, we show convergence of biased client samplings where $m$ clients are selected according to a deterministic criterion,  e.g. when selecting the $m$ clients with the highest loss \citep{PowerOfChoice}, or when selecting the $m$ clients with the most available computation resources \citep{sampling_mobile_edge}. 
In this case, $\mathbb{P}( i \in S_n ) = 0/1$, with 1 if a client satisfies the criterion and 0 otherwise. In this case, no weighting scheme can make an optimization round unbiased.
We also have $\mathbb{P}( \{i, j\} \in S_n ) = \mathbb{P}( i \in S_n ) \mathbb{P}( j \in S_n )$, which gives $\alpha = 1$ with $\beta=0$. 
Without modification, this client sampling cannot satisfy the relaxed sufficient conditions of Theorem \ref{theo:relaxed_sufficient_conditions} and thus converges to a suboptimum point. 
This drawback can be mitigated by allocating a part of time in the window $W$ to sample clients according to the criterion, and the rest of the window to consider clients such that $q_i = p_i$ is satisfied over $W$ optimization rounds. 
%Balancing the amount of time a client is sampled over $W$ is another deterministic criteria. 
%We therefore propose here a combination of two deterministic criteria for FL convergence.
By denoting $\epsilon_{\textsc{FedAvg}}$ the convergence guarantees (\refeq{eq:epsilon_sync_FL}), we have
\begin{equation}
\epsilon
= \epsilon_{\textsc{FedAvg}}
+ \Ocal \left(\eta_g\eta_l (W - 1) K\right)
\label{eq:epsilon_sync_bias}
.
\end{equation}
We note that equation (\refeq{eq:epsilon_sync_bias}) provides a looser bound than equation (\refeq{eq:epsilon_sync_FL}) in term of optimization rounds $N$.
Still, this bound is informative and shows that, with minor changes, biased clients sampling based on a deterministic criterion can be proven to converge to the FL optimum.


==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/conclusion.tex <==
\section{Discussion}


This work introduces equation (\ref{eq:aggreg_SCAFFOLD_general}) which generalizes the expression of \textsc{FedAvg} aggregation scheme by introducing stochastic aggregation weights $\omega_i(n)$ to account for asynchronous client updates. With a simple assumption for clients aggregation weights covariance, Assumption \ref{ass:clients_covariance}, we prove the convergence of FL schemes satisfying equation (\ref{eq:aggreg_SCAFFOLD_general}).
A similar aggregation scheme has been derived in \cite{OnTheImpact} for unbiased client sampling, which this work generalizes. 
In addition, we show that aggregation scheme (\ref{eq:aggreg_SCAFFOLD_general}) and Assumption \ref{ass:clients_covariance} are satisfied by asynchronous FL, \textsc{FedFix}, and \textsc{FedBuff}, Section \ref{sec:applications}. 
Finally, we assume fixed clients update time $T_i$ such that 
we can consider $d_i(n ) = d_i$, and 
give in Section \ref{sec:applications} its close-form 
% for any optimization scheme
% of every client aggregation weight $d_i$ 
to ensure any FL optimization scheme converges to the optimum of problem (\ref{eq:original_problem_general}). Our work remains relevant for applications with $d_i(n) = d_i$ but we let the specific derivations to the reader.
% Finally, we provide in Theorem \ref{theo:relaxed_sufficient_conditions} the close-form of clients aggregation weights $d_i(n)$ in function of its optimization scheme to ensure FL converges to its optimum. 

This work shows theoretically and experimentally that asynchronous \textsc{FedAvg} does not always outperform its synchronous counterpart.
By creating the new global model with the contribution of only one client, asynchronous \textsc{FedAvg} convergence speed is very sensitive to the choice of learning rate and amount of local work $K$. These two hyperparameters need to be fine-tuned to properly balance convergence speed and stability. 
Due to the hardware constraints inherent to the FL setting, fine-tuning is a challenging step for FL and is not necessarily feasible. Therefore, we proposed \textsc{FedFix}, an FL algorithm where the server, after a fixed amount of time, creates the new global model with the contribution of all the participating clients. We prove the convergence of \textsc{FedFix} with our theoretical framework, and experimentally demonstrate its improvement over \textsc{FedAvg} in all the considered scenarios.



% This work proves the convergence of asynchronous FL in the heterogeneous setting, and show that asynchronous \textsc{FedAvg} outperforms its synchronous counterpart in some experimental scenarios. 
% However, by only including the contribution of one client in the new global model, asynchronous FL convergence speed is very sensitive to the choice of learning rate and amount of local work $K$, and these two hyperparameters need to be fine-tuned to properly balance convergence speed and stability. 
% Due to the hardware constraints inherent to the FL setting, fine-tuning is a challenging step for FL and is not necessarily feasible. Therefore, we proposed \textsc{FedFix}, an FL algorithm where the server, after a fixed amount of time, creates the new global model with the contribution of all the participating clients. We prove with our theoretical framework \textsc{FedFix} convergence and experimentally its improvement over \textsc{FedAvg} in every experiment.


==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/generalization.tex <==
\subsection{Generalization}
\label{subsec:generalization}

Coupled with the theoretical method developed in \cite{FedNova}, the proof of Theorem \ref{theo:convergence_convex} can account for FL regularization methods \citep{FedProx, FedDane, FedDyn}, other SGD solvers \citep{Adam, AdaGrad,pmlr-v89-li19c, OnTheLienarSpeedUp, Yu_Yang_Zhu_2019, haddapour2019trading}, and/or gradient compression/quantization \citep{FedPaq, QSparse, Atomo, koloskova2020decentralized}. 

We also note that Theorem \ref{theo:relaxed_sufficient_conditions} can be applied to other distributed optimization schemes using different waiting time policy $\Delta t^n$. With \textsc{FedBuff} \citep{FedBuff}, the server waits for $m$ client updates to create the new global model. The server then communicates to these clients the new global model, while the other clients keep performing local work on the global model they received.

In this section, the sufficient conditions of Theorem \ref{theo:relaxed_sufficient_conditions} regarding the expected aggregation weights $q_i(n)$ were applied to obtain proper aggregation weight $d_i$. We keep identical clients local learning rate $\eta_l$ and amount of local work $K$. 
We could instead get the close-form of a client specific learning rate $\eta_l(i)$ or amount of local work $K(i)$ using the gradient formalization of \cite{FedNova}.



==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/hybrid_FL.tex <==
\subsection{\textsc{FedFix}}
\label{subsec:FedFix}

% The server waiting time for synchronous and asynchronous FL is stochastic and $\Delta t^n$ depends on the clients remaining update time $T_i^n$. 
% With \textsc{FedFix}, we propose to consider the creation of the $n^{th}$ global model at a given clock time $T^n$ decided by the server, which makes the quantity $\Delta t^n = T^{n+1} - T^n$ independent from the clients remaining update time $T_i^n$. 
% For sake of convenience, we further assume that the time between optimization rounds is identical, i.e. $\Delta t^n = \Delta t$, but the following results can be derived for other fixed time policies $\{\Delta t^n\}$. 

The analysis of asynchronous \textsc{FedAvg} (Section \ref{subsec:async_FL}) and its comparison with synchronous \textsc{FedAvg} (Section \ref{subsec:synchronous}), shows that asynchronous \textsc{FedAvg} is not scalable to large cohort of clients. We thus propose \textsc{FedFix} combining the strong points of synchronous and asynchronous \textsc{FedAvg}, where the server creates the new global model at a fixed time $t^n$ with the contributions received since $t^{n-1}$. Therefore, the server does not wait for every client, contrarily to synchronous \textsc{FedAvg}, and considers more than one client per aggregation to have more stable aggregations, contrarily to asynchronous \textsc{FedAvg}. We provide in Figure \ref{fig:illustration} an illustration of \textsc{FedFix} with two clients.

With \textsc{FedFix}, an iteration time $\Delta t^n = t^{n+1} - t^n$ is decided by the server and is independent from the clients remaining update time $T_i^n$. 
For sake of convenience, we further assume that the time between optimization rounds is identical, i.e. $\Delta t^n = \Delta t$, but the following results can be derived for other fixed time policies $\{\Delta t^n\}$. 
% The server waiting time for synchronous and asynchronous FL is stochastic and $\Delta t^n$ depends on the clients remaining update time $T_i^n$. 
% With \textsc{FedFix}, we propose to consider the creation of the $n^{th}$ global model at a given clock time $T^n$ decided by the server, which makes the quantity $\Delta t^n = T^{n+1} - T^n$ independent from the clients remaining update time $T_i^n$. 
% For sake of convenience, we further assume that the time between optimization rounds is identical, i.e. $\Delta t^n = \Delta t$, but the following results can be derived for other fixed time policies $\{\Delta t^n\}$. 
Therefore, $T_i^n$ and $T_j^n$ are independent, and so are $\omega_i$ and $\omega_j$, which gives $\alpha = 1$ and $\beta = 0$.

Every client sends an update to the server in $N_i' = \ceil{T_i / \Delta t }$ optimization steps. 
% To prevent aggregations with no client contributions, we assume $\Delta t \ge \tau_1$, and the update delay $\tau$ satisfies $\tau = \max_i\ceil{ T_i / \Delta t } - 1 = \max_i \floor{T_i / \Delta t} = \Ocal(1)$. 
Contrarily to asynchronous \textsc{FedAvg}, we thus have $\tau = \ceil{\tau_m /\Delta t} = \Ocal(1)$, which is independent from the amount of participating clients $M$. 
In this case,  the smallest window $W$ satisfies $W = lcm(\{N_i'\})$, and clients update $W/ N_i'$ times their work to the server during the window $W$. Therefore, satisfying the conditions of Theorem \ref{theo:relaxed_sufficient_conditions} requires
\begin{equation}
d_i
= \ceil{ \frac{\tau_i }{\Delta t} } p_i
.
\label{eq:aggreg_weights_hybrid}
\end{equation}
With equation (\refeq{eq:aggreg_weights_hybrid}), we can notice the relationship between \textsc{FedFix} and synchronous or asynchronous \textsc{FedAvg}. When $\Delta t \ge \tau_i$, client $i$ participates to every optimization round and is thus considered synchronously, which gives $d_i = p_i$. When $\Delta_t \ge \tau_M$, we retrieve synchronous FL and $d_i = p_i$ for every client. On the contrary, for asynchronous FL, when $\Delta t \ll \tau_i$, we obtain $\ceil{\tau_i / \Delta t}\approx \tau_i /\Delta t$ and we retrieve $\eta_g d_i = \eta_g \left[ \tau_i / \Delta t \right] p_i \propto \tau_i p_i$.

%\begin{property}
%	We denote by $X_A$ and $X_H$ the variable $X$ for respectively asynchronous and hybrid FL.
%	Let us consider $\tau_1 \le  H \le \tau_M$ where $H$ is either bigger or a divider of $\tau_i$, then we have
%	\begin{equation}
%	\tau_H \le \tau_A - (M-2)
%	\text{ and }
%	W_H \le \frac{1}{M} W_A
%	.
%	\end{equation}
%\end{property}
%
%\begin{proof}
%	\begin{equation}
%	\tau_H 
%	=  \floor{\tau_M / H} 
%	\le \ceil{ \tau_M / \tau_1 }
%	\le \sum_{ i = 1 }^{M-1} \ceil{ \tau_M / \tau_i } - \sum_{ i = 2 }^{M-1} \ceil{ \tau_M / \tau_i }
%	= \tau_A - (M - 2)
%	\end{equation} 
%	$H$ is either bigger or a divider of $\tau_i$. Therefore, we have $lcm (\{N_i'\}) \le lcm(\tau_i)/ H$ with equality if and only if $H \le \tau_1$. As a result, we have
%	\begin{equation}
%	W_H 
%	\le \frac{1}{\sum_{ i = 1 }^M \frac{H}{\tau_i}} W_A
%	\le \frac{1}{M \min_i \{H / \tau_i\} } W_A
%	= \frac{1}{M} \frac{\tau_M}{H} W_A
%	\le \frac{1}{M}W_A
%	,
%	\end{equation}
%	where the last inequality comes from $H \le \tau_M$.	
%\end{proof}

Regarding the disparity between the local objectives $R\{\Lcal^n\}$, we know that a client participates to an optimization round with $q_i(n) =d_i$. We thus have $\Lcal^n = \sum_{ i \in S_n } d_i \Lcal_i$, where $S_n$ is the set of the participating clients at optimization step $n$. Considering that $\Lcal^n (\bar{\vtheta}^n)\ge \sum_{ i \in S_n } d_i \Lcal_i(\vtheta_i^*)$, the close form of \textsc{FedFix} is bounded by the one of of asynchronous \textsc{FedAvg}, i.e.
\begin{equation}
	R(\{\Lcal^n\})
	\le  \frac{1}{M} \sum_{ i = 1 }^M \left[\Lcal_i(\vtheta^*) - \Lcal_i(\vtheta_i^*)\right]
	.
\end{equation}
Finally, we simplify the close-form of $\epsilon$ (Theorem \ref{theo:relaxed_sufficient_conditions}) for \textsc{FedFix} to get
% \begin{align}
% \epsilon_{\textsc{FedFix}}
% &= \Ocal\left( \frac{1}{\sqrt{KN}} 
% \left[ \norm{\vtheta^0 -\vtheta^*}^2 
% + R(\{\Lcal^n\}) +\frac{1}{M}\ceil{ \frac{\tau_M }{\Delta_t} } \Sigma 
% \right]
% \right)
% + \Ocal \left(\frac{K-1}{N} \Sigma \right)
% \nonumber\\
% &
% % + \Ocal \left(\tilde{\eta}^2 K^2  \tau^2 R(\{\Lcal^n\}) \right) 
% % + \Ocal \left(\tilde{\eta} R(\{\Lcal^n\}) \right)
% + \Ocal \left( \frac{K}{N} \ceil{\tau_m /\Delta t}^2 
% \left[ R(\{\Lcal^n\}) + \ceil{\tau_m /\Delta t} \frac{1}{M}\Sigma \right] \right)
% + \Ocal\left(  \frac{1}{\sqrt{KN}} (W-1)\right) 
% \label{eq:epsilon_FedFix}
% .
% \end{align}
\begin{align}
	\epsilon_{\textsc{FedFix}}
	&= \frac{1}{ \sqrt{KN}}\E{ \norm{\vtheta^{0} - \vx}^2 }
	+ \Ocal \left(\frac{K-1}{N} \left[ R(\{\Lcal^n\}) + \Sigma \right] \right) 
% 	+ \Ocal \left( \frac{1}{ \sqrt{KN}} \left[ R(\{\Lcal^n\}) + \ceil{\tau_m /\Delta t} \frac{1}{M} \Sigma \right] \right)
	\nonumber\\
	& 
	+ \Ocal \left( \left[ \frac{1}{ \sqrt{KN}} +  \frac{K}{ N} \ceil{\frac{\tau_m}{ \Delta t}}^2 \right] \left[ R(\{\Lcal^n\}) + \ceil{\frac{\tau_m}{ \Delta t}} \frac{1}{M} \Sigma \right] \right)
% 	\nonumber\\
	+ \Ocal\left(  \frac{1}{\sqrt{KN}} (W-1)\right) 
	.\label{eq:epsilon_FedFix}
\end{align}
The first two elements of equation (\refeq{eq:epsilon_FedFix}) are identical for \textsc{FedFix}, synchronous and asynchronous \textsc{FedAvg}. However, thanks to lower values for the different variables (cf Table \ref{tab:summary_comparison}), the last two asymptotic terms of the convergence bound are smaller for \textsc{FedFix} than for asynchronous \textsc{FedAvg}, equation (\refeq{eq:epsilon_FedFix}). Similarly, these two terms are larger with \textsc{FedFix} than with synchronous \textsc{FedAvg}.
The hardware heterogeneity and the amount of participating clients still impacts the convergence bound through $\ceil{\tau_M/ \Delta t}$ and $W$, but can be mitigated with proper selection of $\Delta t$. 
Therefore, after $N$ optimization rounds, synchronous \textsc{FedAvg} outperforms \textsc{FedFix} which outperforms in turn  asynchronous \textsc{FedAvg}. However, in $T$ time, the server performs 
$ N = T / \Delta t$
aggregations with \textsc{FedFix} against $T/ \tau_M$ for synchronous \textsc{FedAvg}. With asynchronous \textsc{FedAvg}, the server thus performs at least $\tau_M/\Delta t$ times more aggregations than with synchronous \textsc{FedAvg}. Overall, $\Delta t$ can be considered as the level of asynchronicity given to Algorithm \ref{alg:FL_with_delayed_gradients}, with \textsc{FedAvg} when $\Delta t  = \tau_M$ and asynchronous \textsc{FedAvg} when $\Delta t \ge \tau_M$.

In the DL case, clients have identical computation time ($\tau_1 = \tau_m$), and we retrieve the convergence bound of synchronous \textsc{FedAvg}.

In addition, we can increase the waiting time for the clients update, since the learning process converges and gets closer to the optimum of optimization problem (\ref{eq:original_problem_general}), to reach a behavior similar to the one of synchronous FL. Indeed, for Theorem \ref{theo:relaxed_sufficient_conditions} to hold, we only need the same optimization time rounds $\Delta t$ over a window $W$ 

==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/introduction.tex <==
\section{Introduction}


Federated learning (FL) is a training paradigm enabling different clients to jointly learn a global model without sharing their respective data. Federated learning is a generalization of distributed learning (DL), which was first introduced to optimize a given model in star-shaped networks composed of a server communicating with computing machines \citep{Bertsekas1989, Nedi2001, SlowLearnersAreFast}. 
In DL, the server owns the dataset and distributes it across machines. 
At every optimization round, the machines return the estimated gradients, and the server aggregates them to perform an SGD step. DL was later extended to account for SGD, and FL extends DL to enable optimization without sharing data between clients. Typical federated training schemes are based on the averaging of clients model parameters optimized locally by each client, such as in \textsc{FedAvg} \citep{FedAvg}, where at every optimization round clients perform a fixed amount of stochastic gradient descent (SGD) steps initialized with the current global model parameters, and subsequently return the optimized parameters to the server. The server computes the new global model as the average of the clients updates weighted by their respective data ratio.

A key methodological difference between the optimization problem solved in FL and the one of DL lies in the assumption of potentially non independent and identically distributed (iid) data instances \citep{OpenProblems, YangFML}.
Proving convergence in the non-iid setup is more challenging, and in some settings, \textsc{FedAvg} has been shown to converge to a sub-optimum, e.g. when each client performs a different amount of local work \citep{FedNova}, or when clients are not sampled in expectation according to their importance \citep{PowerOfChoice}. 

A major drawback of \textsc{FedAvg} concerns the time needed to complete an optimization round, as the server must wait for all the clients to perform their local work to \textit{synchronize} their update and create a new global model.
As a consequence, due to the potential heterogeneity of the hardware across clients, the time for an optimization round is conditioned to the one of the slowest update, while the fastest clients stay idle once they have sent their updates to the server. 
To address these limitations, asynchronous FL has been proposed to take full advantage of the clients computation capabilities \citep{AFLsurvey, Hogwild2, KoloskovaGossip, TamingTheWild}. 
In the asynchronous setting, whenever the server receives a client's contribution, it creates a new global model and sends it back to the client.
In this way, clients are never idle and always perform local work on a different version of the global model.
While asynchronous FL has been investigated in the iid case \citep{ErrorFeedbackFramework}, a unified theoretical and practical investigation in the non-iid scenario is currently missing.


This work introduces a novel theoretical framework for asynchronous FL based on the generalization of the aggregation scheme of \textsc{FedAvg}, where asynchronicity is modeled as a stochastic process affecting clients' contribution at a given federated aggregation step.
More specifically, our framework is based on a stochastic formulation of FL, where clients are given stochastic aggregation weights dependent on their effectiveness in returning an update. 
%While with stochastic \textsc{FedAvg} clients contribute to the new global model with probability 1, our framework associates to each client's weight a probability for sending an update at a given optimization round. 
Based on this formulation, we provide sufficient conditions for asynchronous FL to converge, and we subsequently give sufficient conditions for convergence to the FL optimum of the associated synchronous FL problem. 
Our conditions depend on the clients computation time (which can be eventually estimated by the server), and are independent from the clients data heterogeneity, which is usually unknown to the server.

With asynchronous FL, the server only waits for one client contribution to create the new global. As a result, optimization rounds are potentially faster even though the new global improves only for the participating client at the detriment of the other ones. This aspect may affect the stability of asynchronous \textsc{FedAvg} as compared to synchronous \textsc{FedAvg} and, as we demonstrate in this work, even diverge in some cases. To tackle this issue, we propose \textsc{FedFix}, a robust asynchronous FL scheme, where new global models are created with all the clients contributions received after a fixed amount of time.
We prove the convergence of \textsc{FedFix} and verify experimentally that it outperforms standard asynchronous \textsc{FedAvg} in the considered experimental scenarios.


The paper is structured as follows. 
In Section \ref{sec:background}, we introduce our aggregation scheme and the close-form of its aggregation weights in function of the clients computation capabilities and the considered FL optimization routine.
Based on our aggregation scheme, in Section \ref{sec:convergence}, we provide convergence guarantees, and we give sufficient conditions for the learning procedure to converge to the optimum of the FL optimization problem. 
In Section \ref{sec:applications}, we apply our theoretical framework to synchronous and asynchronous \textsc{FedAvg}, and show that our work extends current state-of-the-art approaches to asynchronous optimization in FL. Finally, in Section \ref{sec:experiments}, we demonstrate experimentally our theoretical results.








==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/main_bias.tex <==
\subsection{Sufficient Conditions for Minimizing the Federated Problem (\ref{eq:original_problem_general})}\label{subsec:sufficient_conditions}



Theorem \ref{theo:convergence_convex} provides convergence guarantees for the history of optimized models $\{\Lcal^n\}$.
Under the same assumptions of Theorem \ref{theo:convergence_convex}, we can provide convergence guarantees for the original FL problem $\Lcal(\vtheta)$ (proof in Appendix \ref{app:sec:theo_bias}). 


\begin{theorem}\label{theo:bias_convex}
	Under the same conditions of Theorem \ref{theo:convergence_convex}, we have
	\begin{multline}
	\frac{1}{N}\sum_{ n = 0 }^{N-1}\frac{1}{K}\sum_{ k = 0 }^{K-1} \E{\norm{\nabla \Lcal (\vtheta^{n, k})}^2}
	\\
	\le 
	\Ocal \left( R(\{\Lcal^n\}) \right) 
	+ P(\{\Lcal^n\})
	+ U(\{\Lcal^n\})
	+ \Ocal \left( \epsilon_F \right)
	+ \epsilon_K
	+ \epsilon_\alpha
	+ \epsilon_\beta
	,
	\end{multline}	
	where 
	\begin{equation}
	P(\{\Lcal^n\})
	= \Ocal \left( \frac{1}{N}\sum_{n=0}^{N-1}\chi_n^2 \sum_{j \in W_n} \tilde{s}_j(n) \left[ F_j(\bar{\vtheta}^n) - F_j(\vtheta_j^*) \right] \right)
	,
	\end{equation}
	\begin{equation}
	U(\{\Lcal^n\})
	= \Ocal \left( \frac{1}{N}\sum_{n=0}^{N-1}  \frac{1}{K} \sum_{k=0}^{K-1} \sum_{j \notin W_n} r_j\left[ \E{F_j(\vtheta^{n , k})} - F_j(\vtheta_j^*) \right] \right)
	,
	\end{equation}
	$\chi_n^2 = \sum_{j\in W_n} (r_j - \tilde{s}_j(n))^2/\tilde{s}_j(n)$, 
%	$\tilde{s}_j(n) =s_j(n)/ \sum_{ k = 1 }^J s_k(n)$, 
	and $W_n = \{j : s_j(n) > 0\}$.
\end{theorem}
Theorem \ref{theo:bias_convex} provides convergence guarantees for the optimization problem (\refeq{eq:original_problem_general}). We retrieve the components of the convergence bound of Theorem \ref{theo:convergence_convex}.
The terms $\epsilon_F$ to $\epsilon_\tau$ can be mitigated by choosing an appropriate local learning rate $\eta_l$, but the same cannot be said for $R(\{\Lcal^n\})$, $P(\{\Lcal^n\})$, $U(\{\Lcal^n\})$. 
Behind these three quantities, Theorem \ref{theo:bias_convex} shows that proper expected representation of every dataset type is needed, i.e. $s_j (n) = r_j$. Indeed, if a client is poorly represented, i.e. $s_j (n) \neq r_j$, then $ R(\{\Lcal^n\})>0$ and $P(\{\Lcal^n\})>0$, while if a client is not represented at all, i.e. $s_j(n) =0$, then $U(\{\Lcal^n\})>0$. Therefore, we propose, with Corollary \ref{cor:bias_distributions}, sufficient conditions for any FL optimization scheme satisfying Algorithm \ref{alg:FL_with_delayed_gradients} to converge to the optimum of the federated problem (\refeq{eq:original_problem_general}).

\begin{corollary}\label{cor:bias_distributions} 
	Under the conditions of Theorem \ref{theo:convergence_convex}, if every client data distribution satisfies $\tilde{s}_j(n) = r_j$, the following convergence bound for optimization problem (\refeq{eq:original_problem_general}) can be obtained 
	\begin{align}
	\frac{1}{N}\sum_{ n = 0 }^{N-1}\frac{1}{K}\sum_{ k = 0 }^{K-1} \left[ \E{\Lcal(\vtheta^{n, k})} - \Lcal(\vtheta^*) \right]
	& \le 
	\epsilon_F 
	+ \epsilon_K
	+ \epsilon_\alpha
	+ \epsilon_\beta
	.
	\end{align}	
\end{corollary}

\begin{proof}
	Follows directly. $\tilde{s}_j(n) = r_j$ implies $\chi_n^2 = 0$, $W_n = \emptyset$, $\Lcal^n = q(n) \Lcal$, and $\bar{\vtheta}^n = \vtheta^*$.
\end{proof}

These theoretical results provide relevant insights for different FL scenarios. 

\textbf{iid data distributions, $\mathcal{Z}_i = \mathcal{Z}$}. Consistently with the extensive literature on synchronous and asynchronous distributed learning, when clients have data points sampled from the same data distribution, FL always converges to its optimum (Corollary \ref{cor:bias_distributions}). Indeed, $\tilde{s}_j(n) = r_j = 1$ regardless of which clients are participating, and what importance $p_i$ or aggregation weight $d_i(n)$ a client is given.

\textbf{non-iid data distributions}. The convergence of FL to the optimum requires to optimize by considering every data distribution type fairly at every optimization round, i.e. $\tilde{s}_j(n) = r_j$  (Corollary \ref{cor:bias_distributions}). This condition is weaker than requiring to treat fairly every client at every optimization round, i.e. $q_i(n) = p_i$.
%which requires every client to participate at every optimization round ($\mathbb{P}( T_i^n \le \Delta t^{n+1})>0$). 
Ideally, only one client per data type needs to have a non-zero participating probability, i.e. $\mathbb{P}( T_i^n \le \Delta t^n )>0$, and an appropriate $d_i(n)$ such that $\tilde{s}_j(n) = r_j$ is satisfied. In practice, knowing the clients data distribution is not possible. Therefore, ensuring FL convergence to its optimum requires at every optimization round $\tilde{q}_i(n) = p_i$ \citep{FedNova}.

We provide in Example \ref{exa:bias} an illustration on these results based on quadratic loss functions to show that considering fairly data distributions is sufficient for an optimization scheme satisfying Algorithm \ref{alg:FL_with_delayed_gradients} to converge to the optimum of the optimization problem (\refeq{eq:original_problem_general}), since $\tilde{s}_j(n) = r_j$ is satisfied at every optimization round, while $\tilde{q}_i(n) \neq p_i$ may not be satisfied. 

\begin{example}\label{exa:bias}
	Let us consider four clients with data distributions such that their loss can be expressed as $\Lcal_i(\vtheta) = \frac{1}{2}\norm{\vtheta - \vtheta_i^*}^2$ with $\vtheta_1^* = \vtheta_2^*$ ($\Zcal_1$), $\vtheta_3^* = \vtheta_4^*$ ($\Zcal_2$), and identical client importance, i.e. $p_i = 1/4$. 
	Therefore, each data type has identical importance, i.e. $r_j = 1/2$, and the optimum satisfies $\vtheta^* = \frac{1}{2}[\vtheta_1^* + \vtheta_3^*]$.
	We consider that clients with odd index participate at odd optimization rounds while the ones with even index at even optimization rounds, i.e. $q_1^{2n+1} = q_3^{2n+1} = q_2^{2n} = q_4^{2n} = 1/2$ and $q_1^{2n} = q_2^{2n} = q_3^{2n+1} = q_4^{2n+1} =  0$ which gives $\tilde{s}_1(n) = \tilde{s}_2(n) = 1 /2$ and $\tilde{q}_i(n)=0$ or $\tilde{q}_i(n)=1/2$ but not $\tilde{q}_i(n)=1/4$.
	With $\eta_g = 1$, equation (\refeq{eq:aggreg_SCAFFOLD_general}) can be rewritten as
	\begin{equation}
		\vtheta^{n+2} = \vtheta^{n+1} + \frac{1}{2}\left[ ( \vtheta_1^{n+1} - \vtheta^n) + ( \vtheta_3^{n+1} - \vtheta^n)\right].
	\label{exa:eq:A1}
	\end{equation}
	Clients update can be rewritten as 
	$
	\vtheta_i^{n+1} - \vtheta^n
	= \phi (\vtheta_i^* - \vtheta^n),
	$
	where $\phi = 1 - ( 1- \eta_l)^K$. Equation (\refeq{exa:eq:A1}) can thus be rewritten as
	\begin{equation}
	\vtheta^{n+2} 
	- \vtheta^{n+1}  
	+ \phi \vtheta^n 
	= \phi \vtheta^*.
	\label{exa:eq:A2}
	\end{equation}
	Solving equation (\refeq{exa:eq:A2}) proves FL asymptotic convergence to the optimum $\vtheta^*$.
	
\end{example}




\subsection{Relaxed Sufficient Conditions for Minimizing the Federated Problem (\ref{eq:original_problem_general})}\label{subsec:relaxed_sufficient}

Theorem \ref{theo:bias_convex} holds for any client's update time $T_i$ and optimization scheme satisfying Algorithm \ref{alg:FL_with_delayed_gradients}, and provides finite convergence guarantees for the optimization  problem (\refeq{eq:original_problem_general}). Corollary \ref{cor:bias_distributions} shows that for the asymptotic convergence of FL, data distribution types should be treated fairly in expectation, i.e. $\tilde{s}_j(n) = r_j$.
This sufficient condition is not necessarily realistic, since the server cannot know the clients data distributions and participation time, and thus needs to give to every client an aggregation weight $d_i(n)$ such that $\tilde{q}_i(n) = p_i$ without knowing $T_i$.

In Example \ref{exa:bias}, we note that we have $\frac{1}{2}\left[q_i^{2n} + q_i^{2n+1}\right] = p_i$. Therefore, every client is given proper consideration every two optimization rounds.
%To provide weaker sufficient conditions than the ones of Corollary \ref{cor:bias_distributions}, 
Based on Example \ref{exa:bias}, in Theorem \ref{theo:relaxed_sufficient_conditions} we provide weaker sufficient conditions than the ones of Corollary \ref{cor:bias_distributions}. To this end, we assume that clients are considered with identical importance across $W$ optimization rounds (Assumption \ref{ass:window}) and that clients gradients are bounded (Assumption \ref{ass:bounded}).

\begin{assumption}[Window]\label{ass:window}	
	$\exists W \ge 1$ such that $\forall s,\ \frac{1}{W}\sum_{n=sW}^{(s+1)W-1} q_i(n) = q_i$.
\end{assumption}
With Assumption \ref{ass:window}, we assume that over a cycle of $W$ aggregations, the sum of the clients expected aggregation weights $q_i(n)$ are constant. 
By definition of $q_i$, Assumption \ref{ass:window} is always satisfied with $W = N$. Also, by construction, we have $ W \ge \tau$.
We note  that Assumption \ref{ass:window} is made on a series of windows of size $W$ and not for any window of size $W$. 


\begin{assumption}[Bounded Gradients]\label{ass:bounded} $\exists B>0$ such that	
	$ \E{\norm{\nabla \Lcal_i(\vx)}} \le B$
	.
\end{assumption}
Gradient clipping is a typical operation performed during the optimization of deep learning models to prevent exploding gradients. A pre-determined gradient threshold $B$ is introduced, and gradients with norm exceeding this threshold are clipped to the norm $B$. Therefore, using Assumption \ref{ass:bounded} and the subadditivity of the norm, the distance between two consecutive global models can be bounded by
\begin{equation}
\E{\norm{\vtheta^{n+1} - \vtheta^{n}}}
\le \eta_g \sum_{ i = 1 }^M q_i(n) \E{\norm{\vtheta_i^{\rho_i(n)+1} - \vtheta^{\rho_i(n)}} }
\le \eta_g \eta_l q(n) K B
,
\end{equation}
which, thanks to the convexity of the clients loss function and to the Cauchy Schwartz inequality, gives 
\begin{equation}
\E{\Lcal_i(\vtheta^{n+1})} - \E{\Lcal_i(\vtheta^{n})}
\le \E{\inner{\nabla  \Lcal_i(\vtheta^{n+1})}{\vtheta^{n+1} - \vtheta^n}}
\le \eta_g \eta_l q(n) B^2 K
\label{eq:ass_bounded}
.
\end{equation}
Finally, using equation (\refeq{eq:ass_bounded}) and Assumption \ref{ass:window}, the performance history on the original optimized problem can be bounded as follows
\begin{multline}
\sum_{n= s W}^{(s+1)W - 1}\sum_{ k = 0 }^{K-1} q_i \E{\Lcal_i(\vtheta^{(n, k)})} 
\le 
\sum_{n= s W}^{(s+1)W - 1}\sum_{ k = 0 }^{K-1} q_i(n) \left[\E{\bar{\Lcal}(\vtheta^{(n, k)})} 
+  \eta_g \eta_l K (W-1) B^2 \right]
.
\label{eq:window_bound}
\end{multline}


%\begin{assumption}[Window]\label{ass:window}	
%	$\exists W \ge 1$ such that $\forall s,\ \frac{1}{W}\sum_{n=sW}^{(s+1)W-1} q_i(n) = q_i$.
%\end{assumption}
%With Assumption \ref{ass:window}, we assume that over a cycle of $W$ aggregations, the sum of the clients expected aggregation weights $q_i(n)$ are identical. 
%By definition of $q_i$, Assumption \ref{ass:window} is always satisfied with $W = N$. Also, by construction, we have $ W \ge \tau$.
%We note Assumption \ref{ass:window} is made on a succession of windows of size $W$ and not for any window of size $W$. 
%Using equation (\refeq{eq:ass_bounded}), the performance history on the original optimized problem can be bounded as follow
%\begin{multline}
%	\sum_{n= s W}^{(s+1)W - 1}\sum_{ k = 0 }^{K-1} q_i \E{\Lcal_i(\vtheta^{(n, k)})} 
%	\le 
%	\sum_{n= s W}^{(s+1)W - 1}\sum_{ k = 0 }^{K-1} q_i(n) \left[\E{\bar{\Lcal}(\vtheta^{(n, k)})} 
%	+  \eta_g \eta_l K (W-1) B^2 \right]
%	.
%	\label{eq:window_bound}
%\end{multline}

\begin{theorem}\label{theo:relaxed_sufficient_conditions}
	Under the conditions of Theorem \ref{theo:convergence_convex}, Assumptions \ref{ass:window} and \ref{ass:bounded}, and considering that $W$ is a divider of  $N$, we get the following convergence bound for the optimization problem (\refeq{eq:surrogate_problem}):
	\begin{equation}
	\frac{1}{N}\sum_{ n = 0 }^{N-1}\frac{1}{K}\sum_{ k = 0 }^{K-1} \left[ \E{\bar{\Lcal}(\vtheta^{n, k})} - \bar{\Lcal}(\bar{\vtheta}) \right]
	\le \epsilon
	\coloneqq 
    \epsilon_F 
	+ \epsilon_K
	+ \epsilon_\alpha
	+ \epsilon_\beta
	+ \epsilon_W
		,
	\end{equation}
	where $\epsilon_W = \Ocal( \eta_g \eta_l (W-1) K)$. 
	Furthermore, we obtain the following convergence guarantees for the federated problem (\refeq{eq:original_problem_general}):
	\begin{align}
	\frac{1}{N}\sum_{ n = 0 }^{N-1}\frac{1}{K}\sum_{ k = 0 }^{K-1} \E{\norm{\nabla \Lcal (\vtheta^{n, k})}^2}
	& \le 
	\epsilon
	+ \Ocal (\chi^2 [\bar{\Lcal}(\bar{\vtheta}) -\sum_{j =1}^J s_j F_j(\vtheta_j^*)])
	,
	\end{align}	
	where $\chi^2 = \sum_{ j = 1 }^J \frac{\left(r_j - \tilde{s}_j\right)^2}{\tilde{s}_j}$.	
\end{theorem}

\begin{proof}
%	We define $q = \sum_{ i = 1 }^M q_i$. 
	\begin{align}
	&\frac{1}{N}\sum_{ n = 0 }^{N-1}\frac{1}{K}\sum_{ k = 0 }^{K-1} \left[ \E{\bar{\Lcal}(\vtheta^{n, k})} - \bar{\Lcal}(\bar{\vtheta}) \right]
	\nonumber\\
	& \le \frac{1}{N}\sum_{ n = 0 }^{N-1}\frac{1}{K}\sum_{ k = 0 }^{K-1}  q_i(n)\left[\E{\Lcal_i(\vtheta^{n, k})} + \tilde{\eta}  K (W - 1) B^2  \right] 
	- \bar{\Lcal}({\bar{\vtheta}})
	\\
	& \le R(\{\Lcal^n\})
	+ \epsilon 
	+ \frac{1}{N} \sum_{n=0}^{N-1} \Lcal^n(\bar{\vtheta}^n) 
	- \bar{\Lcal}(\bar{\vtheta}) 
	= \epsilon 
	,
	\end{align}
	where we use equation (\refeq{eq:window_bound}) for the first inequality and Theorem \ref{theo:convergence_convex} for the second inequality.
	
	Finally, we can obtain convergence guarantees on the optimization problem (\refeq{eq:original_problem_general}) with Theorem \ref{theo:bias_convex} by considering the minimization of the optimization problem $\bar{\Lcal}$. Therefore, the bound of Theorem \ref{theo:bias_convex} can be simplified noting that $\Lcal^n = \bar{\Lcal}$, $\bar{\vtheta}^n = \bar{\vtheta}$, $W_n = \emptyset$, $\chi_n^2 = \chi^2$, and by adding $\epsilon_W$, which completes the proof.
\end{proof}

Theorem \ref{theo:relaxed_sufficient_conditions} shows that the condition $\tilde{s}_j = r_j$ is sufficient to minimize the optimization problem (\refeq{eq:original_problem_general}). In practice, for privacy concerns, clients may not want to share their data distribution with the server, and thus the relaxed sufficient condition becomes $\tilde{q}_i = p_i$. This condition is weaker than the one obtained with Corollary \ref{cor:bias_distributions}, at the detriment of a looser convergence bound including an additional asymptotic term $\epsilon_W$ linearly proportional to the window size $W$. Therefore, for a given learning application, the maximum local work delay $\tau$ and the window size $W$ need to be considered when selecting an FL optimization scheme satisfying Algorithm \ref{alg:FL_with_delayed_gradients}.
%$q_i = p_i$ is a sufficient condition for federated problem (\refeq{eq:original_problem}) to be minimized. 
Also, the server needs to properly allocate clients aggregation weight $d_i(n)$ such that Assumption \ref{ass:window} is satisfied while keeping at a minimum the window size $W$. We note that $W$ depends of the considered FL optimization scheme and clients hardware capabilities.
Based on the results of Theorem \ref{theo:relaxed_sufficient_conditions}, in the following section, we introduce \textsc{FedFix}, a novel asynchronous FL setting based on a waiting policy over fixed time windows $\Delta t^n$. 

Finally, the following example illustrates a practical application of the condition $\tilde{q}_i = p_i$. 
\begin{example}\label{ex:relaxed_sufficient}
	We consider two clients, $i=1, 2$, with $\Lcal_i(\vtheta) = \frac{1}{2}\norm{\vtheta - \vtheta_i^*}^2$ where clients have identical importance, i.e. $p_1 = p_2 = 1/2$. Client 1 contributes at even optimization rounds and Client 2 at odd ones, i.e. $q_1^{2n} =  q_1$, $q_2^{2n+1} = q_2$,  and $q_1^{2n+1} = q_2^{2n} = 0$. 	
	Hence, we have
	\begin{align}
	\vtheta^n 
	&\xrightarrow{n \to \infty } \frac{q_1 \vtheta_1^* + q_2 \vtheta_2^*}{q_1 + q_2}
	,
	\end{align}
	which converges to the optimum of problem (\refeq{eq:original_problem_general}) if and only if $ \frac{1}{2}\left[ \tilde{q}_i^{2n} + \tilde{q}_i^{2n+1} \right] = p_i $ (Theorem \ref{theo:relaxed_sufficient_conditions}).
	
%	\begin{equation}
%	\vtheta_i^{n+1} = ( 1 - \eta_l a_i)^K \vtheta^n - ( 1- ( 1 - \eta_l a_i)^K)\frac{b_i}{a_i}
%	\end{equation}
%	We consider a learning rate such that $\eta_l< a_1$ and $\eta_l< a_2$. We define $\phi_i = ( 1- ( 1 - \eta_l a_i)^K)$.	Hence, we can rewrite the global model aggregation scheme, equation (\refeq{eq:original_problem}), as
%	\begin{equation}
%	\begin{cases}
%	\vtheta^{2n+1} = \vtheta^{2n} + \phi q_1[\vtheta_1^* - \vtheta^{2n}]\\
%	\vtheta^{2n+2} = \vtheta^{2n+1} + \phi q_2[ \vtheta_2^* - \vtheta^{2n+1}]
%	\end{cases}.
%	\end{equation}
%	As a result, we have 
%	\begin{align}
%		\vtheta^{2n+2} 
%		&= (1 - \phi_{2n} q_1)(1 - \phi_{2n+1} q_2)\vtheta^{2n}
%		+ \phi_{2n} q_1(1 - \phi_{2n+1} q_2) \vtheta_1^{*}
%		+ (1 - \phi_{2n+1} q_2)\vtheta_2^{*}
%		\\
%		&\xrightarrow{n \to \infty } \frac{q_1 \vtheta_1^* + q_2 \vtheta_2^*}{q_1 + q_2}
%	\end{align}
%	We also get $\vtheta^{2n+1} \xrightarrow{n \to \infty }  \frac{q_1 \vtheta_1^* + q_2 \vtheta_2^*}{q_1 + q_2}$. Consistently with Theorem \ref{theo:relaxed_sufficient_conditions}, we have $W=2$. Hence, the federated learning process converges. However, the optimum is unbiased if there exists $\alpha$ such that $q_1 = \alpha p1$ and $q_2 = \alpha p_2$. 
\end{example}

The conditions of Corollary \ref{cor:bias_distributions} and Theorem \ref{theo:relaxed_sufficient_conditions} are equivalent when $W=1$, where we retrieve $\epsilon_W=0$. They are also equivalent when clients have the same data distributions, and we retrieve $\tilde{s}_j = r_j = 1$ at every optimization round, which also implies that $W=1$. 




%\begin{example}\label{ex:relaxed_sufficient}
%	We consider two clients with quadratic functions satisfying $\Lcal_i(\vtheta) = \frac{1}{2}\norm{\vtheta - \vtheta_i^*}^2$. Each clients has identical importance in the federated loss function (\refeq{eq:original_problem}), i.e. $p_1 = p_2 = 1/2$. At every even number of optimization steps, client 1 participates and at every odd number of optimization steps, client 2 participates. Hence, we have $q_1^{2n} =  q_1$, $q_2^{2n+1} = q_2$,  and $q_1^{2n+1} = q_2^{2n} = 0$. When the server send a global model to the client, the server waits for the clients to send back its model before creating the new global model. Hence, we have:
%	\begin{equation}
%	\vtheta_i^{n+1} = ( 1 - \eta_l a_i)^K \vtheta^n - ( 1- ( 1 - \eta_l a_i)^K)\frac{b_i}{a_i}
%	\end{equation}
%	We consider a learning rate such that $\eta_l< a_1$ and $\eta_l< a_2$. We define $\phi_i = ( 1- ( 1 - \eta_l a_i)^K)$.	Hence, we can rewrite the global model aggregation scheme, equation (\refeq{eq:original_problem}), as
%	\begin{equation}
%	\begin{cases}
%	\vtheta^{2n+1} = \vtheta^{2n} + \phi q_1[\vtheta_1^* - \vtheta^{2n}]\\
%	\vtheta^{2n+2} = \vtheta^{2n+1} + \phi q_2[ \vtheta_2^* - \vtheta^{2n+1}]
%	\end{cases}.
%	\end{equation}
%	As a result, we have 
%	\begin{align}
%	\vtheta^{2n+2} 
%	&= (1 - \phi_{2n} q_1)(1 - \phi_{2n+1} q_2)\vtheta^{2n}
%	+ \phi_{2n} q_1(1 - \phi_{2n+1} q_2) \vtheta_1^{*}
%	+ (1 - \phi_{2n+1} q_2)\vtheta_2^{*}
%	\\
%	&\xrightarrow{n \to \infty } \frac{q_1 \vtheta_1^* + q_2 \vtheta_2^*}{q_1 + q_2}
%	\end{align}
%	We also get $\vtheta^{2n+1} \xrightarrow{n \to \infty }  \frac{q_1 \vtheta_1^* + q_2 \vtheta_2^*}{q_1 + q_2}$. Consistently with Theorem \ref{theo:relaxed_sufficient_conditions}, we have $W=2$. Hence, the federated learning process converges. However, the optimum is unbiased if there exists $\alpha$ such that $q_1 = \alpha p1$ and $q_2 = \alpha p_2$. 
%\end{example}

The convergence guarantee proposed in Theorem \ref{theo:relaxed_sufficient_conditions} depends on the window size $W$, and to the maximum amount of optimizations needed for a client to update its work $\tau$. 
We provide sufficient conditions in Corollary \ref{cor:sufficient_learning_rate} for the parameters $W$, and $\tau$, such that an optimization scheme satisfying Algorithm \ref{alg:FL_with_delayed_gradients} converges to the optimum of the optimization problem (\refeq{eq:original_problem_general}).


\begin{corollary}\label{cor:sufficient_learning_rate}
	Let us assume there exists $a \ge 0$ and $b \ge 0$ such that $W = \Ocal(N^a)$, $\tau = \Ocal(N^b)$, and $\eta_l \propto N^{-c}$. The convergence bound of Theorem \ref{theo:relaxed_sufficient_conditions} asymptotically converges to 0 if
	\begin{equation}
		W = o(N), 
		\tau = o(N), 
		\text{ and }
		\max (a, b) < c < 1
	\end{equation}
\end{corollary}

\begin{proof}
	The bound of Theorem \ref{theo:relaxed_sufficient_conditions} converges to 0 if the following quantities also do: $\eta_l W$, $\frac{1}{\eta_l N}$, $\tau \eta_l$, $\eta_l$. We get the following conditions on $a$, $b$, and $c$: $ - c + a< 0$, $ c- 1< 0$, $ b - c< 0$, $ - c < 0$, which completes the proof.
\end{proof}

By construction and definition of $q_i$, Assumption \ref{ass:window} is always satisfied with $W=N$. However, Corollary \ref{cor:sufficient_learning_rate} shows that when $W=N$, no learning rate $\eta_l$ can be chosen such that the learning process converges to $\vtheta^*$. 
Also, Corollary \ref{cor:sufficient_learning_rate} shows that Assumption \ref{ass:answering_time} can be relaxed. Indeed, Assumption \ref{ass:answering_time} implies that $\tau = \Ocal (1)$ and Corollary \ref{cor:sufficient_learning_rate} shows that $\tau = o(N)$ is sufficient.
We show in Section \ref{sec:applications} that all the considered optimization schemes satisfy $\tau = \Ocal (1)$ and $W = \Ocal (1)$, and also depend of the clients hardware capabilities and amount of participating clients $M$.

==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/main_convergence.tex <==
\section{Convergence of Federated Problem (\ref{eq:original_problem_general})}\label{sec:convergence}

In this section, we prove the convergence of the optimization based on the stochastic aggregation scheme defined in equation (\ref{eq:aggreg_SCAFFOLD_general}), with implementation given in Algorithm \ref{alg:FL_with_delayed_gradients}. 
We first introduce in Section \ref{subsec:assumptions} the necessary assumptions and then prove with Theorem \ref{theo:convergence_convex} the convergence of the sequence of optimized models (Section \ref{subsec:convergence_convex}).
We show in Section \ref{subsec:sufficient_conditions} the implications of Theorem \ref{theo:convergence_convex} on the convergence of the federated problem (\ref{eq:original_problem_general}), and propose sufficient conditions for the learnt model to be the associated optimum. Finally, with two additional assumptions, we propose in Section \ref{subsec:relaxed_sufficient} simpler and practical sufficient conditions for FL convergence to the optimum of the federated problem (\ref{eq:original_problem_general}).

%\subsection{Single Optimization Step}
%
%Decomposition Theorem \ref{theo:one_FL_step} highlights the impact of an FL optimization scheme on a single FL optimization step.
%For any optimization round, it provides an explicit link between the clients computation time properties 
%and the expected distance between the global model and vector $\vx$. 
%
%\begin{theorem}[Decomposition Theorem]\label{theo:one_FL_step}
%%	We consider clients send at optimization round $n$ their contribution $\vDelta^n$.
%	Under Assumption \ref{ass:clients_covariance}, the following equation holds for any vector $\vx$:
%	\begin{align}
%	\E{\norm{\vtheta^{n+1} - \vx}^2} 
%	&= \E{ \norm{\vtheta^n - \vx}^2 }
%	- 2 \eta_g \underbrace{\E{ \inner { \sum_{i=1}^M q_i(n) \vDelta_i(n)}{\vx - \vtheta^n} }}_{\text{Direction Drift}}
%	+\eta_g^2 Q (n)
%	\label{eq:one_server_iteration}
%	\end{align}
%	with
%	\begin{align}
%	Q(n)
%	 = 
%	\sum_{i=1}^M \gamma_i(n)
%	\underbrace{\E{\norm{\vDelta_i(n) }^2 } }_{\substack{\text{Local Model Drift}\\ = L_i(n)}}
%	+  \alpha
%	\underbrace{\E{\norm{\sum_{i=1}^M q_i(n)\vDelta_i(n) }^2}}_{ \substack{\text{Global Model Drift}\\ = G(n)} }
%	\end{align}
%	where 
%%	$\nu_i(n) = \mathbb{P}( T_i^n \le \Delta t^n) d_i^2(n) $
%%	and 
%	$\gamma_i(n) 
%	= \EE{S_n}{\omega_i^2(n)} - \alpha q_i^2(n) 
%	\ge 0$
%	.
%	
%\end{theorem}
%
%Decomposition Theorem \ref{theo:one_FL_step} (proof in Appendix \ref{app:sec:decompo_theo}) extends \cite{OnTheImpact} to account for asynchronicity. 
%This theorem shows that FL convergence is impacted by an FL optimization scheme through $\gamma_i(n)$ and $\alpha$.
%%which depend on the clients computation hardware capabilities. 
%These variables modulate two quantities, $L_i(n)$ and $G(n)$, representing respectively the \emph{local} and \emph{global} model drift from the current initialization. 
%The local and global drifts are always positive and thus $Q(n)$ is also always positive. 
%Therefore, Decomposition Theorem \ref{theo:one_FL_step} also provides a necessary condition for an optimization step to improve the current global model with respect to $\vx$: the direction drift needs to be positive. This makes optimization schemes based on delay gradients more challenging to optimize as clients contributions are not estimated on the same global model.
%
%\textbf{Application to time based aggregation weights (\ref{eq:agg_weights})}. 
%$Q(n)$ accounts for the aggregation weights $\omega_i(n)$ stochasticity over the optimization rounds $n$. 
%We show in the proof of Decomposition Theorem \ref{theo:one_FL_step} that $Q(n)$ is linearly proportional to $\EE{S_n}{\omega_i^2(n)}$ and $\alpha$. 
%The local model drift is proportional to the aggregation weight variance $\VAR{\omega_i(n)} = \mathbb{P}( T_i^n \le \vDelta t^n) d_i^2(n)$. We note that $\gamma_i(n)$ can be bounded in function of a client expected aggregation weight $q_i(n)$. Indeed, we have
%\begin{equation}
%\gamma_i(n) 
%= \left[d_i(n) - \alpha q_i(n) \right] q_i(n)
%\le \beta q_i(n)
%\end{equation}
%where we define $\beta \coloneqq \max\{d_i(n) - \alpha q_i(n)\}$.






\subsection{Assumptions}\label{subsec:assumptions}

We make the following assumptions regarding the Lipschitz smoothness and convexity of the clients local loss functions (Assumption \ref{ass:smoothness} and  \ref{ass:strong_convexity}), 
unbiased gradients estimators (Assumption \ref{ass:unbiased}), finite answering time for the clients (Assumption \ref{ass:answering_time}), and the clients aggregation weights (Assumption \ref{ass:clients_covariance}). 
Assumption \ref{ass:unbiased} \citep{Khaled2020} considers unbiased gradient estimators without assuming bounded variance, giving in turn more interpretable convergence bounds.
Assumption \ref{ass:clients_covariance} states that the covariance between two aggregation weights can be expressed as the product of their expected aggregation weight up to a positive multiplicative factor $\alpha$. We show in Section \ref{sec:applications} that Assumption \ref{ass:clients_covariance} is not limiting as it is satisfied by all the standard FL optimization schemes considered in this work.

\begin{assumption}[Smoothness]\label{ass:smoothness}
    Clients local objective functions are $L$-Lipschitz smooth, that is, $\forall i \in \{1, ..., n\},\ \norm{\nabla \Lcal_i(\vx) - \nabla \Lcal_i(\vy)} \le L \norm{\vx - \vy}$.
\end{assumption}

% \begin{assumption}[Strong convexity]\label{ass:strong_convexity}
% 	The clients local objective function is $\mu$-strongly convex, that is, $\forall i \in \{1, ..., n\},\ \inner{\nabla \Lcal_i(\vx)}{\vx - \vy}
% 	\ge \Lcal_i(\vx) - \Lcal_i(\vy) + \frac{\mu}{2}\norm{\vx - \vy}^2$.
% \end{assumption}
\begin{assumption}[Convexity]\label{ass:strong_convexity}
	Clients local objective functions are convex.
\end{assumption}

\begin{assumption}[Unbiased Gradient]\label{ass:unbiased}
	Every client stochastic gradient $g_i(\vx) = \nabla \Lcal_i(\vx, \vz_i)$ of a model with parameters $\vx$ evaluated on batch $\vz_i$ is an unbiased estimator of the local gradient, i.e. $\EE{\vz_i}{g_i(\vx)} = \nabla \Lcal_i(\vx)$.
\end{assumption}

\begin{assumption}[Finite Answering Time]\label{ass:answering_time}
	The server receives a client local work in at most $\tau \coloneqq \max_{i, n} (n - \rho_i(n))$ optimization steps, which satisfy $\mathbb{P}( \tau < \infty)  = 1$.
\end{assumption}

%We also consider the aggregation weights covariance satisfies Assumption \ref{ass:clients_covariance} \citep{OnTheImpact}. We provide in Section \ref{sec:applications} $\alpha$ close-form for all the considered optimization schemes. 
\begin{assumption}\label{ass:clients_covariance}
	There exists $\alpha \in (0, 1)$ such that $\E{\omega_i(n)\omega_j(n)} = \alpha q_i(n) q_j(n) $.
\end{assumption}


\subsection{Convergence of Algorithm \ref{alg:FL_with_delayed_gradients}}\label{subsec:convergence_convex}

%At optimization round $n$, client $i$ is considered with expected importance $\{q_i(n)\}$. No assumption is made on the clients importance $\{q_i(n)\}$ which can change over time. The expected clients contribution $\sum_{ i = 1 }^M q_i(n)\vDelta_i(n)$ helps minimize $\Lcal^n$ the optimization problem defined as
%\begin{equation}
%\label{eq:surrogate_loss_fucntion}
%\Lcal^n(\vtheta) 
%\coloneqq
%%\frac{1}{\bar{q}^n}
%\sum _{i=1}^M q_i(n) \Lcal_i(\vtheta)
%.
%\end{equation}
%%where $\bar{q}^n = \sum _{i=1}^M q_i(n)$. 
%We define by $\bar{\vtheta}^n$ the optimum of $\Lcal^n$ and by $\vtheta^*$ the optimum of optimization problem $\Lcal$ defined in equation (\ref{eq:original_problem_general}). Finally, we define $q_i = \frac{1}{N}\sum_{ n = 0 }^{N-1}q_i(n)$ the expected importance given to client $i$ over the FL process and $\tilde{q_i}$ its normalized expected importance $\tilde{q_i} = \frac{1}{N}\sum_{ n = 0 }^{N-1} \tilde{q_i}(n)$. We define $\tilde{\Lcal}$ the associated optimization problem where clients have importance $q_i$ with optimum $\bar{\vtheta}$ and defined as
%\begin{equation}
%\label{eq:surrogate_problem}
%\tilde{\Lcal}(\vtheta) 
%\coloneqq
%%\frac{1}{\bar{q}^n}
%\sum _{i=1}^M q_i \Lcal_i(\vtheta)
%=
%\frac{1}{N}\sum _{ n = 0}^{N-1} q_i(n) \Lcal^n(\vtheta)
%.
%\end{equation}
%Finally, we define $\Sigma_1$ and $\Sigma_2$ respectively the expected and variance convergence residual
%\begin{equation}
%	\Sigma_1 
%	\coloneqq \sum_{ i = 1 }^M q_i \EE{\vxi_i}{\norm{\nabla \Lcal_i(\bar{\vtheta}, \vxi_i)}^2}
%	\text{ and }
%	\Sigma_2 
%	\coloneqq \sum_{ i = 1 }^M \left[ \frac{1}{N}\sum_{ n = 0 }^{N-1} q_i^2(n) \right] 
%	\EE{\vxi_i}{\norm{\nabla \Lcal_i(\bar{\vtheta}, \vxi_i)}^2}
%	.
%\end{equation}

We first prove with Theorem \ref{theo:convergence_convex} the convergence of Algorithm \ref{alg:FL_with_delayed_gradients}. 

\begin{theorem}\label{theo:convergence_convex}
	Under Assumptions \ref{ass:smoothness} to \ref{ass:clients_covariance}, 
	with $\eta_l \le 1/48KL
	\min \left(1, 1/ {3 \rho^{2} \eta_g (\tau+1)}\right)$,
	we obtain the following convergence bound:
	\begin{align}
	\frac{1}{N}\sum_{ n = 0 }^{N-1}\frac{1}{K}\sum_{ k = 0 }^{K-1} \left[ \E{\Lcal^n(\vtheta^{n, k})} - \Lcal^n(\bar{\vtheta}^n) \right]
	& \le R(\{\Lcal^n\})
	+ \epsilon_F
	+ \epsilon_K
	+ \epsilon_\alpha
	+ \epsilon_\beta
	,
	\end{align}
	where 
	\begin{align}
	R(\{\Lcal^n\})
	= \frac{1}{N}\sum_{ n = 0 }^{N-1} \left[ \Lcal^n(\bar{\vtheta}) - \Lcal^n(\bar{\vtheta}^n)\right]
	,
	&&
	\epsilon_{F}
    = \frac{1}{\tilde{\eta} K N}\norm{\vtheta^{0} - \bar{\vtheta}}^2
    ,
	\end{align}
	\begin{align}
	    \epsilon_K
		= \Ocal \left(\eta_l^2 (K-1)^2 \left[ R(\{\Lcal^n\}) + \Sigma_1 \right] \right)
		,
		&&
		\epsilon_\alpha
	    = \Ocal \left( \alpha \left[\tilde{\eta} + \tilde{\eta}^2 K^2 \tau^2 \right] \left[ R(\{\Lcal^n\}) + 
	    \max q_i(n) \Sigma \right] \right)
	    ,
	\end{align}
	\begin{align}
	    \epsilon_\beta = \Ocal\left(\beta \left[\tilde{\eta} + \tilde{\eta}^2 K^2 \tau^2 \right] \left[ R(\{\Lcal^n\}) + \Sigma\right]\right)
	    ,
	    &&
    	\tilde{\eta} 
    	= \eta_g \eta_l
    	,
    	&&
    	\beta 
    	\coloneqq \max\{d_i(n) - \alpha q_i(n)\}
    	,
	\end{align}
    and $\Ocal$ accounts for numerical constants and the loss function Lipschitz smoothness $L$.

\end{theorem}
Theorem \ref{theo:convergence_convex} is proven in Appendix \ref{app:sec:convergence_convex}. The convergence guarantee provided in Theorem \ref{theo:convergence_convex} is composed of 5 terms: $R(\{\Lcal^n\})$, 
$\epsilon_F$, 
$\epsilon_K$,
$\epsilon_\alpha$,
$\epsilon_\beta$.
In the following, we describe these terms and explain their origin in a given optimization scheme.

\textbf{Optimized expected residual $R(\{\Lcal^n\})$}. 
The residual $R(\{\Lcal^n\})$ 
quantifies the sensitivity of $\Lcal^n$ between its optimum $\bar{\vtheta}^n$ and the optimum $\bar{\vtheta}$ of the overall expected minimized problem across optimization rounds $\tilde{\Lcal}$. 
As such, the residual accounts for the heterogeneity in the history of optimized problems, and is minimized to 0 when the same optimization problem is minimized at every round $n$, i.e. $\Lcal^n = \tilde{\Lcal}$. This condition is always satisfied when clients have identical data distributions, but requires for the server to set properly every client aggregation weight $d_i(n)$ in function of the server waiting time policy $\Delta t^n$ and the clients hardware capabilities $T_i^n$ in the general case (Section \ref{subsec:sufficient_conditions} and \ref{subsec:relaxed_sufficient}). 

\textbf{Initialization quality $\epsilon_{F}$}. 
$\epsilon_{F}$ only depends of the quality of the initial model $\vtheta^0$ through its distance with respect to the optimum $\bar{\vtheta}$ of the overall expected minimized problem across optimization rounds $\tilde{\Lcal}$. 
This convergence term can only be minimized by performing as many serial SGD steps $K N$.

\textbf{Clients data heterogeneity $\epsilon_K$}. 
This term accounts for the disparity in the clients updated models, and is proportional to the clients amount of local work $K$ (quadratically) and to the heterogeneity of their data distributions $\Zcal_i$ through $\Sigma_1$.  
When $K=1$, every client perform its SGD on the same model, which reduces the server aggregation to a traditional centralized SGD. We retrieve $\epsilon_K = 0$. 

\textbf{Gradient delay $\tau$ through $\epsilon_\alpha$ and $\epsilon_\beta$}.
Decreasing the server time policy $\Delta t^n$ allows faster optimization rounds but decreases a client's participation probability $\mathbb{P}( T_i^n \le \Delta t^n )$ resulting in an increased maximum answering time $\tau$. 
In turn, we note that $\epsilon_\alpha$ and $\epsilon_\beta$ are quadratically proportional to the maximum amount of serial SGD $K \tau$.
This latter terms quantifies the maximum amount of SGD integrated in the global model $\vtheta^n$.


% \textbf{Aggregation policy $\epsilon_\omega$ and delayed updates $\epsilon_\tau$}.
% Decreasing the server time policy $\Delta t^n$ allows faster optimization rounds but decreases a client's participation probability $\mathbb{P}( T_i^n \le \Delta t^n )$ resulting in an increased maximum answering time $\tau$. 
% In turn, we note that $\epsilon_\tau$ is quadratically proportional to the amount of serial SGD $K \tau$, the maximum amount of SGD integrated in the global model $\vtheta^n$ since a client received its global model $(\rho_i(n) \le \tau)$, which makes the selection of $\Delta t^n$ detrimental for the convergence residual after $T$ time. Finally, when every client has the same data distribution, we have $\Sigma_1 = \Sigma_2 = 0$ which gives $\epsilon_\omega = \epsilon_\tau = 0$.



==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/main_experiments.tex <==
\section{Experiments}\label{sec:experiments}

In this section, we experimentally demonstrate the theoretical claims of Section \ref{sec:convergence} and \ref{sec:applications}.
We first introduce the information needed to understand how the experiments are run in Section \ref{subsec:setting}. Finally, in Section \ref{subsec:exp_results}, we provide our experiments and their interpretation. 

\subsection{Experimental Setting}\label{subsec:setting}

We introduce in this subsection the dataset and the predictive models used for federated optimization, the hardware scenarios proposed to simulate hardware heterogeneity, the clients aggregation weights strategies, and how the different hyperparameters are set.

\textbf{Optimization Problems.}
We consider learning a predictive model for optimization problem (\ref{eq:original_problem_general}) where clients have identical importance ($p_i = 1/M$) based on the following datasets with their associated learning scenarios. 
\begin{itemize}
	
%	\item \textbf{Synthetic}. 
%	Every client has 100 data features generated with $X_i \sim U(0, 1)$, $\mu_i \sim U(0, 1)$, and predictive value $y_i = X_i \mu_i$. With asynchronous federated learning, we learn the optimal model parameters $\vtheta$ minimizing the federated mean squared error.
	
	\item \textbf{MNIST} \citep{MNIST} and \textbf{MNIST-shard}. MNIST is a dataset of 28x28 pixel grayscale images of handwritten single digits between 0 and 9 composed of 60 000 training and 10 000 testing samples split equally among the clients. 
	We use a logistic regression to predict the images class. Clients are randomly allocated digits to match their number of samples. 
	With MNIST-shard, we split instead data samples among clients using a Dirichlet distribution of parameter 0.1, i.e. $Dir(0.1)$.
	Therefore, with MNIST and MNIST-shard, we evaluate our theory on a convex optimization problem.
	
%	\item \textbf{MNIST-shard}. MNIST is split equally among clients with a Dirichlet distribution of parameter 0.1, i.e. $Dir(0.1)$.
%	Therefore, with MNIST-shard, we evaluate our theory on a convex optimization where clients have non-iid data.
	
%	\item \textbf{FEMNIST} \citep{Leaf}. FEMNIST is a federated version of MNIST where a client has data samples written by the same person. We train a logistic regression to have a convex optimization where clients have different data distributions. 
%%	By default, clients have different amount of data which makes FEMNIST unbalanced.
	
	\item \textbf{CIFAR-10} \citep{CIFAR-10}. The dataset consists of 10 classes of 32x32 images with three RGB channels.  There are 50000 training and 10000 testing examples. The model architecture was taken from \citep{FedAvg} which consists of two convolutional layers and a linear transformation layer to produce logits. 
	Clients get the same amount of samples but their percentage for each class vary and is determined with a Dirichlet distribution of parameter 0.1, i.e. $Dir(0.1)$ \citep{FL_and_CIFAR_dir}. 
	
	\item \textbf{Shakespeare} \citep{Leaf}. We study a LSTM model for next character prediction on the dataset of \textit{The Complete Works of William Shakespeare}. The model architecture is composed of a two-layer LSTM classifier containing 100 hidden units with an 8 dimensional embedding layer taken from \citep{FedProx}. The model takes as an input a sequence of 80 characters, embeds each of the characters into a learned 8-dimensional space and outputs one character per training sample after 2 LSTM layers and a fully connected one.
\end{itemize}





\textbf{Hardware Scenarios.}
In the following experimental scenarios, clients computation time are obtained according to the time policy $FX$. We consider that clients have fixed update times that can be up to X\% slower than the fastest client. Clients computation time are uniformly distributed from the upper to the lower bound.
Clients have thus identical hardware with $F0$. To simulate heterogeneous clients hardware, we consider the time scenario $F80$.

\textbf{Clients Aggregation Weights.}
To compare asynchronous FL with and without the close-form of $d_i$ provided in Section \ref{sec:applications}, we introduce \textsc{Identical} where $d_i =1$ for every client regardless of the time scenario $FX$, and \textsc{Time-based} where $d_i$ satisfies equation (\ref{eq:aggreg_weights_async}) derived in Section \ref{sec:applications}.

\textbf{Hyperparameters.}
Unless specified otherwise, we consider a global learning rate $\eta_g = 1$. We finetune the local learning rate $\eta_l$ with values ranging from $10^{-5}$ to $1$. We consider a batch size $B=64$ for every dataset. 
We report mean and standard deviation on 5 random seeds. 
Every comparison of \textsc{Identical} with \textsc{Time-Based} is done using the same local learning rate. We give an advantage to \textsc{Identical} by finetuning the learning rate on this clients aggregation weight scenario. 



\subsection{Experimental Results}\label{subsec:exp_results}

We experimentally show that asynchronous FL has better performances with \textsc{Time-based} than with \textsc{Identical}, and thus we demonstrate the correctness of Theorem \ref{theo:relaxed_sufficient_conditions} with Figure \ref{fig:improvement_conv_async} in Section \ref{subsubsec:convergence_async}. We however show in Figure \ref{fig:amount_of_SGD} that \textsc{Time-based} is less stable than \textsc{Identical} to the change in amount of local work $K$. Finally, we compare synchronous \textsc{FedAvg} and asynchronous \textsc{FedAvg} in Figure \ref{fig:all_opt_scheme}. 

\subsubsection{Impact of the Clients Aggregation Weights on Asynchronous \textsc{FedAvg}}\label{subsubsec:convergence_async}

\begin{figure}
	\includegraphics[width=\linewidth]{./plots/fig_conv_async_all.pdf}
	\caption{We consider the loss evolution over time of federated problem (\ref{eq:original_problem_general}) (FP) and surrogate problem (\ref{eq:surrogate_problem}) (SP) for MNIST, MNIST-shard, CIFAR10, and Shakespeare; and the respective standard deviation of the loss over clients in (b) and (d).
	We consider $M=10$ for a time scenario $F80$ with $K=1$. 
	}
	\label{fig:improvement_conv_async}
\end{figure}


Figure \ref{fig:improvement_conv_async}(a) experimentally shows the interest of coupling asynchronous FL with \textsc{Time-based} instead of \textsc{Identical} for different applications (MNIST, MNIST-shard, CIFAR10, and Shakespeare). The learnt model with \textsc{Time-based} has better minima on the federated problem (\ref{eq:original_problem_general}). 
In addition, Figure \ref{fig:improvement_conv_async}(b) shows that losses across clients are more homogeneous with \textsc{Time-based}, resulting in generally lower standard deviations. 

Focusing on MNIST and MNIST-shard, we see the impact of data heterogeneity on the learnt model performances. With \textsc{Identical}, asynchronous FL converges to a suboptimum point and the differences between the learnt model losses is twice as large for MNIST-shard than for MNIST, Figure \ref{fig:improvement_conv_async}(a). 
Figure \ref{fig:improvement_conv_async}(b) shows a similar result concerning the clients loss heterogeneity.
Therefore, data heterogeneity degrades the suboptimum loss and cannot be ignored in asynchronous FL applications. Indeed, \textsc{Identical} and \textsc{Time-based} curves are significantly different even for the simplest application on MNIST, where the dataset is uniformly distributed across $M=10$ clients.
Hence, the assumption of identical data distributions should generally not be made and the aggregation scheme \textsc{Time-based} should be used instead for any asynchronous FL (or DL). 

With Figure \ref{fig:improvement_conv_async}(c), we can also appreciate the performances of the learning procedure on the surrogate problem (\ref{eq:surrogate_problem}) based on the clients computation times $T_i$. Due to clients hardware heterogeneity, in the scenario $F80$, clients communicate with the server up to 5 more times than the slowest one. \textsc{Time-based} balances this amount of updates disparity across clients. As a result, \textsc{Identical} has better performances than \textsc{Time-based} on the surrogate problem (\ref{eq:surrogate_problem}) for MNIST, MNIST-shard, and CIFAR10, while for Shakespeare, \textsc{Time-based} shows better performances. We attribute this fact to the depth of the predictive model enabling overfitting. As such, \textsc{Time-based} outperforms \textsc{Identical} on the federated problem (\ref{eq:original_problem_general}), Figure \ref{fig:improvement_conv_async}(a), while preventing catastrophic forgetting and thus leading to better losses on fast clients, Figure \ref{fig:improvement_conv_async}(c). Finally, Figure \ref{fig:improvement_conv_async}(d) shows that in addition, the weighted standard deviation of the surrogate loss is always worse for \textsc{Identical}.


 



\subsubsection{Impact of the amount of local work on asynchronous FL convergence}
\label{subsubsec:async_nSGD}

\begin{figure}
	\centering
	\includegraphics[width=0.5 \linewidth]{./plots/fig_evo_SGD.pdf}
	\caption{Evolution of the loss of optimization problem (\ref{eq:original_problem_general}) for CIFAR10 with $M=10$, time scenario $F80$, $\eta_g = 1$, $\eta_l = 0.005$, and varying amount of local work $K$ ranging from 1 to 25.}
	\label{fig:amount_of_SGD}
\end{figure}

With Figure \ref{fig:amount_of_SGD}, we consider the impact of the amount of local work on the convergence speed of Asynchronous FL with CIFAR10, time scenario $F80$, and $M=10$ clients. For every simulation, we consider $\eta_l = 0.0005$, the optimal local learning rate for $K=1$ with \textsc{Identical}. The server aggregates the clients contribution over $T = 25000$ units of time, and we report in Figure \ref{fig:amount_of_SGD} mean and standard deviation over the 5\% last server optimization rounds of the loss of the optimization problem (\ref{eq:original_problem_general}).

Figure \ref{fig:amount_of_SGD} shows that increasing the amount of local work $K$ first decreases the loss of optimization problem (\ref{eq:original_problem_general}) evaluated on the expected learnt model before increasing it. This point justifies asking to clients to perform $K>1$ SGDs but requires proper finetuning of the amount of local work $K$. In particular, we notice that the variance strictly increases with $K$, which shows that the learning procedure becomes less stable.

These behaviors of asynchronous FL are due to the disparity between clients contributions induced by clients data heterogeneity, and can only be mitigated with a smaller global learning rate $\eta_g$, local learning rate $\eta_l$, and amount of local work $K$. 
Figure \ref{fig:amount_of_SGD} shows that \textsc{Time-based} is however more sensitive to an increase in amount of local work $K$ than \textsc{Identical}. \textsc{Time-based} is associated with higher variance after $K=8$, and higher mean after $K=15$, while \textsc{Identical} has  very similar mean and standard deviation from $K=8$ to $K=16$. 

This difference in convergence behavior is due to the FL aggregation scheme (\ref{eq:aggreg_SCAFFOLD_general}), and to the difference between the clients aggregation weights $d_i$ for \textsc{Identical} and \textsc{Time-based}. We have indeed $d_i =1$ for every client with \textsc{Identical}, while with \textsc{time-based} fast clients are given lower aggregation weights $d_i<1$, and slow clients higher weights $d_i>1$. 
Therefore, whenever a slow client contributes, the new global model is more perturbed with \textsc{Time-based} than with \textsc{Identical}, which makes \textsc{Time-based} convergence speed more sensitive to a small change in the choice of $K$ and other hyperparameters. 
This point can also be noticed in Figure \ref{fig:improvement_conv_async}(a) where \textsc{Identical} first converges faster than \textsc{Time-based}. Still, \textsc{Identical} converges to a suboptimum. 

\textsc{Identical} outperforms \textsc{Time-based} in Figure \ref{fig:amount_of_SGD} because we consider $\eta_l = 0.0005$.
We note that considering our time budget $T$, doing a grid search for $\eta_l$ would always provide a learnt model with better optimization loss for \textsc{Time-based}.






%\subsubsection*{Importance of the amount of clients}
%
%\begin{figure}
%	\caption{text}
%	\label{fig:amount_of_clients}
%\end{figure}
%
%We investigate the impact of the amount of clients $M$. With Figure \ref{fig:amount_of_clients}, we consider CIFAR10 partitioned in $M \in \{1, 2, 5, 10, 20, 50, 100\}$. 


%\subsubsection*{Robustness}
%
%\begin{figure}
%	\caption{text}
%	\label{fig:robustness_eta_l}
%\end{figure}
%
%We investigate the impact of the local learning rate $\eta_l$ on the convergence speed. Indeed, due to communication constraints, fine-tuning hyperparameters in FL is challenging. We also investigate the impact of $\eta_g$ with Figure \ref{fig:robustness_eta_g}. 
%With Figure \ref{fig:robustness_eta_l}, we consider CIFAR10 with $M=20$. 
%
%\begin{figure}
%	\caption{text}
%	\label{fig:robustness_eta_g}
%\end{figure}



\subsubsection{Partial Asynchronicity with \textsc{FedFix}}\label{subsubsec:partial_asynchronicity}


\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{./plots/fig_best_opt_scheme.pdf}
	\caption{Evolution of federated problem (\ref{eq:original_problem_general}) loss for CIFAR10 and Shakespeare and time scenario $F0$ and $F80$, with $M=20$ (a) and $M=50$ (b). We consider $\eta_g = 1$, $K = 10$, and $\Delta t=0.5$ for \textsc{FedFix}.}
	\label{fig:all_opt_scheme}
\end{figure}

The theory derived in Section \ref{sec:convergence} can be applied to asynchronous FL but also synchronous FL, \textsc{FedAvg}, and other asynchronous FL schemes like \textsc{FedFix} (Section \ref{sec:applications}). 
We show with Figure \ref{fig:all_opt_scheme} that allowing asynchronicity does not necessarily provide faster learning processes, e.g. comparison between synchronous and asynchronous \textsc{FedAvg} above, but \textsc{FedFix} always outperforms \textsc{FedAvg} by balancing convergence speed and stability.

With a small enough learning rate $\eta_l$, asynchronous \textsc{FedAvg} outperforms \textsc{FedFix}, which outperforms synchronous FL (see Figure \ref{app:fig:explore_CIFAR10_20} and \ref{app:fig:explore_Shakespeare_20} in Appendix \ref{app:sec:experiments}). Indeed, in this case, global models change slowly and we can consider that the server receives contributions with no gradient delay. As such, the learning procedure including the most serial contributions in the global model is the fastest. 
% Hence, asynchronous FL outperforms \textsc{FedFix}, which outperforms synchronous FL. 
However, in the other cases, the learning rate $\eta_l$ does not mitigate the discrepancy between clients update, which slows down convergence for asynchronous FL, and can even prevent it.

Identifying the fastest optimization scheme must be done by comparing optimization schemes based on their best local learning rate $\eta_l$ (Figure \ref{fig:all_opt_scheme}). 
Synchronous FL always outperforms asynchronous FL when clients have heterogeneous hardware ($F0$). Even with heterogeneous hardware ($F80$), synchronous FL can outperform asynchronous FL (Shakespeare). Indeed, the server needs to reduce its amount of aggregations to balance convergence speed and convergence stability. We see that \textsc{FedFix-0.5} provides this trade-off and outperforms synchronous FL in every scenario. 

We note that, even for synchronous FL, FL convergence is not monotonous. Indeed, for synchronous FL to have a better convergence speed than asynchronous FL, the server needs to consider a high local learning rate leading to convergence instability. Figure \ref{fig:all_opt_scheme} shows this instability for Shakespeare and $t>4000$, and Figure \ref{app:fig:explore_CIFAR10_20} to \ref{app:fig:explore_Shakespeare_20} in Appendix \ref{app:sec:experiments} provides the evolution of this instability as the learning rate $\eta_l$ increases.

We note that even when clients have homogeneous hardware ($F0$), \textsc{FedFix} outperforms synchronous FL. This can be explained by the close-form of \textsc{FedFix} weights $d_i$, equation (\ref{eq:aggreg_weights_hybrid}), which accounts for server aggregations where no client participates. As a result, \textsc{FedFix-0.5} behaves as asynchronous FL but with an higher server learning rate $\eta_g =2$ which provides faster convergence.









==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\left \lceil #1 \right \rceil}
\def\floor#1{\left \lfloor #1 \right \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vDelta{{\bm{\Delta}}}
\def\vtheta{{\bm{\theta}}}
\def\vxi{{\bm{\xi}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\vR{{\bm{R}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

%\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
%\newcommand{\KL}{D_{\mathrm{KL}}}
%\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
%\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/math_formulas.tex <==
% Abbreviations
\newcommand{\rhs}[0]{right hand side}  % right hand side
\newcommand{\lhs}[0]{left hand side}  % left hand side
\newcommand{\snr}[0]{snr}  % signal-to-noise ratio
% Definitions
\newcommand{\realnumbers}[0]{\mathbb{R}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
% boldface symbols
\newcommand{\ab}[0]{\mathbf{a}}
\newcommand{\bb}[0]{\mathbf{b}}
\newcommand{\xb}[0]{\mathbf{x}}
\newcommand{\setx}[0]{\mathbf{x}_1,\ldots,\mathbf{x}_C}
\newcommand{\setxn}[0]{\mathbf{x}_1^{(n)},\ldots,\mathbf{x}_C^{(n)}}
\newcommand{\yb}[0]{\mathbf{y}}
\newcommand{\zb}[0]{\mathbf{z}}
\newcommand{\dz}[0]{d\zb}
% colored symbols
\newcommand{\xc}[0]{\color{blue}x\color{black}}
\newcommand{\xbc}[0]{\color{blue}\xb\color{black}}
\newcommand{\yc}[0]{\color{olive}y\color{black}}
\newcommand{\ybc}[0]{\color{olive}\yb\color{black}}
% bold symbols
\newcommand{\alphab}[0]{\boldsymbol{\alpha}}
\newcommand{\thetab}[0]{\boldsymbol{\theta}}
\newcommand{\thetaset}[0]{\thetab_1,\ldots,\thetab_C}
\newcommand{\phib}[0]{\boldsymbol{\phi}}
\newcommand{\phiset}[0]{\phib_1,\ldots,\phib_C}
\newcommand{\etab}[0]{\boldsymbol{\eta}}
\newcommand{\epsilonb}[0]{\boldsymbol{\epsilon}}
\newcommand{\x}[0]{\xb}
\newcommand{\z}[0]{\zb}
\newcommand{\Lin}[0]{\mathbf{L}}
\newcommand{\mub}[0]{\boldsymbol{\mu}}
\newcommand{\Sigmab}[0]{\boldsymbol{\Sigma}}
\newcommand{\sigmab}[0]{\boldsymbol{\sigma}}
% cal symbols
\newcommand{\Dcal}[0]{\mathcal{D}}
\newcommand{\Lcal}[0]{\mathcal{L}}
\newcommand{\Mcal}[0]{\mathcal{M}}
\newcommand{\Ocal}[0]{\mathcal{O}}
\newcommand{\Pcal}[0]{\mathcal{P}}
\newcommand{\Qcal}[0]{\mathcal{Q}}
\newcommand{\Rcal}[0]{\mathcal{R}}
\newcommand{\Ucal}[0]{\mathcal{U}}
\newcommand{\Zcal}[0]{\mathcal{Z}}
% Gaussian
\newcommand{\Gauss}[2]{\mathcal{N}\left(#1;#2\right)}
\newcommand{\Gaussof}[1]{\mathcal{N}\left(#1\right)}
\newcommand{\Gausstd}[0]{\Gauss{\mathbf{0}}{\mathbf{I}}}
\newcommand{\GaussStdDim}[1]{\Gauss{\mathbf{0}}{\mathbf{I}_{#1}}}
% Kullback-Leibler
\newcommand{\kl}[0]{\operatorname{\mathcal{D}_{KL}}}
\newcommand{\KL}[2]{\kl\bigg(#1\bigg\vert\bigg\vert#2\bigg)}
% Expected Value
\newcommand{\expect}{\operatorname{\mathbb{E}}}
\newcommand{\Var}{\operatorname{Var}}
\newcommand{\Cov}{\operatorname{Cov}}
\newcommand{\VAR}[1]{\Var\left[#1\right]}
\newcommand{\VARR}[2]{\Var_{#1}\left[#2\right]}
\newcommand{\COV}[2]{\Cov\left[#1 , #2\right]}
\newcommand{\E}[1]{\expect\left[#1\right]}
\newcommand{\EE}[2]{\expect_{#1}\left[#2\right]}
% Marginal / Joint probabilities
\newcommand{\q}[1]{q\left(#1\right)}
\newcommand{\p}[1]{p\left(#1\right)}
\newcommand{\px}[0]{\p{\x}}
\newcommand{\pz}[0]{\p{\z}}
\newcommand{\pxz}[0]{\p{\x,\z}}
\newcommand{\psetx}[0]{\p{\setx}}
\newcommand{\psetxz}[0]{\p{\setx,\z}}
% Conditional probabilities
\newcommand{\pxgz}[0]{\p{\x|\z}} % x Given z
\newcommand{\psetxgz}[0]{\p{\setx|\z}}
\newcommand{\pzgsetx}[0]{\p{\z|\setx}}
\newcommand{\pzgx}[0]{\p{\z|\x}}
% Posterior
\newcommand{\pzsetx}[0]{\p{\z|\setx}}
% Variational approximation
\newcommand{\qz}[0]{\q{\z}}
\newcommand{\qzgx}[0]{\q{\z|\x}}
\newcommand{\qzgsetx}[0]{\q{\z|\setx}}
\newcommand{\qzg}[1]{\q{\z|#1}}
\newcommand{\qzx}[1]{\q{\z|\x_{#1}}}
% Lower Bound
\newcommand{\LB}[0]{\mathcal{L}\left(\thetab, \phib, \x \right)}
% EXPECTATION PROPAGATION
\newcommand{\qi}[0]{q_i(\thetab)}
\newcommand{\qj}[0]{q_j(\thetab)}
\newcommand{\cavity}[0]{Q_{\backslash i}(\thetab)}
%Complexity

%Innner Product
\newcommand{\inner}[2]{\langle #1, #2 \rangle}





==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/one_client.tex <==
\subsection{Centralized Learning}\label{subsec:centralized_learning}

In this setting, one client, i.e. $M = 1$, learns a predictive model on its own data. In this case, we always have $\tilde{q}_1(n) =1$, and the resulting optimization problem is always proportional to $\Lcal = \Lcal_1$ which thus gives $R(\{\Lcal^n\}) \le R(\Lcal) = 0$. 
%The server/client only has to wait for its participation to compute the next global model. 
There is no gradient delay ($\tau =1$), while the clients always participate at each optimization round ($\alpha = 1$ and $\beta=0$), while the global learning rate is redundant with the local learning rate ($\eta_g =1$). The server performs $KN$ SGD steps. All these considered elements give
\begin{equation}
\label{eq:epsilon_centra}
\epsilon
= \Ocal\left(\frac{\norm{\vtheta^0 - \vtheta^*}^2}{\eta_l K N}\right)
+ \Ocal \left(\eta_l \EE{\vxi}{\norm{\nabla \Lcal(\vx, \vxi)}^2} \right)
.
\end{equation}
With equation (\refeq{eq:epsilon_centra}), we retrieve standard convergence guarantees for centralized ML derived in \cite{SGD_review}.

%We consider the server has the hardware capabilities of the fastest client and thus perform $K$ SGD steps in time $\tau_1$. Therefore, the server performs $N = T/ \tau_1$ optimization steps in $T$ time, which gives 
%
%\begin{equation}
%\epsilon'
%= \Ocal\left(\frac{\sqrt{\tau_1}}{\sqrt{K T}}\right)
%%+ \Ocal \left( \eta_l^2 (K -1) \sigma^2 \right)
%+ \Ocal \left(\frac{\sqrt{\tau_1}}{\sqrt{K T}} \EE{\vxi}{\norm{\nabla \Lcal(\vx, \vxi)}^2} \right)
%.
%\end{equation}


==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/priorities.tex <==
\section{Priorities}

\begin{enumerate}
	
%	\item Finish the literature review
	
%	\item Write properly the intro
	
	\item Update Schematic F1
	
	\item Experiments: Figure with FedFix
	
	\item Submission at JMLR
	

\end{enumerate}

==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/quadratic_example.tex <==
\section{Example with quadratic functions}\label{app:sec:quadratic}

To show in this work that provided convergence bound are tight, we consider an FL applications where clients local loss functions are convex and quadratic, i.e. 
\begin{equation}
	\Lcal_i(\theta) = a_i \theta^2 + b_i \theta + c_i,
	\label{eq:example_local_loss}
\end{equation}
where $\theta \in \mathbb{R}$ and $a_i \ge 0$. Taking the gradient of this local loss function, we get $\nabla \Lcal_i(\theta) = 2 a_i \theta +  b_i$ which leads to 
\begin{equation}
	\theta_i^* = - b_i / (2 a_i) 
	\text{ and }
	\Lcal_i(\theta_i^*) = - b_i^2 / (4 a_i) + c_i .
	\label{eq:example_local_optimum}
\end{equation}
A parallel can be done with this local loss function to a linear regression with one parameter and a modelization with no bias, i.e. $\Lcal_i(\theta) = \frac{1}{2}\norm{X_i \theta - y_i}^2$ where $X_i$ is the parameter vector and $y_i$ is the output vector which leads to  $a_i = X_i^T X_i /2$, $b_i = - X_i^T y_i$, and $c_i = y_i^Ty_i/2$. We also have:
\begin{equation}
	\theta^* = - (\sum_{i=1}^{n}p_i b_i) / (2 \sum_{i=1}^{n}p_i a_i)
	\text{ and }
	\Lcal(\theta^*) = - (\sum_{i =1 }^n p_i b_i)^2 / (4 \sum_{i=1}^{n}p_i a_i) + \sum_{i=1}^{n}p_i c_i .
\end{equation}


Let us consider a local SGD process. $y_{i, k}^n$ is the local model obtained for client $i$ after $k$ SGD. One gradient descent of a client satisfies $\nabla \Lcal_i(x) = - (x - \theta_i^*)$ hence one descent of gradient can be expressed as:
\begin{equation}
y_{i, k+1}^n 
= y_{i, k}^n - \eta_l (y_{i, k}^n - \theta_i^*)
= (1 - \eta_l) y_{i, k}^n + \eta_l \theta_i^* 
\end{equation}
which leads to 
\begin{equation}
\theta_i^{n+1} 
= (1 - \eta_l)^K \theta^n + \sum_{k=0}^{K-1} ( 1 - \eta_l)^k \eta_l \theta_i^*. 
\end{equation}
We note that $\sum_{k=0}^{K-1} ( 1 - \eta_l)^k = [1 - ( 1 - \eta_l )^K]/ \eta_l$. By defining $\phi = 1 -  ( 1 - \eta_l )^K$, we get:
\begin{equation}
\theta_i^{n+1} 
= ( 1 - \eta_l )^K \theta^n + \phi \theta_i^*,
\label{eq:local_work_quadratic}
\end{equation}
which leads to 
\begin{equation}
\theta_i^{n+1} - \theta^n
%= (1 - \eta_l)^K \theta^n + \left[1 - ( 1 - \eta_l )^K \right] \theta_i^* - \theta^n
= \phi (\theta_i^* - \theta^n). 
\label{eq:diff_local_work_quadratic}
\end{equation} 






\subsection{Expected Convergence}

Hence, considering equation (\ref{eq:aggreg_SCAFFOLD_general}), we have:
\begin{equation}
	\theta^{n+1}
	= \theta^n + \eta_g \sum_{ i = 1 }^M\omega_i^n \phi \left[\theta_i^* - \theta^{\rho_i(n)} \right] 
%	= \left[ 1 - \eta_g \phi \sum_{ i = 1 }^M\omega_i^n \right]\theta^n 
%	+ \eta_g \phi \sum_{ i = 1 }^M\omega_i^n \theta_i^* 
\end{equation}
We note that $\E{\theta^{\rho_i(n)}} = \sum_{k=0}^{n}\mathbb{P}(\rho_i(n) = k) \E{\theta^k}$. We have $q_{n, k} = \mathbb{P}(\rho_i(n) = k) $. and $\E{\omega_i^n} = 1/C$ which gives:
\begin{align}
\E{\theta^{n+1}}
& = \E{\theta^n} 
+ \eta_g \phi \frac{1}{M} \sum_{ i = 1 }^M\theta_i^* 
- \eta_g \phi \sum_{ k = 0 }^n q_{n, k} \E{\theta^k} 
%& = ( 1 - \eta_g \phi q_{n, n})\E{\theta^n} 
%- \eta_g \phi \sum_{ k = 0 }^{n-1} q_k \E{\theta^k}
%+ \eta_g \phi \theta^* 
\end{align}

We consider that we can write 
\begin{equation}
	\E{\theta^n }
	= A^n \theta^0 + B^n
	\label{eq:U_2}
\end{equation}
with $A^0 = 1$ and $B^0 = 0$.

Hence, we have:
\begin{align}
\E{\theta^{n+1}}
& = A^n \theta^0 + B^n
- \eta_g \phi \sum_{ k = 0 }^n q_{n, k} [A^k \theta^0 + B^k]
+ \eta_g \phi \theta^* 
\end{align}

which gives $ A^{n+1} = A^n - \eta_g \phi \sum_{ k = 0 }^n q_{n, k} A^k$ and $B^{n+1} = B^n - \eta_g \phi \sum_{ k = 0 }^n q_{n, k} B^k + \eta_g\phi \theta^*$.

\subsection{Variance}
All the clients have the same importance, $p_i = 1 /C$ and the same hardware, $\tau_i = \tau = 1$. Hence, we have: $R_i = R$, $\gamma_i = \gamma = \left[\mathbb{P}( T_i \le \Delta t^{n+1}) - R^2 \right] d^2$ and $d_i = d$. Using the Decomposition Theorem \ref{theo:one_FL_step}, we get:


\begin{align}
\E{\norm{\theta^{n+1} - \theta^*}^2} 
&= \E{ \norm{\theta^n - \theta^*}^2 }
- 2 \E{ \inner { \sum_{i} \frac{1}{M} \phi [\theta_i^* - \theta^{\rho_i(n)}] }{\theta^* - \theta^n} } \nonumber\\
&+ \sum_{i=1}^M\gamma \phi^2  \E{\norm{\theta_i^* - \theta^{\rho_i(n)}}^2} 
+ \phi^2 \E{\norm{\sum_{i=1}^{n} R d(\theta_i^* - \theta^{\rho_i(n)})}^2}
\\
&= \E{ \norm{\theta^n - \theta^*}^2 }
- 2 \phi \E{ \inner { \theta^* - \theta^{\rho(n)} }{\theta^* - \theta^n} } \nonumber\\
&+ \gamma \phi^2 \sum_{i=1}^M  \left[ \E{\norm{\theta_i^* - \theta^*}^2}  + \E{\norm{\theta^* - \theta^{\rho(n)}}^2}  \right] \nonumber\\
& + \phi^2 R^2 d^2 \left[ M\E{\norm{\theta^* - \theta^{\rho(n)}}^2} + M(M- 1) \E{\inner{\theta^* - \theta^{\rho(n)}}{\theta^* - \theta^{\rho'(n)}}} \right] 
\end{align}

We define $U_{u, v} = \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v}}}$. Hence, we have:
\begin{equation}
\E{\inner { \theta^* - \theta^{\rho(n)}}{\theta^* - \theta^{n}}}
= \sum_{k=0}^{n} q_{n, k}\E{\inner { \theta^* - \theta^{k}}{\theta^* - \theta^{n}}}
= \sum_{k=0}^{n} q_{n, k}U_{k, n}
\end{equation}
and 
\begin{equation}
	\E{\inner{\theta^* - \theta^{\rho(n)}}{\theta^* - \theta^{\rho'(n)}}} 
	= \sum_{s=0}^n \sum_{u=0}^n q_{n,s} q_{n, u} U_{s, u}
\end{equation}

We note that $U_{u,v}$ can be calculated with the following sequence:
\begin{align}
U_{u, v+1}
& =  \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v+1}}}\\
& =  \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v} - \sum_{ i = 1 }^M\omega_i^{v}\phi [\theta_i^* - \theta^{\rho(v)}]}}\\
& =  \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v}}}
-  \phi \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{\rho(v)}}}\\
& =  \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v}}}
-  \phi \sum_{s=0}^{v}q_{v , s}\E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{s}}}\\
& =  U_{u, v} 
-  \phi \sum_{s=0}^{v}q_{v , s}U_{u, s}
\end{align}

As a result, we have:
\begin{align}
\E{\norm{\theta^{n+1} - \theta^*}^2} 
&= \E{ \norm{\theta^n - \theta^*}^2 }
- 2 \phi \sum_{s=0}^{n}q_{n , s}U_{n, s}\nonumber\\
&+ \gamma \phi^2 \sum_{i=1}^M  \norm{\theta_i^* - \theta^*}^2  
+ \phi^2 \left[ \gamma  M + R^2 d^2 M\right] \sum_{s=0}^n q_{n , s} \E{\norm{\theta^* - \theta^s }^2}   \nonumber\\
& + \phi^2 R^2 d^2 M (M- 1) \sum_{s=0}^n \sum_{u=0}^n q_{n,s} q_{n, u} U_{s, u}
\end{align}







\subsection{Synchronous FL}

For Synchronous FL, we have $q_{n, n} =1 $ and $\forall k \neq n,\ q_{n, k} = 0 $. Hence, we can rewrite $A^{n+1} = ( 1- \phi)A^n$ and $B^{n+1} = ( 1 - \phi)B^n + \phi \theta^*$ which gives 
\begin{equation}
	\E{\theta^n - \theta^*} = ( 1- \phi)^n [\theta^0 - \theta^*]
	\label{eq:U_1}
%	\label(eq:U_1)
\end{equation} 

We also have $\mathbb{P}( T_i^n \le \Delta t^{n+1}) = \mathbb{P}( T_i \le \Delta t^{n+1}) = 1$ and $R = 1 $ giving $\gamma = 0$ and $d = 1/C$. As a result, we have:
\begin{align}
\E{\norm{\theta^{n+1} - \theta^*}^2} 
&= \E{ \norm{\theta^n - \theta^*}^2 }
- 2 \E{ \inner { \sum_{i} \frac{1}{M} \phi [\theta_i^* - \theta^n] }{\theta^* - \theta^n} } \nonumber\\
& + \phi^2 \E{\norm{\sum_{i=1}^{n} \frac{1}{M}(\theta_i^* - \theta^n)}^2} \\
&= ( 1 - \phi)^2\E{ \norm{\theta^n - \theta^*}^2 }
,
\end{align}
Considering the close from of the expectation, we have $\VAR{\theta^n - \theta^*} = 0$.







\subsection{Synchronous FL + Uniform sampling}

Similarly to Synchronous FL when considering all the clients, we still have $q_{n, n} =1 $ and $\forall k \neq n,\ q_{n, k} = 0 $. Hence equation (\ref{eq:U_1}) still holds for synchronous FL + uniform client sampling.

We define by $S_n$ the set of sampled clients at optimizations step $n$. With Uniform sampling, $m$ clients are sampled without replacement which gives $\mathbb{P}( T_i^n \le \Delta t^{n+1}) = \mathbb{P}( i \in S_n) = m / C$ and $R^2 = m(m-1)/M(C-1)$ implying $d= 1/m$ and $\gamma = [m/M- R^2]d^2$.

By structure, of $q_{n, s}$, we have $\sum_{s=0}^{n}q_{n , s}U_{u, s} = q_{n, n} U_{n, n} = \E{\norm{\theta^n - \theta^*}^2}$, and $\sum_{s=0}^n \sum_{u=0}^n q_{n,s} q_{n, u} U_{s, u} =  q_{n, n}^2 U_{n, n} = \E{\norm{\theta^n - \theta^*}^2}$


\begin{align}
\E{\norm{\theta^{n+1} - \theta^*}^2} 
&= (1 - 2 \phi + \phi^2 R^2 d^2 M^2+ \gamma \phi^2 M )\E{ \norm{\theta^n - \theta^*}^2 } 
+ \gamma \phi^2  \sum_{i=1}^M\E{\norm{\theta^*- \theta_i^*}^2}
\\
&= (1 - 2 \phi + \phi^2 )\E{ \norm{\theta^n - \theta^*}^2 } 
+ \gamma \phi^2  \sum_{i=1}^M\E{\norm{\theta_i^* - \theta^* }^2}
,
\end{align} 

We retrieve the case when considering all the clients as we have $ m = M$ and $\gamma = 0$. 




\subsection{Asynchronous FL}

For every $k > 0$, we have:
\begin{equation}
q_{n, k} 
= \mathbb{P}(\rho_i(n) = k) 
= \mathbb{P}(T_i >  \min_i T_i)^{n-k} \mathbb{P}(T_i =  \min_i T_i)
= \left[\frac{M-1}{M}\right]^{n-k}\frac{1}{M}
,
\end{equation}
and when $k=0$, we have:
\begin{equation}
q_{n, 0} 
= 1 - \sum_{k=1}^n q_{n, k}
= \left[\frac{M-1}{M}\right]^n
\end{equation}

We can use the formulation in equation (\ref{eq:U_2}) to express the expected global at every optimization step. Regarding the variance at every optimization step, we have $\mathbb{P}( T_i^n \le \Delta t^{n+1}) = 1/C$ and $R = 0$ implying $d= 1$ and $\gamma = 1/C$, which gives:
\begin{align}
\E{\norm{\theta^{n+1} - \theta^*}^2} 
&= \E{ \norm{\theta^n - \theta^*}^2 }
- 2 \phi \sum_{s=0}^{n} q_{n, s} U_{n, s} \nonumber\\
&+ \sum_{i=1}^M\frac{1}{M}  \phi^2  \norm{\theta_i^* - \theta^*}^2 
+ \phi^2  \sum_{ s = 0 }^n q_{n, s} \norm{\theta^s - \theta^* }^2 
\end{align}


%
%\begin{align}
%\E{\norm{\theta^{n+1} - \theta^*}^2} 
%&= \E{ \norm{\theta^n - \theta^*}^2 }
%- 2 \E{ \inner { \sum_{i} \frac{1}{M} \phi [\theta_i^* - \theta^{\rho_i(n)}] }{\theta^* - \theta^n} } \nonumber\\
%&+ \sum_{i=1}^M\frac{1}{M}  \phi^2  \E{\norm{\theta_i^* - \theta^{\rho_i(n)}}^2}\\
%&= \E{ \norm{\theta^n - \theta^*}^2 }
%- 2 \phi \E{\inner { \theta^* - \theta^{\rho(n)}}{\theta^* - \theta^n}}\nonumber\\
%&+ \sum_{i=1}^M\frac{1}{M}  \phi^2  \E{\norm{\theta_i^* - \theta^*}^2 + \norm{\theta^* - \theta^{\rho(n)}}^2+ 2 \inner{\theta_i^* - \theta^*}{\theta^* - \theta^{\rho(n)}} }\\
%&= \E{ \norm{\theta^n - \theta^*}^2 }
%- 2 \phi \E{\inner { \theta^* - \theta^{\rho(n)}}{\theta^* - \theta^n}}\nonumber\\
%&+ \sum_{i=1}^M\frac{1}{M}  \phi^2  \left[ \norm{\theta_i^* - \theta^*}^2 + \sum_{ k = 0 }^n q_{n, k} \norm{\theta^* - \theta^k}^2 \right]\\
%&= \E{ \norm{\theta^n - \theta^*}^2 }
%- 2 \phi \E{\inner { \theta^* - \theta^{\rho(n)}}{\theta^* - \theta^n}}\nonumber\\
%&+ \sum_{i=1}^M\frac{1}{M}  \phi^2  \norm{\theta_i^* - \theta^*}^2 
%+ \phi^2  \sum_{ k = 0 }^n q_{n, k} \norm{\theta^* - \theta^k}^2 \\
%\end{align}
%
%We define $U_{u, v} = \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v}}}$. We have:
%\begin{align}
%U_{u, v+1}
%& =  \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v+1}}}\\
%& =  \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v} - \sum_{ i = 1 }^M\omega_i^{v}\phi [\theta_i^* - \theta^{\rho(v)}]}}\\
%& =  \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v}}}
%-  \phi \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{\rho(v)}}}\\
%& =  \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v}}}
%-  \phi \sum_{s=0}^{v}q_{v , s}\E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{s}}}\\
%& =  U_{u, v} 
%-  \phi \sum_{s=0}^{v}q_{v , s}U_{u, s}
%\end{align}
%
%
%Hence, we have:
%\begin{align}
%\E{\inner { \theta^* - \theta^{\rho(n)}}{\theta^* - \theta^{n}}}
%& = \sum_{k=0}^{n} q_{n, k}\E{\inner { \theta^* - \theta^{k}}{\theta^* - \theta^{n}}}\\
%& = \sum_{k=0}^{n} q_{n, k}U_{k, n}
%\end{align}
%






\subsection{Hybrid FL}
When $k>0$, we have:
\begin{align}
q_{n, k} 
&= \mathbb{P}(\rho_i(n) = k) \\
&= \mathbb{P}(T_i  \le  (n -k+1) T) - \mathbb{P}(T_i  \le  (n -k) T)\\
& = ( 1 - e^{-(n-k+1)T}) -  ( 1 - e^{-(n-k )T} ) \\
& =  e^{-(n-k )T } - e^{-(n-k+1)T}
,
\end{align}
and when $k =0$, we have:
\begin{equation}
q_{n, 0} 
= 1 - \sum_{k=1}^n q_{n, k}
= 1 - \sum_{k=1}^n \left[ e^{-(n-k )T } - e^{-(n-k+1)T} \right]
= 1 - \left[e^{-(n-n )T } - e^{-nT} \right]
= e^{-nT} 
\end{equation}



We have $\mathbb{P}( T_i^n \le T) = \mathbb{P}( T_i \le T) =1 - e^{-T}$, which also gives by independence of the clients computation time $R = 1 - e^{-T}$. Thus, we have $\gamma = R ( 1- R) d^2$ with $d = 1 /RC$. Hence, $\gamma = e^{-T}/ ( 1 - e^{-T})M^2$. Hence for $T$ big enough, hybrid FL behaves similarly to Synchronous FL.
\begin{align}
\E{\norm{\theta^{n+1} - \theta^*}^2} 
&= \E{ \norm{\theta^n - \theta^*}^2 }
- 2 \phi \sum_{s=0}^{n}q_{n , s}U_{n, s}\nonumber\\
&+ \gamma \phi^2 \sum_{i=1}^M  \norm{\theta_i^* - \theta^*}^2  
+ \phi^2 \frac{1}{M} \frac{1}{1 - e^{-T}}\sum_{s=0}^n q_{n , s} \E{\norm{\theta^* - \theta^s }^2}   \nonumber\\
& + \phi^2 \frac{M-1}{M} \sum_{s=0}^n \sum_{u=0}^n q_{n,s} q_{n, u} U_{s, u}
\end{align}


\subsection{Hybrid  Evo FL}
When $k>0$, we have:
\begin{align}
q_{n, k} 
&= \mathbb{P}(\rho_i(n) = k) \\
&= \mathbb{P}(T_i  \le  T^{n+1} - T^k) - \mathbb{P}(T_i  \le  T^{n+1} - T^{k+1})\\
& = ( 1 - e^{-(T^{n+1} - T^k)}) -  ( 1 - e^{-(T^{n+1} - T^{k+1})} ) \\
& =  e^{-(T^{n+1} - T^{k+1}) } - e^{-(T^{n+1} - T^k)}
,
\end{align}
and when $k =0$, we have:
\begin{equation}
q_{n, 0} 
= 1 - \sum_{k=1}^n q_{n, k}
= e^{-T^{n+1}} 
\end{equation}



%
%
%
%\begin{align}
%\E{\norm{\theta^{n+1} - \theta^*}^2} 
%&= \E{ \norm{\theta^n - \theta^*}^2 }
%- 2 \phi \E{ \inner {  \theta^* - \theta^{\rho(n)} }{\theta^* - \theta^n} } \nonumber\\
%&+ \gamma \phi^2  \sum_{i=1}^M \E{\norm{\theta_i^* - \theta^{\rho_i(n)}}^2}\nonumber\\
%&+ \phi^2 R^2 d^2 \E{\norm{\sum_{i=1}^{M} (\theta_i^* - \theta^{\rho_i(n)})}^2}
%\\
%&= \E{ \norm{\theta^n - \theta^*}^2 }
%- 2 \phi \E{ \inner {  \theta^* - \theta^{\rho(n)} }{\theta^* - \theta^n} } \nonumber\\
%&+ \gamma \phi^2  \left[ \sum_{i=1}^M  \E{\norm{\theta_i^* - \theta^*}}^2 + C\E{\norm{\theta^* - \theta^{\rho(n)}}^2} \right] \nonumber\\
%&+ \phi^2 R^2 d^2 \left[ M\E{\norm{ \theta^* - \theta^{\rho(n)}}^2} + C(C-1) \E{\inner{\theta^* - \theta^{\rho_i(n)}}{\theta^* - \theta^{\rho_j(n)}} }\right]
%,
%\end{align}
%
%
%We have:
%\begin{align}
%	\E{\inner{\theta^* - \theta^{\rho_i(n)}}{\theta^* - \theta^{\rho_j(n)}}}
%	&= \sum_{s=0}^{n} \sum_{u=0}^{n} \mathbb{P}( \rho_i(n) = s)\mathbb{P}( \rho_j(n) = u) \E{\inner{\theta^* - \theta^u}{\theta^* - \theta^v}}
%	\\
%	&= \sum_{s=0}^{n} \sum_{u=0}^{n} q_{n , s} q_{n , u} U_{s, u}
%	\\
%\end{align}
%which gives
%\begin{align}
%\E{\norm{\theta^{n+1} - \theta^*}^2} 
%&= \E{ \norm{\theta^n - \theta^*}^2 }
%- 2 \phi \sum_{s=0}^{n} q_{n , s} U_{n, s} \nonumber\\
%&+ \phi^2 R^2 d^2 \left[ M\sum_{s=0}^{n} q_{n , s} \E{\norm{ \theta^s - \theta^*}^2} + C(C-1)\sum_{s=0}^{n} \sum_{u=0}^{n} q_{n , s} q_{n , u} U_{s, u}\right]
%,
%\end{align}
%


\subsection{Computation Time}

With synchronous FL, we have:
\begin{equation}
	\E{\Delta t^{n}}
	= \E{\max_i{T_i}}
	= \sum_{ k = 0 }^{M-1} \frac{1}{(M - k)\lambda}
\end{equation}
When combining synchronous FL with sampling uniformly $m$ clients, we get:
\begin{equation}
\E{\Delta t^{n}}
= \sum_{ k = 0 }^{m-1} \frac{1}{(m - k)\lambda}
\end{equation}
When sampling client asynchronously, an optimization step time is the one for a client to perform its local given that all the clients are performing their local work.
\begin{equation}
\E{\Delta t^{n}}
= \E{\min_i{T_i}}
= \frac{1}{M \lambda}
\end{equation}









==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/related_work.tex <==
%\section{Related Work}
%\label{sec:related}
%
%\begin{definition}[Unbiased Sampling]\label{def:sampling} 
%	A client sampling scheme is said unbiased if the expected value of the client aggregation is equal to the global deterministic aggregation obtained when considering all the clients, i.e.
%	\begin{equation}
%	\EE{S_t}{\vtheta^t}
%	=
%	\EE{S_t}{\sum_{j \in S_t}w_j(S_t)\vtheta_j^t}
%	\coloneqq
%	\sum_{i =1 }^n p_i\vtheta_i^t ,
%	\end{equation}
%	where $w_j(S_t)$ is the aggregation weight of client $j$ for subset of clients $S_t$.
%\end{definition}






%\subsection{FL convergence with MD client sampling}
%
%Theoretical guarantees regarding the convergence of FedAvg were given in \cite{FedNova}. The proof relies on assumptions classically used in Stochastic Gradient Descent (SGD) analysis \cite{Bottou2018} (Assumptions \ref{ass:smoothness} and \ref{ass:unbiased} below), or commonly used in the federated optimization literature \cite{FedProx, ontheconvergence, Haddadpour2019, SCAFFOLD, MATCHA} to capture the dissimilarities of local objectives (Assumption \ref{ass:dissimilarity} below). 
%
%%\cite{FedNova} also proves that to avoid inducing bias in the trained model, when sampled every client needs to perform the same amount of Stochastic Gradient Descent (SGD) $N$ with an SGD optimizer. Clients, when participating at an iteration, performs therefore $N$ SGD with and SGD optimizer.
%
%%The authors assume the following 3 assumptions regarding each client's local loss function $\Lcal_i$. Using Assumptions \ref{ass:smoothness} to \ref{ass:dissimilarity}, \cite{FedNova} gives an upper bound on the gradient of the global loss function $\Lcal$ at the end of the FL process when considering all the clients and when sampling $m$ clients using FedProx sampling scheme. The theorem for the later result is given in Theorem \ref{theo:convergence_FP}.
%
%\begin{assumption}[Smoothness]\label{ass:smoothness}
%	The clients local objective function is Lipschitz smooth, that is, $\norm{\nabla \Lcal_i(x) - \nabla \Lcal_i(y)} \le L \norm{x - y}, \forall i \in \{1, ..., n\}$.
%\end{assumption}
%
%\begin{assumption}[Unbiased Gradient and Bounded Variance]\label{ass:unbiased}
%	For each client $i$ local model, the stochastic gradient $g_i(x|\xi)$ of model $x$ evaluated on batch $\xi$ is an unbiased estimator of the local gradient: $\EE{\xi}{g_i(x|\xi)} = \nabla \Lcal_i(x)$, and has bounded variance $\EE{\xi}{\norm{g_i(x|\xi) - \nabla \Lcal_i(x)}} \le \sigma^2, \forall i \in \{1,..., n\}$ with $\sigma^2\ge 0$.
%\end{assumption}
%
%\begin{assumption}[Bounded Dissimilarity]\label{ass:dissimilarity}
%	For any set of weights $\{ w_i\le 0\}_{i=1}^n$ such that $\sum_{i=1}^{n}w_i =1$, there exists constants $\beta^2\ge 1$ and $\kappa^2 \ge 0$ such that $\sum_{i=1}^{m}w_i \norm{\nabla \Lcal_i(x)}^2 \le \beta^2 \norm{\sum_{i=1}^{m}w_i \nabla \Lcal_i(x)}^2 + \kappa^2$. If all the local loss functions are identical, then we have $\beta^2 =1$ and $\kappa^2 =0$. 
%\end{assumption}
%
%The following theorem was proven in \cite{FedNova} and provides theoretical guarantees for MD client sampling.
%
%\begin{theorem}\label{theo:convergence_FP}
%	Under Assumptions \ref{ass:smoothness} to \ref{ass:dissimilarity}, and local learning rate $\eta = \sqrt{m/NT}$, 
%	FL with $FedAvg$ when sampling $m$ clients with MD
%	converges to a stationary point of $\Lcal(\vtheta)$:
%	\begin{equation}
%		\frac{1}{T}\sum_{t=0}^{T}\E{\norm{\nabla \Lcal(\vtheta^t)}^2}
%		\le \Ocal(\frac{1}{\sqrt{mNT}}) + \Ocal(\frac{mN}{T}).
%	\end{equation}
%\end{theorem}
%The proof of Theorem \ref{theo:convergence_FP} can be found in \cite{FedNova} and shows that considering a subset of workers with MD client sampling is enough to ensure convergence of the global model to a local minimum of the federated loss function, equation (\ref{eq:global_loss}). 
%
%Following the conclusions of this work, to avoid optimizing a surrogate loss function instead of the federated one in equation (\ref{eq:global_loss}), the server asks from every client to compute the same amount of SGD steps $N$. 
%
%%However, clients need to be sampled such that the expected aggregation is equal to the aggregation with all the workers considered. At iteration $t$, we denote by $S_t$ the $m$ sampled workers, by $\vtheta_i^t$ the updated model of worker $i$ , and by $\omega_i(S_t)$ the weight given to worker $i$ for the aggregation. The expected aggregation must then follow


%\subsection{Sampling schemes comparison}
%
%Other client sampling schemes have been proposed. For example, with \cite{ontheconvergence}, the server sends the global model to every client before creating the new global model out of the first $m$ updated models the server receives; with \cite{Richtarik_optimal_sampling}, the server waits for every client to send the norm of their work before selecting the $m$ clients with the most relevant updates; with \cite{sampling_mobile_edge}, clients transmit information about their available computation resources before the server selects $m$ of them in function of their availability. Contrarily to FedAvg and MD sampling, these sampling schemes require additional communications and sometimes even computation from all the clients. On the contrary, FedAvg and MD sampling have the appealing property of maintaining to a minimum the amount of clients-server communications at each iteration. The global model is sent only to the sampled clients, and the amount of local work is set for those clients to only $N$ SGD updates. 
%To the best of our knowledge, FedAvg and MD sampling schemes are the only approaches minimizing the effective work and communications asked to the clients.
%Moreover, while FedAvg sampling has no theoretical guarantees regarding its convergence, neither regarding the unbiasedness of its global model, MD sampling is shown to converge to a stationary point of the global loss function (\ref{eq:global_loss}) (Theorem \ref{theo:convergence_FP}).  Based on these considerations and given that \cite{ontheconvergence} shows experimentally that MD sampling outperforms FedAvg, in the rest of this work we consider MD sampling as reference sampling technique.


%\section{Introduction}
%
%
%Federated learning is a training paradigm that has gained popularity in the last years as it enables different clients to jointly learn a global model without sharing their respective data. Federated training schemes based on model averaging of clients contributions are the most common, among which FedAvg (\cite{FedAvg}) is the most popular. 
%
%First, we begin by defining the stochastic distributed prediction problem. Suppose that we have $M$ participants and for each participant observe $n_i$ inputs $\{\vz_{k, i}\}_{k=1}^{n_i}$ independently sampled from a fixed unknown distribution over a sample space $\mathcal{Z}_i$. Models are defined by a set of parameters $\vtheta$ which are learnt based on the clients training data quantified on loss $l(\vtheta, \vz_{k, i})$. This formalization accounts both for supervised learning with $\vz_{k, i} = (\vx_{k, i}, \vy_{k, i})$ where $\vx_{k, i}$ is regarded as the input of the statistical model and $\vy_{k, i}$ is desired output, and unsupervised learning with $\vz_{k, i} = \vx_{k, i}$. We aim at building a statistical model providing the smallest averaged loss of the clients data points defined as
%\begin{equation}
%\label{eq:original_problem}
%\Lcal(\vtheta) 
%\coloneqq \frac{1}{\sum_{i=1}^M n_i}\sum_{i=1}^M \sum_{k=1}^{n_i} l(\vtheta, \vz_{k, i})
%.
%\end{equation}
%
%We note that every stochastic distributed prediction problem aims at minimizing a loss function $\Lcal$ that can be expressed as in equation (\ref{eq:original_problem}). The focus of this work is on applications for federated learning. More precisely, participants, called clients, communicate with a server orchestrating the learning process, and never share their data with the server and the other clients. We concentrate in the rest of this work on FedAvg (\cite{FedAvg}), the most popular federated learning approach to solving the problem in equation (\ref{eq:original_problem}) while respecting the constraints discussed before. At every optimization step, each client performs in parallel a fix amount of stochastic gradient descents (SGD) on the current global model before sending back the resulting model to the server. Once in possession of all the clients contributions, the server creates the new global model as the weighted mean of the clients updates based on their data ratio. 
%
%Speak about security and the amount of average is important for that.
%
%
%Federated learning is a generalization of distributed learning which was first introduced for statistical inference with a star-shape network composed of a server communicating with computation machines. The server owns the dataset and splits it among the machines. At every optimization round, machines send gradient estimated on the current global model and their data to the server that using the machines' gradients to perform a gradient descent (GD). Distributed learning was later extended to account for SGD and more local computation like federated learning. The main optimization difference between federated and distributed learning lies in their data distributions respectively non-iid and iid. Therefore, proving FedAvg convergence was more challenging and done in [XX]. In some settings, FedAvg is also shown to converge to a sub-optimum, e.g. when each client performs a different amount of local work \citep{FedNova}, or when clients are not sampled in expectation according to their importance \citep{PowerOfChoice}.
%
%A major drawback behind FedAvg is the time needed for the server to create two consecutive global models. The server has to wait for all the clients to perform their local work to \textit{synchronize} their update and create a new global model.
%Therefore, the time for an optimization step is conditioned on the one of the slowest client. Also, the fastest clients are idle once they have sent their updates to the server. In addition of having heterogeneous data distributions $\mathcal{Z}_i$, clients have heterogeneous hardware which can translate in major FL slow-down. Considering a subset of clients at every optimization step is shown to provide faster optimization rounds and in turn faster FL \citep{OnTheConvergence}. However, client sampling increases clients idle time and thus does not take full advantage of the clients computation power either.
%
%We propose in this work to consider an asynchronous version of FedAvg. The server creates a new global model whenever a client send its local work and send this model to this client. As a result, clients are never idle and each perform their local work on a different global model. Similarly to the synchronous case, asynchronous distributed learning has already been investigated in [XX]. We position our work as an extension of asynchronous distributed learning. To the best of our knowledge, asynchronous FedAvg for non-iid data distributions has also been investigated in [XX]. We introduce a new theoretical convergence framework for averaging aggregation schemes with which we can prove synchronous FedAvg convergence. We also show that in most FL applications asynchronous FL applications do not converge to their optimum. Finally, we propose instead to consider fixed period of time at which the server aggregates 
%
%
%Our paper is structured as follow...
%
%
%
%What happens when the amount fo local work is increased to more than one SGD ?
%
%What happens when clients do not result from the same data distribution ?
%
%
%%By eliminating the required coordination overhead, asynchronous operations become simultaneously more appealing (in physically clustered systems) and more scalable (in massively parallel and volunteer computing grids).
%%
%%Distributed asynchronous stochastic gradient descent is one of the most widely deployed methods for training large-scale machine learning models. More concretely, there are two types of distributed computing architectures that are common in practice,: the first is a shared-memory multi-core/multi-GPU cluster where different processors independently compute stochastic gradients and update a global model parameter using a hared memory. The second is a "master-slave" architecture where each worker independently computes a stochastic gradient of the objective; these gradients are sent asynchronously to the master as they become available. 
%
%
%
%
%
%
%
%
%%\subsection{Original Problem}
%%We consider the following distributed optimization problem:
%%\begin{equation}
%%\label{eq:original_problem}
%%\Lcal(\vtheta) = \sum_{i=1}^{C}p_i \Lcal_i(\vtheta)
%%\end{equation}












==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/review_papers.tex <==
\section{Background}

asynchronous DL convergence \cite{DistributedDelayed}
\cite{OptimalDistributedOnline} \cite{SlowLearnersAreFast}
\cite{AsyncParallelSGDforNonconvex} 

experimental asynchrnous FL \cite{RevisitingDistributedSynchronousSGD} \cite{EfficientAndRobust} 
\cite{PrivacyPreservingAsynchronous}
\cite{HowSlowCanYouGo}

asynchronous FL \cite{ErrorFeedbackFramework}

FedBuff \cite{RevisitingDistributedSynchronousSGD} 
\cite{FedBuff}

Heterogeneous amount of local work \cite{AsynchronousFOpti}




For in-depth discussion of SGD and its application in machine learning, we refer to the book of \cite{BottouBookSGD}. For in-depth discussion of Federated Learning please refer to \cite{OpenProblems} and for in depth discussion of Asynchronous FL please refer to \cite{AFLsurvey}. 

\cite{DistributedDelayed} about asynchronous distributed learning. This work is theoretical and assumes convex functions with updates using projected gradients and a primal/dual optimization approach. The learning rate considered is decreasing. The authors show that asynchronicity can speed-up convergence: theoretically with a $1/m$ ratio and experimentally. 

\cite{DataDependent} about distributed learning. The authors consider the problem of distributed learning for a network where clients can communicate between each other. Authors show that the resulting convergence bound is proportional to the eigen value of the matrix for this network. Data is assumed to be iid and shared among the clients/processors by the server.

\cite{RevisitingDistributedSynchronousSGD} about asynchronous FL. This work is experimental. The server asks to more than $m$ clients to perform their local work and creates the new global model with the first $m$ clients updating their contribution. This setup is identical to the one considered for client sampling in \cite{OnTheConvergence}.

\cite{TowardsAsynchronousFL} about clients performing different amount of local work $K_i$. 
At fixed clock times, clients share with the server their communication capabilities and the amount of SGD conducted on their local work. The server uses these information to optimally select a subset of clients used for aggregation. These clients receive the new global model while other clients keep performing local work on their current local model.
No theoretical work is conducted. The asynchronicity comes from the heterogeneous amount of local work in clients considered for aggregation. 

\cite{EfficientAndRobust} about asynchronous FL. The authors make an interesting assumption about the gradients enabling consideration of unbiased gradients. The underlying idea is to tailor the amount fo local work a client should perform in function of its data difference with other clients and its communication and computation capabilities. While theoretical and experimental proof are provided, I do not trust the theoretical derivation in this work. Especially assumptions are pretty strong and results in this work goes against the one in \cite{FedNova}. 
THIS WORK SHOULD BE COMPARED TO OURS AS CONVERGENCE PROOF TO OPTIMUM IS PROVIDED.

\cite{OptimalDistributedOnline} about distributed learning. Interesting article published at JMLR. The notion of regret is interesting as convergence to the optimum in that case reduces to a null regret. A star shape network is assumed with $M$ processors. Clients data distributions are assumed to be identical and partitioned by the server. The local optimization is based on projected gradients. POTENTIAL COMPARISON WITH OUR BOUND ? Definition of the difference between online and optimization.

\cite{TamingTheWild} about asynchronous DL. Speaks about the worst case expected delay. Very interesting work based on submartingales. Authors provide an upper bound on the probability an algorithm has performed its work in $N$ optimization rounds in function of the desired residual $\epsilon$ and learning parameters. We note that this method required to bound the gradients.

\cite{FedBuff} Introduces a new asynchronous FL algorithm \textsc{FedBuff}. The server waits for $m$ clients to perform their local update before considering clients contribution for aggregation. The server sends the new model to these clients.
Author have strong assumptions (bounded gradients, bounded dissimilarity) but do not assume convexity. COMPARE OUR CONVERGENCE BOUNDS.

\cite{ParallelizingSGD} about SGD for least square. Published at JMLR. Different parallelization methods are proposed to have faster SGD for this kind of problems. Not directly applicable to DL or FL. 

\cite{SlowLearnersAreFast} about asynchronous DL. This work is very similar to ours and prove the convergence of a sequence of optimizations schemes.
Authors consider convex loss functions, bound the distance between two consecutive models $\norm{\vtheta^{n+1} -\vtheta^n}^2 \le D^2$ and bound the gradient norms.
However, it seems that the bound in Theorem 2 cannot help draw any conclusion. Indeed, the lower bound cannot be 0 and a residual like the one in Theorem \ref{theo:convergence_convex} needs to appear to prove convergence. 
Also, authors restrict themselves to the asynchronous case where clients send their update with fixed delay $\tau = M - 1 $.
COMPARE THEIR CONVERGENCE RATE TO OURS.

\cite{AsyncParallelSGDforNonconvex} about asynchronous DL. Clients have identical data distributions but no assumption convexity are made. The second part of this work is on a lock free approach which does not seem to hold and be relevant for this work. 
COMPARE THEIR LEARNING RATE AND CONVERGENCE BOUND WITH OURS.

\cite{ADPSGD} for asynchronous decentralized DL. The work does not consider a star shape network with theoretical guarantees.

\cite{PrivacyPreservingAsynchronous} for asynchronous FL. No theoretical work and only experiments are provided. The considered experimental scenario consider few clients (3 for MNIST) and data partitioning is iid.

\cite{Hogwild} for lock free DL. $M$ processors have access to the same dataset. 

\cite{DynamicFL} for FL. Clients are sample according to a MD distribution and asked to perform their local work according to client specific hyperparameters. Proofs for their theorem is not provided. 

\cite{Samarakoon2019} for (asynchronous) FL. This work is around optimization of communications based on Lyapunov equations but without proving FL convergence to its optimum. A synchronous and asynchronous version of their algorithm is available.

\cite{ErrorFeedbackFramework} for (asynchronous) FL. The authors make the same assumptions as us while also proving convergence for non convex functions. However, authors assume iid data distributions. Authors also introduce the notion of compressors. The delay scenario considered is $\tau = M$.

\cite{WhenEdgeMeetsLearning} for FL. Authors propose an optimization method to choose the appropriate amount of local SGD $K$ to perform for a given amount $N$ of optimization rounds. Theoretical convergence provided assuming a bounded gradient divergence and convex local loss functions.

\cite{IsLocalSGD} for FL. Authors show that for quadratic loss functions, $K>1$ is better than $K=1$. They also show that local work sometimes improve convergence for convex functions and the other way around. Clients data distributions are assumed iid (dataset split among clients).

\cite{AsynchronousFOpti} for asynchronous FL. Authors propose a weighting scheme to account properly for clients updates in function of a function they design proportional to an hyperparameter and clients staleness. Clients perform heterogeneous amount of local work $K$. Theoretical work is proposed for weakly convex functions but with bounded gradients and assumptions not easy to verify.

\cite{ParallelSGDWhenDoesAveragingHelp} for FL. Impact of $K$ on FL convergence. Authors propose theoretical considerations around simple convex functions and non conclusive experiments are given.

\cite{FedPD} for FL.
Answers questions on the impact of FL assumptions, local work and aggregation on FL convergence. The theoretical part is informal and either based on simple functions or with informal theory. Clear formalization of FL assumptions in introduction.

\cite{AsyncSGDwithDelay} for asynchronous DL. Authors propose a novel async-DL algorithm which they theoretically show improves async-DL. Their method aims at compensating the clients delay with a Taylor expansion of the gradient using Hessian Approximation. Computing the Hessian can be costly. Clients data is assumed centralized and then split among the participants.

\cite{Zhou2018} for FL. Theoretical proof of FL convergence in non convex settings. Clients data are assumed iid. Authors work is redundant with current work on FL with weaker assumptions and without citing any FL papers.
Unfair experimental comparison based on the amount of aggregations and not on the amount of time needed for training.

\cite{HowSlowCanYouGo} for asynchronous DL. Assumptions are made on the shape of the delay $\tau$. Delays $\tau$ are paired with learning rate structures $\eta_l$. Theoretical convergence is proven without providing convergence bound and thus convergence rate. Nice paragraph citing a lot of papers in the introduction about asynchronous DL.  






\cite{AFLsurvey} Survey on AFL with more than 50 papers. Most of them are experimental papers. Describe the potential ongoing work for AFL: Node selection, weighted aggregation, gradient compression, semi-asynchronous, cluster FL, model split.

\cite{FLUnderArbitraryCommPatterns} Identical convergence speed for their asynchronous algorithm and synchronous FL. The authors assume that clients perform their local work with the same amount of time. The asynchronicity only comes from the communication time which helps the server to know how many local work has been done. Theoretical justification for non convex and Lipschitz smooth loss functions is provided. After T server aggregations, every client has performed T optimization steps which prevents bias.

\cite{GraphOracleModels} The answering delay is assumed to be fixed.

\cite{stich2018local} Proposed optimization problem by bounding the clients gradient dissimilarity. A synchronous and asynchronous framework are proposed while considering non-iid data distributions. 

\cite{Chen2021}

\cite{Wang2019adaptive}

\cite{Chen2018}

\cite{arjevani20a}



%%%
%FL with only experiments: \citep{PrivacyPreservingAsynchronous, Wang2019adaptive}(few clients + iid), \cite{Samarakoon2019}
%
%FL with broken theory: \cite{Chen2021}(issues with assumption + proof), \cite{AsynchronousFOpti} (bounded gradients)
%
%Parallel SGD Star shape network: \citep{Chen2018, AsyncParallelSGDforNonconvex, AsyncSGDwithDelay} (iid data) \cite{stich2018local}(niid)
%
%Parallel SGD Star distributed network: \cite{ADPSGD} (niid data)
%
%ML with delayed gradients: \citep{ErrorFeedbackFramework, arjevani20a}
%
%FL papers using asynchronous or stragglers to speak about clients hardware constraints but keeping synchronization: \citep{FedProx, FedNova, DynamicFL} (accounting for different amount of local work), \citep{PrivacyPreservingAsynchronous, AsynchronousFOpti} (accounting for different local computation time)




==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/schematic.tex <==
\begin{figure}
	\begin{tikzpicture}
%	[scale = 0.7, line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm]
	
	%Global models
	\node[fill, draw, circle,label=above: $\theta^t$, minimum size = 3pt, inner sep =0] (A) at (0,0){} ;
	\node[fill, draw, circle,label=below: $\theta^{t+1}$, minimum size = 3pt, inner sep =0] (B) at (-7.5/4/2, -7.5/2/4){} ;
	
	%Connect the globsl models
	\draw [line width=1pt, ->] (A)-- (B);
	%	\draw [line width=1pt, ->] (B)-- (C);
	%	
	%Local optima and local update
	\node[fill, draw, circle,label=left: $\theta_1^*$, minimum size = 3pt, inner sep =0] (E) at (-0.5,-2.7){} ;
	\node[fill, draw, circle,label=below: $\theta_1^{t+1}$, minimum size = 3pt, inner sep =0] (F) at (-0.5/2,-2.7/2){} ;
	
	\node[fill, draw, circle,label=left: $\theta_2^*$, minimum size = 3pt, inner sep =0] (G) at (0.5,-3){} ;
	\node[fill, draw, circle,label=right: $\theta_2^{t+1}$, minimum size = 3pt, inner sep =0] (H) at (0.5/2,-3/2){} ;
	
	\node[fill, draw, circle,label=left: $\theta_3^*$, minimum size = 3pt, inner sep =0] (I) at (-3,0){} ;
	\node[fill, draw, circle,label=above: $\theta_3^{t+1}$, minimum size = 3pt, inner sep =0] (J) at (-3/2,-0/2){} ;
	
	\node[fill, draw, circle,label=below: $\theta_4^*$, minimum size = 3pt, inner sep =0] (K) at (-3.5, -0.5){} ;
	\node[fill, draw, circle,label=below: $\theta_4^{t+1}$, minimum size = 3pt, inner sep =0] (L) at (-3.5/2,-0.5/2){} ;
	
	%Connect the updates
	\draw [line width=0.5pt, ->] (A)-- (F);
	\draw [line width=0.5pt, dashed] (F)-- (E);
	
	\draw [line width=0.5pt, ->] (A)-- (H);
	\draw [line width=0.5pt, dashed] (H)-- (G);
	
	\draw [line width=0.5pt, ->] (A)-- (J);
	\draw [line width=0.5pt, dashed] (J)-- (I);
	
	\draw [line width=0.5pt, ->] (A)-- (L);
	\draw [line width=0.5pt, dashed] (L)-- (K);
	
	
	%\end{scriptsize}
	\end{tikzpicture}
	%	\hspace{1cm}
	\begin{tikzpicture}[scale = 0.7, line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm]
	
	%Global models
	\node[fill, draw, circle,label=above: $\theta^t$, minimum size = 3pt, inner sep =0] (A) at (0,0){} ;
	\node[fill, draw, circle,label=right: $\theta^{t+1}$, minimum size = 3pt, inner sep =0] (B) at (-2.5/2/2, -3/2/2){} ;
	\node[fill, draw, circle,label=below: $\theta^{t+2}$, minimum size = 3pt, inner sep =0] (C) at (-1.9, -1.6){} ;
	
	%Connect the globsl models
	\draw [line width=1pt, ->] (A)-- (B);
	\draw [line width=1pt, ->] (B)-- (C);
	%	
	%Local optima and local update
	\node[fill, draw, circle,label=left: $\theta_1^*$, minimum size = 3pt, inner sep =0] (E) at (-0.5,-2.7){} ;
	\node[fill, draw, circle,label=below: $\theta_1^{t+2}$, minimum size = 3pt, inner sep =0] (F) at (-0.55,-1.7){} ;
	
	\node[fill, draw, circle,label=left: $\theta_2^*$, minimum size = 3pt, inner sep =0] (G) at (0.5,-3){} ;
	\node[fill, draw, circle,label=right: $\theta_2^{t+1}$, minimum size = 3pt, inner sep =0] (H) at (0.5/2,-3/2){} ;
	
	\node[fill, draw, circle,label=left: $\theta_3^*$, minimum size = 3pt, inner sep =0] (I) at (-3,0){} ;
	\node[fill, draw, circle,label=above: $\theta_3^{t+1}$, minimum size = 3pt, inner sep =0] (J) at (-3/2,-0/2){} ;
	
	\node[fill, draw, circle,label=below: $\theta_4^*$, minimum size = 3pt, inner sep =0] (K) at (-3.5, -0.5){} ;
	\node[fill, draw, circle,label=below: $\theta_4^{t+2}$, minimum size = 3pt, inner sep =0] (L) at (-2.25,-0.62){} ;
	
	%Connect the updates
	\draw [line width=0.5pt, ->] (B)-- (F);
	\draw [line width=0.5pt, dashed] (F)-- (E);
	
	\draw [line width=0.5pt, ->] (A)-- (H);
	\draw [line width=0.5pt, dashed] (H)-- (G);
	
	\draw [line width=0.5pt, ->] (A)-- (J);
	\draw [line width=0.5pt, dashed] (J)-- (I);
	
	\draw [line width=0.5pt, ->] (B)-- (L);
	\draw [line width=0.5pt, dashed] (L)-- (K);
	
	\end{tikzpicture}
	
	\caption{Schematics illustrating the clients' similarities detection method when considering all the clients, left, and when sampling clients, right. $\theta^t$ is the global model at iteration $t$ and $\theta_i^{t+1}$ is the updated local model of client $i$ on $\theta^t$ while converging to its local optimum $\theta_i^*$.}
	\label{fig:schematic_sim}
\end{figure}

==> arXiv - A General Theory for Federated Optimization with Delayed Gradients and Heterogeneous Data/tex/specifications.tex <==
\subsection{Heterogeneity of clients hardware and data distributions}\label{subsec:specifications}

\textbf{Clients importance.}
%We provide $\epsilon$ for centralized learning, synchronous FL, asynchronous FL and hybrid FL in function of the amount of server aggregations $N$ and the amount of time $T$ elapsed since the beginning of the learning process.
We restrict our investigation to the case where clients have identical aggregation weights during the learning process, i.e. $d_i(n) = d_i$.  
We also consider identical client importance $p_i = 1/M$.
We can therefore define the averaged optimum residual $\Sigma$ defined as the average of the clients SGD evaluated on the global optimum, i.e.
\begin{equation}
	\Sigma
	\coloneqq
	\frac{1}{M} \sum_{ i = 1 }^M \EE{\vxi_i}{\norm{\nabla \Lcal_i(\vtheta^*, \vxi_i)}^2}
	.
\end{equation}
When clients have identical data distributions, $\Sigma$ can be simplified as $\Sigma = \EE{\vxi}{\norm{\nabla \Lcal(\vtheta^*, \vxi)}^2}$, and $\Sigma =0$ when clients perform GD. We note that in the DL and FL literature $\Sigma$ is often simplified by assuming bounded variance of the stochastic gradients, i.e. $\Sigma \le \sigma^2$, where $\sigma^2$ is the bounded variance of any client SG.

%We compare the theoretical bounds we obtain for these state-of-the-art optimization schemes with the state-of-the-art bounds obtained for each of these learning procedures. 
%Lastly, we consider the federated learning case where clients have heterogeneous data and perform $K>1$ SGD step. Our theory still works when assuming that clients have identical data, e.g. the server allocates data samples to clients, or perform $K=1$ SGD step, e.g. distributed learning, but we let the specific derivation to the reader.

\textbf{Clients computation time.} 
In the rest of this work, we consider that clients guarantee reliable computation and communication, although with heterogeneous hardware capabilities, i.e. $\exists \tau_i \in \mathbb{R},\text{ s.t. }T_i = \tau_i$.
Without loss of generality, we assume that clients are ordered by increasing $\tau_i$, i.e. $\tau_i \le \tau_{i+1}$, where the unit of $\tau_i$ is such that $\tau_i$ is an integer. 
In what follows, we provide the close form of $d_i$ for all the considered optimization schemes. This derivation still holds for applications where clients have unreliable hardware capabilities that can be modeled as an exponential distribution, i.e. $T_i \sim \exp(\tau_i^{-1})$ which gives $\E{T_i} = \tau_i$.

\textbf{Clients data distributions.}
Unless stated otherwise, we will consider the FL setting where each client has its unique data distribution. 
Therefore, clients have heterogeneous hardware and non-iid data distributions. 
The obtained results can be simplified for the DL setting where a dataset is made available to $M$ processors.
In this special case, clients have iid data distributions ($\Zcal_i = \Zcal_1$)
, and identical computation times ($\tau_i = \tau_1$, $W = M$, and $\tau = M-1$).

\textbf{Learning rates.} 
For sake of clarity, we ignore the server learning rate when expressing the convergence bounds $\epsilon$, i.e. $\eta_g = 1$. 
Also, we consider a local learning rate $\eta_l$ inversely proportional to the serial amount of SGD included in the global model, i.e. $\eta_l \propto 1 / \sqrt{KN}$, consistently with the rest of the distributed optimization literature.

We propose Table \ref{tab:summary_comparison} to summarize the close form or bounds of the different parameters used in Section \ref{sec:convergence}.

\begin{table}
	\begin{center}
		\begin{tabular}{ | c || c | c | c| }
			\hline
			& Sync. \textsc{FedAvg} 
			& Async. \textsc{FedAvg} 
			& \textsc{FedFix}\\
			\hline
			$d_i$   
			& $= p_i$ 
			& $= \left[\sum_{ i = 1 }^M \frac{1}{\tau_i}\right] \tau_i p_i$
			& $= \ceil{ \tau_i /\Delta t } p_i$
			\\
			$N$ 
			&   $T/\tau_M $
			& $\sum_{i=1}^M T/\tau_i $
            & $ T/\Delta t $
			\\
			$\Delta t$ 
			& = $\max T_i^n$ 
			& = $\min T_i^n$
			& = $\Delta t$
			\\
			$\alpha$ 
			& $1$ 
			& 0
			& 1
			\\
			$\beta$
			& 0 
			& $\max d_i \le \tau_m / \tau_0$
			& 0
			\\
			$\tau$ 
			& 0 
			& $\Omega(M)$, $\Ocal(M \tau_M / \tau_0)$
			& 0, $\floor{\tau_m / \tau_0}$
			\\
			$W$ 
			& 1 
			& $\Omega(M)$, $\Ocal(M (\tau_M)^M)$
			& 1, $M \ceil{\tau_m / \tau_0}^M$
			\\
			$R(\{\Lcal^n\})$ 
			& $= 0$
			& $= \frac{1}{M} \sum_{ i = 1 }^M \left[\Lcal_i(\vtheta^*) - \Lcal_i(\vtheta_i^*)\right]$
			& $\le \frac{1}{M} \sum_{ i = 1 }^M \left[\Lcal_i(\vtheta^*) - \Lcal_i(\vtheta_i^*)\right]$
			\\
			\hline
		\end{tabular}
	\end{center}

\caption{The different variables used to account for the importance of clients or data distributions at every optimization round and during the full FL process. For $\tau$ and $W$, we give two values which correspond to their respective lower and upper bound.}
\label{tab:summary_comparison}
\end{table}



% \begin{corollary}
% % \label{cor:simplification}
% 	Under Assumptions \ref{ass:smoothness} to \ref{ass:clients_covariance}, we obtain the following convergence bound:
% 	\begin{align}
% 	\epsilon
% 	&=
% 	\Ocal\left(\frac{1}{\sqrt{KN}}\left[\norm{\vtheta^{0} - \bar{\vtheta}}^2 + R(\{\Lcal^n\})\right]\right)
% 	+
% 	\Ocal \left(\frac{K\tau^2}{N} R(\{\Lcal^n\}) \right) 
%     + 
%     \Ocal \left( \frac{K-1}{N} \Sigma \right)
%     \nonumber\\
% 	&+
% 	\Ocal \left( \frac{1}{\sqrt{KN}} \left[ \alpha \Sigma_2 + \beta \Sigma_1\right] \right)
% 	+ 
% 	\Ocal \left( \frac{K}{N} \tau^2 \left[ \alpha \Sigma_2 + \beta \Sigma_1\right]\right)
% 	+
% 	\Ocal \left( \frac{\sqrt{K}}{\sqrt{N}} (W-1)\right)
% 	\end{align}
% 	with $\eta_g =1$ and $\eta_l \propto 1/ \sqrt{KN}$.

% \end{corollary}

% \begin{corollary}
% \label{cor:simplification}
% 	Under Assumptions \ref{ass:smoothness} to \ref{ass:clients_covariance}, we obtain the following convergence bound:
% 	\begin{align}
% 	\epsilon
% 	&=
% 	\Ocal\left(\frac{1}{\sqrt{KN}}\left[\norm{\vtheta^{0} - \bar{\vtheta}}^2 + R(\{\Lcal^n\})\right]\right)
%     +
% 	\Ocal \left( \frac{1}{\sqrt{KN}} \left[ \alpha \Sigma_2 + \beta \Sigma_1\right] \right)
% 	+ 
% 	\Ocal \left( \frac{\sqrt{K}}{\sqrt{N}} (W-1)\right)
% 	\end{align}
% 	with $\eta_g =1$ and $\eta_l \propto 1/ \sqrt{KN}$.

% \end{corollary}

% As discussed in Section \ref{sec:convergence}, when clients have identical data distributions, the sufficient conditions of Corollary \ref{cor:bias_distributions} are always satisfied. 
% In theory, in the heterogeneous case, these conditions can still be satisfied. If every client has a non-null probability to participate at a round, i.e.$\mathbb{P}( T_i^n \le \Delta t^n) >0$, there exists an appropriate $d_i(n)$ such that $\tilde{q}_i(n) = p_i$, equation (\refeq{eq:agg_weights}).
% Yet, in practice clients generally may not even know their update time distribution $\mathbb{P}( T_i^n)$ making the computation of $d_i(n)$ intractable. In what follows, we thus use Theorem \ref{theo:relaxed_sufficient_conditions} to obtain the close-form of $\epsilon$ which only requires from the server to know the clients time $\tau_i$.
% Providing convergence guarantees for distributed applications coupled with non-iid data distributions is of paramount importance. 

% Corollary \ref{cor:bias_distributions} shows that the knowledge of the clients computation time is not necessary to achieve convergence to the global optimum. Indeed, when clients have identical data distributions, at every optimization round the data distribution common to all the clients is properly represented regardless of the aggregation weights and stochastic computation time $T_i$ given to them. Therefore, the sufficient conditions of Corollary \ref{cor:bias_distributions} are always satisfied, and convergence to the global optimum is always ensured.

% In theory, when clients have non-iid data distributions, the sufficient conditions of Corollary \ref{cor:bias_distributions} can still be satisfied. If $\mathbb{P}( T_i^n \le \Delta t^n) >0$ for every client, there exists an appropriate $d_i(n)$ such that $\tilde{q}_i(n) = p_i$. 
% Yet, in practice clients generally may not even know their update time distribution $\mathbb{P}( T_i^n)$ making the computation of $d_i(n)$ intractable. 
% Providing convergence guarantees for distributed applications coupled with non-iid data distributions is of paramount importance. 

%\textbf{non-iid data distributions by default.} 
% Unless stated otherwise, we will consider the FL setting where clients have their unique data distribution. Therefore, clients have heterogeneous hardware and non-iid data distributions. The obtained results can be simplified for the DL setting where a dataset is made available to $M$ processors.
% In this special case, clients have iid data distributions ($\Zcal_i = \Zcal_1$ and $W=1$), identical computation times ($\tau_i = \tau_1$), and negligible communication times ($K=1$).

==> delayed_proofs/Calculus_applications.tex <==
\section{Calculus Applications}\label{app:sec:calculus_applications}

We assume that $\tau$, $W$, $\nu$, $\beta$ are independent from $N$, and $K \ll N$, $M \ll N$

\begin{align}
\epsilon_{F}
= \Ocal\left(\frac{\sqrt{W}}{\sqrt{K N}}\right)
+ \Ocal \left( \frac{1}{W N } \sigma^2 \right)
,
\end{align}

\begin{align}
\epsilon_{opt}
&= \Ocal\left(\frac{1}{\sqrt{WKN}} \nu \sigma^2 \right)
+ \Ocal \left(\frac{(\tau +  1)  \tau}{WN } \nu \sigma^2 \right)
+ \Ocal\left(\frac{\sqrt{K}}{W^{3/2}N^{3/2}}  \beta   \sigma^2 \right)
\nonumber\\
&+ \Ocal \left( \frac{\tau}{WN} \sigma^2 \right)
+ \Ocal \left(\beta \frac{K(\tau+1)\tau}{W^2N^2 }\sigma^2 \right)
\\
&= \Ocal\left(\frac{1}{\sqrt{WKN}} \nu \sigma^2 \right)
,
\end{align}
\begin{align}
\epsilon_H
= \Ocal\left(\frac{\sqrt{K}}{\sqrt{WN}} \right)
+ \Ocal \left( \frac{\tau}{WN} K \right)
+ \Ocal \left((\tau +  1) \frac{\tau}{WN} K \right)
= \Ocal\left(\frac{\sqrt{K}}{\sqrt{WN}} \right)
%+ \Ocal \left( \frac{\tau}{WN} K \right)
%+ \Ocal \left((\tau +  1) \frac{\tau}{WN} K \right)
,
\end{align}
\begin{equation}
\nu 
= \frac{1}{N}\sum_{ n = 0 }^{N-1} \sum_{i=1}^M \mathbb{P}( T_i^n \le \Delta t^n ) d_i^2(n) 
,
\end{equation}
and
\begin{equation}
\beta = \nu + \frac{1}{N}\sum_{ n = 0 }^{N-1}
\left[
\left[\sum_{i=1}^M  R_i(n) d_i(n)\right]^2
- \sum_{i=1}^M R_i^2(n) d_i^2(n)
\right]
.
\end{equation}




\begin{equation}
	\epsilon_W = \Ocal( \frac{\sqrt{K (W-1)}}{\sqrt{N}})
\end{equation}

As a result, we have 

\begin{align}
\epsilon_{iid}
= \Ocal \left(\frac{1}{\sqrt{KN}}\right)
%+ \Ocal\left(\frac{\sqrt{K(W-1)}}{\sqrt{N}}\right)
+ \Ocal\left(\frac{1}{\sqrt{KN}} \nu \sigma^2 \right)
\end{align}

\begin{align}
	\epsilon_{non-iid}
	= \Ocal \left(\frac{\sqrt{K}}{\sqrt{WN}}\right)
	+ \Ocal\left(\frac{\sqrt{K(W-1)}}{\sqrt{N}}\right)
	+ \Ocal\left(\frac{1}{\sqrt{WKN}} \nu \sigma^2 \right)
\end{align}


\subsection{Synchronous FL: naive FedAvg}





\begin{equation}
\nu 
= \sum_{i=1}^M p_i^2
,
\end{equation}
and
%\begin{equation}
%\beta = \sum_{i=1}^M p_i^2 + 
%\left[ 1 - \sum_{i=1}^M p_i^2
%\right] =1 
%.
%\end{equation}
$W=1$, $\tau = 0$.

Hence, we have
\begin{align}
\epsilon
= \Ocal \left(\frac{\sqrt{K}}{\sqrt{WN}}\right)
+ \Ocal\left(\frac{\sqrt{K(W-1)}}{\sqrt{N}}\right)
+ \Ocal\left(\frac{1}{\sqrt{WKN}} \nu \sigma^2 \right)
\end{align}



\subsection{Synchronous FL : sampling with windows}




==> delayed_proofs/app_bias_bound_2.tex <==
\section{Include Bias in the error bound}

\begin{lemma} \label{lem:async_FL_bias}
%	For any model parameters $\theta$, the difference between the gradients of $\Lcal(\theta)$ and $\tilde{\Lcal}(\theta)$ can be bounded as follow:
	\begin{align}
	\norm{\nabla \Lcal(\theta) - \nabla \Lcal^n (\theta)}^2
	\le 2 \chi^n \norm{\nabla \Lcal^n (\theta)}^2 
+ 2  \norm{ \sum_{j \notin W_n} r_j  \nabla \Lcal_j(\theta) }^2  ,
%	\label{app:eq:U_1}
	\end{align}
	where $\chi^n$ denote the chi-square distance between $p$ and $q^n$, i.e. $\chi^n = \sum_{j \in W_n } (r_j - s_j^n)^2/s_j^n$ and $W_n = \{j | s_j^n > 0\}$.
\end{lemma}

\begin{proof}
	We define $s_j^n = \frac{1}{\bar{q}^n}q_j^n $ and $\bar{q}^n = \sum_{j=1}^{J}q_j^n = \sum_{i=1}^{C}q_i^n $.
	
	According to the definition of $\Lcal(\theta)$ and $\Lcal^n(\theta)$, we have:
	\begin{align}
		\nabla \Lcal(\theta) - \nabla \Lcal^n(\theta)
		& = \sum_{j=1}^{J} (r_j - s_j^n ) \nabla \Lcal_j(\theta)
		\\
%		& = \sum_{i=1}^{n} (r_j - s_j^n) [\nabla \Lcal_j(\theta) -  \nabla \Lcal^n (\theta)]\\
		& = \sum_{j \in W_n} \frac{r_j - s_j^n}{\sqrt{s_j^n}} \sqrt{s_j^n}\nabla \Lcal_j(\theta)
		+ \sum_{j \notin W_n} r_j \nabla \Lcal_j(\theta) ,
	\end{align}
	where 
%	the second equality comes from $\sum_{i=1}^{n}r_j = \sum_{i=1}^{n}s_j^n = 1$ and 
	$W_n = \{j | s_j^n > 0\}$.
	
	Applying the Jensen inequality and the Cauchy-Schwartz inequality, it follows that:
	\begin{align}
		\norm{\nabla \Lcal(\theta) - \nabla \Lcal^n (\theta)}^2
		& \le 2 \norm{ \sum_{j \in W_n} \frac{r_j - s_j^n}{\sqrt{s_j^n}} \sqrt{s_j^n} \nabla \Lcal_j(\theta) }^2 
		+ 2 \norm{ \sum_{j \notin W_n} r_j \nabla \Lcal_j(\theta)}^2 
		\\
		& \le 2 \left[\sum_{j \in W_n} \frac{(r_j - s_j^n)^2}{s_j^n}  \right] \norm{\sum_{j \in W_n} s_j^n \nabla \Lcal_j(\theta) }^2 
		+ 2  \norm{ \sum_{j \notin W_n} r_j  \nabla \Lcal_j(\theta) }^2 
%	& \le  \left[\sum_{j \notin W_n}  r_j\right] \sum_{j \notin W_n} r_j  [\Lcal_j(\theta^n) - \Lcal_j(\theta_j^*)] 
	\end{align}
	
	
	
\end{proof}

\begin{proof}	
	\begin{align}
	\norm{\nabla \Lcal (\theta)}^2
	& \le 2 \norm{\nabla \Lcal ( \theta) - \nabla \Lcal^n( \theta)}^2 
	+ 2 \norm{ \nabla \Lcal^n (\theta)}^2\\
	& \le \left[ 4 \chi^n + 2 \right] \norm{ \nabla \Lcal^n (\theta)}^2 
	+ 4  \norm{ \sum_{j \notin W_n} r_j  \nabla \Lcal_j(\theta) }^2 
	,
	%	\label{app:eq:U_1}
	\end{align}
	We define $B = \frac{1}{N}\sum_{i=0}^{N-1}B^n$. 
%	We define $\chi_{p ||q}^2 = \max_n \chi^n$.  
	Hence, using Theorem XX, we have:
	\begin{align}
	\frac{1}{N}\sum_{n=0}^{N-1} \norm{\nabla \Lcal (\theta^n)}^2
	& \le 
%	4L \left[\chi_{p ||q}^2 + 1\right] \epsilon_{opt}
	\epsilon
	+ \frac{1}{N}\sum_{n=0}^{N-1}\chi^n A^n 
	+ B \nonumber\\
	& + 4L \max_n\left[\left[\chi^n + 1\right]\frac{1}{\bar{q}^n}\right] 
	\min_x\left[ \frac{1}{N}  \sum_{n=0}^{N-1} \left[ \E{\Lcal^n(x)} - \Lcal^n(\tilde{\theta}^n) \right] \right]
	,
	%	\label{app:eq:U_1}
	\end{align}	
	
	\begin{align}
	\frac{1}{N}\sum_{n=0}^{N-1} \norm{\nabla \Lcal (\theta^n)}^2
	& \le 
	%	4L \left[\chi_{p ||q}^2 + 1\right] \epsilon_{opt}
	\epsilon
	+ \Ocal (\frac{1}{N}\sum_{n=0}^{N-1}\chi^n [\Lcal^n(\tilde{\theta}^n) -\sum_{j \in W_n} {q}_j^n \Lcal_j(\theta_j^*)])\nonumber\\
	& + \Ocal(\frac{1}{N}\sum_{n=0}^{N-1}\sum_{j \notin W_n} r_j [\Lcal_j(\theta^n) - \Lcal_j(\theta_j^*)]) \nonumber\\
	& + \Ocal(\min_x \{\frac{1}{N} \sum_{n=0}^{N-1} \left[ \E{\Lcal^n(x)} - \Lcal^n(\tilde{\theta}^n) \right]\} )
	\end{align}	
	
	

\end{proof}














==> delayed_proofs/app_convergence_convexity.tex <==

\section{Convergence Guarantees Proofs}

\begin{table}
	\caption{Common Notation Summary.}
	\label{table:parameters}
	\centering
	\begin{tabular}{cc}
%		\toprule
		Symbol     & Description    \\
%		\midrule
		$C$ & Number of clients. \\
		$K$ & Number of local SGD.  \\
		$\eta_l$ & Local/Client learning rate.\\
		$\eta_g$ & Global/Server learning rate.\\
		$\tilde{\eta}$ & Effective learning rate, $\tilde{\eta} = \eta_l \eta_g$.\\
		
		$n$ & optimization round. \\
		$\theta^n$ & Global model at server iteration $n$.  \\
		$\tilde{\theta}$ & Optimum of the federated loss function, equation (\ref{eq:global_loss}). \\
		$\theta_i^{n+1}$ & Local update of client $i$ on model $\theta^n$.\\
		$y_{i, k}^n$ & Local model of client i after $k$ SGD updates ($y_{i, k}^n = \theta_i^{n+1}$ and $y_{i, 0}^{t} = \theta^n$). \\
		
		$p_i$ & Importance of client $i$ in the federated loss function, equation (\ref{eq:global_loss}).  \\
		$m$ & Maximum amount of clients the server can communicate with.\\
		$S_n$ & Set of participating clients considered at iteration $n$.\\
		$\omega_i(S_n)$ & Aggregation weight for client $i$ given $S_n$.\\
		$\alpha$ & Covariance parameter.\\
		$\delta_i, \delta_i^*$ & cf Section \ref{sec:convergence}\\
		$\gamma^*$ & Jensen gap upper bound parameter, cf Section \ref{sec:convergence}\\
		
		$n$ & time variable since the start of the learning process.\\
		$t^n$ & time at the aggregation $n$.\\
		$\rho_i(n)$ & expected computation time of client $i$. \\
		
		$\EE{n}{\cdot}$ & Expected value conditioned on $\theta^n$.\\
		$\Lcal(\cdot)$ & Federated loss function, equation \ref{eq:global_loss}\\
		$\Lcal_i(\cdot)$ & Local loss function of client $i$.\\
		$g_i(\cdot)$ & SGD. We have $\EE{\xi_i}{g_i(\cdot)} = \nabla \Lcal_i(\cdot)$ with Assumption \ref{ass:unbiased}.\\
		$\xi_i$ & Random batch of samples from client $i$ of size $B$.\\

		
		$L$ & Lipschitz smoothness parameter, Assumption \ref{ass:smoothness}.\\
		$\sigma^2$ & Uniform bound on the variance of the stochastic gradients, Assumption \ref{ass:unbiased}.\\
		$\beta$, $\kappa$ & Assumption \ref{ass:dissimilarity} parameters on the clients gradient bounded dissimilarity.\\
		$\mu$ & Strong convexity parameter. \\
		
%		$\rho_i(n)$ & step at which the server communicated to client $i$ its global model for local computation.\\
		
		
%		\bottomrule
	\end{tabular}
\end{table}


In Table \ref{table:parameters}, we provide the definition of the different notation used in this work.






\begin{equation}
\label{app:eq:SGD_process}
y_{i, k}^{\rho_i(n)} - \theta^{\rho_i(n)} 
= - \eta_l \sum_{l=0}^{k-1} g_i( y_{i, l}^{\rho_i(n)})
\end{equation}
By taking the expected value while considering Assumption \ref{ass:unbiased} we get:
\begin{equation}
\label{app:eq:E_SGD_process}
\E{y_{i, k}^{\rho_i(n)} - \theta^{\rho_i(n)}} 
= - \eta_l \sum_{ l = 0 }^{k - 1} \nabla \Lcal_i( y_{i, l}^{\rho_i(n)})
\end{equation}


By rewriting equation (\ref{eq:aggreg_SCAFFOLD_general}) with equation (\ref{app:eq:SGD_process}), we get:
\begin{align}
\label{app:eq:global_update_rewrote}
\theta^{n+1} - \theta^n
& = \eta_g \sum_{i=1}^n \omega_i^n \left[\theta_i^{\rho_i(n)+1} - \theta^{\rho_i(n)} \right] \\
& = -\tilde{\eta} \sum_{i=1}^n \omega_i^n \sum_{k=1}^{K} g_i( y_{i, k}^{\rho_i(n)})
\end{align}
We take the expected value of equation (\ref{app:eq:global_update_rewrote}). The aggregation weight $\omega_i^n$ is independent from the local work $\theta_i^{\rho_i(n)+1} - \theta^{\rho_i(n)}$. Hence, using equation (\ref{app:eq:E_expected_weight}) and (\ref{app:eq:E_SGD_process}), one gets:
\begin{equation}
\label{app:eq:E_global_update_rewrote}
\E{\theta^{n+1} - \theta^n}
= -\tilde{\eta} \sum_{i=1}^n q_i^n \sum_{k=1}^{K} \nabla \Lcal_i( y_{i, k}^{\rho_i(n)})
\end{equation}



%\input{./tex/Lemma_equality.tex}
\input{./tex/bounding_client_drift.tex}
\input{./tex/property_convex_functions.tex}
\input{./tex/convergence_convex.tex}


















%\subsection{Proof of Theorem \ref{theo:convergence}}\label{app:proof:convergence}
%
%\begin{proof}
%	
%	With Lemma \ref{lem:equality_update_without_Jenken}, we get:
%	\begin{align}
%	\EE{n}{\norm{\theta^{n+1} - \tilde{\theta}}^2} 
%	&\le \norm{\theta^n - \tilde{\theta}}^2 
%	\underbrace{- 2 \tilde{\eta} \inner{\sum_{k, i}d_i \nabla \Lcal_i(y_{i,k}^{\rho_i(n)})}{\theta^n - \tilde{\theta}}}_{T_1} \nonumber\\
%	&+ \underbrace{\eta_g^2 \sum_{i=1}^{n} \EE{n}{\omega_i^2} \EE{n}{\norm{\theta_i^{\rho_i(n) + 1} - \theta^{\rho_i(n)}}^2 }}_{T_2}. \label{app:eq:C_1}
%	\end{align}
%	
%	
%	
%	
%	\subsubsection*{Bounding $T_1$}
%	Using Lemma \ref{lem:perturbed_strong_convexity} with convex functions ($\mu = 0$), we can bound $T_1$ as :
%	\begin{align}
%	T_1 
%	&\le - 2 \tilde{\eta} \sum_{k, i}d_i \left[ \Lcal_i(\theta^n) - \Lcal_i(\tilde{\theta}) - L \norm{y_{i, k}^{\rho_i(n)} - \theta^n}^2
%	%			+ \frac{\mu}{4}\norm{\theta^n - \tilde{\theta}}^2
%	\right]\\
%	&\le - 2 \tilde{\eta} K \left[ \Lcal(\theta^n) - \Lcal(\tilde{\theta}) 
%	%			+ \frac{\mu}{4}\norm{\theta^n - \tilde{\theta}}^2
%	\right] 
%	+ 2 L \tilde{\eta} \sum_{i}d_i\sum_{k}\EE{n}{\norm{y_{i,k}^{\rho_i(n)} - \theta^n}^2},
%	\end{align}
%	where $\EE{n}{\norm{y_{i,k}^{\rho_i(n)} - \theta^n}^2}$ can be bounded using Lemma \ref{lem:bounded_drift_asynchronous}:
%	\begin{align}
%	T_1 
%	&\le - 2 \tilde{\eta} K\left[ \Lcal(\theta^n) - \Lcal(\tilde{\theta}) 
%	%		+ \frac{\mu}{4}\norm{\theta^n - \tilde{\theta}}^2
%	\right] 
%	+ 4 L \tilde{\eta} \eta_l^2 K^2 (\Delta \tau + 1) \left[ [\sigma^2 + 3 L^2 G^2 ][1 + \eta_g^2 \delta^{t, \Delta \tau}]  
%	+3 \rho
%	+ 3 \eta_g^2 \nu^t \right],
%	\label{app:eq:C_2}
%	\end{align}
%	where $\rho = \sum_{i=1}^{n} d_i \EE{\xi_i}{\norm{\nabla \Lcal_i (\tilde{\theta})}^2}$.
%	
%	
%	
%	
%	
%	
%	
%	\subsubsection*{Bounding $T_2$}
%	Using Lemma \ref{lem:bounded_drift_asynchronous}, we can rewrite $T_2$ as :
%	\begin{equation}
%	T_2
%	\le 2 \tilde{\eta}^2 K^2 (\Delta \tau + 1) \left[ \delta [\sigma^2 + 3 L^2 G^2 ][1 + \eta_g^2 \delta^{t, \Delta \tau}]  
%	+3 \epsilon 
%	+ 3 \eta_g^2 \delta  \nu^t \right], 
%	\label{app:eq:C_4}
%	\end{equation}
%	where we define $\delta_i  = \EE{n}{{\omega_i^n}^2}$, $\delta = \sum_{i=1}^{n}\delta_i$, and $\epsilon =\sum_{i=1}^{n}\delta_i \EE{\xi_i}{\norm{\nabla \Lcal_i(\tilde{\theta})}^2 }$. 
%	
%	
%	
%	
%	\subsubsection*{Bounding equation (\ref{app:eq:C_1})}
%	
%	
%	Substituting equation (\ref{app:eq:C_4}) and (\ref{app:eq:C_2}) in equation (\ref{app:eq:C_1}), we get:	
%	
%	\begin{align}
%	\EE{n}{\norm{\theta^{n+1} - \tilde{\theta}}^2} 
%	&\le \norm{\theta^n - \tilde{\theta}}^2 
%	- 2 \tilde{\eta} K\left[ \Lcal(\theta^n) - \Lcal(\tilde{\theta}) 
%	%	+ \frac{\mu}{4}\norm{\theta^n - \tilde{\theta}}^2
%	\right] \nonumber\\
%	& + 4 L \tilde{\eta} \eta_l^2 K^2 (\Delta \tau + 1) \left[ [\sigma^2 + 3 L^2 G^2 ][1 + \eta_g^2 \delta^{t, \Delta \tau}]  
%	+3 \rho
%	+ 3 \eta_g^2 \nu^t \right] \nonumber\\
%	&+ 2 \tilde{\eta}^2 K^2 (\Delta \tau + 1) \left[ \delta [\sigma^2 + 3 L^2 G^2 ][1 + \eta_g^2 \delta^{t, \Delta \tau}]  
%	+3 \epsilon 
%	+ 3 \eta_g^2 \delta  \nu^t \right]. 
%	\end{align}
%	
%	Finally, by rearranging the terms, we get:
%	\begin{align}
%	\E{\Lcal(\theta^n)} - \Lcal(\tilde{\theta}) 	
%	& \le \frac{1}{2 \tilde{\eta} K} \left[\E{\norm{\theta^n - \tilde{\theta}}^2} - \E{\norm{\theta^{n+1} - \tilde{\theta}}^2}  \right] \nonumber\\
%	& + 2 L \eta_l^2 K (\Delta \tau + 1) \left[ [\sigma^2 + 3 L^2 G^2 ][1 + \eta_g^2 \delta^{t, \Delta \tau}]  
%	+3 \rho
%	+ 3 \eta_g^2 \nu^t \right] \nonumber\\
%	&+ \tilde{\eta} K (\Delta \tau + 1) \left[ \delta [\sigma^2 + 3 L^2 G^2 ][1 + \eta_g^2 \delta^{t, \Delta \tau}]  
%	+3 \epsilon 
%	+ 3 \eta_g^2 \delta  \nu^t \right],
%	\label{app:eq:C_5}
%	\end{align}
%	
%	We note that we have:
%	\begin{align}
%	\delta = 
%	&\frac{1}{T+1}\sum_{t=0}^{T} \delta^{t, \Delta \tau}\\
%	& =  \frac{1}{T+1}\sum_{t=0}^{T}\sum_{s=0}^{\Delta \tau - 1} \delta^{t-s}\\
%	& \le \frac{1}{T+1}\sum_{t=0}^{T}\sum_{s=0}^{\Delta \tau - 1}  \sum_{i=1}^C \E{{\omega_i^{t-s}}^2}\\
%	& \le \frac{1}{T+1}\sum_{t=0}^{T}\Delta \tau \sum_{i=1}^C \E{{\omega_i^{t}}^2}
%	\label{app:eq:C_6}
%	\end{align}
%	Similarly, we have:
%	\begin{equation}
%	\nu
%	= \frac{1}{T+1 } \sum_{t=0}^{T} \nu^{t} 
%	\le \frac{\Delta \tau}{T+1}\sum_{t=0}^{T}  \sum_{i=1}^C \EE{n}{{\omega_i^n}^2}
%	\EE{\xi_i}{\norm{\nabla \Lcal_i(\tilde{\theta}) }^2}
%	\label{app:eq:C_7}
%	\end{equation}
%	Substituting equation (\ref{app:eq:C_6}) and equation (\ref{app:eq:C_7}) in equation (\ref{app:eq:C_5}) gives:
%	\begin{align}
%	\frac{1}{T+1} \sum_{t=0}^{T}\E{\Lcal(\theta^n)} - \Lcal(\tilde{\theta}) 	
%	& \le \frac{1}{2 \tilde{\eta} K(T+1)} \E{\norm{\theta^0 - \tilde{\theta}}^2} \nonumber\\
%	& + 2 L \eta_l^2 K (\Delta \tau + 1) \left[ [\sigma^2 + 3 L^2 G^2 ][1 + \eta_g^2 \delta]  
%	+3 \rho
%	+ 3 \eta_g^2 \nu \right] \nonumber\\
%	&+ \tilde{\eta} K (\Delta \tau + 1) \left[ \delta [\sigma^2 + 3 L^2 G^2 ][1 + \eta_g^2 \delta]  
%	+3 \epsilon 
%	+ 3 \eta_g^2 \delta  \nu \right]\\
%	& = \Ocal (\frac{1}{\tilde{\eta} K(T+1)}) \nonumber\\
%	& + \Ocal( \eta_l^2 K (\Delta \tau + 1) [1 + \eta_g^2 \delta])
%	+ \Ocal( \eta_l^2 K (\Delta \tau + 1) (\rho
%	+ \eta_g^2 \nu ))\nonumber\\
%	&+ \Ocal( \tilde{\eta} K (\Delta \tau + 1) \delta [1 + \eta_g^2 \delta] ) 
%	+ \Ocal (\tilde{\eta} K (\Delta \tau + 1) (\epsilon 
%	+ \eta_g^2 \delta  \nu )).
%	\end{align}
%	
%	
%	
%	
%	
%	
%\end{proof}




==> delayed_proofs/app_convergence_without_convexity.tex <==
\section{No convexity}


\begin{proof}
	With the Lipschitz-smooth assumption \ref{ass:smoothness}, it follows:
	\begin{equation}
		\EE{n}{\Lcal^n(\theta^{n+1})} - \Lcal^n(\theta^n)
		\le \underbrace{\EE{n}{\inner{\nabla \Lcal^n(\theta^n)}{\theta^{n+1} - \theta^n}}}_A 
		+ \frac{L}{2}\underbrace{\EE{n}{\norm{\theta^{n+1} - \theta^n}^2}}_B
		\label{app:eq:M_0}
	\end{equation}	
	By construction, equation (\ref{eq:aggreg_SCAFFOLD_general}), we have $\theta^{n+1} - \theta^n =  \eta_g \sum_{i}\omega_i^n(\theta_i^{\rho_i(n) +  1} - \theta^{\rho_i(n)})$. The considered client sampling satisfies $\EE{n}{\omega_i^n} = q_i^n$ and the aggregation weight is independent of a client's local work. Therefore, $\EE{n}{\theta^{n+1} - \theta^n} = \eta_g \sum_{i} q_i^n \EE{n}{\theta_i^{\rho_i(n)+1} - \theta^{\rho_i(n)}}$. 
	\begin{align}
	A 
	&= \eta_g \inner{\nabla \Lcal^n(\theta^n)}{\sum_{i} q_i^n \EE{n}{\theta_i^{t+1} - \theta_i^{\rho_i(n)}}}
	\\
	&= - \tilde{\eta}\inner{\nabla \Lcal^n(\theta^n)}{\sum_{i, k} q_i^n \EE{n}{\nabla \Lcal^n_i(y_{k, i}^{\rho_i(n)})}}
	\\
	&= - K\bar{q}^n\tilde{\eta}\inner{\nabla \Lcal^n(\theta^n)}{\sum_{i, k} \frac{1}{\bar{q}^n} q_i^n \frac{1}{K}\EE{n}{\nabla \Lcal^n_i(y_{k, i}^{\rho_i(n)})}}
	\\
	&= - K\tilde{\eta} \bar{q}^n\frac{1}{2} 
	[\norm{\nabla \Lcal^n(\theta^n)}^2 
	+ \EE{n}{\norm{\sum_{i, k}\frac{1}{\bar{q}^n} q_i^n \frac{1}{K}\nabla \Lcal^n_i(y_{k, i}^{\rho_i(n)})}^2} \nonumber\\
	&- \underbrace{\EE{n}{\norm{\nabla \Lcal^n(\theta^n) - \sum_{i, k} \frac{1}{\bar{q}^n} q_i^n\frac{1}{K} \nabla \Lcal^n_i(y_{k, i}^{\rho_i(n)})}^2}}_C]
	\\
	&\le - K\tilde{\eta} \bar{q}^n\frac{1}{2} 
	[\norm{\nabla \Lcal^n(\theta^n)}^2 
	+ H^2 - C ],
	\label{app:eq:M_1}
	\end{align}
	where the second equality comes from XXX and the last inequality comes from using $2 \inner{a}{b} = \norm{a}^2 + \norm{b}^2 - \norm{a-b}^2$.
	
	
	\begin{align}
		C 
		&=  \EE{n}{\norm{\sum_{i} \frac{1}{\bar{q}^n} q_i^n [\nabla \Lcal_i(\theta^n) - \sum_{k}\frac{1}{K} \nabla \Lcal_i(y_{k, i}^{\rho_i(n)})]}^2}
		\\
%		& \le \sum_{i} q_i^n  \EE{n}{\norm{ \sum_{k}\frac{1}{K} [\nabla \Lcal_i(\theta^n) - \nabla \Lcal_i(y_{k, i}^{\rho_i(n)}) ] }^2}\\
		& \le \sum_{k, i} \frac{1}{\bar{q}^n}q_i^n  \frac{1}{K}\EE{n}{\norm{ \nabla \Lcal_i(\theta^n) - \nabla \Lcal_i(y_{k, i}^{\rho_i(n)}) }^2}\\
		& \le \sum_{k, i} \frac{1}{\bar{q}^n} q_i^n  \frac{1}{K} L^2 \EE{n}{\norm{ \theta^n - y_{k, i}^{\rho_i(n)} }^2}
		\\
		& = \sum_{i} \frac{1}{\bar{q}^n} q_i^n  L^2 \left[ (\Delta \tau + 1 ) (\eta_l^2 K^2 (\sigma^2 + H^2 )) + (\Delta \tau + 1 ) \eta_g^2 \beta(n) (\eta_l^2 K^2 (\sigma^2 + H^2 )) \right]
		\\
		& = L^2 (\Delta \tau + 1 ) (\eta_l^2 K^2 (\sigma^2 + H^2 )) ( 1 + \eta_g^2 \beta(n) )
		\label{app:eq:M_2}
	\end{align}
	
	
	
	
	
	
	
	
	\begin{align}
		B 
		& = \EE{n}{\norm{\theta^{n+1} - \theta^n}^2}
		\\
		&  \le \eta_g^2 \sum_{i=1}^{C}\beta_i^n \EE{n}{\norm{\theta_i^{\rho_i(n)+1} - \theta_i^{\rho_i(n)}}^2}
		\\
		&  \le \tilde{\eta}^2 \sum_{i=1}^{C}\beta_i^n \EE{n}{\norm{\sum_{k=0}^{K-1} g_i(y_{i, k}^{\rho_i(n)})}^2}
		\\
		&  \le \tilde{\eta}^2 \sum_{i=1}^{C}\beta_i^n \left[ K \sigma^2 + \EE{n}{\norm{\sum_{k=0}^{K-1} \nabla \Lcal_i(y_{i, k}^{\rho_i(n)})}^2} \right]
		\\
		&  \le \tilde{\eta}^2 \sum_{i=1}^{C}\beta_i^n 
		\left[ K \sigma^2 
		+ K H^2\right]
		\label{app:eq:M_3}
	\end{align}
	where the last inequality comes from using Assumption \ref{ass:unbiased}.
	
	Substituting equation (\ref{app:eq:M_2}) and equation (\ref{app:eq:M_3}) in equation (\ref{app:eq:M_0}), we get:
	\begin{equation}
		\EE{n}{\Lcal^n(\theta^{n+1})} - \Lcal^n(\theta^n)
		\le \EE{n}{\inner{\nabla \Lcal^n(\theta^n)}{\theta^{n+1} - \theta^n}}
		+ \frac{L}{2}\EE{n}{\norm{\theta^{n+1} - \theta^n}^2}
	\end{equation}
	
	
	
	
	
	
	
	
\end{proof}

==> delayed_proofs/convergence_convex.tex <==
\subsection{Proof of Theorem \ref{theo:convergence_convex}}\label{sec:app:proof:convergence}

\begin{proof}
	Equation (\ref{eq:FedAvg_one_server_iteration_bound})
	\begin{align}
	\E{\norm{\vtheta^{n+1} - \vx}^2} 
	&= \E{ \norm{\vtheta^n - \vx}^2 }
	\underbrace{- 2 \eta_g \E{ \inner { \sum_{i=1}^M q_i(n) \E{\vtheta_i^{\rho_i(n)+1} - \vtheta^{\rho_i(n)}} }{x - \vtheta^n} }}_{T_1}
	+ \tilde{\eta}^2 Q(\vtheta^n)
%	\nonumber\\
%	&+ \underbrace{\eta_g^2 \sum_{i=1}^M \beta_i^n \E{\norm{\vtheta_i^{\rho_i(n) + 1} - \vtheta^{\rho_i(n)}}^2}}_{T_2},
	\label{app:eq:C_1}
	\end{align}
	
	
	
	
	\subsubsection*{Bounding $T_1$}
	\begin{align}
	T_1 
	& = - 2 \tilde{\eta} \sum_{i=1}^M q_i(n) \sum_{k=0}^{K-1}  \underbrace{\E{ \inner { \nabla \Lcal_i (\vy_{i, k}^{\rho_i(n)}) }{\vx - \vtheta^n} }}_{T_2}
%	\\
	\end{align}
	
	\begin{align}
	T_2 
	& = \E{ \inner { \nabla \Lcal_i (\vy_{i, k}^{\rho_i(n)}) }{\vx - y_{i, k}^{\rho_i(n)}} }
	\nonumber\\
	& + \E{ \inner { \nabla \Lcal_i (\vy_{i, k}^{\rho_i(n)}) }{y_{i, k}^{\rho_i(n)} - \vtheta^{\rho_i(n)}} }
	\nonumber\\
	& + \E{ \inner { \nabla \Lcal_i (\vy_{i, k}^{\rho_i(n)}) }{\vtheta^{\rho_i(n)} - \vtheta^n} }
	\end{align}
	
	Using Cauchy Schwartz inequality and AM-GM inequality, we have
	\begin{equation}
		- 2 \inner{\va}{\vb} 
		\le 2 \sqrt{\norm{\va}^2\norm{\vb}^2}
		= 2 \sqrt{\frac{1}{\tilde{\eta}}\norm{\va}^2 \tilde{\eta} \norm{\vb}^2}
		\le \left[ \frac{1}{\tilde{\eta}}\norm{\va}^2 + \tilde{\eta} \norm{\vb}^2\right] 
	\end{equation}
	Also, the strong convexity of $\Lcal_i$ gives us:
	\begin{equation}
		\inner { \nabla \Lcal_i (\vy_{i, k}^{\rho_i(n)}) }{\vx - y_{i, k}^{\rho_i(n)}} 
		\ge \Lcal_i(\vy_{i, k}^{\rho_i(n)}) - \Lcal_i(\vx) + \frac{\mu}{2}\norm{\vy_{i, k}^{\rho_i(n)} - \vx}^2
	\end{equation}
	
	\begin{align}
	T_1 
	& \le - 2 \tilde{\eta} \sum_{i=1}^M q_i(n) \sum_{k=0}^{K-1} 
	\E{
	\Lcal_i(\vy_{i, k}^{\rho_i(n)}) - \Lcal_i(\vx) + \frac{\mu}{2}\norm{\vy_{i, k}^{\rho_i(n)} - \vx}^2
}
	\nonumber\\
	& + \sum_{i=1}^M q_i(n) \sum_{k=0}^{K-1}
	\E{
	2 \tilde{\eta}^2 \norm{\nabla \Lcal_i (\vy_{i, k}^{\rho_i(n)})}^2 
	+  \norm{y_{i, k}^{\rho_i(n)} - \vtheta^{\rho_i(n)}}^2 
	+ \norm{\vtheta^{\rho_i(n)} - \vtheta^n}^2
}
	%	\\
	\end{align}
	


	
	
	
	\subsubsection*{Bounding $T_2$}
	Using Lemma \ref{lem:bounded_drift_convex}, we can rewrite $T_2$ as :	
%	\begin{align}
%	T_2
%	&\le 2\tilde{\eta}^2  (H +  1) K^2 \underbrace{ \sum_{i=1}^{C}\beta_i^n \phi_i(x)}_{U^n}\nonumber\\
%	& + 2 \tilde{\eta}^2  (H +  1) K^2  \eta_g^2 H \underbrace{\left[\sum_{i=1}^{C}\beta_i^n \right]\frac{1}{\max(H, 1)}\sum_{s=0}^{H - 1} \sum_{i=1}^{C} \beta_i^{n-s}
%	\phi_i(x)}_{V^n} 
%	,
%	\label{app:eq:C_4}
%	\end{align}
%
	\begin{align}
	T_2
	&\le 2 \tilde{\eta}^2 K^2 \underbrace{\sum_{i=1}^{C} \beta_i^n \phi_i(x)}_{U^n}
	,
	\label{app:eq:C_4}
	\end{align}
	
	
	
	\subsubsection*{Bounding equation (\ref{app:eq:C_1})}
	
	
	Substituting equation (\ref{app:eq:C_4}) and (\ref{app:eq:C_2}) in equation (\ref{app:eq:C_1}), we get:	
	\begin{align}
	\E{\norm{\vtheta^{n+1} - \vx}^2} 
	&\le \E{ \norm{\vtheta^n - \vx}^2 }
	- 2 \tilde{\eta} K  \E{ \Lcal^n(\vtheta^n) - \Lcal^n(x) 
	%	+ \frac{\mu}{4}\norm{\vtheta^n - \vx}^2
	}\nonumber\\
	&+ 2 \tilde{\eta} (H +  1) \eta_l^2 K^3 [R^n + \eta_g^2 H S^n] 
	+ 2 \tilde{\eta}^2  K^2 U^n . 
	\end{align}	

	Finally, by rearranging the terms, we get:
	\begin{align}
	\E{\Lcal^n(\vtheta^n)} - \Lcal^n(x) 	
	& \le \frac{1}{2  \tilde{\eta} K} \left[\E{\norm{\vtheta^n - \vx}^2} - \E{\norm{\vtheta^{n+1} - \vx}^2}  \right] \nonumber\\
	&+ (H +  1) \eta_l^2 K^2 [R^n + \eta_g^2 H S^n ]  
	+ \tilde{\eta}  K . 
	\label{app:eq:C_5}
	\end{align}

	Summing over $N$ gives:
	\begin{align}
	\frac{1}{N} \sum_{n=0}^{N-1} \left[ \E{\Lcal^n(\vtheta^n)} - \Lcal^n(x) \right]	
	& \le \frac{1}{2 \tilde{\eta} K N} \E{\norm{\vtheta^0 - \vx}^2} \nonumber\\
	& + (H +  1) \eta_l^2 K^2 \frac{1}{N} \sum_{n=0}^{N-1} [R^n + \eta_g^2 H S^n ] 
	+ \tilde{\eta}   K \frac{1}{N} \sum_{n=0}^{N-1} U^n  
	\\
	& = \Ocal(\frac{1}{\tilde{\eta} K N})
	+\Ocal[(H +  1) \eta_l^2 K^2] 
	+ \Ocal[\tilde{\eta}^2  (H +  1)H  K ]
	+\Ocal[\tilde{\eta} K] 
	\label{app:eq:R_1}
	.
	\end{align}
	
	We note that the result in equation (\ref{app:eq:R_1}) works for any model $x$. FL is a succession of minimization problems $\Lcal^n$ with respective optimum $\tilde{\vtheta}^n$. 
	As a result, we have:
	\begin{align}
	\frac{1}{N} \sum_{n=0}^{N-1} \left[ \E{\Lcal^n(\vtheta^n)} - \Lcal^n(\tilde{\vtheta}^n) \right]
	& \le \frac{1}{N} \sum_{n=0}^{N-1} \left[ \E{\Lcal^n(x)} - \Lcal^n(\tilde{\vtheta}^n) \right]
	 + \Ocal(\frac{1}{\tilde{\eta} K N}) \nonumber\\
	&+\Ocal[(H +  1) \eta_l^2 K^2] 
	+ \Ocal[\tilde{\eta}^2  (H +  1)H  K ]
	+\Ocal[\tilde{\eta} K]
	\label{app:eq:R_2}
	.
	\end{align}
	


	

	
	
\end{proof}

==> delayed_proofs/decomposition_theorem.tex <==
\section{Decomposition Theorem \ref{theo:decomposition_theorem}} \label{app:sec:decomposition_theorem}

\input{tex/variables}
In Table \ref{table:parameters}, we provide the definition of the different notations used in this work.

%\input{./tex/Lemma_equality.tex}

\subsection{Useful Lemma}
We first introduce and prove the following useful lemma before introducing the proof of Decomposition Theorem \ref{theo:decomposition_theorem}.

\begin{lemma}\label{lem:decompo_Xi}
	Let us consider $n$ vectors $\vx_i, ..., \vx_n$ and a client sampling satisfying $\EE{S_t}{\omega_i(S_t)} = p_i$ and $\COV{\omega_i(S_t)}{\omega_j(S_t)} = - \alpha p_i p_j$. We have:
	\begin{equation}
		\EE{S_t}{\norm{\sum_{i=1}^{n}\omega_i(S_t)\vx_i}^2} 
		= \sum_{i=1}^{n} \gamma_i \norm{\vx_i}^2
		+ (1 - \alpha)\norm{\sum_{i=1}^{n}p_i \vx_i}^2,
	\end{equation}
	where $\gamma_i =  \VARR{S_t}{\omega_i(S_t)} + \alpha p_i^2 $.
\end{lemma}


\begin{proof}
	\begin{align}
		\EE{S_t}{\norm{\sum_{i=1}^{n}\omega_i(S_t)\vx_i}^2} 
		& = \sum_{i=1}^{n} \EE{S_t}{\omega_i(S_t)^2} \norm{\vx_i}^2
		+ \sum_{i=1}^{n}\sum_{\substack{j=1\\ j\neq i}}^{n}\EE{S_t}{\omega_i(S_t)\omega_j(S_t)}\inner{\vx_i}{\vx_j}
		\label{app:eq:AA1}
	\end{align}
	
	In addition, we have:
	\begin{equation}
		\EE{S_t}{\omega_i(S_t)\omega_j(S_t)}
		= \COV{\omega_i(S_t)}{\omega_j(S_t)} + p_i p_j
		= (- \alpha + 1) p_i p_j,
		\label{app:eq:AA2}
	\end{equation}
	where the last equality comes from the client sampling covariance assumption.
	
	We also have:
	\begin{equation}
		\sum_{i=1}^{n}\sum_{\substack{j=1\\ j\neq i}}^{n}\inner{p_i \vx_i}{p_j \vx_j} 
		= \norm{\sum_{i=1}^{n}p_i \vx_i}^2 - \sum_{i=1}^{n}p_i^2 \norm{\vx_i}^2
		\label{app:eq:AA3}
	\end{equation}
	
	Substituting equation (\ref{app:eq:AA2})  and equation (\ref{app:eq:AA3}) in equation (\ref{app:eq:AA1}) gives:
	\begin{equation}
		\EE{S_t}{\norm{\sum_{i=1}^{n}\omega_i(S_t)\vx_i}^2} 
		= \sum_{i=1}^{n} \left[ \EE{S_t}{\omega_i(S_t)^2} - (-\alpha +1 )p_i^2 \right] \norm{\vx_i}^2
		+ (-\alpha +  1)\norm{\sum_{i=1}^{n}p_i \vx_i}^2
		\label{app:eq:AA4}
	\end{equation}
	
	Considering that we have $\EE{S_t}{\omega_i(S_t)^2} = \VAR{\omega_i(S_t)} + p_i^2$, we have :
	\begin{equation}
	\EE{S_t}{\omega_i(S_t)^2} + (\alpha - 1) p_i^2
	= \VARR{S_t}{\omega_i(S_t)} + \alpha p_i^2
	\label{app:eq:AA5}
	\end{equation}
	
	Substituting equation (\ref{app:eq:AA5}) in equation (\ref{app:eq:AA4}) completes the proof.

\end{proof}





\subsection{Proof of the Decomposition Theorem \ref{theo:decomposition_theorem}}
\begin{proof}
	\begin{align}
	\EE{t}{\norm{\theta^{t+1} - \theta^*}^2} 
	&= \EE{t}{\norm{(\theta^{t+1} - \theta^t) + (\theta^t - \theta^*)}^2}\\
	&= \norm{\theta^t - \theta^*}^2 
	+ 2 \inner{\EE{t}{\theta^{t+1} - \theta^t}}{\theta^t - \theta^*} + \EE{t}{\norm{\theta^{t+1} - \theta^t}^2} 
	\end{align}
	By construction, equation (\ref{eq:aggreg_SCAFFOLD_general}), we have 
	$\theta^{t+1} - \theta^t 
	=  \eta_g \sum_{i=1}^n\omega_i(S_t)(\theta_i^{t+1} - \theta^t) 
	%= - \tilde{\eta} \sum_{i, k}\omega_i(S_t)g_i(y_{i,k}^t)
	$. The sampling scheme follows Definition \ref{def:sampling} which gives $\EE{S_t}{\theta^{t+1} - \theta^t} = \eta_g \sum_{i=1}^n p_i (\theta_i^{t+1} - \theta^t)$. Hence , we get:
	\begin{align}
	\EE{t}{\norm{\theta^{t+1} - \theta^*}^2} 
	&= \norm{\theta^t - \theta^*}^2 
	+ 2 \eta_g \inner{\sum_{i=1}^n p_i \EE{t}{\theta_i^{t+1} - \theta^t}}{\theta^t - \theta^*} \nonumber\\
	&+ \eta_g^2 \underbrace{\EE{t}{\norm{\sum_{i=1}^n\omega_i(S_t) (\theta_i^{t+1} - \theta^t)}^2}}_{= \eta_l^2 Q(\theta^t)} 
	\label{app:eq:A1}
	\end{align}
	
	Using Lemma \ref{lem:decompo_Xi}, we bound $Q(\theta^t)$ as follow:
	\begin{equation}
		\eta_l^2 Q(\theta^t) 
		= \sum_{i=1}^n \gamma_i \EE{t}{\norm{ \theta_i^{t+1} - \theta^t}^2}
		+ (1 - \alpha) \EE{t}{\norm{\sum_{i=1}^n p_i (\theta_i^{t+1} - \theta^t)}^2}.
		\label{app:eq:A2}
	\end{equation}
	
	
	By construction, we have $\theta_i^{t+1} - \theta^t = - \sum_{k=0}^{K-1} \eta_l g_i(y_{i,k}^t)$. Considering Assumption \ref{ass:unbiased} gives
	\begin{align}
	\E{\norm{\theta_i^{t+1} - \theta^t}^2}
	%        = \E{\norm{\theta_i^{t+1}-\theta^t}^2}
	%        \\
%	= \eta_l^2 \E{\norm{d_i^t}^2}
	%        \\
	%        = \eta_l^2 \left[ \E{\norm{d_i^t - h_i^t}^2 }
	%        +  \E{\norm{h_i^t}^2}\right]
	%        \\
	= \eta_l^2 \left[ \E{\norm{\xi_i^t}^2 }
	+ \E{\norm{\Delta_i^t}^2} \right] 
	%        \\
	.
	\label{app:eq:A3}
	\end{align}
	
	Similarly by using twice Assumption \ref{ass:unbiased} for the global model drift, we have
	\begin{align}
%	G(\{p_i\}, \theta^t)
%	%        &= \E{\norm{\sum_{i=1}^n p_i (\theta_i^{t+1}-\theta^t)}^2}
%	%        \\
%	&= 
	\eta_l^2 \E{\norm{\sum_{i=1}^n p_id_i^t }^2}
%	&= \eta_l^2 \E{\norm{\sum_{i=1}^n p_i (d_i^t - h_i^t)}^2}
%	+ \eta_l^2 \E{\norm{\sum_{i=1}^n p_i h_i^t }^2}
%	\\
	&= \eta_l^2 \E{\norm{\sum_{i=1}^n p_i \xi_i^t }^2}
	+ \eta_l^2 \E{\norm{\sum_{i=1}^n p_i \Delta_i^t }^2}
	\\
	&= \eta_l^2 \left[ \sum_{i=1}^n p_i^2 \E{\norm{ \xi_i^t }^2}
	+ \E{\norm{\sum_{i=1}^n p_i \Delta_i^t }^2} \right],
	\label{app:eq:A4}
	\end{align}
	where, for the last equality, Assumption \ref{ass:unbiased} gives $\E{\inner{\xi_i^t}{\xi_j^t}} = \E{\xi_i^t}^T \E{\xi_j^t} =  0 $.
	
	Combining equation (\ref{app:eq:A3}) with equation (\ref{app:eq:A4}) gives
	\begin{align}
	Q(\theta^t)
%	& = \sum_{i=1}^{n} \left[ \VAR{\omega_i(S_t)} 
%	+ \alpha p_i^2\right] L_i(\theta^t) + ( 1- \alpha) G(\theta^t)
%	\\
%	& = \eta_l^2 \sum_{i=1}^{n} \left[ \VAR{\omega_i(S_t)} + \alpha p_i^2\right]  \left[ \E{\norm{\xi_i^t}^2 } + \E{\norm{h_i^t}^2} \right] 
%	\nonumber\\
%	& + \eta_l^2 ( 1- \alpha)  \left[ \sum_{i=1}^n p_i^2 \E{\norm{ \xi_i^t }^2}
%	+ \E{\norm{\sum_{i=1}^n p_i h_i^t }^2} \right]
%	\\
	& = \sum_{i=1}^{n} \left[ \VAR{\omega_i(S_t)} + p_i^2 \right] \E{\norm{\xi_i^t}^2 } 
	\nonumber\\
	& +  \sum_{i=1}^{n} \gamma_i  \E{\norm{\Delta_i^t}^2} 
	+ ( 1- \alpha)  \E{\norm{\sum_{i=1}^n p_i \Delta_i^t }^2} .
	\label{app:eq:A5}
%	\\
%	& = \eta_l^2 \sum_{i=1}^{n} \left[ \VAR{\omega_i(S_t)} + p_i^2 \right] \E{\norm{\xi_i^t}^2 } 
%	\nonumber\\
%	& + \eta_l^2 \sum_{i=1}^{n} \left[\VAR{\omega_i(S_t)} + p_i^2 \right]  \E{\norm{h_i^t}^2} 
%	+ \eta_l^2 ( 1- \alpha) \sum_{i=1}^{n}\sum_{\substack{j=1\\ j\neq i}}^{n} \E{\inner{h_i^t}{h_j^t}} 
	\end{align}
	
%	where the equality comes from the unbiasedness of the SGD estimator, Assumption \ref{ass:unbiased}, and the last inequality comes from the bounded variance of the SGD estimator, Assumption \ref{ass:unbiased}.
%	
%	
%	Let us consider the special case where clients have the same data distribution. Clients perform identical local work. Therefore, we can define $h^t \coloneqq h_i^t$. By definition, equation (\ref{eq:global_loss}), we have $\sum_{i=1}^{n}p_i = 1$ which gives $h^t = \sum_{i=1}^{n} p_i h_i^t$ which gives	
%	\begin{align}
%	\sum_{i=1}^{n} \gamma_i L_i(\theta^t) + ( 1- \alpha) G(\theta^t)
%	& \le \eta_l^2 \sum_{i=1}^{n} \left[ \VAR{\omega_i(S_t)} + p_i^2 \right] K \sigma^2 
%	\nonumber\\
%	& + \eta_l^2 \left[ \sum_{i=1}^{n} \gamma_i  + (1 - \alpha ) \right] \E{\norm{h^t}^2} 
%	%	+ \eta_l^2 ( 1- \alpha)  \E{\norm{\sum_{i=1}^n p_i h_i^t }^2} 
%	\\& = \eta_l^2 \sum_{i=1}^{n} \left[ \VAR{\omega_i} + p_i^2 \right] K \sigma^2 
%	+ \eta_l^2 \left[ \VAR{\sum_{i=1}^{n}\omega_i}  + 1 \right] \E{\norm{h^t}^2} 
%	\end{align}
	
	Substituting equation (\ref{app:eq:A5}) in equation (\ref{app:eq:A1}) completes the proof.
	
\end{proof}


\subsection{Adaptation to Clustered Sampling}

Instead of Lemma \ref{lem:decompo_Xi} which requires $\COV{\omega_i(S_t)}{\omega_j(S_t)} = - \alpha p_i p_j$, we propose the following Lemma for clustered sampling expressed in function of MD sampling covariance parameter $\alpha_{MD}$ showing that a sufficient condition for MD sampling to perform as Clustered sampling is $\vx_i$ to all be identical or for all the distributions to be identical, i.e. $r_{k, i} = p_i$. 

\begin{lemma}\label{lem:decompo_Xiclustered}
	Let us consider $n$ vectors $\vx_i, ..., \vx_n$ and a client sampling satisfying $\EE{S_t}{\omega_i(S_t)} = p_i$ and $\COV{\omega_i(S_{Cl})}{\omega_j(S_{Cl})} = - \alpha p_i p_j$. We have:
	\begin{equation}
	\EE{S_{Cl}}{\norm{\sum_{i=1}^{n}\omega_i(S_{Cl})\vx_i}^2} 
	\le \sum_{i=1}^{n} \gamma_i(MD) \norm{\vx_i}^2
	+ (1 - \alpha_{MD})\norm{\sum_{i=1}^{n}p_i \vx_i}^2,
	\label{eq:decompo_clustered}
	\end{equation}
	where $\gamma_i(MD)$ and $\alpha_{MD}$ are the aggregation weights statistics of MD sampling. Equation (\ref{eq:decompo_clustered}) is an equality if and only if $\sum_{i=1}^{n} r_{k, i} \vx_i = \sum_{j=1}^{n} r_{k, j} \vx_j$.
\end{lemma}


\begin{proof}
	Substituting equation (\ref{app:eq:T1}) in equation (\ref{app:eq:AA1}) gives
	\begin{align}
	\EE{S_{Cl}}{\norm{\sum_{i=1}^{n}\omega_i(S_{Cl})\vx_i}^2} 
	& = \sum_{i=1}^{n} \EE{ S_{Cl} }{\omega_i( S_{Cl} )^2} \norm{\vx_i}^2
	+ \sum_{i=1}^{n}\sum_{\substack{j=1\\ j\neq i}}^{n} p_i p_j \inner{\vx_i}{\vx_j}
	\nonumber\\
	&- \frac{1}{m^2} \sum_{k=1}^{m} \sum_{i=1}^{n}\sum_{\substack{j=1\\ j\neq i}}^{n}  r_{k, i}r_{k, j} \inner{\vx_i}{\vx_j}
	\label{app:eq:U1}
	\end{align}
	
	Substituting equation (\ref{app:eq:AA3}) in equation (\ref{app:eq:AA1}) gives:
	\begin{align}
	\EE{ S_{Cl} }{\norm{\sum_{i=1}^{n}\omega_i( S_{Cl} )\vx_i}^2} 
	& = \sum_{i=1}^{n} \EE{ S_{Cl} }{\omega_i( S_{Cl} )^2} \norm{\vx_i}^2
	+ \norm{\sum_{i=1}^{n}p_i \vx_i }^2 
	- \sum_{i=1}^{n}p_i^2 \norm{ \vx_i }^2 
	\nonumber\\
	&- \frac{1}{m^2} \sum_{k=1}^m \left[\norm{\sum_{i=1}^{n}r_{k, i} \vx_i }^2 
	- \sum_{i=1}^{n} r_{k, i}^2 \norm{ \vx_i }^2 \right]
	\label{app:eq:U2}
	\end{align}
	
	With rearrangements and using equation (\ref{app:eq:clustered_prop}) we get:
	\begin{align}
	\EE{ S_{Cl} }{\norm{\sum_{i=1}^{n}\omega_i( S_{Cl} )\vx_i}^2} 
	& = \sum_{i=1}^{n} \left[ \VAR{\omega_i( S_{Cl} )} + \frac{1}{m^2}\sum_{k=1}^m r_{k, i}^2 \right] \norm{\vx_i}^2
	+ \norm{\sum_{i=1}^{n}p_i \vx_i }^2 
	\nonumber\\
	&- \frac{1}{m^2} \sum_{k=1}^m \norm{\sum_{i=1}^{n}r_{k, i} \vx_i }^2 
	\label{app:eq:U3}
	\end{align}
	
	Using the expression of clustered sampling variance, equation (\ref{app:eq:T2}), for the first term and using Jensen inequality on the third term completes the proof. Jensen inequality is an equality if and only if $\sum_{i=1}^{n} r_{k, i} \vx_i = \sum_{j=1}^{n} r_{k, j} \vx_j$.
%	\begin{align}
%	\EE{S_t}{\norm{\sum_{i=1}^{n}\omega_i(S_t)\vx_i}^2} 
%	& = \frac{1}{m}\sum_{i=1}^{n} p_i \norm{\vx_i}^2
%	+ \norm{\sum_{i=1}^{n}p_i \vx_i }^2 
%	- \frac{1}{m^2} \sum_{k=1}^m \norm{\sum_{i=1}^{n}r_{k, i} \vx_i }^2 
%	\label{app:eq:U4}
%	\end{align}
%	Substituting equation (\ref{app:eq:AA5}) in equation (\ref{app:eq:AA4}) completes the proof.
	
\end{proof}



%\input{tex/coro_decomposition_theorem}

==> delayed_proofs/proof_based_Wang.tex <==
\newpage
\section{FL Convergence}\label{app:sec:convergence_Wang}

Our work is made possible thanks to the one of \cite{FedNova}. We use their developed theoretical framework to prove Theorem \ref{theo:convergence_paper}. The focus of our work (and Theorem \ref{theo:convergence_paper}) is on FedAvg. Yet, the proof devised in this section, like in \cite{FedNova}, keeps $a_i$ which can account for a wide-range of regularization method on FedAvg or optimizer different of the Vanilla SGD one. This proof can easily be extended to account for different amount of local work from the clients \citep{FedNova}. 

Before diving in the proof of Theorem \ref{theo:convergence_paper} in Section \ref{app:sec:proof_convergence}, we introduce the notation we use in Section \ref{app:sec:notation}, some useful lemmas in Section \ref{app:sec:lemmas} and Theorem \ref{theo:intermediary} generalizing Theorem \ref{theo:convergence_paper} in Section \ref{app:sec:intermediary_theo}.



%\subsection{Notations}\label{app:sec:notation}
%We define by $\vy_{i, k}^n$ the local model of client $i$ after $k$ SGD initialized on $\vtheta^n$ which enables us to also define the normalized stochastic gradients $\vs_i^n$ and the normalized gradient $\vDelta_i^n$ defined as
%\begin{equation}
%\vs_i^n = \frac{1}{a_i} \sum_{k=0}^{K-1} a_{i,k} g_i(\vy_{i, k}^n)
%\text{ and }
%\vDelta_i^n = \frac{1}{a_i} \sum_{k=0}^{K-1} a_{i, k} \nabla \Lcal_i (\vy_{i, k}^n),
%\label{app:eq:formalism_sum_grad}
%\end{equation}
%where $a_{i, k}$ is an arbitrary scalar set by the client to its $k$th computed gradient, $\va_i = [a_{i, 0}, .., a_{i, K -1}]^T$, and $a_i = \norm{\va_i}_1$. In the special case of FedAvg, we have $\va_i = [1, ..., 1]$ and in the one of FedProx, we have $\va_i = [(1 - \mu)^{K-1}, ..., 1]$ where $\mu$ is the FedProx regularization parameter. 
%
%With the formalism in equation (\ref{app:eq:formalism_sum_grad}), we can express a client contribution as $\theta_i^{n+1} - \vtheta^n  = - \eta_l a_i \vs_i^n $ and rewrite the server aggregation scheme defined in equation (\ref{eq:aggreg_SCAFFOLD_general}) as 
%\begin{align}
%\vtheta^{n+1} - \vtheta^n  
%&= - \eta_g \eta_l \sum_{i=1}^M\omega_i(n) a_i \vs_i^{\rho_i(n)}
%%	& = - \tilde{\eta} \underbrace{\left(\sum_{i=1}^M\omega_i(n) a_i \right)}_{K_{eff}} \sum_{i=1}^M \underbrace{\left(\frac{\omega_i(n) a_i}{\sum_{i=1}^M\omega_i(n) a_i}\right)}_{w_i} \vs_i^n\\
%,
%\end{align}
%which in expectation over the set of sampled clients $S_n$ gives
%\begin{align}
%\EE{S_n}{\vtheta^{n+1} - \vtheta^n}  
%&= - \tilde{\eta} \sum_{i=1}^M q_i(n) a_i \vs_i^n
%\\
%& = - \tilde{\eta} \underbrace{\left(\sum_{i=1}^M q_i(n) a_i \right)}_{K_{eff}} \sum_{i=1}^M \underbrace{\left(\frac{q_i(n) a_i}{\sum_{i=1}^M q_i(n) a_i}\right)}_{q_i(n)} \vs_i^{\rho_i(n)}
%\label{app:eq:expected_client_contrib}
%\end{align}
%
%We define the surrogate objective $\Lcal^n(\vx) = \sum_{i=1}^M q_i(n) \Lcal_i(\vx)$, where $\sum_{i=1}^Mq_i(n) =1 $. 
%
%In what follows, for $\va_i$ we specify the norm used can either be L1, $\norm{\cdot}_1$, or L2, $\norm{\cdot}_2$, For other variables the norm is always the euclidean  one and $\norm{\cdot}$ is used instead of $\norm{\cdot}_2$. Also, regarding the client sampling metrics, for ease of writing, due to the independence of the client sampling statistics with the current optimization round we use $\omega_i(n)$ instead of $\omega_i(S_n)$.


\begin{align}
\EE{S_n}{\vtheta^{n+1} - \vtheta^n}  
&= - \tilde{\eta} \sum_{i=1}^M q_i(n) \Delta_i^n
%\\
%& = - \tilde{\eta} \underbrace{\left(\sum_{i=1}^M q_i(n) a_i \right)}_{K_{eff}} \sum_{i=1}^M \underbrace{\left(\frac{q_i(n) a_i}{\sum_{i=1}^M q_i(n) a_i}\right)}_{q_i(n)} \vs_i^{\rho_i(n)}
\label{app:eq:expected_client_contrib}
\end{align}



%
%\subsection{Useful Lemmas}\label{app:sec:lemmas}
%
%
%
%\begin{lemma}\label{lem:decompo_Xi}
%	Let us consider $n$ vectors $\vx_i, ..., \vx_n$ and a client sampling satisfying $\EE{S_n}{\omega_i(n)} = \mathbb{P}( T_i^n \le \Delta t^{n+1}) d_i^2(n)$ and $\EE{S_n}{\omega_i(n)\omega_j(n)} = - R_i(n) R_j(n) p_i p_j$. We have:
%	\begin{equation}
%	\EE{S_n}{\norm{\sum_{i=1}^M\omega_i(n)\vx_i}^2} 
%	= \sum_{i=1}^M \gamma_i(n) \norm{\vx_i}^2
%	+ \norm{\sum_{i=1}^MR_i(n)d_i(n) \vx_i}^2
%	\end{equation}
%	where $\gamma_i(n)=  \left[ \mathbb{P}( T_i^n \le \Delta t^n) -R_i^2(n) \right] d_i^2(n)$.
%\end{lemma}
%
%
%\begin{proof}
%	\begin{align}
%	\EE{S_n}{\norm{\sum_{i=1}^M\omega_i(n)\vx_i}^2} 
%	& = \sum_{i=1}^M \EE{S_n}{\omega_i^2(n)} \norm{\vx_i}^2
%	+ \sum_{i=1}^M\sum_{\substack{j=1\\ j\neq i}}^M\EE{S_n}{\omega_i(n)\omega_j(n)}\inner{\vx_i}{\vx_j}
%	\\
%	& = \sum_{i=1}^M \mathbb{P}( T_i^n \le \Delta t^n) d_i^2(n) \norm{\vx_i}^2 
%	+ \sum_{i, j \neq i}^M R_i(n) d_i(n) R_j(n) d_j(n) \inner{\vx_i}{\vx_j}
%	\label{app:eq:AA1}
%	\end{align}
%	In addition, we have:
%	\begin{equation}
%	\sum_{i=1}^M\sum_{\substack{j=1\\ j\neq i}}^M\inner{R_i(n)d_i(n) \vx_i}{R_j(n) d_j(n) \vx_j} 
%	= \norm{\sum_{i=1}^M R_i(n) d_i(n) \vx_i}^2 - \sum_{i=1}^MR_i^2(n) d_i^2(n) \norm{\vx_i}^2
%	\label{app:eq:AA3}
%	\end{equation}
%	Substituting equation (\ref{app:eq:AA3}) in equation (\ref{app:eq:AA1}) completes the proof.
%\end{proof}
%
%
%
%\begin{lemma}[\cite{OnTheImpact}]\label{lem:dif_grads}
%	Under Assumptions \ref{ass:unbiased} to \ref{ass:dissimilarity}, we can prove
%	\begin{align}
%%		\frac{1}{2}\sum_{i=1}^M q_i(n) 
%		\E{\norm{\nabla \Lcal_i(\vtheta^n) - \vDelta_i^n}^2}
%		&\le \frac{\eta_l^2 L^2 \sigma^2}{1 -R} 
%		\left( \norm{\va_i}_2^2 - a_{i, -1}^2\right)
%%		\nonumber\\
%%		&
%		+ \frac{R \beta^2 }{1 - R}\E{\norm{\nabla \Lcal^n(\vtheta^n)}^2}
%		+ \frac{R \kappa^2 }{ 1 -R},
%	\end{align}
%	with $R = 2 \eta_l^2 L^2 \max_{i}\{\norm{\va_i}_1 (\norm{\va_i}_1 - a_{i, -1})\}$ with a learning rate such that $R < 1$.
%	
%	\begin{align}
%	%		\frac{1}{2}\sum_{i=1}^M q_i(n) 
%	\E{\norm{\nabla \Lcal_i(\vtheta^n) - \vDelta_i^n}^2}
%	&\le \frac{3}{2}\eta_l^2 L^2 \sigma^2
%	\left( \norm{\va_i}_2^2 - a_{i, -1}^2\right)
%	%		\nonumber\\
%	%		&
%%	+ \frac{R \beta^2 }{1 - R}\E{\norm{\nabla \Lcal^n(\vtheta^n)}^2}
%	+ \frac{1}{2} \kappa^2 ,
%	\end{align}
%	
%	\begin{equation}
%	\E{\norm{\nabla \Lcal_i(\vtheta^n) - \vDelta_i^n}^2}
%	\le
%		L^2 \eta_l^2 \left[ \left(\norm{a_i}_2^2 - a_{i, -1}^2\right) \sigma^2 
%		+  a_i \left( a_i - a_{i, -1} \right) \kappa^2 \right]
%	\end{equation}
%\end{lemma}
%
%\begin{proof}
%	\begin{align}
%		\E{\norm{\nabla \Lcal_i(\vtheta^n) - h_i^n}^2}
%		& = \E{\norm{\frac{1}{a_i} \sum_{ k = 0 }^{K-1} a_{i, k} \left(\nabla \Lcal_i(\vtheta^n) - \nabla \Lcal_i(\vy_{i, k}^n)\right)}^2}
%		\\
%		& \le \frac{1}{a_i} \sum_{ k = 0 }^{K-1} a_{i, k}  \E{\norm{\nabla \Lcal_i(\vtheta^n) - \nabla \Lcal_i(\vy_{i, k}^n )}^2}
%		\\
%		& \le L^2 \frac{1}{a_i} \sum_{ k = 0 }^{K-1} a_{i, k}  \E{\norm{\vtheta^n - \vy_{i, k}^n }^2}
%		\label{app:eq:Q1}
%	\end{align}
%	
%	We also have:
%	\begin{align}
%		\E{\norm{\vtheta^n - \vy_{i, k}^n }^2}
%		& = \eta_l^2 \E{\norm{\sum_{s=0}^{k-1} a_{i, s} g_i(\vy_{i, s}^n)}^2}
%		\\
%		& = \eta_l^2 \left[ \E{\norm{\sum_{s=0}^{k-1} a_{i, s} \left(g_i(\vy_{i, s}^n) - \nabla \Lcal_i(\vy_{i, s}^n)\right)}^2}
%		+  \E{\norm{\sum_{s=0}^{k-1} a_{i, s} \nabla \Lcal_i(\vy_{i, s}^n)}^2}\right]
%		\\
%		& \le \eta_l^2 \left[ \sum_{s=0}^{k-1} a_{i, s}^2 \sigma^2 
%		+  \left( \sum_{s=0}^{k-1} a_{i, s}\right)^2 \kappa^2 \right]
%		\\
%		& \le \eta_l^2 \left[ \left(\norm{a_i}_2^2 - a_{i, -1}^2\right) \sigma^2 
%		+  a_i \left( a_i - a_{i, -1} \right) \kappa^2 \right]
%		\label{app:eq:Q2}
%	\end{align}
%	
%	Plugging equation (\ref{app:eq:Q2}) in equation (\ref{app:eq:Q1}) completes the proof.
%\end{proof}
%
%
%%\begin{proof}
%%	The proof is in Section C.5 of \cite{FedNova}.
%%	
%%	The bound provided here is slightly tighter in term of numerical constants than \cite{FedNova}. Indeed, equation (70) in \cite{FedNova} uses the Jensen inequality $\norm{ \va + \vb}^2 \le 2 \norm{\va}^2 + 2 \norm{\vb}^2$ which could instead be obtained with:
%%	\begin{equation}
%%		\E{\norm{\sum_{s=0}^{k-1}a_{i,s} g_i(\vy_{i, s}^n)}^2}
%%		= \E{\norm{\sum_{s=0}^{k-1}a_{i,s} \left(g_i(\vy_{i, s}^n ) - \nabla \Lcal_i(\vy_{i, s}^n) \right)}^2}
%%		+ \E{\norm{\sum_{s=0}^{k-1}a_{i,s} \nabla \Lcal_i(\vy_{i, s}^n)}^2},
%%	\end{equation}
%%	which uses Assumption \ref{ass:unbiased} giving $\E{\inner{\sum_{s=0}^{k-1}a_{i,s} \left(g_i(\vy_{i, s}^n ) - \nabla \Lcal_i(\vy_{i, s}^n )\right)}{\sum_{s=0}^{k-1}a_{i,s} \nabla \Lcal_i(\vy_{i, s}^n )}} = 0$ with the same reasoning as for $U$ in equation(\ref{app:eq:B2}).
%%\end{proof}
%
%
%
%
%
%\begin{lemma}[\cite{OnTheImpact}]\label{lem:contrib_client_sampling}
%	Under Assumptions \ref{ass:unbiased} to \ref{ass:dissimilarity}, we can prove
%	\begin{align}
%	\E{\norm{ a_i \vDelta_i^{n}}^2}
%	&\le \frac{1}{1 - R}  \left(\norm{\va_i}_2^2 - (a_{i, -1}^2) \right) \sigma^2 
%	+ 2  \left[ L^2 \frac{R}{1 - R} +1 \right] a_i^2 \left(\beta^2 \E{\norm{\nabla  \Lcal^n (\vtheta^n)}^2} + \kappa^2 \right)
%	%	\label{app:eq:C5}
%	\end{align}
%	where $2 \eta_l^2 L^2 \max_i \{ \norm{a_i}_1^2 \} <1$.
%%	 $R' = 2 \eta_l^2 L^2 \max_i \{ \norm{a_i}_1^2 \} <1$.
%
%	\begin{align}
%	\E{\norm{ a_i \vDelta_i^{n}}^2}
%	&\le \frac{3}{2}  \left(\norm{\va_i}_2^2 - (a_{i, -1}^2) \right) \sigma^2 
%	+ \left[ L^2 + 2\right] a_i^2 \kappa^2 
%	%	\label{app:eq:C5}
%	\end{align}
%	
%\end{lemma}
%
%\begin{proof}
%	Due to the definition of $\vDelta_i^n$, we have:
%	\begin{align}
%	\E{\norm{ \vDelta_i^{n}}^2}
%	= \E{\norm{\sum_{k=0}^{K-1} \frac{1}{a_i} a_{i, k} \nabla \Lcal_i (\vy_{i, k}^{n})}^2}
%	\le \sum_{k=0}^{K-1}\frac{1}{a_i} a_{i, k} \E{\norm{\nabla \Lcal_i (\vy_{i, k}^{n})}^2}
%	\le \kappa^2
%	,
%	\label{app:eq:C1}
%	\end{align}
%	where the first inequality comes from using Jensen inequality and the second inequality from using Assumption 
%	XX.
%\end{proof}
%
%
%%\begin{proof}
%%	Due to the definition of $\vDelta_i^n$, we have:
%%	\begin{align}
%%	\E{\norm{ a_i \vDelta_i^{\rho_i(n)}}^2}
%%	& = a_i^2 \E{\norm{\sum_{k=0}^{K-1} \frac{1}{a_i} a_{i, k} \nabla \Lcal_i (\vy_{i, k}^{\rho_i(n)})}^2}\\
%%	&\le a_i^2 \sum_{k=0}^{K-1}\frac{1}{a_i} a_{i, k} \E{\norm{\nabla \Lcal_i (\vy_{i, k}^{\rho_i(n)})}^2}
%%	\label{app:eq:C1}
%%	\end{align}
%%	
%%	Using Jensen inequality, we have
%%	\begin{align}
%%	\E{\norm{\nabla \Lcal_i (\vy_{i, k}^{\rho_i(n)})}^2}
%%	&\le 2 \E{ \norm{\nabla \Lcal_i (\vy_{i, k}^n) - \nabla \Lcal_i (\vtheta^n)}^2}
%%	+ 2 \E{\norm{\nabla \Lcal_i (\vtheta^n)}^2}\\
%%	&\le 2 L^2 \E{ \norm{ \vy_{i, k}^n - \vtheta^n}^2}
%%	+ 2 \E{\norm{\nabla \Lcal_i (\vtheta^n)}^2},
%%	\label{app:eq:C2}
%%	\end{align}
%%	where the second equality comes from using Assumption \ref{ass:smoothness}.
%%	
%%	Also, Section C.5 of \cite{FedNova} proves
%%	\begin{equation}
%%	\frac{1}{a_i} \sum_{k=0}^{K-1} a_{i, k}\E{ \norm{ \vy_{i, k}^n - \vtheta^n}^2}
%%	\le \frac{1}{1 - R}\eta_l^2 \sigma^2 \left(\norm{\va_i}_2^2 - (a_{i, -1}^2) \right)
%%	+ \frac{R}{1 - R} \E{\norm{\nabla \Lcal_i (\vtheta^n)}^2}
%%	.
%%	\label{app:eq:C3}
%%	\end{equation}
%%	
%%	Plugging equation (\ref{app:eq:C2}) and then equation (\ref{app:eq:C3}) in equation (\ref{app:eq:C1}), we get:
%%	\begin{align}
%%	\E{\norm{ a_i \vDelta_i^{\rho_i(n)}}^2}
%%	&\le a_i^2 \sum_{k=0}^{K-1}\frac{1}{a_i} a_{i, k} \left[2 L^2 \E{ \norm{ \vy_{i, k}^n - \vtheta^n}^2}
%%	+ 2 \E{\norm{\nabla \Lcal_i (\vtheta^n)}^2}\right]
%%	\\
%%	&= 2 L^2  a_i^2 \sum_{k=0}^{K-1}\frac{1}{a_i} a_{i, k}  \E{ \norm{ \vy_{i, k}^n - \vtheta^n}^2}
%%	+ 2 a_i^2 \E{\norm{\nabla \Lcal_i (\vtheta^n)}^2}
%%	\\
%%	&\le 2 L^2  a_i^2 \left[\frac{1}{1 - R}\eta_l^2 \sigma^2 \left(\norm{\va_i}_2^2 - (a_{i, -1}^2) \right)
%%	+ \frac{R}{1 - R} \E{\norm{\nabla \Lcal_i (\vtheta^n)}^2}\right]
%%	\nonumber\\
%%	&+ 2 a_i^2 \E{\norm{\nabla \Lcal_i (\vtheta^n)}^2}
%%	\\
%%	&\le \frac{R'}{1 - R} \sigma^2 \left(\norm{\va_i}_2^2 - (a_{i, -1}^2) \right)
%%	+ 2 a_i^2 \left[ L^2 \frac{R}{1 - R} +1 \right] \E{\norm{\nabla \Lcal_i (\vtheta^n)}^2}
%%	\label{app:eq:C4}
%%	\end{align}
%%	
%%	Summing over $M$ gives
%%	\begin{align}
%%	\sum_{i=1}^M \gamma_i(n) \E{\norm{ a_i \vDelta_i^{\rho_i(n)}}^2}
%%	&\le 2 L^2 \frac{1}{1 - R}\eta_l^2 \sigma^2 \sum_{i=1}^M \gamma_i(n) a_i^2\left(\norm{\va_i}_2^2 - (a_{i, -1}^2) \right)
%%	\nonumber\\
%%	&+ 2  \left[ L^2 \frac{R}{1 - R} +1 \right] \sum_{i=1}^M\gamma_i(n) a_i^2 \E{\norm{\nabla \Lcal_i (\vtheta^n)}^2}
%%	\label{app:eq:C5}
%%	\end{align}
%%	
%%	Using Assumption \ref{ass:dissimilarity} in equation (\ref{app:eq:C5}) and $R' < 1$ completes the proof.	
%%	
%%\end{proof}
%
%
%
%
%
%
%
\begin{lemma}\label{lem:delta_n}
	\begin{align}
	\Delta^n
	\coloneqq \E{\norm{\vtheta^{n+1} - \vtheta^n}^2}
	\le \tilde{\eta}^2 \alpha(n) \sigma^2
	+\tilde{\eta}^2 \beta(n)
	+\tilde{\eta}^2 U^2 K_{eff}^2 \Gamma(n)
	.
	\end{align}
	where $\alpha(n) = \sum_{i=1}^M \E{\omega_i^2(n)} \norm{\va_i}_2^2$, $\beta(n) = \sum_{i=1}^M \gamma_i(n) \E{\norm{ a_i \vDelta_i^{\rho_i(n)}}^2}$, and $\Gamma(n) =  \E{\norm{\sum_{i=1}^M q_i(n)\vDelta_i^{\rho_i(n)} }^2}$.
\end{lemma}
%
%\begin{proof}
%	
%	\begin{align}
%	\Delta^n 
%	& = \tilde{\eta}^2 \E{\norm{\sum_{i=1}^M \omega_i(n) a_i \vs_i^{\rho_i(n)}}^2}
%	\\
%	& = \tilde{\eta}^2 \E{\norm{\sum_{i=1}^M \omega_i(n) a_i \left(\vs_i^{\rho_i(n)} - \vDelta_i^{\rho_i(n)}\right) 
%			+ \sum_{i=1}^M \omega_i(n) a_i \vDelta_i^{\rho_i(n)}}^2}
%	\\
%	& = \tilde{\eta}^2 \E{\norm{\sum_{i=1}^M \omega_i(n) a_i \left(\vs_i^{\rho_i(n)} - \vDelta_i^{\rho_i(n)}\right) }^2 }
%	+\tilde{\eta}^2 \E{\norm{\sum_{i=1}^M \omega_i(n) a_i \vDelta_i^{\rho_i(n)}}^2}
%	\nonumber\\
%	& + 2 \tilde{\eta} \underbrace{\E{\inner{\sum_{i=1}^M \omega_i(n) a_i \left(\vs_i^{\rho_i(n)} - \vDelta_i^{\rho_i(n)}\right)}{\sum_{i=1}^M \omega_i(n) a_i \vDelta_i^{\rho_i(n)}}}}_V
%	.
%	\label{app:eq:B2}
%	\end{align}
%	Using Assumption \ref{ass:unbiased}, we have $\E{\inner{g_i(\vy_{i, k}^n) - \nabla \Lcal^n(\vy_{i, k}^n) }{\nabla \Lcal^n(\vy_{i, k}^n)}} = 0$. Hence, we get $V=0$ and can simplify $\Delta^n$ as: 
%	\begin{align}
%	\Delta^n
%	& = \tilde{\eta}^2 \sum_{i=1}^M \E{\omega_i^2(n)} a_i^2\E{\norm{ \vs_i^{\rho_i(n)} - \vDelta_i^{\rho_i(n)} }^2 }
%	+\tilde{\eta}^2 \E{\norm{\sum_{i=1}^M \omega_i(n) a_i \vDelta_i^{\rho_i(n)}}^2}
%	.
%	\label{app:eq:B3}
%	\end{align}
%	
%	Using Lemma \ref{lem:decompo_Xi} on the second term, we get:
%	\begin{align}
%	\Delta^n
%	& = \tilde{\eta}^2 \sum_{i=1}^M \E{\omega_i^2(n)} a_i^2\E{\norm{ \vs_i^{\rho_i(n)} - \vDelta_i^{\rho_i(n)} }^2 }
%	\nonumber\\
%	&+\tilde{\eta}^2 \sum_{i=1}^M \gamma_i(n) \E{\norm{ a_i \vDelta_i^{\rho_i(n)}}^2}
%	+\tilde{\eta}^2 \E{\norm{\sum_{i=1}^M R_i(n)d_i(n) a_i \vDelta_i^{\rho_i(n)} }^2}
%	.
%	\label{app:eq:B4}
%	\end{align} 
%	We can bound the first term using Assumption \ref{ass:unbiased}
%%	 and the second term with Lemma \ref{lem:contrib_client_sampling}
%	 . Also, using Assumption \ref{ass:clients_covariance} and the definition of $q_i(n)$, we can rewrite the third term as$\E{\norm{\sum_{i=1}^M R_i(n)d_i(n) a_i \vDelta_i^n}^2} = U^2 K_{eff}^2 \E{\norm{\sum_{i=1}^M q_i(n) \vDelta_i^n}^2}$. Hence, we have:
%	\begin{align}
%	\Delta^n
%	& = \tilde{\eta}^2 \sum_{i=1}^M \E{\omega_i^2(n)} \sum_{k=0}^{K-1} a_{i, k}^2 \E{\norm{ g_i(\vy_{i, k}^n) - \nabla \Lcal_i(\vy_{i, k}^n) }^2 }
%	\nonumber\\
%	&+\tilde{\eta}^2 \sum_{i=1}^M \gamma_i(n) \E{\norm{ a_i \vDelta_i^{\rho_i(n)}}^2}
%	+\tilde{\eta}^2 U^2 K_{eff}^2\E{\norm{\sum_{i=1}^M q_i(n)\vDelta_i^{\rho_i(n)} }^2}
%	\\
%	& \le \tilde{\eta}^2 \sum_{i=1}^M \E{\omega_i^2(n)} \norm{\va_i}_2^2 \sigma^2
%	+\tilde{\eta}^2 \sum_{i=1}^M \gamma_i(n) \E{\norm{ a_i \vDelta_i^{\rho_i(n)}}^2}
%	\nonumber\\
%	&
%	+\tilde{\eta}^2 U^2 K_{eff}^2\E{\norm{\sum_{i=1}^M q_i(n)\vDelta_i^{\rho_i(n)} }^2}
%	.
%	\label{app:eq:B5}
%	\end{align}
%\end{proof}
%
%
%
%\begin{lemma}\label{lem:dif_grads_async}
%	Under Assumptions \ref{ass:unbiased} to \ref{ass:dissimilarity}, we can prove
%	\begin{align}
%	\sum_{ i = 1 }^M q_i(n) \E{ \norm{\nabla \Lcal_i(\vtheta^n) - \vDelta_i^{\rho_i(n)}}^2}
%	& \le  \tilde{\eta}^2 L^2  (\tau+1) \sum_{s=1}^{H}
%	\left[ \alpha(n) \sigma^2
%	+\beta(n)
%	+U^2 K_{eff}^2 \Gamma(n) \right] 
%	\nonumber\\
%	&+ (\tau+1) 
%	\eta_l^2 \left[ \left(\norm{a_i}_2^2 - a_{i, -1}^2\right) \sigma^2 
%	+  a_i \left( a_i - a_{i, -1} \right) \kappa^2 \right]
%	.
%	\end{align}	
%	with $\Delta^n = \E{\norm{\vtheta^{n+1} - \vtheta^n}^2}$.
%	
%	with $R = 2 \eta_l^2 L^2 \max_{i}\{\norm{\va_i}_1 (\norm{\va_i}_1 - a_{i, -1})\}$ with a learning rate such that $R < 1$.
%\end{lemma}
%
%
%\begin{proof}
%	We note that we have:
%	\begin{align}
%		&\norm{\nabla \Lcal_i(\vtheta^n) - \vDelta_i^{\rho_i(n)}}^2
%		\nonumber\\
%		& = \norm{\sum_{s=0}^{n - \rho_i(n) -1 } \left[ \nabla \Lcal_i(\vtheta^{\rho_i(n)+ s + 1}) - \nabla \Lcal_i(\vtheta^{\rho_i(n) + s})\right] + \left[\nabla \Lcal_i(\vtheta^{\rho_i(n)}) - \vDelta_i^{\rho_i(n)}\right]}^2		
%		\nonumber\\
%		& \le (H +1 ) \sum_{s=0}^{n - \rho_i(n) -1 } \norm{ \nabla \Lcal_i(\vtheta^{\rho_i(n)+ s + 1}) - \nabla \Lcal_i(\vtheta^{\rho_i(n) + s})}^2 
%		+ (\tau+1)\norm{ \nabla \Lcal_i(\vtheta^{\rho_i(n)}) - \vDelta_i^{\rho_i(n)} }^2	
%		\nonumber\\
%		& \le (\tau+1) L^2  \sum_{s=0}^{n - \rho_i(n) -1 } \norm{ \vtheta^{\rho_i(n)+ s + 1} - \vtheta^{\rho_i(n) + s}}^2 
%		+ (\tau+1) \norm{ \nabla \Lcal_i(\vtheta^{\rho_i(n)}) - \vDelta_i^{\rho_i(n)} }^2	
%		,
%	\end{align}
%	where the first inequality comes from using Jensen inequality and the second inequality from using Assumption \ref{ass:smoothness}.
%	
%	Taking the expectation gives
%	\begin{align}
%	\E{\norm{\nabla \Lcal_i(\vtheta^n) - \vDelta_i^{\rho_i(n)}}^2}
%	\le  L^2  (\tau+1) \sum_{s=1}^{H} \Delta^{n - s} 
%	+ (\tau+1) \left[ \left(\norm{a_i}_2^2 - a_{i, -1}^2\right) \sigma^2 
%	+  a_i \left( a_i - a_{i, -1} \right) \kappa^2 \right]
%	,
%	\end{align}	
%	which with reordering completes the proof.
%	
%	
%	
%	Using Lemma \ref{lem:delta_n} and Lemma \ref{lem:dif_grads} yields, 
%	\begin{align}
%	\E{ \norm{\nabla \Lcal_i(\vtheta^n) - \vDelta_i^{\rho_i(n)}}^2}
%%	&\le  L^2  (\tau+1) \sum_{s=1}^{H} \Delta^{n - s} 
%%	+ (\tau+1) \E{ \norm{ \nabla \Lcal_i(\vtheta^{\rho_i(n)}) - \vDelta_i^{\rho_i(n)} }^2 }
%%	\\
%	& \le  \tilde{\eta}^2 L^2  (\tau+1) \sum_{s=1}^\tau
%	\left[ \alpha(n) \sigma^2
%	+\beta(n)
%	+U^2 K_{eff}^2 \Gamma(n) \right] 
%	\nonumber\\
%	&+ (\tau+1) 
%	\left[\frac{\eta_l^2 L^2 \sigma^2}{1 -R} 
%	\left( \norm{\va_i}_2^2 - a_{i, -1}^2\right)
%	+ \frac{1}{2}\E{\norm{\nabla \Lcal^n(\vtheta^{\rho_i(n)})}^2}
%	+ \frac{1}{2} \kappa^2  \right]
%	.
%	\end{align}	
%	
%	If we assume that $R \le \frac{1}{2 \beta^2 +1}$ and considering that $\beta^2 \ge 1$, then we have $\frac{1}{1 - R} \le 1 + \frac{1}{2 \beta^2}\le \frac{3}{2}$, $\frac{R}{1-R} \le \frac{1}{2}$ , $\frac{R \beta^2}{1 -R} \le \frac{1}{2 \beta^2 + 1} (1 + \frac{1}{2 \beta^2})\beta^2 = \frac{1}{2}$, and $1 - \frac{R \beta^2}{1 - R} \ge \frac{1}{2}$, which gives:
%	%	 We also define $\Omega = L \tilde{\eta} \frac{1}{K_{eff}}   \left[ L^2  + 2 \right] \left(\sum_{i=1}^M\gamma_i(n)a_i^2\right)\beta^2 \le \frac{1}{2}$. Plugging all these components in equation (\ref{app:eq:B66}) gives
%	\begin{align}
%	\E{ \norm{\nabla \Lcal_i(\vtheta^n) - \vDelta_i^{\rho_i(n)}}^2}
%	%	&\le  L^2  (\tau+1) \sum_{s=1}^{H} \Delta^{n - s} 
%	%	+ (\tau+1) \E{ \norm{ \nabla \Lcal_i(\vtheta^{\rho_i(n)}) - \vDelta_i^{\rho_i(n)} }^2 }
%	%	\\
%	& \le  \tilde{\eta}^2 L^2  (\tau+1) \sum_{s=1}^{H}
%	\left[ \alpha(n) \sigma^2
%	+\beta(n)
%	+U^2 K_{eff}^2 \Gamma(n) \right] 
%	\nonumber\\
%	&+ (\tau+1) 
%	\eta_l^2 \left[ \left(\norm{a_i}_2^2 - a_{i, -1}^2\right) \sigma^2 
%	+  a_i \left( a_i - a_{i, -1} \right) \kappa^2 \right]
%	.
%	\end{align}	
%	
%	Taking the summation over $M$ completes the proof.	
%
%	
%	
%	
%\end{proof}
%







\subsection{Intermediary Theorem}\label{app:sec:intermediary_theo}

%\begin{theorem}\label{theo:intermediary}
%\begin{align}
%\frac{1}{T}\sum_{t=0}^{T-1} \E{\norm{\nabla \Lcal^n(\vtheta^n)}^2}
%&\le \Ocal(\frac{1}{ ( 1 - \Omega) \tilde{\eta} \left(\sum_{i=1}^M p_i a_i\right) T}) 
%+ \Ocal (\tilde{\eta}A' \sigma^2\frac{1}{m})
%+ \Ocal( \eta_l^2 \sigma^2 B')
%\nonumber\\
%& + \Ocal (\eta_l^2 C' \kappa^2 )
%+ \Ocal(\tilde{\eta} D' \sigma^2)
%+ \Ocal(\tilde{\eta} E' \kappa^2)
%,
%\end{align}
%where $A$-$E$ are defined in the following proof from equation (\ref{app:eq:def_A}) to equation (\ref{app:eq:def_E}).
%\end{theorem}


\begin{proof}
$\Lcal^n$ is $L$-Lipschitz smooth, Assumption \ref{ass:smoothness}, which gives
\begin{equation}
	\E{\Lcal^n(\vtheta^{n+1}) - \Lcal^n(\vtheta^n)}
	\le \underbrace{\E{\inner{\nabla \Lcal^n(\vtheta^n)}{\vtheta^{n+1} - \vtheta^n}}}_{T_1}
	+ \frac{L}{2}\underbrace{\E{\norm{\vtheta^{n+1} - \vtheta^n }^2}}_{ T_2 }
%	\le \underbrace{\E{\inner{\nabla \Lcal^n(\vtheta^n)}{- \tilde{\eta} \sum_{i=1}^M \omega_i(n) a_i \vs_i^n}}}_{T_1}
%	+ \frac{L}{2}\underbrace{\E{\norm{\tilde{\eta}\sum_{i=1}^M\omega_ia_i \vs_i^n}^2}}_{T_2}
,
\label{app:eq:B1}
\end{equation}
where the expectation is taken over the subset of randomly sampled clients $S_n$ and the clients gradient estimator noises $\xi_i^n$ but we use $\E{\cdot}$ instead of $\EE{\{\xi_i^n\}, S_n}{\cdot}$ for ease of writing.


\subsubsection*{Bounding $T_1$}
By conditioning on $\{\xi_i^n \}$ and using equation (\ref{app:eq:expected_client_contrib}), we get:
\begin{equation}
	T_1 
	= \E{\inner{\nabla \Lcal^n(\vtheta^n)}{{\EE{S_n}{\vtheta^{n+1} - \vtheta^n}}}} 
	= - \tilde{\eta} \E{\inner{\nabla \Lcal^n(\vtheta^n)}{ \sum_{i=1}^M q_i(n) \vDelta_i^{\rho_i(n)}}},
\end{equation}
which, using $2 \inner{a}{b} = \norm{a}^2 + \norm{b}^2 - \norm{a - b}^2$ can be rewritten as:
\begin{equation}
T_1 
= - \frac{1}{2}\tilde{\eta} K \E{ \norm{\nabla \Lcal^n(\vtheta^n)}^2 
+ \norm{ \sum_{i=1}^M q_i(n) \frac{1}{K} \vDelta_i^{\rho_i(n)}}^2 
- \norm{\nabla \Lcal^n(\vtheta^n) -  \sum_{i=1}^M q_i(n) \frac{1}{K}\vDelta_i^{\rho_i(n)}}^2 } ,
\label{app:eq:BB1}
\end{equation}


\subsubsection*{Bounding $T_2$}

\begin{align}
	T_2 
	& = \tilde{\eta}^2 \E{\norm{\sum_{i=1}^M \omega_i(n) \left[\vtheta_i^{\rho_i(n)+1} - \vtheta^{\rho_i(n)}\right]}^2}
	\\
	& = \tilde{\eta}^2 \E{\norm{\sum_{i=1}^M \omega_i(n) \vxi_i^{\rho_i(n)}  
			+ \sum_{i=1}^M \omega_i(n) \vDelta_i^{\rho_i(n)}}^2|S_n}
	\\
	& = \tilde{\eta}^2 \sum_{i=1}^M \E{\omega_i^2(n)} \E{\norm{ \vxi^{\rho_i(n)} }^2 }
	+\tilde{\eta}^2 \E{\norm{\sum_{i=1}^M \omega_i(n) \vDelta_i^{\rho_i(n)}}^2}
%	\nonumber\\
%	& + 2 \tilde{\eta} \underbrace{\E{\inner{\sum_{i=1}^M \omega_i(n)  \left(\vs_i^{\rho_i(n)} - \vDelta_i^{\rho_i(n)}\right)}{\sum_{i=1}^M \omega_i(n) \vDelta_i^{\rho_i(n)}}}}_V
	.
	\label{app:eq:B2}
\end{align}
%Using Assumption \ref{ass:unbiased}, we have $\E{\inner{g_i(\vy_{i, k}^n) - \nabla \Lcal^n(\vy_{i, k}^n) }{\nabla \Lcal^n(\vy_{i, k}^n)}} = 0$. Hence, we get $V=0$ and can simplify $T_2$ as: 
%\begin{align}
%T_2 
%& = \tilde{\eta}^2 \sum_{i=1}^M \E{\omega_i^2(n)} a_i^2\E{\norm{ \vs_i^{\rho_i(n)} - \vDelta_i^{\rho_i(n)} }^2 }
%+\tilde{\eta}^2 \E{\norm{\sum_{i=1}^M \omega_i(n) a_i \vDelta_i^{\rho_i(n)}}^2}
%.
%\label{app:eq:B3}
%\end{align}
%
%
%Finally, by bounding the gradient estimators with Assumption \ref{ass:unbiased}, and noting that $p_i a_i = q_i(n)K_eff$. we get:
We note that $\E{\omega_i^2(n)} = \mathcal{P}(T_i^n \le \Delta t^n)d_i^2(n) = \nu_i(n)$. Therefore $\sum_{i=1}^M \E{\omega_i^2(n)}  = \nu(n)$.
Using Assumption \ref{ass:unbiased} on the first term and Lemma \ref{lem:decompo_Xi} on the second term, we get:
\begin{align}
T_2 
& = \tilde{\eta}^2 \left[ \nu(n) K \sigma^2
+  \sum_{i=1}^M \gamma_i(n) \E{\norm{ \vDelta_i^{\rho_i(n)}}^2}
+ U^2 \E{\norm{\sum_{i=1}^M q_i(n) \vDelta_i^{\rho_i(n)} }^2}
\right]
.
\label{app:eq:B4}
\end{align} 
%By  bounding the first term using Assumption \ref{ass:unbiased}, and noting that there exists $U$ such that $\E{\norm{\sum_{i=1}^M R_i(n)d_i(n) a_i \vDelta_i^n}^2} = U K_{eff}^2 \E{\norm{\sum_{i=1}^M q_i(n) \vDelta_i^n}^2}$ for the second term, we get:
%\begin{align}
%T_2 
%& = \tilde{\eta}^2 \sum_{i=1}^M \E{\omega_i^2(n)} \sum_{k=0}^{K-1} a_{i, k}^2 \E{\norm{ g_i(\vy_{i, k}^n) - \nabla \Lcal_i(\vy_{i, k}^n) }^2 }
%\nonumber\\
%&+\tilde{\eta}^2 \sum_{i=1}^M \gamma_i(n) \E{\norm{ a_i \vDelta_i^{\rho_i(n)}}^2}
%+\tilde{\eta}^2 U K_{eff}^2\E{\norm{\sum_{i=1}^M q_i(n)\vDelta_i^{\rho_i(n)} }^2}
%\\
%& \le \tilde{\eta}^2 \sum_{i=1}^M \E{\omega_i^2(n)} \norm{\va_i}_2^2 \sigma^2
%+\tilde{\eta}^2 \sum_{i=1}^M \gamma_i(n) \E{\norm{ a_i \vDelta_i^{\rho_i(n)}}^2}
%+\tilde{\eta}^2 U K_{eff}^2\E{\norm{\sum_{i=1}^M q_i(n)\vDelta_i^{\rho_i(n)} }^2}
%.
%\label{app:eq:B5}
%\end{align}


\subsubsection*{Going back to equation (\ref{app:eq:B1})}



Substituting equation (\ref{app:eq:BB1}) and equation (\ref{app:eq:B4})
%Lemma \ref{lem:delta_n} 
in equation (\ref{app:eq:B1}), we get:
\begin{align}
	\E{\Lcal^n(\vtheta^{n+1}) - \Lcal^n(\vtheta^n)}
	&\le - \frac{1}{2}\tilde{\eta} K \norm{\nabla \Lcal^n(\vtheta^n)}^2 
	+ \frac{1}{2}\tilde{\eta} K \E{\norm{\nabla \Lcal^n(\vtheta^n) -  \sum_{i=1}^M q_i(n) \frac{1}{K} \vDelta_i^{\rho_i(n)} }^2}
	\nonumber\\
	& - \frac{1}{2}\tilde{\eta} K \left[1 - L\tilde{\eta} U^2 K\right] \E{\norm{ \sum_{i=1}^M q_i(n) \frac{1}{K} \vDelta_i^{\rho_i(n)}}^2}
	\nonumber\\
	&+\frac{L}{2} \tilde{\eta}^2 \nu(n) K \sigma^2
	+ \frac{L}{2} \tilde{\eta}^2 \sum_{i=1}^M \gamma_i(n) \E{\norm{ \vDelta_i^{\rho_i(n)}}^2}
	,
	\label{app:eq:B55}
\end{align}
We consider that the local learning rate $\eta_l$ satisfies $1 - L\tilde{\eta} U^2 K>0$. Therefore, using Jensen inequality and with reordering equation (\ref{app:eq:B55}) can be simplified as
\begin{align}
\frac{\E{\Lcal^n(\vtheta^{n+1}) - \Lcal^n(\vtheta^n)}}{\frac{1}{2}\tilde{\eta} K}
&\le - \norm{\nabla \Lcal^n(\vtheta^n)}^2 
+ \sum_{i=1}^M q_i(n)\E{ \norm{\nabla \Lcal_i(\vtheta^n) -   \frac{1}{K}\vDelta_i^{\rho_i(n)}}^2}
\nonumber\\
%& - \frac{1}{2} \left[1 - L\tilde{\eta} U^2 K_{eff}\right] \Gamma(n)
%\nonumber\\
&+L \tilde{\eta} \nu(n) \sigma^2
+ L \tilde{\eta} \frac{1}{K} \sum_{i=1}^M \gamma_i(n) \E{\norm{ \vDelta_i^{\rho_i(n)}}^2}
.
\label{app:eq:B6}
\end{align}

Using Lemma \ref{lem:dif_grads} and \ref{lem:contrib_client_sampling}, we get:
\begin{align}
&\frac{\E{\Lcal^n(\vtheta^{n+1}) - \Lcal^n(\vtheta^n)}}{\tilde{\eta} K_{eff}}\\
&\le - \frac{1}{2}\norm{\nabla \Lcal^n(\vtheta^n)}^2 
+ \frac{1}{2}\tilde{\eta}^2 L^2  (\tau+1) \sum_{s=1}^{H}
\left[ \alpha(n) \sigma^2
+\beta(n)
+U^2 K_{eff}^2 \Gamma(n) \right] 
\nonumber\\
&
+ \frac{1}{2}(\tau+1) \eta_l^2 \left[ \left(\norm{a_i}_2^2 - a_{i, -1}^2\right) \sigma^2 
+  a_i \left( a_i - a_{i, -1} \right) \kappa^2 \right]
\nonumber\\
&
- \frac{1}{2}\left[1 - L\tilde{\eta} U^2 K_{eff}\right] \Gamma(n)
\nonumber\\
&+\frac{L}{2} \tilde{\eta} \frac{1}{K_{eff}} \sum_{i=1}^M \E{\omega_i^2(n)} \norm{\va_i}_2^2 \sigma^2
+ \frac{L}{2} \tilde{\eta} \frac{1}{K_{eff}} \sum_{i=1}^M \gamma_i(n) a_i^2 \kappa^2
.
\label{app:eq:B66}
\end{align}

We denote by $\bar{\alpha} = \frac{1}{N} \sum_{ n = 0 }^{N-1}\alpha(n)$. Hence, we have $\sum_{ n = 0 }^{N-1} \sum_{s=1}^\tau \alpha(n - s) \le \tau \bar{\alpha}$. We similarly define $\bar{\beta}$. Hence, by taking the average over $N$ rounds, we get:
\begin{align}
\frac{1}{N}\sum_{ n = 0 }^{N-1}\norm{\nabla \Lcal^n(\vtheta^n)}^2 
& \le 2 \frac{1}{N}\sum_{ n = 0 }^{N-1}\frac{\E{\Lcal^n(\vtheta^{n+1}) - \Lcal^n(\vtheta^n)}}{\tilde{\eta} K_{eff}}\\ 
&+ \tilde{\eta}^2 L^2  (\tau+1) 
\left[ \tau \bar{\alpha} \sigma^2
+ \bar{\beta} a_i^2 \kappa^2 
%+U^2 K_{eff}^2 \Gamma(n) 
\right] 
\nonumber\\
&
+ (\tau+1) \eta_l^2 \left[ \left(\norm{a_i}_2^2 - a_{i, -1}^2\right) \sigma^2 
+  a_i \left( a_i - a_{i, -1} \right) \kappa^2 \right]
\nonumber\\
&
- \frac{1}{N}\sum_{ n = 0 }^{N-1} \left[1 - L\tilde{\eta} U^2 K_{eff} + \tilde{\eta}^2 L^2 \tau (\tau+1) U^2 K_{eff}^2\right] \Gamma(n)
\nonumber\\
&+ L \tilde{\eta} \frac{1}{K_{eff}} \sum_{i=1}^M \E{\omega_i^2(n)} \norm{\va_i}_2^2 \sigma^2
+  L \tilde{\eta} \frac{1}{K_{eff}} \sum_{i=1}^M \gamma_i(n) a_i^2 \kappa^2
.
\label{app:eq:B66}
\end{align}




\begin{align}
\frac{\E{\Lcal^n(\vtheta^{n+1}) - \Lcal^n(\vtheta^n)}}{\tilde{\eta} K_{eff}}
&\le - \frac{1}{4}\left[1 - \Omega \right]\norm{\nabla \Lcal^n(\vtheta^n)}^2 
%	+ \norm{\sum_{i=1}^M q_i(n)\vDelta_i^n}^2 
+ \frac{3}{4} \eta_l^2 L^2 \sigma^2 \sum_{i=1}^M q_i(n)\left( \norm{\va_i}_2^2 - a_{i, -1}^2\right)
\nonumber\\
&+ \frac{3}{2}\eta_l^2 L^2\max_i\{a_i (a_i - a_{i, -1})\} \kappa^2 
\nonumber\\
&+\frac{L}{2} \tilde{\eta} \frac{1}{K_{eff}} \left[\sum_{i=1}^M \E{\omega_i^2(n)} \norm{\va_i}_2^2 
+ \frac{3}{2}\sum_{i=1}^M \gamma_i(n)\left(\norm{\va_i}_2^2 - (a_{i, -1}^2) \right)\right] \sigma^2
\nonumber\\
&+ L \tilde{\eta} \frac{1}{K_{eff}}   \left[  \frac{L^2}{2} +1 \right] \left(\sum_{i=1}^M\gamma_i(n)a_i^2\right)  \kappa^2
,
\end{align}


\subsection{Old}



Taking average across all rounds, we get:
\begin{align}
\frac{1 - \Omega}{T}\sum_{t=0}^{T-1} \E{\norm{\nabla \Lcal^n(\vtheta^n)}^2}
&\le 4   \frac{\Lcal^n(\theta^0) - \Lcal^n(\theta^*)}{\tilde{\eta} K_{eff}T} 
%	+ \norm{\sum_{i=1}^M q_i(n)\vDelta_i^n}^2 
+ 3 \eta_l^2 L^2 \sigma^2 \sum_{i=1}^M q_i(n)\left( \norm{\va_i}_2^2 - a_{i, -1}^2\right)
\nonumber\\
&+ 6\eta_l^2 L^2\max_i\{a_i (a_i - a_{i, -1})\} \kappa^2 
\nonumber\\
&+ L \tilde{\eta} \frac{1}{K_{eff}} \left[2 \sum_{i=1}^M \E{\omega_i^2(n)} \norm{\va_i}_2^2
+ 3  \sum_{i=1}^M \gamma_i(n)\left(\norm{\va_i}_2^2 - (a_{i, -1}^2) \right)\right] \sigma^2
\nonumber\\
&+ 4 L \tilde{\eta} \frac{1}{K_{eff}}   \left[ \frac{L^2}{2} +1 \right] \left(\sum_{i=1}^M\gamma_i(n)a_i^2\right)  \kappa^2
,
\end{align}


We define the following auxiliary variables
\begin{equation}
	A 
	= m \frac{1}{K_{eff}} \sum_{i=1}^M \E{\omega_i^2(n)} \norm{\va_i}_2^2 
	= m \frac{1}{\sum_{i=1}^Mp_i a_i} \sum_{i=1}^M \left[\VAR{\omega_i} + p_i^2\right] \norm{\va_i}_2^2 ,
	\label{app:eq:def_A}
\end{equation}

\begin{equation}
B
= \sum_{i=1}^M q_i(n)\left( \norm{\va_i}_2^2 - a_{i, -1}^2\right)
= \sum_{i=1}^M\frac{p_i a_i}{\sum_{j=1}^{n} p_j a _j}  \left( \norm{\va_i}_2^2 - a_{i, -1}^2\right)
,
\end{equation}

\begin{equation}
C
= \max_i\{a_i (a_i - a_{i, -1})\}
,
\end{equation}

\begin{equation}
D 
= \frac{1}{K_{eff}} \max_i\{a_i (a_i - a_{i, -1})\} \sum_{i=1}^M\gamma_i(n) 
= \frac{1}{\sum_{i=1}^Mp_i a_i} C \left( \sum_{i=1}^M \VAR{\omega_i} + \alpha \sum_{i=1}^Mp_i^2 \right)
,
\end{equation}

\begin{equation}
E 
%= \frac{1}{K_{eff}} \left(\sum_{i=1}^M\gamma_i(n)a_i^2\right)
= \frac{1}{K_{eff}}\max_{i} \{a_i^2\}\left(\sum_{i=1}^M\gamma_i(n)\right) 
= \frac{1}{\sum_{i=1}^Mp_i a_i} \max_{i} \{a_i^2\}\left(\sum_{i=1}^M \VAR{\omega_i} + \alpha \sum_{i=1}^M p_i^2 \right)
\label{app:eq:def_E}
.
\end{equation}
%where $E$ and $F$ are obtained using Property \ref{prop:sum_weights} with $\alpha
%= \frac{\sum_{i=1}^M\VAR{\omega_i(S_n)} - \VAR{ \sum_{i=1}^M  \omega_i(S_n)}}{1 - \sum_{i=1}^M p_i^2}$

%with $\gamma = \sum_{i=1}^M\gamma_i$.


We define for $A$ -$E$, $A'$-$E'$ such that $X' = \frac{1}{1 -\Omega} X$.
\begin{align}
\frac{1}{T}\sum_{t=0}^{T-1} \E{\norm{\nabla \Lcal^n(\vtheta^n)}^2}
&\le 4   \frac{\Lcal^n(\theta^0) - \Lcal^n(\theta^*)}{( 1- \Omega) \tilde{\eta} \left(\sum_{i=1}^M p_i a_i\right) T} 
+ 2L \tilde{\eta} A' \sigma^2\frac{1}{m}
+ 3 \eta_l^2 L^2 \sigma^2 B'
\nonumber\\
& + 6\eta_l^2 L^2 C' \kappa^2 
+ 3L \tilde{\eta} D\sigma^2
+ 4 L \left[  \frac{L^2}{2} +1 \right] \tilde{\eta} E \kappa^2
,
\label{app:eq:end_intermediary}
\end{align}

\end{proof}




\subsection{Theorem \ref{theo:convergence_paper}}\label{app:sec:proof_convergence}


\begin{proof}
With FedAvg, every client performs vanilla SGD. As such, we have $a_{i, k} = 1$ which gives $a_i = K$ and $\norm{a_i}_2 = \sqrt{K}$. In addition we consider a local learning rate $\eta_l$ such that $\Omega \le \frac{1}{2}$ as such we can bound $A'$-$E'$ as $ X' \le \frac{1}{2}X$. 

Finally, considering that the variables $A$ to $E$ can be simplified as
\begin{equation}
A 
= m \sum_{i=1}^M \left[\VAR{\omega_i} + p_i^2\right]
,
\end{equation}

\begin{equation}
B
= (K -1)
,
\end{equation}

\begin{equation}
C
= K (K-1)
,
\end{equation}

\begin{equation}
D 
= (K - 1) \left( \sum_{i=1}^M \VAR{\omega_i} + \alpha \sum_{i=1}^M p_i^2  \right)
,
\end{equation}

and
\begin{equation}
E 
= K  \left( \sum_{i=1}^M \VAR{\omega_i} + \alpha \sum_{i=1}^M p_i^2 \right)
,
\end{equation}
the convergence bound of Theorem \ref{theo:intermediary} can be reduced to
\begin{align}
\frac{1}{T}\sum_{t=0}^{T-1} \E{\norm{\nabla \Lcal^n(\vtheta^n)}^2}
&\le \Ocal \left( \frac{1}{\eta_g \eta_l K T} \right)
+  \Ocal \left( \eta_g \eta_l \sum_{i=1}^M \left[\VAR{\omega_i} + p_i^2\right] \sigma^2 \right)
\nonumber\\
&+ \Ocal \left(  \eta_l^2 (K-1) \sigma^2 \right)
+ \Ocal \left( \eta_l^2 K(K-1) \kappa^2 \right)
\nonumber\\
& + \Ocal \left( \eta_g \eta_l \left(\sum_{i=1}^M\VAR{\omega_i} + \alpha \sum_{i=1}^M p_i^2  \right) \left[(K-1)\sigma^2 + K \kappa^2 \right] \right)
\label{app:eq:F1}
,
\end{align}
which completes the proof.

\end{proof}    

$\Omega$ is proportional to $\sum_{i=1}^M\gamma_i(n)= \sum_{i=1}^M\VAR{\omega_i} + \alpha \sum_{i=1}^M p_i^2 $. With full participation, we have $\Omega = 0$. However, with client sampling, all the terms in equation (\ref{app:eq:F1}) are proportional with $\frac{1}{1 - \Omega}$. Yet, we provide a looser bound in equation (\ref{app:eq:F1}) independent from $\Omega$ as the conclusions drawn are identical. Through $\Omega$, $\sum_{i=1}^M\VAR{\omega_i}$ and  $\alpha$ needs to be minimized which are conclusions already reached with the impact of $E$ and $F$.

We note that equation (\ref{app:eq:F1}) is function of the client sampling through $\sigma^2$ an indicator of the clients SGD quality and $\kappa^2$ an indicator of the clients data heterogeneity. In the special case where clients have the same data distribution and perform full gradient descent, based on the arguments discussed in the previous paragraph, we can still provide the following bound showing the influence of a client sampling on the convergence speed and the interest of minimizing $\sum_{i=1}^M\VAR{\omega_i}$ and  $\alpha$.
\begin{align}
\frac{1}{T}\sum_{t=0}^{T-1} \E{\norm{\nabla \Lcal^n(\vtheta^n)}^2}
&\le \Ocal \left( \frac{1}{(1 - \Omega)\eta_g \eta_l K T} \right)
,
\end{align}

                                                                                                                                                                                                                       
                                                                                                                                                                                                                                      
                                                                                                                                                                                                                                      
When setting the server learning rate at 1, $\eta_g=1$ with client full participation, i.e. $\VAR{\omega_i} = \VAR{\sum_{i=1}^M\omega_i} = \alpha = 0$ and $m=n$, we have $E= F=0$ and can simplify $A$ to                          
\begin{equation}                                                                                                         
A
= n \sum_{i=1}^M p_i^2                                                                                                                                                                                                              
.                                                                                                                                                                                                                                     
\end{equation}                                                                                                                                                                                                                        
Therefore, our provided convergence guarantee is $\frac{1}{\eta_lKT} + \eta_l \sum_{i=1}^Mp_i^2 \sigma^2 + \eta_l^2 (K-1) \sigma^2 + \eta_l^2 K(K-1) \kappa^2 $ which is identical to the one of \cite{FedNova} (equation (97) in their work), where $\sum_{i=1}^Mp_i^2$ can be replaced by $1/n$ when clients have identical importance, i.e. $p_i = 1/n$.

In the special case, where we use $\eta_l = \sqrt{m/KT}$ \citep{FedNova}, we retrieve their asymptotic convergence bound $\frac{1}{\sqrt{mKT}} + \sqrt{\frac{m}{KT}} \sum_{i=1}^Mp_i^2 \sigma^2 + \frac{m}{T} \sigma^2 + \frac{m}{T} K \kappa^2 $.


\subsection{Application to Clustered Sampling}\label{app:sec:clustered_convergence}

We adapt Theorem \ref{theo:convergence_paper} to clustered sampling. \cite{ClusteredSampling} proves the convergence of FL with clustered sampling by giving identical convergence guarantees to the one of FL with MD sampling. As a result, their convergence bound does not depend of the clients selection probability in the different clusters $r_{k, i}$. \cite{ClusteredSampling} claim reducing the aggregation weight variance provides faster FL convergence while only providing experimental proofs. Corollary \ref{cor:clustered} complements \cite{ClusteredSampling} by theoretically proving the influence of one clustered sampling on the convergence rate. For ease of writing, Corollary \ref{cor:clustered} is formatted for FedAvg but can easily be extended to account for any local $\va_i$ using the proof of Theorem \ref{theo:intermediary} in Section \ref{app:sec:intermediary_theo}.

\begin{corollary}\label{cor:clustered}
	Even with no $\alpha$ such that $\COV{\omega_i(S_n)}{\omega_j(S_n)} = - \alpha p_i p_j$, the bound of Theorem \ref{theo:convergence_paper} still holds with $B$, $C$, and $D$ defined as in Section \ref{app:sec:intermediary_theo} and 
	\begin{equation}
	A = m \left[\frac{1}{m}
	- \frac{1}{m^2} \sum_{i=1}^M \sum_{k=1}^{m}r_{k, i}^2 + \sum_{i=1}^Mp_i^2\right]
	,\
	E 
	= \frac{1}{m}(K-1)
	,
	\text{ and }
	F
	= \frac{1}{m}K
	,
	\end{equation}
	where $E$ and $F$ are identical to the one for MD sampling and $A$ is smaller than the one for Clustered sampling.
\end{corollary}


\begin{proof}
	The covariance property required for Theorem \ref{theo:intermediary} is only used for Lemma \ref{lem:decompo_Xi}. In the proof of Theorem \ref{theo:intermediary}, Lemma \ref{lem:decompo_Xi} is only used in equation (\ref{app:eq:B4}). We can instead use Lemma \ref{lem:decompo_Xiclustered} and keep the rest of the proof as it is in Section \ref{app:sec:intermediary_theo}. Therefore, the bound of Theorem \ref{theo:intermediary} remains unchanged for clustered sampling where $E$ and $F$ use the aggregation weight statistics of MD sampling instead of clustered sampling. Statistics for MD sampling can be found in Section \ref{app:sec:MD} and gives
	\begin{equation}
	\VAR{\sum_{i=1}^M\omega_i(S_{MD})} =0
	\text{ and }
	\alpha_{MD} = \frac{1}{m}.
	\end{equation}
	and the ones of clustered sampling in Section \ref{app:sec:clustered} gives
	\begin{equation}
	\sum_{i=1}^M \VAR{\omega_i(S_{Cl})} 
	= \frac{1}{m}
	- \frac{1}{m^2} \sum_{i=1}^M \sum_{k=1}^{m}r_{k, i}^2
	\le \sum_{i=1}^M \VAR{\omega_i(S_{MD})} 
	.
	\end{equation}
	
\end{proof}



%\cite{ClusteredSampling} introduces \textit{clustered sampling}, a client sampling satisfying Definition \ref{def:sampling} and generalizing MD sampling. Coupling \textit{clustered sampling} with FL was proposed in \cite{ClusteredSampling} to improve MD sampling. Instead of sampling $m$ clients from $m$ the same distribution, $m$ clients are sampled from $m$ different distributions. As a result, clustered sampling generalizes MD sampling and $\VAR{\sum_{i=1}^M\omega_i(S_n)} = 0$. \cite{ClusteredSampling} provide identical convergence rate for clustered and MD sampling and experimentally show clustered sampling improvements over MD sampling. Based on the proof of Theorem \ref{theo:convergence_paper}, we differ to Appendix \ref{app:sec:clustered_convergence} the adjustment of Theorem \ref{theo:convergence_paper} for clustered sampling where we theoretically show the advantages of clustered sampling over MD sampling.




\subsection{ Proof of Corollary \ref{cor:sufficient_conditions}}\label{app:sec:sufficient_conditions} 

\begin{proof}
	
	Combining equation (\ref{app:eq:R1}) with equation (\ref{app:eq:S2}) gives
	\begin{align}
		\Sigma_{MD}
		- \Sigma_U
		& = \left[ - \frac{1}{m} \sum_{i=1}^Mp_i^2 + \frac{1}{m} \right]
		- \left( \frac{n}{m} - 1 \right) \sum_{i=1}^Mp_i^2
		\\
		& = - \frac{1}{m}\left[(n- m +1) \sum_{i=1}^M p_i^2 -1 \right]
		.
		\label{app:eq:N1}
	\end{align}
	Therefore, we have
	\begin{equation}
		\Sigma_{MD} \le \Sigma_U
		\Leftrightarrow
		\sum_{i=1}^Mp_i^2 
		\le 
		\frac{1}{n - m +1}
	\end{equation}
	
	Combining equation (\ref{app:eq:R2}), (\ref{app:eq:R3}), (\ref{app:eq:S5}), and (\ref{app:eq:S6}) gives
	\begin{align}
	\gamma_{MD} - \gamma_{U}
	&= \sum_{i=1}^M \VAR{  \omega_i(S_{MD})} + \alpha_{MD} \sum_{i=1}^M p_i^2
	- \left( \sum_{i=1}^M   \VAR{ \omega_i(S_{U})} + \alpha_U \sum_{i=1}^M  p_i^2 \right)
	\\
	& = \frac{1}{m} - \frac{n-m}{m (n-1)} n \sum_{i=1}^Mp_i^2
	.
	\label{app:eq:N2}
	\end{align}
	
	Therefore, we have
	\begin{equation}
	\gamma_{MD} \le \gamma_U
	\Leftrightarrow
	\sum_{i=1}^Mp_i^2 
	\le 
	\frac{1}{n-m} \frac{n-1}{n}
	.
	\end{equation}

	Noting that 
	\begin{equation}
		\frac{1}{n - m +1} - \frac{1}{n-m} \frac{n-1}{n} 
		= \frac{-m +1}{n (n-m )(n-m+1)}
		\le 0
	\end{equation}
	completes the proof.
%	We also consider a local learning rate $\eta_l$ such that $ \Omega_{MD} \ll 1$ and $ \Omega_{U} \ll 1$. Hence, subtracting equation (\ref{app:eq:end_intermediary}) estimated for FedAvg with Uniform sampling to equation (\ref{app:eq:end_intermediary}) estimated for FedAvg with MD sampling gives
%	\begin{align}
%		D
%		& =  2L  \tilde{\eta} \left[ \sum_{i=1}^M \VAR{\omega_i(S_{MD})}
%		- \sum_{i=1}^M \VAR{\omega_i(S_{U})} \right] \sigma^2 
%		\nonumber\\
%		& + \tilde{\eta} R \left[ 3L (K-1) \sigma^2 + 2 L \left( L^2 + 2 \right) K \kappa^2 \right]
%		\label{app:eq:N5}
%	\end{align}
%	Substituting equation (\ref{app:eq:N1}) and (\ref{app:eq:N2}) in equation (\ref{app:eq:N5}) gives
%	\begin{align}
%		D
%		& \le  2L  \tilde{\eta} \frac{1}{m} \abs{ 1 - (n- m +1) \sum_{i=1}^M p_i^2 } \sigma^2 
%		\nonumber\\
%		& + \tilde{\eta} \frac{1}{m} \abs{1 - \frac{n-m}{n-1} n \sum_{i=1}^Mp_i^2} \left[ 3L (K-1) \sigma^2 + 2 L \left( L^2 + 2 \right) K \kappa^2 \right]
%		\label{app:eq:N6}
%	\end{align}
%	Considering that clients importance satisfy $p_i = \Ocal(\frac{1}{n})$, we have $\sum_{i=1}^Mp_i^2 = \Ocal(\frac{1}{n})$ which gives
%	\begin{align}
%	D
%	& = \Ocal \left( \eta_g \eta_l \left(- \frac{1}{m}\left[(n- m +1) \frac{1}{n} -1 \right] \right) \sigma^2 \right)
%	\nonumber\\
%	& + \Ocal\left(\eta_g \eta_l \left( \frac{1}{m} - \frac{n-m}{m (n-1)} \right) [(K -1)\sigma^2 + K \kappa^2] \right)
%	\\
%	& = \Ocal \left( \eta_g \eta_l \frac{m-1}{m n} \sigma^2 \right)
%	+ \Ocal\left(\eta_g \eta_l \frac{m-1}{m (n-1)} [(K -1)\sigma^2 + K \kappa^2] \right)
%	\\
%	& = \Ocal \left( \eta_g \eta_l \frac{1}{n} \sigma^2 \right)
%	+ \Ocal\left(\eta_g \eta_l \frac{1}{n} [(K -1)\sigma^2 + K \kappa^2] \right)
%	\\
%	& = \Ocal\left(\eta_g \eta_l \frac{1}{n} K[\sigma^2 + \kappa^2] \right)
%	,
%	\label{app:eq:N7}
%	\end{align}
%	which completes the proof.
	
\end{proof}


































==> tex/priorities.tex <==
\section{Priorities}

\begin{enumerate}
	
%	\item Finish the literature review
	
%	\item Write properly the intro
	
	\item Update Schematic F1
	
	\item Experiments: Figure with FedFix
	
	\item Submission at JMLR
	

\end{enumerate}

==> tex/quadratic_example.tex <==
\section{Example with quadratic functions}\label{app:sec:quadratic}

To show in this work that provided convergence bound are tight, we consider an FL applications where clients local loss functions are convex and quadratic, i.e. 
\begin{equation}
	\Lcal_i(\theta) = a_i \theta^2 + b_i \theta + c_i,
	\label{eq:example_local_loss}
\end{equation}
where $\theta \in \mathbb{R}$ and $a_i \ge 0$. Taking the gradient of this local loss function, we get $\nabla \Lcal_i(\theta) = 2 a_i \theta +  b_i$ which leads to 
\begin{equation}
	\theta_i^* = - b_i / (2 a_i) 
	\text{ and }
	\Lcal_i(\theta_i^*) = - b_i^2 / (4 a_i) + c_i .
	\label{eq:example_local_optimum}
\end{equation}
A parallel can be done with this local loss function to a linear regression with one parameter and a modelization with no bias, i.e. $\Lcal_i(\theta) = \frac{1}{2}\norm{X_i \theta - y_i}^2$ where $X_i$ is the parameter vector and $y_i$ is the output vector which leads to  $a_i = X_i^T X_i /2$, $b_i = - X_i^T y_i$, and $c_i = y_i^Ty_i/2$. We also have:
\begin{equation}
	\theta^* = - (\sum_{i=1}^{n}p_i b_i) / (2 \sum_{i=1}^{n}p_i a_i)
	\text{ and }
	\Lcal(\theta^*) = - (\sum_{i =1 }^n p_i b_i)^2 / (4 \sum_{i=1}^{n}p_i a_i) + \sum_{i=1}^{n}p_i c_i .
\end{equation}


Let us consider a local SGD process. $y_{i, k}^n$ is the local model obtained for client $i$ after $k$ SGD. One gradient descent of a client satisfies $\nabla \Lcal_i(x) = - (x - \theta_i^*)$ hence one descent of gradient can be expressed as:
\begin{equation}
y_{i, k+1}^n 
= y_{i, k}^n - \eta_l (y_{i, k}^n - \theta_i^*)
= (1 - \eta_l) y_{i, k}^n + \eta_l \theta_i^* 
\end{equation}
which leads to 
\begin{equation}
\theta_i^{n+1} 
= (1 - \eta_l)^K \theta^n + \sum_{k=0}^{K-1} ( 1 - \eta_l)^k \eta_l \theta_i^*. 
\end{equation}
We note that $\sum_{k=0}^{K-1} ( 1 - \eta_l)^k = [1 - ( 1 - \eta_l )^K]/ \eta_l$. By defining $\phi = 1 -  ( 1 - \eta_l )^K$, we get:
\begin{equation}
\theta_i^{n+1} 
= ( 1 - \eta_l )^K \theta^n + \phi \theta_i^*,
\label{eq:local_work_quadratic}
\end{equation}
which leads to 
\begin{equation}
\theta_i^{n+1} - \theta^n
%= (1 - \eta_l)^K \theta^n + \left[1 - ( 1 - \eta_l )^K \right] \theta_i^* - \theta^n
= \phi (\theta_i^* - \theta^n). 
\label{eq:diff_local_work_quadratic}
\end{equation} 






\subsection{Expected Convergence}

Hence, considering equation (\ref{eq:aggreg_SCAFFOLD_general}), we have:
\begin{equation}
	\theta^{n+1}
	= \theta^n + \eta_g \sum_{ i = 1 }^M\omega_i^n \phi \left[\theta_i^* - \theta^{\rho_i(n)} \right] 
%	= \left[ 1 - \eta_g \phi \sum_{ i = 1 }^M\omega_i^n \right]\theta^n 
%	+ \eta_g \phi \sum_{ i = 1 }^M\omega_i^n \theta_i^* 
\end{equation}
We note that $\E{\theta^{\rho_i(n)}} = \sum_{k=0}^{n}\mathbb{P}(\rho_i(n) = k) \E{\theta^k}$. We have $q_{n, k} = \mathbb{P}(\rho_i(n) = k) $. and $\E{\omega_i^n} = 1/C$ which gives:
\begin{align}
\E{\theta^{n+1}}
& = \E{\theta^n} 
+ \eta_g \phi \frac{1}{M} \sum_{ i = 1 }^M\theta_i^* 
- \eta_g \phi \sum_{ k = 0 }^n q_{n, k} \E{\theta^k} 
%& = ( 1 - \eta_g \phi q_{n, n})\E{\theta^n} 
%- \eta_g \phi \sum_{ k = 0 }^{n-1} q_k \E{\theta^k}
%+ \eta_g \phi \theta^* 
\end{align}

We consider that we can write 
\begin{equation}
	\E{\theta^n }
	= A^n \theta^0 + B^n
	\label{eq:U_2}
\end{equation}
with $A^0 = 1$ and $B^0 = 0$.

Hence, we have:
\begin{align}
\E{\theta^{n+1}}
& = A^n \theta^0 + B^n
- \eta_g \phi \sum_{ k = 0 }^n q_{n, k} [A^k \theta^0 + B^k]
+ \eta_g \phi \theta^* 
\end{align}

which gives $ A^{n+1} = A^n - \eta_g \phi \sum_{ k = 0 }^n q_{n, k} A^k$ and $B^{n+1} = B^n - \eta_g \phi \sum_{ k = 0 }^n q_{n, k} B^k + \eta_g\phi \theta^*$.

\subsection{Variance}
All the clients have the same importance, $p_i = 1 /C$ and the same hardware, $\tau_i = \tau = 1$. Hence, we have: $R_i = R$, $\gamma_i = \gamma = \left[\mathbb{P}( T_i \le \Delta t^{n+1}) - R^2 \right] d^2$ and $d_i = d$. Using the Decomposition Theorem \ref{theo:one_FL_step}, we get:


\begin{align}
\E{\norm{\theta^{n+1} - \theta^*}^2} 
&= \E{ \norm{\theta^n - \theta^*}^2 }
- 2 \E{ \inner { \sum_{i} \frac{1}{M} \phi [\theta_i^* - \theta^{\rho_i(n)}] }{\theta^* - \theta^n} } \nonumber\\
&+ \sum_{i=1}^M\gamma \phi^2  \E{\norm{\theta_i^* - \theta^{\rho_i(n)}}^2} 
+ \phi^2 \E{\norm{\sum_{i=1}^{n} R d(\theta_i^* - \theta^{\rho_i(n)})}^2}
\\
&= \E{ \norm{\theta^n - \theta^*}^2 }
- 2 \phi \E{ \inner { \theta^* - \theta^{\rho(n)} }{\theta^* - \theta^n} } \nonumber\\
&+ \gamma \phi^2 \sum_{i=1}^M  \left[ \E{\norm{\theta_i^* - \theta^*}^2}  + \E{\norm{\theta^* - \theta^{\rho(n)}}^2}  \right] \nonumber\\
& + \phi^2 R^2 d^2 \left[ M\E{\norm{\theta^* - \theta^{\rho(n)}}^2} + M(M- 1) \E{\inner{\theta^* - \theta^{\rho(n)}}{\theta^* - \theta^{\rho'(n)}}} \right] 
\end{align}

We define $U_{u, v} = \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v}}}$. Hence, we have:
\begin{equation}
\E{\inner { \theta^* - \theta^{\rho(n)}}{\theta^* - \theta^{n}}}
= \sum_{k=0}^{n} q_{n, k}\E{\inner { \theta^* - \theta^{k}}{\theta^* - \theta^{n}}}
= \sum_{k=0}^{n} q_{n, k}U_{k, n}
\end{equation}
and 
\begin{equation}
	\E{\inner{\theta^* - \theta^{\rho(n)}}{\theta^* - \theta^{\rho'(n)}}} 
	= \sum_{s=0}^n \sum_{u=0}^n q_{n,s} q_{n, u} U_{s, u}
\end{equation}

We note that $U_{u,v}$ can be calculated with the following sequence:
\begin{align}
U_{u, v+1}
& =  \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v+1}}}\\
& =  \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v} - \sum_{ i = 1 }^M\omega_i^{v}\phi [\theta_i^* - \theta^{\rho(v)}]}}\\
& =  \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v}}}
-  \phi \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{\rho(v)}}}\\
& =  \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v}}}
-  \phi \sum_{s=0}^{v}q_{v , s}\E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{s}}}\\
& =  U_{u, v} 
-  \phi \sum_{s=0}^{v}q_{v , s}U_{u, s}
\end{align}

As a result, we have:
\begin{align}
\E{\norm{\theta^{n+1} - \theta^*}^2} 
&= \E{ \norm{\theta^n - \theta^*}^2 }
- 2 \phi \sum_{s=0}^{n}q_{n , s}U_{n, s}\nonumber\\
&+ \gamma \phi^2 \sum_{i=1}^M  \norm{\theta_i^* - \theta^*}^2  
+ \phi^2 \left[ \gamma  M + R^2 d^2 M\right] \sum_{s=0}^n q_{n , s} \E{\norm{\theta^* - \theta^s }^2}   \nonumber\\
& + \phi^2 R^2 d^2 M (M- 1) \sum_{s=0}^n \sum_{u=0}^n q_{n,s} q_{n, u} U_{s, u}
\end{align}







\subsection{Synchronous FL}

For Synchronous FL, we have $q_{n, n} =1 $ and $\forall k \neq n,\ q_{n, k} = 0 $. Hence, we can rewrite $A^{n+1} = ( 1- \phi)A^n$ and $B^{n+1} = ( 1 - \phi)B^n + \phi \theta^*$ which gives 
\begin{equation}
	\E{\theta^n - \theta^*} = ( 1- \phi)^n [\theta^0 - \theta^*]
	\label{eq:U_1}
%	\label(eq:U_1)
\end{equation} 

We also have $\mathbb{P}( T_i^n \le \Delta t^{n+1}) = \mathbb{P}( T_i \le \Delta t^{n+1}) = 1$ and $R = 1 $ giving $\gamma = 0$ and $d = 1/C$. As a result, we have:
\begin{align}
\E{\norm{\theta^{n+1} - \theta^*}^2} 
&= \E{ \norm{\theta^n - \theta^*}^2 }
- 2 \E{ \inner { \sum_{i} \frac{1}{M} \phi [\theta_i^* - \theta^n] }{\theta^* - \theta^n} } \nonumber\\
& + \phi^2 \E{\norm{\sum_{i=1}^{n} \frac{1}{M}(\theta_i^* - \theta^n)}^2} \\
&= ( 1 - \phi)^2\E{ \norm{\theta^n - \theta^*}^2 }
,
\end{align}
Considering the close from of the expectation, we have $\VAR{\theta^n - \theta^*} = 0$.







\subsection{Synchronous FL + Uniform sampling}

Similarly to Synchronous FL when considering all the clients, we still have $q_{n, n} =1 $ and $\forall k \neq n,\ q_{n, k} = 0 $. Hence equation (\ref{eq:U_1}) still holds for synchronous FL + uniform client sampling.

We define by $S_n$ the set of sampled clients at optimizations step $n$. With Uniform sampling, $m$ clients are sampled without replacement which gives $\mathbb{P}( T_i^n \le \Delta t^{n+1}) = \mathbb{P}( i \in S_n) = m / C$ and $R^2 = m(m-1)/M(C-1)$ implying $d= 1/m$ and $\gamma = [m/M- R^2]d^2$.

By structure, of $q_{n, s}$, we have $\sum_{s=0}^{n}q_{n , s}U_{u, s} = q_{n, n} U_{n, n} = \E{\norm{\theta^n - \theta^*}^2}$, and $\sum_{s=0}^n \sum_{u=0}^n q_{n,s} q_{n, u} U_{s, u} =  q_{n, n}^2 U_{n, n} = \E{\norm{\theta^n - \theta^*}^2}$


\begin{align}
\E{\norm{\theta^{n+1} - \theta^*}^2} 
&= (1 - 2 \phi + \phi^2 R^2 d^2 M^2+ \gamma \phi^2 M )\E{ \norm{\theta^n - \theta^*}^2 } 
+ \gamma \phi^2  \sum_{i=1}^M\E{\norm{\theta^*- \theta_i^*}^2}
\\
&= (1 - 2 \phi + \phi^2 )\E{ \norm{\theta^n - \theta^*}^2 } 
+ \gamma \phi^2  \sum_{i=1}^M\E{\norm{\theta_i^* - \theta^* }^2}
,
\end{align} 

We retrieve the case when considering all the clients as we have $ m = M$ and $\gamma = 0$. 




\subsection{Asynchronous FL}

For every $k > 0$, we have:
\begin{equation}
q_{n, k} 
= \mathbb{P}(\rho_i(n) = k) 
= \mathbb{P}(T_i >  \min_i T_i)^{n-k} \mathbb{P}(T_i =  \min_i T_i)
= \left[\frac{M-1}{M}\right]^{n-k}\frac{1}{M}
,
\end{equation}
and when $k=0$, we have:
\begin{equation}
q_{n, 0} 
= 1 - \sum_{k=1}^n q_{n, k}
= \left[\frac{M-1}{M}\right]^n
\end{equation}

We can use the formulation in equation (\ref{eq:U_2}) to express the expected global at every optimization step. Regarding the variance at every optimization step, we have $\mathbb{P}( T_i^n \le \Delta t^{n+1}) = 1/C$ and $R = 0$ implying $d= 1$ and $\gamma = 1/C$, which gives:
\begin{align}
\E{\norm{\theta^{n+1} - \theta^*}^2} 
&= \E{ \norm{\theta^n - \theta^*}^2 }
- 2 \phi \sum_{s=0}^{n} q_{n, s} U_{n, s} \nonumber\\
&+ \sum_{i=1}^M\frac{1}{M}  \phi^2  \norm{\theta_i^* - \theta^*}^2 
+ \phi^2  \sum_{ s = 0 }^n q_{n, s} \norm{\theta^s - \theta^* }^2 
\end{align}


%
%\begin{align}
%\E{\norm{\theta^{n+1} - \theta^*}^2} 
%&= \E{ \norm{\theta^n - \theta^*}^2 }
%- 2 \E{ \inner { \sum_{i} \frac{1}{M} \phi [\theta_i^* - \theta^{\rho_i(n)}] }{\theta^* - \theta^n} } \nonumber\\
%&+ \sum_{i=1}^M\frac{1}{M}  \phi^2  \E{\norm{\theta_i^* - \theta^{\rho_i(n)}}^2}\\
%&= \E{ \norm{\theta^n - \theta^*}^2 }
%- 2 \phi \E{\inner { \theta^* - \theta^{\rho(n)}}{\theta^* - \theta^n}}\nonumber\\
%&+ \sum_{i=1}^M\frac{1}{M}  \phi^2  \E{\norm{\theta_i^* - \theta^*}^2 + \norm{\theta^* - \theta^{\rho(n)}}^2+ 2 \inner{\theta_i^* - \theta^*}{\theta^* - \theta^{\rho(n)}} }\\
%&= \E{ \norm{\theta^n - \theta^*}^2 }
%- 2 \phi \E{\inner { \theta^* - \theta^{\rho(n)}}{\theta^* - \theta^n}}\nonumber\\
%&+ \sum_{i=1}^M\frac{1}{M}  \phi^2  \left[ \norm{\theta_i^* - \theta^*}^2 + \sum_{ k = 0 }^n q_{n, k} \norm{\theta^* - \theta^k}^2 \right]\\
%&= \E{ \norm{\theta^n - \theta^*}^2 }
%- 2 \phi \E{\inner { \theta^* - \theta^{\rho(n)}}{\theta^* - \theta^n}}\nonumber\\
%&+ \sum_{i=1}^M\frac{1}{M}  \phi^2  \norm{\theta_i^* - \theta^*}^2 
%+ \phi^2  \sum_{ k = 0 }^n q_{n, k} \norm{\theta^* - \theta^k}^2 \\
%\end{align}
%
%We define $U_{u, v} = \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v}}}$. We have:
%\begin{align}
%U_{u, v+1}
%& =  \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v+1}}}\\
%& =  \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v} - \sum_{ i = 1 }^M\omega_i^{v}\phi [\theta_i^* - \theta^{\rho(v)}]}}\\
%& =  \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v}}}
%-  \phi \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{\rho(v)}}}\\
%& =  \E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{v}}}
%-  \phi \sum_{s=0}^{v}q_{v , s}\E{\inner { \theta^* - \theta^{u}}{\theta^* - \theta^{s}}}\\
%& =  U_{u, v} 
%-  \phi \sum_{s=0}^{v}q_{v , s}U_{u, s}
%\end{align}
%
%
%Hence, we have:
%\begin{align}
%\E{\inner { \theta^* - \theta^{\rho(n)}}{\theta^* - \theta^{n}}}
%& = \sum_{k=0}^{n} q_{n, k}\E{\inner { \theta^* - \theta^{k}}{\theta^* - \theta^{n}}}\\
%& = \sum_{k=0}^{n} q_{n, k}U_{k, n}
%\end{align}
%






\subsection{Hybrid FL}
When $k>0$, we have:
\begin{align}
q_{n, k} 
&= \mathbb{P}(\rho_i(n) = k) \\
&= \mathbb{P}(T_i  \le  (n -k+1) T) - \mathbb{P}(T_i  \le  (n -k) T)\\
& = ( 1 - e^{-(n-k+1)T}) -  ( 1 - e^{-(n-k )T} ) \\
& =  e^{-(n-k )T } - e^{-(n-k+1)T}
,
\end{align}
and when $k =0$, we have:
\begin{equation}
q_{n, 0} 
= 1 - \sum_{k=1}^n q_{n, k}
= 1 - \sum_{k=1}^n \left[ e^{-(n-k )T } - e^{-(n-k+1)T} \right]
= 1 - \left[e^{-(n-n )T } - e^{-nT} \right]
= e^{-nT} 
\end{equation}



We have $\mathbb{P}( T_i^n \le T) = \mathbb{P}( T_i \le T) =1 - e^{-T}$, which also gives by independence of the clients computation time $R = 1 - e^{-T}$. Thus, we have $\gamma = R ( 1- R) d^2$ with $d = 1 /RC$. Hence, $\gamma = e^{-T}/ ( 1 - e^{-T})M^2$. Hence for $T$ big enough, hybrid FL behaves similarly to Synchronous FL.
\begin{align}
\E{\norm{\theta^{n+1} - \theta^*}^2} 
&= \E{ \norm{\theta^n - \theta^*}^2 }
- 2 \phi \sum_{s=0}^{n}q_{n , s}U_{n, s}\nonumber\\
&+ \gamma \phi^2 \sum_{i=1}^M  \norm{\theta_i^* - \theta^*}^2  
+ \phi^2 \frac{1}{M} \frac{1}{1 - e^{-T}}\sum_{s=0}^n q_{n , s} \E{\norm{\theta^* - \theta^s }^2}   \nonumber\\
& + \phi^2 \frac{M-1}{M} \sum_{s=0}^n \sum_{u=0}^n q_{n,s} q_{n, u} U_{s, u}
\end{align}


\subsection{Hybrid  Evo FL}
When $k>0$, we have:
\begin{align}
q_{n, k} 
&= \mathbb{P}(\rho_i(n) = k) \\
&= \mathbb{P}(T_i  \le  T^{n+1} - T^k) - \mathbb{P}(T_i  \le  T^{n+1} - T^{k+1})\\
& = ( 1 - e^{-(T^{n+1} - T^k)}) -  ( 1 - e^{-(T^{n+1} - T^{k+1})} ) \\
& =  e^{-(T^{n+1} - T^{k+1}) } - e^{-(T^{n+1} - T^k)}
,
\end{align}
and when $k =0$, we have:
\begin{equation}
q_{n, 0} 
= 1 - \sum_{k=1}^n q_{n, k}
= e^{-T^{n+1}} 
\end{equation}



%
%
%
%\begin{align}
%\E{\norm{\theta^{n+1} - \theta^*}^2} 
%&= \E{ \norm{\theta^n - \theta^*}^2 }
%- 2 \phi \E{ \inner {  \theta^* - \theta^{\rho(n)} }{\theta^* - \theta^n} } \nonumber\\
%&+ \gamma \phi^2  \sum_{i=1}^M \E{\norm{\theta_i^* - \theta^{\rho_i(n)}}^2}\nonumber\\
%&+ \phi^2 R^2 d^2 \E{\norm{\sum_{i=1}^{M} (\theta_i^* - \theta^{\rho_i(n)})}^2}
%\\
%&= \E{ \norm{\theta^n - \theta^*}^2 }
%- 2 \phi \E{ \inner {  \theta^* - \theta^{\rho(n)} }{\theta^* - \theta^n} } \nonumber\\
%&+ \gamma \phi^2  \left[ \sum_{i=1}^M  \E{\norm{\theta_i^* - \theta^*}}^2 + C\E{\norm{\theta^* - \theta^{\rho(n)}}^2} \right] \nonumber\\
%&+ \phi^2 R^2 d^2 \left[ M\E{\norm{ \theta^* - \theta^{\rho(n)}}^2} + C(C-1) \E{\inner{\theta^* - \theta^{\rho_i(n)}}{\theta^* - \theta^{\rho_j(n)}} }\right]
%,
%\end{align}
%
%
%We have:
%\begin{align}
%	\E{\inner{\theta^* - \theta^{\rho_i(n)}}{\theta^* - \theta^{\rho_j(n)}}}
%	&= \sum_{s=0}^{n} \sum_{u=0}^{n} \mathbb{P}( \rho_i(n) = s)\mathbb{P}( \rho_j(n) = u) \E{\inner{\theta^* - \theta^u}{\theta^* - \theta^v}}
%	\\
%	&= \sum_{s=0}^{n} \sum_{u=0}^{n} q_{n , s} q_{n , u} U_{s, u}
%	\\
%\end{align}
%which gives
%\begin{align}
%\E{\norm{\theta^{n+1} - \theta^*}^2} 
%&= \E{ \norm{\theta^n - \theta^*}^2 }
%- 2 \phi \sum_{s=0}^{n} q_{n , s} U_{n, s} \nonumber\\
%&+ \phi^2 R^2 d^2 \left[ M\sum_{s=0}^{n} q_{n , s} \E{\norm{ \theta^s - \theta^*}^2} + C(C-1)\sum_{s=0}^{n} \sum_{u=0}^{n} q_{n , s} q_{n , u} U_{s, u}\right]
%,
%\end{align}
%


\subsection{Computation Time}

With synchronous FL, we have:
\begin{equation}
	\E{\Delta t^{n}}
	= \E{\max_i{T_i}}
	= \sum_{ k = 0 }^{M-1} \frac{1}{(M - k)\lambda}
\end{equation}
When combining synchronous FL with sampling uniformly $m$ clients, we get:
\begin{equation}
\E{\Delta t^{n}}
= \sum_{ k = 0 }^{m-1} \frac{1}{(m - k)\lambda}
\end{equation}
When sampling client asynchronously, an optimization step time is the one for a client to perform its local given that all the clients are performing their local work.
\begin{equation}
\E{\Delta t^{n}}
= \E{\min_i{T_i}}
= \frac{1}{M \lambda}
\end{equation}









==> tex/related_work.tex <==
%\section{Related Work}
%\label{sec:related}
%
%\begin{definition}[Unbiased Sampling]\label{def:sampling} 
%	A client sampling scheme is said unbiased if the expected value of the client aggregation is equal to the global deterministic aggregation obtained when considering all the clients, i.e.
%	\begin{equation}
%	\EE{S_t}{\vtheta^t}
%	=
%	\EE{S_t}{\sum_{j \in S_t}w_j(S_t)\vtheta_j^t}
%	\coloneqq
%	\sum_{i =1 }^n p_i\vtheta_i^t ,
%	\end{equation}
%	where $w_j(S_t)$ is the aggregation weight of client $j$ for subset of clients $S_t$.
%\end{definition}






%\subsection{FL convergence with MD client sampling}
%
%Theoretical guarantees regarding the convergence of FedAvg were given in \cite{FedNova}. The proof relies on assumptions classically used in Stochastic Gradient Descent (SGD) analysis \cite{Bottou2018} (Assumptions \ref{ass:smoothness} and \ref{ass:unbiased} below), or commonly used in the federated optimization literature \cite{FedProx, ontheconvergence, Haddadpour2019, SCAFFOLD, MATCHA} to capture the dissimilarities of local objectives (Assumption \ref{ass:dissimilarity} below). 
%
%%\cite{FedNova} also proves that to avoid inducing bias in the trained model, when sampled every client needs to perform the same amount of Stochastic Gradient Descent (SGD) $N$ with an SGD optimizer. Clients, when participating at an iteration, performs therefore $N$ SGD with and SGD optimizer.
%
%%The authors assume the following 3 assumptions regarding each client's local loss function $\Lcal_i$. Using Assumptions \ref{ass:smoothness} to \ref{ass:dissimilarity}, \cite{FedNova} gives an upper bound on the gradient of the global loss function $\Lcal$ at the end of the FL process when considering all the clients and when sampling $m$ clients using FedProx sampling scheme. The theorem for the later result is given in Theorem \ref{theo:convergence_FP}.
%
%\begin{assumption}[Smoothness]\label{ass:smoothness}
%	The clients local objective function is Lipschitz smooth, that is, $\norm{\nabla \Lcal_i(x) - \nabla \Lcal_i(y)} \le L \norm{x - y}, \forall i \in \{1, ..., n\}$.
%\end{assumption}
%
%\begin{assumption}[Unbiased Gradient and Bounded Variance]\label{ass:unbiased}
%	For each client $i$ local model, the stochastic gradient $g_i(x|\xi)$ of model $x$ evaluated on batch $\xi$ is an unbiased estimator of the local gradient: $\EE{\xi}{g_i(x|\xi)} = \nabla \Lcal_i(x)$, and has bounded variance $\EE{\xi}{\norm{g_i(x|\xi) - \nabla \Lcal_i(x)}} \le \sigma^2, \forall i \in \{1,..., n\}$ with $\sigma^2\ge 0$.
%\end{assumption}
%
%\begin{assumption}[Bounded Dissimilarity]\label{ass:dissimilarity}
%	For any set of weights $\{ w_i\le 0\}_{i=1}^n$ such that $\sum_{i=1}^{n}w_i =1$, there exists constants $\beta^2\ge 1$ and $\kappa^2 \ge 0$ such that $\sum_{i=1}^{m}w_i \norm{\nabla \Lcal_i(x)}^2 \le \beta^2 \norm{\sum_{i=1}^{m}w_i \nabla \Lcal_i(x)}^2 + \kappa^2$. If all the local loss functions are identical, then we have $\beta^2 =1$ and $\kappa^2 =0$. 
%\end{assumption}
%
%The following theorem was proven in \cite{FedNova} and provides theoretical guarantees for MD client sampling.
%
%\begin{theorem}\label{theo:convergence_FP}
%	Under Assumptions \ref{ass:smoothness} to \ref{ass:dissimilarity}, and local learning rate $\eta = \sqrt{m/NT}$, 
%	FL with $FedAvg$ when sampling $m$ clients with MD
%	converges to a stationary point of $\Lcal(\vtheta)$:
%	\begin{equation}
%		\frac{1}{T}\sum_{t=0}^{T}\E{\norm{\nabla \Lcal(\vtheta^t)}^2}
%		\le \Ocal(\frac{1}{\sqrt{mNT}}) + \Ocal(\frac{mN}{T}).
%	\end{equation}
%\end{theorem}
%The proof of Theorem \ref{theo:convergence_FP} can be found in \cite{FedNova} and shows that considering a subset of workers with MD client sampling is enough to ensure convergence of the global model to a local minimum of the federated loss function, equation (\ref{eq:global_loss}). 
%
%Following the conclusions of this work, to avoid optimizing a surrogate loss function instead of the federated one in equation (\ref{eq:global_loss}), the server asks from every client to compute the same amount of SGD steps $N$. 
%
%%However, clients need to be sampled such that the expected aggregation is equal to the aggregation with all the workers considered. At iteration $t$, we denote by $S_t$ the $m$ sampled workers, by $\vtheta_i^t$ the updated model of worker $i$ , and by $\omega_i(S_t)$ the weight given to worker $i$ for the aggregation. The expected aggregation must then follow


%\subsection{Sampling schemes comparison}
%
%Other client sampling schemes have been proposed. For example, with \cite{ontheconvergence}, the server sends the global model to every client before creating the new global model out of the first $m$ updated models the server receives; with \cite{Richtarik_optimal_sampling}, the server waits for every client to send the norm of their work before selecting the $m$ clients with the most relevant updates; with \cite{sampling_mobile_edge}, clients transmit information about their available computation resources before the server selects $m$ of them in function of their availability. Contrarily to FedAvg and MD sampling, these sampling schemes require additional communications and sometimes even computation from all the clients. On the contrary, FedAvg and MD sampling have the appealing property of maintaining to a minimum the amount of clients-server communications at each iteration. The global model is sent only to the sampled clients, and the amount of local work is set for those clients to only $N$ SGD updates. 
%To the best of our knowledge, FedAvg and MD sampling schemes are the only approaches minimizing the effective work and communications asked to the clients.
%Moreover, while FedAvg sampling has no theoretical guarantees regarding its convergence, neither regarding the unbiasedness of its global model, MD sampling is shown to converge to a stationary point of the global loss function (\ref{eq:global_loss}) (Theorem \ref{theo:convergence_FP}).  Based on these considerations and given that \cite{ontheconvergence} shows experimentally that MD sampling outperforms FedAvg, in the rest of this work we consider MD sampling as reference sampling technique.


%\section{Introduction}
%
%
%Federated learning is a training paradigm that has gained popularity in the last years as it enables different clients to jointly learn a global model without sharing their respective data. Federated training schemes based on model averaging of clients contributions are the most common, among which FedAvg (\cite{FedAvg}) is the most popular. 
%
%First, we begin by defining the stochastic distributed prediction problem. Suppose that we have $M$ participants and for each participant observe $n_i$ inputs $\{\vz_{k, i}\}_{k=1}^{n_i}$ independently sampled from a fixed unknown distribution over a sample space $\mathcal{Z}_i$. Models are defined by a set of parameters $\vtheta$ which are learnt based on the clients training data quantified on loss $l(\vtheta, \vz_{k, i})$. This formalization accounts both for supervised learning with $\vz_{k, i} = (\vx_{k, i}, \vy_{k, i})$ where $\vx_{k, i}$ is regarded as the input of the statistical model and $\vy_{k, i}$ is desired output, and unsupervised learning with $\vz_{k, i} = \vx_{k, i}$. We aim at building a statistical model providing the smallest averaged loss of the clients data points defined as
%\begin{equation}
%\label{eq:original_problem}
%\Lcal(\vtheta) 
%\coloneqq \frac{1}{\sum_{i=1}^M n_i}\sum_{i=1}^M \sum_{k=1}^{n_i} l(\vtheta, \vz_{k, i})
%.
%\end{equation}
%
%We note that every stochastic distributed prediction problem aims at minimizing a loss function $\Lcal$ that can be expressed as in equation (\ref{eq:original_problem}). The focus of this work is on applications for federated learning. More precisely, participants, called clients, communicate with a server orchestrating the learning process, and never share their data with the server and the other clients. We concentrate in the rest of this work on FedAvg (\cite{FedAvg}), the most popular federated learning approach to solving the problem in equation (\ref{eq:original_problem}) while respecting the constraints discussed before. At every optimization step, each client performs in parallel a fix amount of stochastic gradient descents (SGD) on the current global model before sending back the resulting model to the server. Once in possession of all the clients contributions, the server creates the new global model as the weighted mean of the clients updates based on their data ratio. 
%
%Speak about security and the amount of average is important for that.
%
%
%Federated learning is a generalization of distributed learning which was first introduced for statistical inference with a star-shape network composed of a server communicating with computation machines. The server owns the dataset and splits it among the machines. At every optimization round, machines send gradient estimated on the current global model and their data to the server that using the machines' gradients to perform a gradient descent (GD). Distributed learning was later extended to account for SGD and more local computation like federated learning. The main optimization difference between federated and distributed learning lies in their data distributions respectively non-iid and iid. Therefore, proving FedAvg convergence was more challenging and done in [XX]. In some settings, FedAvg is also shown to converge to a sub-optimum, e.g. when each client performs a different amount of local work \citep{FedNova}, or when clients are not sampled in expectation according to their importance \citep{PowerOfChoice}.
%
%A major drawback behind FedAvg is the time needed for the server to create two consecutive global models. The server has to wait for all the clients to perform their local work to \textit{synchronize} their update and create a new global model.
%Therefore, the time for an optimization step is conditioned on the one of the slowest client. Also, the fastest clients are idle once they have sent their updates to the server. In addition of having heterogeneous data distributions $\mathcal{Z}_i$, clients have heterogeneous hardware which can translate in major FL slow-down. Considering a subset of clients at every optimization step is shown to provide faster optimization rounds and in turn faster FL \citep{OnTheConvergence}. However, client sampling increases clients idle time and thus does not take full advantage of the clients computation power either.
%
%We propose in this work to consider an asynchronous version of FedAvg. The server creates a new global model whenever a client send its local work and send this model to this client. As a result, clients are never idle and each perform their local work on a different global model. Similarly to the synchronous case, asynchronous distributed learning has already been investigated in [XX]. We position our work as an extension of asynchronous distributed learning. To the best of our knowledge, asynchronous FedAvg for non-iid data distributions has also been investigated in [XX]. We introduce a new theoretical convergence framework for averaging aggregation schemes with which we can prove synchronous FedAvg convergence. We also show that in most FL applications asynchronous FL applications do not converge to their optimum. Finally, we propose instead to consider fixed period of time at which the server aggregates 
%
%
%Our paper is structured as follow...
%
%
%
%What happens when the amount fo local work is increased to more than one SGD ?
%
%What happens when clients do not result from the same data distribution ?
%
%
%%By eliminating the required coordination overhead, asynchronous operations become simultaneously more appealing (in physically clustered systems) and more scalable (in massively parallel and volunteer computing grids).
%%
%%Distributed asynchronous stochastic gradient descent is one of the most widely deployed methods for training large-scale machine learning models. More concretely, there are two types of distributed computing architectures that are common in practice,: the first is a shared-memory multi-core/multi-GPU cluster where different processors independently compute stochastic gradients and update a global model parameter using a hared memory. The second is a "master-slave" architecture where each worker independently computes a stochastic gradient of the objective; these gradients are sent asynchronously to the master as they become available. 
%
%
%
%
%
%
%
%
%%\subsection{Original Problem}
%%We consider the following distributed optimization problem:
%%\begin{equation}
%%\label{eq:original_problem}
%%\Lcal(\vtheta) = \sum_{i=1}^{C}p_i \Lcal_i(\vtheta)
%%\end{equation}












==> tex/review_papers.tex <==
\section{Background}

asynchronous DL convergence \cite{DistributedDelayed}
\cite{OptimalDistributedOnline} \cite{SlowLearnersAreFast}
\cite{AsyncParallelSGDforNonconvex} 

experimental asynchrnous FL \cite{RevisitingDistributedSynchronousSGD} \cite{EfficientAndRobust} 
\cite{PrivacyPreservingAsynchronous}
\cite{HowSlowCanYouGo}

asynchronous FL \cite{ErrorFeedbackFramework}

FedBuff \cite{RevisitingDistributedSynchronousSGD} 
\cite{FedBuff}

Heterogeneous amount of local work \cite{AsynchronousFOpti}




For in-depth discussion of SGD and its application in machine learning, we refer to the book of \cite{BottouBookSGD}. For in-depth discussion of Federated Learning please refer to \cite{OpenProblems} and for in depth discussion of Asynchronous FL please refer to \cite{AFLsurvey}. 

\cite{DistributedDelayed} about asynchronous distributed learning. This work is theoretical and assumes convex functions with updates using projected gradients and a primal/dual optimization approach. The learning rate considered is decreasing. The authors show that asynchronicity can speed-up convergence: theoretically with a $1/m$ ratio and experimentally. 

\cite{DataDependent} about distributed learning. The authors consider the problem of distributed learning for a network where clients can communicate between each other. Authors show that the resulting convergence bound is proportional to the eigen value of the matrix for this network. Data is assumed to be iid and shared among the clients/processors by the server.

\cite{RevisitingDistributedSynchronousSGD} about asynchronous FL. This work is experimental. The server asks to more than $m$ clients to perform their local work and creates the new global model with the first $m$ clients updating their contribution. This setup is identical to the one considered for client sampling in \cite{OnTheConvergence}.

\cite{TowardsAsynchronousFL} about clients performing different amount of local work $K_i$. 
At fixed clock times, clients share with the server their communication capabilities and the amount of SGD conducted on their local work. The server uses these information to optimally select a subset of clients used for aggregation. These clients receive the new global model while other clients keep performing local work on their current local model.
No theoretical work is conducted. The asynchronicity comes from the heterogeneous amount of local work in clients considered for aggregation. 

\cite{EfficientAndRobust} about asynchronous FL. The authors make an interesting assumption about the gradients enabling consideration of unbiased gradients. The underlying idea is to tailor the amount fo local work a client should perform in function of its data difference with other clients and its communication and computation capabilities. While theoretical and experimental proof are provided, I do not trust the theoretical derivation in this work. Especially assumptions are pretty strong and results in this work goes against the one in \cite{FedNova}. 
THIS WORK SHOULD BE COMPARED TO OURS AS CONVERGENCE PROOF TO OPTIMUM IS PROVIDED.

\cite{OptimalDistributedOnline} about distributed learning. Interesting article published at JMLR. The notion of regret is interesting as convergence to the optimum in that case reduces to a null regret. A star shape network is assumed with $M$ processors. Clients data distributions are assumed to be identical and partitioned by the server. The local optimization is based on projected gradients. POTENTIAL COMPARISON WITH OUR BOUND ? Definition of the difference between online and optimization.

\cite{TamingTheWild} about asynchronous DL. Speaks about the worst case expected delay. Very interesting work based on submartingales. Authors provide an upper bound on the probability an algorithm has performed its work in $N$ optimization rounds in function of the desired residual $\epsilon$ and learning parameters. We note that this method required to bound the gradients.

\cite{FedBuff} Introduces a new asynchronous FL algorithm \textsc{FedBuff}. The server waits for $m$ clients to perform their local update before considering clients contribution for aggregation. The server sends the new model to these clients.
Author have strong assumptions (bounded gradients, bounded dissimilarity) but do not assume convexity. COMPARE OUR CONVERGENCE BOUNDS.

\cite{ParallelizingSGD} about SGD for least square. Published at JMLR. Different parallelization methods are proposed to have faster SGD for this kind of problems. Not directly applicable to DL or FL. 

\cite{SlowLearnersAreFast} about asynchronous DL. This work is very similar to ours and prove the convergence of a sequence of optimizations schemes.
Authors consider convex loss functions, bound the distance between two consecutive models $\norm{\vtheta^{n+1} -\vtheta^n}^2 \le D^2$ and bound the gradient norms.
However, it seems that the bound in Theorem 2 cannot help draw any conclusion. Indeed, the lower bound cannot be 0 and a residual like the one in Theorem \ref{theo:convergence_convex} needs to appear to prove convergence. 
Also, authors restrict themselves to the asynchronous case where clients send their update with fixed delay $\tau = M - 1 $.
COMPARE THEIR CONVERGENCE RATE TO OURS.

\cite{AsyncParallelSGDforNonconvex} about asynchronous DL. Clients have identical data distributions but no assumption convexity are made. The second part of this work is on a lock free approach which does not seem to hold and be relevant for this work. 
COMPARE THEIR LEARNING RATE AND CONVERGENCE BOUND WITH OURS.

\cite{ADPSGD} for asynchronous decentralized DL. The work does not consider a star shape network with theoretical guarantees.

\cite{PrivacyPreservingAsynchronous} for asynchronous FL. No theoretical work and only experiments are provided. The considered experimental scenario consider few clients (3 for MNIST) and data partitioning is iid.

\cite{Hogwild} for lock free DL. $M$ processors have access to the same dataset. 

\cite{DynamicFL} for FL. Clients are sample according to a MD distribution and asked to perform their local work according to client specific hyperparameters. Proofs for their theorem is not provided. 

\cite{Samarakoon2019} for (asynchronous) FL. This work is around optimization of communications based on Lyapunov equations but without proving FL convergence to its optimum. A synchronous and asynchronous version of their algorithm is available.

\cite{ErrorFeedbackFramework} for (asynchronous) FL. The authors make the same assumptions as us while also proving convergence for non convex functions. However, authors assume iid data distributions. Authors also introduce the notion of compressors. The delay scenario considered is $\tau = M$.

\cite{WhenEdgeMeetsLearning} for FL. Authors propose an optimization method to choose the appropriate amount of local SGD $K$ to perform for a given amount $N$ of optimization rounds. Theoretical convergence provided assuming a bounded gradient divergence and convex local loss functions.

\cite{IsLocalSGD} for FL. Authors show that for quadratic loss functions, $K>1$ is better than $K=1$. They also show that local work sometimes improve convergence for convex functions and the other way around. Clients data distributions are assumed iid (dataset split among clients).

\cite{AsynchronousFOpti} for asynchronous FL. Authors propose a weighting scheme to account properly for clients updates in function of a function they design proportional to an hyperparameter and clients staleness. Clients perform heterogeneous amount of local work $K$. Theoretical work is proposed for weakly convex functions but with bounded gradients and assumptions not easy to verify.

\cite{ParallelSGDWhenDoesAveragingHelp} for FL. Impact of $K$ on FL convergence. Authors propose theoretical considerations around simple convex functions and non conclusive experiments are given.

\cite{FedPD} for FL.
Answers questions on the impact of FL assumptions, local work and aggregation on FL convergence. The theoretical part is informal and either based on simple functions or with informal theory. Clear formalization of FL assumptions in introduction.

\cite{AsyncSGDwithDelay} for asynchronous DL. Authors propose a novel async-DL algorithm which they theoretically show improves async-DL. Their method aims at compensating the clients delay with a Taylor expansion of the gradient using Hessian Approximation. Computing the Hessian can be costly. Clients data is assumed centralized and then split among the participants.

\cite{Zhou2018} for FL. Theoretical proof of FL convergence in non convex settings. Clients data are assumed iid. Authors work is redundant with current work on FL with weaker assumptions and without citing any FL papers.
Unfair experimental comparison based on the amount of aggregations and not on the amount of time needed for training.

\cite{HowSlowCanYouGo} for asynchronous DL. Assumptions are made on the shape of the delay $\tau$. Delays $\tau$ are paired with learning rate structures $\eta_l$. Theoretical convergence is proven without providing convergence bound and thus convergence rate. Nice paragraph citing a lot of papers in the introduction about asynchronous DL.  






\cite{AFLsurvey} Survey on AFL with more than 50 papers. Most of them are experimental papers. Describe the potential ongoing work for AFL: Node selection, weighted aggregation, gradient compression, semi-asynchronous, cluster FL, model split.

\cite{FLUnderArbitraryCommPatterns} Identical convergence speed for their asynchronous algorithm and synchronous FL. The authors assume that clients perform their local work with the same amount of time. The asynchronicity only comes from the communication time which helps the server to know how many local work has been done. Theoretical justification for non convex and Lipschitz smooth loss functions is provided. After T server aggregations, every client has performed T optimization steps which prevents bias.

\cite{GraphOracleModels} The answering delay is assumed to be fixed.

\cite{stich2018local} Proposed optimization problem by bounding the clients gradient dissimilarity. A synchronous and asynchronous framework are proposed while considering non-iid data distributions. 

\cite{Chen2021}

\cite{Wang2019adaptive}

\cite{Chen2018}

\cite{arjevani20a}



%%%
%FL with only experiments: \citep{PrivacyPreservingAsynchronous, Wang2019adaptive}(few clients + iid), \cite{Samarakoon2019}
%
%FL with broken theory: \cite{Chen2021}(issues with assumption + proof), \cite{AsynchronousFOpti} (bounded gradients)
%
%Parallel SGD Star shape network: \citep{Chen2018, AsyncParallelSGDforNonconvex, AsyncSGDwithDelay} (iid data) \cite{stich2018local}(niid)
%
%Parallel SGD Star distributed network: \cite{ADPSGD} (niid data)
%
%ML with delayed gradients: \citep{ErrorFeedbackFramework, arjevani20a}
%
%FL papers using asynchronous or stragglers to speak about clients hardware constraints but keeping synchronization: \citep{FedProx, FedNova, DynamicFL} (accounting for different amount of local work), \citep{PrivacyPreservingAsynchronous, AsynchronousFOpti} (accounting for different local computation time)




==> tex/schematic.tex <==
\begin{figure}
	\begin{tikzpicture}
%	[scale = 0.7, line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm]
	
	%Global models
	\node[fill, draw, circle,label=above: $\theta^t$, minimum size = 3pt, inner sep =0] (A) at (0,0){} ;
	\node[fill, draw, circle,label=below: $\theta^{t+1}$, minimum size = 3pt, inner sep =0] (B) at (-7.5/4/2, -7.5/2/4){} ;
	
	%Connect the globsl models
	\draw [line width=1pt, ->] (A)-- (B);
	%	\draw [line width=1pt, ->] (B)-- (C);
	%	
	%Local optima and local update
	\node[fill, draw, circle,label=left: $\theta_1^*$, minimum size = 3pt, inner sep =0] (E) at (-0.5,-2.7){} ;
	\node[fill, draw, circle,label=below: $\theta_1^{t+1}$, minimum size = 3pt, inner sep =0] (F) at (-0.5/2,-2.7/2){} ;
	
	\node[fill, draw, circle,label=left: $\theta_2^*$, minimum size = 3pt, inner sep =0] (G) at (0.5,-3){} ;
	\node[fill, draw, circle,label=right: $\theta_2^{t+1}$, minimum size = 3pt, inner sep =0] (H) at (0.5/2,-3/2){} ;
	
	\node[fill, draw, circle,label=left: $\theta_3^*$, minimum size = 3pt, inner sep =0] (I) at (-3,0){} ;
	\node[fill, draw, circle,label=above: $\theta_3^{t+1}$, minimum size = 3pt, inner sep =0] (J) at (-3/2,-0/2){} ;
	
	\node[fill, draw, circle,label=below: $\theta_4^*$, minimum size = 3pt, inner sep =0] (K) at (-3.5, -0.5){} ;
	\node[fill, draw, circle,label=below: $\theta_4^{t+1}$, minimum size = 3pt, inner sep =0] (L) at (-3.5/2,-0.5/2){} ;
	
	%Connect the updates
	\draw [line width=0.5pt, ->] (A)-- (F);
	\draw [line width=0.5pt, dashed] (F)-- (E);
	
	\draw [line width=0.5pt, ->] (A)-- (H);
	\draw [line width=0.5pt, dashed] (H)-- (G);
	
	\draw [line width=0.5pt, ->] (A)-- (J);
	\draw [line width=0.5pt, dashed] (J)-- (I);
	
	\draw [line width=0.5pt, ->] (A)-- (L);
	\draw [line width=0.5pt, dashed] (L)-- (K);
	
	
	%\end{scriptsize}
	\end{tikzpicture}
	%	\hspace{1cm}
	\begin{tikzpicture}[scale = 0.7, line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm]
	
	%Global models
	\node[fill, draw, circle,label=above: $\theta^t$, minimum size = 3pt, inner sep =0] (A) at (0,0){} ;
	\node[fill, draw, circle,label=right: $\theta^{t+1}$, minimum size = 3pt, inner sep =0] (B) at (-2.5/2/2, -3/2/2){} ;
	\node[fill, draw, circle,label=below: $\theta^{t+2}$, minimum size = 3pt, inner sep =0] (C) at (-1.9, -1.6){} ;
	
	%Connect the globsl models
	\draw [line width=1pt, ->] (A)-- (B);
	\draw [line width=1pt, ->] (B)-- (C);
	%	
	%Local optima and local update
	\node[fill, draw, circle,label=left: $\theta_1^*$, minimum size = 3pt, inner sep =0] (E) at (-0.5,-2.7){} ;
	\node[fill, draw, circle,label=below: $\theta_1^{t+2}$, minimum size = 3pt, inner sep =0] (F) at (-0.55,-1.7){} ;
	
	\node[fill, draw, circle,label=left: $\theta_2^*$, minimum size = 3pt, inner sep =0] (G) at (0.5,-3){} ;
	\node[fill, draw, circle,label=right: $\theta_2^{t+1}$, minimum size = 3pt, inner sep =0] (H) at (0.5/2,-3/2){} ;
	
	\node[fill, draw, circle,label=left: $\theta_3^*$, minimum size = 3pt, inner sep =0] (I) at (-3,0){} ;
	\node[fill, draw, circle,label=above: $\theta_3^{t+1}$, minimum size = 3pt, inner sep =0] (J) at (-3/2,-0/2){} ;
	
	\node[fill, draw, circle,label=below: $\theta_4^*$, minimum size = 3pt, inner sep =0] (K) at (-3.5, -0.5){} ;
	\node[fill, draw, circle,label=below: $\theta_4^{t+2}$, minimum size = 3pt, inner sep =0] (L) at (-2.25,-0.62){} ;
	
	%Connect the updates
	\draw [line width=0.5pt, ->] (B)-- (F);
	\draw [line width=0.5pt, dashed] (F)-- (E);
	
	\draw [line width=0.5pt, ->] (A)-- (H);
	\draw [line width=0.5pt, dashed] (H)-- (G);
	
	\draw [line width=0.5pt, ->] (A)-- (J);
	\draw [line width=0.5pt, dashed] (J)-- (I);
	
	\draw [line width=0.5pt, ->] (B)-- (L);
	\draw [line width=0.5pt, dashed] (L)-- (K);
	
	\end{tikzpicture}
	
	\caption{Schematics illustrating the clients' similarities detection method when considering all the clients, left, and when sampling clients, right. $\theta^t$ is the global model at iteration $t$ and $\theta_i^{t+1}$ is the updated local model of client $i$ on $\theta^t$ while converging to its local optimum $\theta_i^*$.}
	\label{fig:schematic_sim}
\end{figure}
